Partial Synchrony for Free? New Upper Bounds for Byzantine Agreement

Byzantine agreement allows n processes to decide on a common value, in spite of arbitrary failures. The seminal Dolev-Reischuk bound states that any deterministic solution to Byzantine agreement exchanges Omega(n^2) bits. In synchronous networks, solutions with optimal O(n^2) bit complexity, optimal fault tolerance, and no cryptography have been established for over three decades. However, these solutions lack robustness under adverse network conditions. Therefore, research has increasingly focused on Byzantine agreement for partially synchronous networks. Numerous solutions have been proposed for the partially synchronous setting. However, these solutions are notoriously hard to prove correct, and the most efficient cryptography-free algorithms still require O(n^3) exchanged bits in the worst case. In this paper, we introduce Oper, the first generic transformation of deterministic Byzantine agreement algorithms from synchrony to partial synchrony. Oper requires no cryptography, is optimally resilient (n >= 3t+1, where t is the maximum number of failures), and preserves the worst-case per-process bit complexity of the transformed synchronous algorithm. Leveraging Oper, we present the first partially synchronous Byzantine agreement algorithm that (1) achieves optimal O(n^2) bit complexity, (2) requires no cryptography, and (3) is optimally resilient (n >= 3t+1), thus showing that the Dolev-Reischuk bound is tight even in partial synchrony. Moreover, we adapt Oper for long values and obtain several new partially synchronous algorithms with improved complexity and weaker (or completely absent) cryptographic assumptions.

==> sections/crusader_agreement.tex <==
\section{Crusader Agreement}


Crusader Agreement \cite{Dolev82} is similar to agreement, but allows some parties to output a special $\bot$ value. More specifically, it guarantees (1) Validity: when all non-faulty parties have the same input, this is the only
output; and (2) Agreement: no two honest parties output two distinct non-$\bot$ values.
We can extend BCA to Graded-BCA, where each party outputs a value and a grade $g \in \{0, 1, 2\}$, intuitively corresponding to how confident they are in their output. Roughly speaking, in
Graded-BCA, a grade of 2 implies that all parties have the same value.
More generally, we can define connected consensu sthat generalize these concepts \cite{AttiyaWelch23}.
With binary inputs, this description of the problems resembles approximate agreement on the $[0,1]$ real interval with parameter $\varepsilon$.
 Processes start at the two extreme points of the interval, 0 or 1, and must decide on values that are at most $\varepsilon$ apart from each other. Decisions must also be valid, i.e., contained in the interval of the inputs. Approximate agreement is a way to sidestep the impossibility of solving consensus in asynchronous systems and there are many algorithms for approximate agreement.
Indeed, crusader agreement reduces to approximate agreement with $\varepsilon = 1/2$ : Run approximate agreement with your input (0 or 1) to get some output y, then choose the value in {0, 1/2 , 1} that is closest to $y$ (taking the smaller one if there are two such values, e.g., for $y = 1/4$ ). Finally, return $\bot$ if $1/2$ is chosen. (A similar observation is noted in Mahaney and Shneider, PODC'85.) Likewise, adopt-commit reduces to approximate agreement with $\varepsilon = 1/3$, and graded consensus to taking $\varepsilon = 1/4$ . This connection makes it clear why binary crusader agreement, adopt-commit and graded broadcast can be solved in an asynchronous message-passing system, in the presence of crash and malicious (unauthenticated Byzantine) failures, within a small number of communication rounds.
Connected consensus elegantly unifies seemingly-diverse problems, including crusader agreement, graded broadcast, and adopt-commit, and generalizes them to accept multi-valued inputs. It can be viewed as approximate agreement on a restricted class of graphs: spider graphs consisting of a central clique (which could be a single vertex) to which are attached $|V |$ paths (“branches”) of length $R$, where $R$ is the refinement parameter


\begin{algorithm}
\caption{Asynchronous Binding Crusader Agreement for Byzantine Faults instance $\text{id}$ ($\text{BCA}_{\text{Byz}}$) (Algorithm 4 of \cite{Abraham22crusader})}
\label{algorithm:bcabyz}
\begin{algorithmic}[1]
\State \textbf{Input:} $ x $
\State $ \text{approvedVals} \gets \{\} $
\State \textbf{send} $\langle \text{echo}, \text{id}, x \rangle$ \textbf{to all}
\State \textbf{upon receiving} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from} $ t + 1 $ \textbf{parties}:
\State \hskip2em \textbf{if} haven’t echoed $ v $ \textbf{yet then send} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{to all}
\State \textbf{upon receiving} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from} $ n - t $ \textbf{parties}:
\State \hskip2em $ \text{approvedVals} \gets \text{approvedVals} \cup \{v\} $
\State \hskip2em \textbf{if} haven’t sent any echo2 message \textbf{yet then send} $\langle \text{echo2}, \text{id}, v \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $ |\text{approvedVals}| > 1 $ \textbf{or}
\State \hskip2em (2) received $\langle \text{echo2}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from} $ n - t $ \textbf{parties}
\State \hskip2em \textbf{if} (1) \textbf{then send} $\langle \text{echo3}, \text{id}, \bot \rangle$ \textbf{to all}
\State \hskip2em \textbf{else send} $\langle \text{echo3}, \text{id}, v \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $ |\text{approvedVals}| > 1 $ \textbf{and received echo3 messages from at least} $ n - t $ \textbf{parties or}
\State \hskip2em (2) received $\langle \text{echo3}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from at least} $ n - t $ \textbf{parties}
\State \hskip2em \textbf{if} (1) \textbf{then decide} $\bot$
\State \hskip2em \textbf{else decide} $ v $
\end{algorithmic}
\end{algorithm}


%%%%%%%%

\begin{algorithm}
\caption{Asynchronous Graded Binding Crusader Agreement for Byzantine Faults instance $\text{id}$ ($\text{GBCA}_{\text{Byz}})$ (Algorithm 6 of \cite{Abraham22crusader})}
\label{algorithm:gbcabyz}
\begin{algorithmic}[1]
\State \textbf{Input:} $ x $
\State $ \text{approvedVals} \gets \{\} $
\State \textbf{send} $\langle \text{echo}, \text{id}, x \rangle$ \textbf{to all}
\State \textbf{upon receiving} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from} $ t + 1 $ \textbf{parties}:
\State \hskip2em \textbf{if} haven’t echoed $ v $ \textbf{yet then send} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{to all}
\State \textbf{upon receiving} $\langle \text{echo}, \text{id}, v \rangle$ \textbf{for the same non-}$\bot v$ \textbf{from} $ n - t $ \textbf{parties}:
\State \hskip2em $ \text{approvedVals} \gets \text{approvedVals} \cup \{v\} $
\State \hskip2em \textbf{if} haven’t sent an echo2 message \textbf{yet then send} $\langle \text{echo2}, \text{id}, v \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $\langle \text{echo2}, \text{id}, v \rangle$ \textbf{has been received from} $ n - t $ \textbf{parties for the same non-}$\bot v$ \textbf{or}
\State \hskip2em (2) $\langle \text{echo2}, \text{id}, * \rangle$ \textbf{messages have been received from} $ n - t $ \textbf{parties and} $ |\text{approvedVals}| > 1 $
\State \hskip2em \textbf{if} 1 \textbf{then send} $\langle \text{echo3}, \text{id}, v \rangle$ \textbf{to all}
\State \hskip2em \textbf{else send} $\langle \text{echo3}, \text{id}, \bot \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $\langle \text{echo3}, \text{id}, v \rangle$ \textbf{has been received from} $ n - t $ \textbf{parties for the same non-}$\bot v$ \textbf{or}
\State \hskip2em (2) $\langle \text{echo3}, \text{id}, * \rangle$ \textbf{messages have been received from} $ n - t $ \textbf{parties and} $ |\text{approvedVals}| > 1 $
\State \hskip2em \textbf{if} (1) \textbf{then send} $\langle \text{echo4}, \text{id}, v \rangle$ \textbf{to all}
\State \hskip2em \textbf{else send} $\langle \text{echo4}, \text{id}, \bot \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $\langle \text{echo4}, \text{id}, v \rangle$ \textbf{has been received from} $ n - t $ \textbf{parties for the same non-}$\bot v$ \textbf{or}
\State \hskip2em (2) $\langle \text{echo4}, \text{id}, * \rangle$ \textbf{messages have been received from} $ n - t $ \textbf{distinct parties and} $ |\text{approvedVals}| > 1 $
\State \hskip2em \textbf{if} (1) \textbf{then send} $\langle \text{echo5}, \text{id}, v \rangle$ \textbf{to all}
\State \hskip2em \textbf{else send} $\langle \text{echo5}, \text{id}, \bot \rangle$ \textbf{to all}
\State \textbf{wait until}
\State \hskip2em (1) $\langle \text{echo5}, \text{id}, v \rangle$ \textbf{has been received from} $ n - t $ \textbf{parties for the same non-}$\bot v$ \textbf{or}
\State \hskip2em (2) $\langle \text{echo5}, \text{id}, * \rangle$ \textbf{messages have been received from at least} $ n - t $ \textbf{distinct parties, at least one of which}
\State \hskip4em \textbf{is} $\langle \text{echo5}, \text{id}, v \rangle$ \textbf{s.t.} $ v $ \textbf{is non-}$\bot$, $\langle \text{echo4}, \text{id}, v \rangle$ \textbf{messages have been received from at least} $ t + 1 $ \textbf{distinct parties,}
\State \hskip4em \textbf{and} $ |\text{approvedVals}| > 1 $ \textbf{or}
\State \hskip2em (3) $\langle \text{echo5}, \text{id}, \bot \rangle$ \textbf{messages have been received from at least} $ n - t $ \textbf{distinct parties and}
\State \hskip4em $ |\text{approvedVals}| > 1 $
\State \hskip2em \textbf{if} (1) \textbf{then decide} $ v, 2 $
\State \hskip2em \textbf{else if} (2) \textbf{then decide} $ v, 1 $
\State \hskip2em \textbf{else decide} $\bot, 0$
\end{algorithmic}
\end{algorithm}


%%%%%%%%%

\begin{algorithm}
\small
\caption{Connected Consensus algorithm with Binding for $ R = 1, 2 $ with $ n $ processes, $ f < n/3 $ of which may be malicious; code for process $ p $ (Algorithm 3 of \cite{AttiyaWelch23})}
\label{algorithm:connected-consensus}
\begin{algorithmic}[1]
\State \textbf{initially:}
\State $ \text{approved} \gets \emptyset $ (\textit{subset of} $ V \cup \{\bot\} $)
\State $ \text{num\_echo}[v] \gets 0 $ \textbf{for} $ v \in V \cup \{\bot\} $
\State $ \text{num\_echoi}[v] \gets 0 $ \textbf{for} $ 2 \leq i \leq 5, v \in V \cup \{\bot\} $
\State $ \text{sent\_echo}[v] \gets \text{false} $ \textbf{for} $ v \in V \cup \{\bot\} $
\State $ \text{sent\_echoi} \gets \text{false} $ \textbf{for} $ 2 \leq i \leq 5 $
\State $ \text{decided} \gets \text{false} $
\Comment{initialization}

\medskip
\State \textbf{wakeup:}
\State \hskip2em \textbf{send} $ \langle \text{echo}, \text{input} \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo}[\text{input}] \gets \text{true} $
\Comment{initiate echo for $ p $'s input}

\medskip
\State \textbf{receive} $ \langle \text{echo}, v \rangle $:
\State \hskip2em $ \text{num\_echo}[v] \gets \text{num\_echo}[v] + 1 $
\State \hskip2em \textbf{if} $ (\text{num\_echo}[v] = f + 1) $ \textbf{and} $ \lnot \text{sent\_echo}[v] $ \textbf{then}
\State \hskip4em \textbf{send} $ \langle \text{echo}, v \rangle $ \textbf{to all;}
\State \hskip4em $ \text{sent\_echo}[v] \gets \text{true} $
\Comment{echo $ v $ if enough support but only once}
\State \hskip2em \textbf{else if} $ (\text{sum}(\text{num\_echo}) - \text{num\_echo}[m] \geq f + 1) $ \textbf{and} $ \lnot \text{sent\_echo}[\bot] $,
\State \hskip4em \textbf{where} $ m $ \textbf{is s.t.} $ \text{num\_echo}[m] \geq \text{num\_echo}[u] $ \textbf{for all} $ u \in V \cup \{\bot\} $ \textbf{then}
\State \hskip4em \textbf{send} $ \langle \text{echo}, \bot \rangle $ \textbf{to all;}
\State \hskip4em $ \text{sent\_echo}[\bot] \gets \text{true} $
\Comment{if evidence for multiple correct inputs then initiate echo for $ \bot $}

\medskip
\State \textbf{else if} $ \text{num\_echo}[v] = n - f $ \textbf{then if} $ \lnot \text{sent\_echo2} $ \textbf{then}
\State \hskip2em \textbf{send} $ \langle \text{echo2}, v \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo2} \gets \text{true} $
\State \hskip2em \textbf{add} $ v $ \textbf{to} $ \text{approved} $
\State \hskip2em \textbf{if} $ (|\text{approved}| > 1 ) $ \textbf{and} $ \lnot \text{sent\_echo3} $ \textbf{then}
\State \hskip2em \textbf{send} $ \langle \text{echo3}, \bot \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo3} \gets \text{true} $

\medskip
\State \textbf{receive} $ \langle \text{echo2}, v \rangle $:
\State \hskip2em $ \text{num\_echo2}[v] \gets \text{num\_echo2}[v] + 1 $
\State \hskip2em \textbf{if} $ (\text{num\_echo2}[v] = n - f) $ \textbf{and} $ \lnot \text{sent\_echo3} $ \textbf{then}
\State \hskip2em \textbf{send} $ \langle \text{echo3}, v \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo3} \gets \text{true} $

\medskip
\State \textbf{receive} $ \langle \text{echo3}, v \rangle $:
\State \hskip2em $ \text{num\_echo3}[v] \gets \text{num\_echo3}[v] + 1 $
\State \hskip2em \textbf{if} $ (\text{sum}(\text{num\_echo3}) \geq n - f ) $ \textbf{and} $ (|\text{approved}| > 1 $ \textbf{or} $ \bot \in \text{approved}) $ \textbf{then}
\State \hskip4em \textbf{if} $ (R = 1) $ \textbf{and} $ \lnot \text{decided} $ \textbf{then}
\State \hskip6em \textbf{decide} $ (\bot, 0) $; $ \text{decided} \gets \text{true} $
\State \hskip4em \textbf{else if} $ (R = 2) $ \textbf{and} $ \lnot \text{sent\_echo4} $ \textbf{then}
\State \hskip6em \textbf{send} $ \langle \text{echo4}, \bot \rangle $ \textbf{to all;}
\State \hskip6em $ \text{sent\_echo4} \gets \text{true} $
\State \hskip2em \textbf{else if} $ \text{num\_echo3}[v] \geq n - f $ \textbf{then if} $ (R = 1) $ \textbf{and} $ \lnot \text{decided} $ \textbf{then}
\State \hskip4em \textbf{decide} $ (v, 1) $; $ \text{decided} \gets \text{true} $
\State \hskip4em \textbf{else if} $ (R = 2) $ \textbf{and} $ \lnot \text{sent\_echo4} $ \textbf{then}
\State \hskip6em \textbf{send} $ \langle \text{echo4}, v \rangle $ \textbf{to all;}
\State \hskip6em $ \text{sent\_echo4} \gets \text{true} $

\medskip
\State \textbf{receive} $ \langle \text{echo4}, v \rangle $:
\State \hskip2em $ \text{num\_echo4}[v] \gets \text{num\_echo4}[v] + 1 $
\State \hskip2em \textbf{if} $ (\text{num\_echo4}[v] = n - f) $ \textbf{and} $ \lnot \text{sent\_echo5} $ \textbf{then}
\State \hskip2em \textbf{send} $ \langle \text{echo5}, v \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo5} \gets \text{true} $
\State \hskip2em \textbf{else if} $ (\ \text{sum}(\text{num\_echo4}) \geq n - f ) $ \textbf{and} $ (|\text{approved}| > 1 $ \textbf{or} $ \bot \in \text{approved}) $ \textbf{and} $ \lnot \text{sent\_echo5} $ \textbf{then}
\State \hskip2em \textbf{send} $ \langle \text{echo5}, \bot \rangle $ \textbf{to all;}
\State \hskip2em $ \text{sent\_echo5} \gets \text{true} $

\medskip
\State \textbf{receive} $ \langle \text{echo5}, v \rangle $:
\State \hskip2em $ \text{num\_echo5}[v] \gets \text{num\_echo5}[v] + 1 $
\State \hskip2em \textbf{if} $ \lnot \text{decided} $ \textbf{then}
\State \hskip4em \textbf{if} $ (v \in V) $ \textbf{and} $ (\text{num\_echo5}[v] \geq n - f) $ \textbf{then}
\State \hskip6em \textbf{decide} $ (v, 2) $; $ \text{decided} \gets \text{true} $
\State \hskip4em \textbf{else if} $ (\text{sum}(\text{num\_echo5}) \geq n - f ) $ \textbf{and} $ (|\text{approved}| > 1 $ \textbf{or} $ \bot \in \text{approved}) $ \textbf{and}
\State \hskip6em \textbf{there exists} $ w \in V $ \textbf{s.t.} $ (\text{num\_echo5}[w] \geq 1) $ \textbf{and} $ (\text{num\_echo4}[w] \geq f + 1) $ \textbf{then}
\State \hskip6em \textbf{decide} $ (w,1) $; $ \text{decided} \gets \text{true} $
\State \hskip4em \textbf{else if} $ \text{num\_echo5}[\bot] \geq n - f $ \textbf{then}
\State \hskip6em \textbf{decide} $ (\bot, 0) $
\end{algorithmic}
\end{algorithm}




==> sections/crux_proof_main_body.tex <==
\subsection{\block's Correctness \& Complexity} \label{subsection:block_correctness_complexity}

This subsection gives a proof of the following theorem:

\begin{theorem} \label{theorem:block}
\Cref{algorithm:block} satisfies the specification of \block.
Moreover, correct processes collectively send
\begin{equation*}
    \mathit{bit}(\block) = \mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B} \text{ bits, where}
\end{equation*}
\begin{compactitem}
    \item $\mathit{bit}(\mathcal{X})$ denotes the number of bits sent in $\mathcal{X} \in \{\mathcal{GC}_1, \mathcal{GC}_2, \mathcal{VB}\}$ (see \Cref{subsection:graded_consensus_building_blocks} and \Cref{subsection:validation_broadcast_building_blocks})
    
    \item $\mathcal{B}$ denotes the maximum number of bits any correct process sends in $\mathcal{BA}^S$.
\end{compactitem}
%(1) $\mathit{bit}(\mathcal{GC}_1)$ denotes the number of bits sent in $\mathcal{GC}_1$, (2) $\mathit{bit}(\mathcal{GC}_2)$ denotes the number of bits sent in $\mathcal{GC}_2$, (3) $\mathit{bit}(\mathcal{VB})$ denotes the number of bits sent in $\mathcal{VB}$, and (4) $\mathcal{B}$ denotes the maximum number of bits any correct process sends in $\mathcal{BA}^S$.
\end{theorem}

% A formal proof of \Cref{theorem:block} is relegated to \Cref{appendix:proof}.
% The rest of the subsection informally shows how each of the \block's properties is satisfied, and argues about \block's complexity.
We start by proving strong validity.

\begin{theorem} [Strong validity]
\block satisfies strong validity.
\end{theorem}
\begin{proof}
Suppose that all correct processes that propose to \block do propose the same value $v$.
This implies that all correct processes that propose to $\mathcal{GC}_1$ do so with $v$ (Step 1 of Task 1).
Hence, due to the strong validity property of $\mathcal{GC}_1$, every correct process that decides from $\mathcal{GC}_1$ decides $(v, 1)$.
Therefore, every correct process $p_i$ sets its $\mathit{est}_i$ local variable to $v$ (Step 3 of Task 1), and proposes $v$ to $\mathcal{GC}_2$ (Step 4 of Task 1).
The strong validity property of $\mathcal{GC}_2$ further ensures that every correct process that decides from $\mathcal{GC}_2$ does decide $(v, 1)$ (Step 4 of Task 1), which implies that no correct process decides any value $v' \neq v$ from \block (Step 5 of Task 1).
Furthermore, every correct process that broadcasts using the $\mathcal{VB}$ primitive does broadcast $v$ (Step 6 of Task 1).
Due to the strong validity property of $\mathcal{VB}$, no correct process validates any value $v' \neq v$ (Step 1 of Task 3), thus ensuring strong validity.
\end{proof}

%\pierre{I would merge theorems about external validity, integrity, and completion time, with a very short proof.}\pierre{Not anymore if we do not care about the page limit}

Next, we prove external validity.
\begin{theorem} [External validity]
\name satisfies external validity.
\end{theorem}
\begin{proof}
At the end of Step 3 of Task 1, the $\mathit{est}_i$ local variable of every correct process $p_i$ contains a valid value.
Let us consider all three possibilities for $p_i$ to update its $\mathit{est}_i$ local variable (according to the logic of Step 3):
\begin{compactitem}
    \item Process $p_i$ decided $(\mathit{est}_i, 1)$ from $\mathcal{GC}_1$.
    In this case, $\mathit{est}_i$ is valid due to the external validity property of $\mathcal{GC}_1$.
    % As no correct process proposes an invalid value to $\mathcal{GC}_1$ (given that no correct process proposes an invalid value to \block), the safety property of $\mathcal{GC}_1$ guarantees that $\mathit{est}_i$ is proposed by a/ correct process.
    % Hence, $\mathit{est}_i$ is valid.

    \item Process $p_i$ decided $(\cdot, 0)$ from $\mathcal{GC}_1$, and decided $\mathit{est}_i \neq \bot$ from $\mathcal{BA}^S$.
    Prior to updating the $\mathit{est}_i$ local variable, $p_i$ checks that the value is valid, thus ensuring that the statement holds in this case.
b
    \item Process $p_i$ updates $\mathit{est}_i$ to its proposal to \block.
    In this case, $\mathit{est}_i$ is valid as no correct process proposes an invalid value to \block.
\end{compactitem}
Therefore, every correct process that proposes to $\mathcal{GC}_2$ does propose a valid value (Step 4 of Task 1).
If any correct process $p_i$ decides $(v_2, 1)$ from $\mathcal{GC}_2$ (thus, deciding $v_2$ from \block in Step 5), then $v_2$ is a valid value due to the external validity property of $\mathcal{GC}_2$.
Similarly, if any correct process validates any value from \block (Step 1 of Task 3), then that value is valid due to the external validity property of $\mathcal{VB}$ (all correct processes that broadcast via $\mathcal{VB}$ do so with valid values due to the external validity property of $\mathcal{GC}_2$).
\end{proof}

The following theorem proves the agreement property.

\begin{theorem} [Agreement]
\block satisfies agreement.
\end{theorem}
\begin{proof}
No two correct processes decide different values from \block (Step 5 of Task 1) due to the consistency property of $\mathcal{GC}_2$.
Moreover, if a correct process decides some value $v$ from \block (Step 5 of Task 1), every correct process that broadcasts via $\mathcal{VB}$ does broadcast value $v$ (ensured by the consistency property of $\mathcal{GC}_2$).
Thus, the strong validity property of $\mathcal{VB}$ ensures that no correct process validates any value $v' \neq v$ from \block (Step 1 of Task 3).
\end{proof}

Next, we prove the integrity property of \block.

\begin{theorem} [Integrity]
\block satisfies integrity.
\end{theorem}
\begin{proof}
Any correct process $p_i$ decides or completes \block only in Task 1 (see Task 1). 
As $p_i$ starts executing Task 1 only after it has proposed to \block, the integrity property is satisfied.
\end{proof}

Next, we prove the termination property.

\begin{theorem} [Termination]
\block satisfies termination.
\end{theorem}
\begin{proof}
Suppose that all correct processes propose to \block and no correct process ever abandons \block.
Hence, every correct process proposes to $\mathcal{GC}_1$ (Step 1 of Task 1), and no correct process ever abandons it.
Thus, every correct process decides from $\mathcal{GC}_1$ (due to the termination property of $\mathcal{GC}_1$), and proposes to $\mathcal{BA}^S$ (Step 2 of Task 1).
As every correct process executes $\mathcal{BA}^S$ for exactly $\mathcal{R}$ synchronous rounds, every correct process eventually concludes Step 2 of Task 1.
Therefore, every correct process proposes to $\mathcal{GC}_2$ (Step 4 of Task 1), and no correct process ever abandons it.
Hence, the termination property of $\mathcal{GC}_2$ ensures that every correct process decides from $\mathcal{GC}_2$, which implies that every correct process broadcasts its decision via $\mathcal{VB}$ (Step 6 of Task 1).
Finally, as no correct process ever abandons $\mathcal{VB}$, every correct process eventually receives a $\mathsf{completed}$ indication from $\mathcal{VB}$ (Step 6 of Task 1), which implies that every correct process completes \block (Step 7 of Task 1).
\end{proof}

The following theorem proves totality.

\begin{theorem} [Totality]
\block satisfies totality.
\end{theorem}
\begin{proof}
Suppose that a correct process receives a $\mathsf{completed}$ indication from \block at some time $\tau$ (Step 7 of Task 1).
Hence, that correct process has received a $\mathsf{completed}$ indication from $\mathcal{VB}$ at time $\tau$ (Step 6 of Task 1).
Therefore, the totality property of $\mathcal{VB}$ ensures that every correct process validates a value from $\mathcal{VB}$ by time $\max(\tau, \text{GST}) + 2\delta$.
Therefore, every correct process validates a value from \block by time $\max(\tau, \text{GST}) + 2\delta$ (Step 1 of Task 3).
\end{proof}

We now prove the synchronicity property of \block.

\begin{theorem} [Synchronicity]
\block satisfies synchronicity.
\end{theorem}
\begin{proof}
Suppose that $\tau$ denotes the first time a correct process proposes to \block.
Moreover, suppose that (1) $\tau \geq \text{GST}$, (2) all correct processes propose to \block by time $\tau + \Delta_{\mathit{shift}}$, and (3) no correct process abandons \block by time $\tau + \Delta_{\mathit{total}}$.
(Hence, let the precondition of the synchronicity property be satisfied.)

As $\mathcal{GC}_1$ terminates in $\mathit{round}(\mathcal{GC}_1)$ asynchronous rounds, every correct process decides from $\mathcal{GC}_1$ by time $\tau + \Delta_{\mathit{shift}} + \Delta_1$ (as all correct processes overlap for $\Delta_1 = \mathit{round}(\mathcal{GC}_1) \cdot \delta$ time in $\mathcal{GC}_1$).
Moreover, all correct processes start executing $\mathcal{BA}^S$ within $\Delta_{\mathit{shift}}$ time of each other (as they execute $\mathcal{GC}_1$ for at least $\Delta_{\mathit{shift}} + \Delta_1$ time even if they decide from $\mathcal{GC}_1$ before).
As $\mathcal{BA}^S$ is executed after GST with the round duration of $\Delta_{\mathit{shift}} + \delta$ time \pierre{do not forget applying the modification due to \Cref{lemma:simulation_correct}, i.e. round duration of $2\Delta_{\mathit{shift}} + \delta$, applied to \block as well}, $\mathcal{BA}^S$ exhibits a valid synchronous execution.
Hence, all correct process decide the same valid (non-$\bot$) value from $\mathcal{BA}^S$ by time $\tau + (\Delta_{\mathit{shift}} + \Delta_1) + \mathcal{R}(\Delta_{\mathit{shift}} + \delta)$.
\replace{To prove the synchronicity property of \block, we show that the $\mathit{est}_i$ local variable of any correct process $p_i$ and the $\mathit{est}_j$ local variable of any other correct process $p_j$ have the same value at the end of Step 3 of Task 1}{
To prove \block's synchronicity property, we show that, at the end of Task 1's Step 3, the local variables $\mathit{est}_i$ and $\mathit{est}_j$ of any pair of correct processes $p_i$ and $p_j$, respectively, are identical.}:
\begin{compactitem}
    \item \add{Assume a correct process $p_i$ decides $\mathit{est}_i$ with grade $1$ from $\mathcal{GC}_1$ (Step 1 of Task 1). Hence, by consistency property of $\mathcal{GC}_1$, all correct processes have decided $(\mathit{est}_i, \cdot)$ from $\mathcal{GC}_1$, and then have proposed $\mathit{est}_i$ to $\mathcal{BA}^S$.
    As $\mathcal{BA}^S$ satisfies strong validity, every correct process $p_j$ decides $\mathit{est}_i$ from $\mathcal{BA}^S$.
    As stated above, $\mathit{est}_i \neq \bot$ and $\mathsf{valid}(\mathit{est}_i) = \mathit{true}$. Let $p_j$ be a correct process.
    \begin{compactitem}
    \item  If process $p_j$ has decided $(\mathit{est}_i, 1)$ from $\mathcal{GC}_1$, it applies $\mathit{est}_j \gets \mathit{est}_i$ as the output of $\mathcal{GC}_1$
    \item  If process $p_j$ has decided $(\mathit{est}_i, 0)$ from $\mathcal{GC}_1$, it applies $\mathit{est}_j \gets \mathit{est}_i$ as the output of $\mathcal{BA}^S$
    \end{compactitem}
    In both cases, $\mathit{est}_i = \mathit{est}_j$, at the end of Task 1's Step 3.

    \item Let both $p_i$ and $p_j$ decide with grade $0$ from $\mathcal{GC}_1$ (Step 1 of Task 1).
    In this case, $\mathit{est}_i = \mathit{est}_j$ due to the agreement property of $\mathcal{BA}^S$.
    }

    \item Let both $p_i$ and $p_j$ decide with grade $1$ from $\mathcal{GC}_1$ (Step 1 of Task 1).
    In this case, $\mathit{est}_i = \mathit{est}_j$ due to the consistency property of $\mathcal{GC}_1$, which proves that $\mathit{est}_i = \mathit{est}_j$.

    \item Let $p_i$ decide with grade $1$ from $\mathcal{GC}_1$, whereas $p_j$ decides with grade $0$ from $\mathcal{GC}_1$ (Step 1 of Task 1).
    Moreover, let $p_j$ decide $v'$ from $\mathcal{BA}^S$ (Step 2 of Task 1).
    As stated above, $v' \neq \bot$ and $\mathsf{valid}(v') = \mathit{true}$.
    % As $\mathcal{SBA}$ exhibits a valid execution, $\mathit{val}' \neq \bot$ and $\mathsf{valid}(\mathit{val}') = \mathit{true}$, i.e., $p_j$ decides a valid value from $\mathcal{SBA}$.
    Moreover, as $p_i$ decided $\mathit{est}_i$ with grade $1$ from $\mathcal{GC}_1$, all correct processes have decided $(\mathit{est}_i, \cdot)$ from $\mathcal{GC}_1$ (due to the consistency property of $\mathcal{GC}_1$).
    Therefore, all correct processes propose $\mathit{est}_i$ to $\mathcal{BA}^S$.
    As $\mathcal{BA}^S$ satisfies strong validity, $v' = \mathit{est}_i$, which proves that $\mathit{est}_i = \mathit{est}_j$.

    \item Let both $p_i$ and $p_j$ decide with grade $0$ from $\mathcal{GC}_1$ (Step 1 of Task 1).
    In this case, $\mathit{est}_i = \mathit{est}_j$ due to the agreement property of $\mathcal{BA}^S$.
\end{compactitem} 
Thus, all correct processes propose to $\mathcal{GC}_2$ the same valid value $v$, and they do so within $\Delta_{\mathit{shift}}$ time of each other.
Every correct process decides $(v, 1)$ by time $\tau + (\Delta_{\mathit{shift}} + \Delta_1) + \mathcal{R}(\Delta_{\mathit{shift}} + \delta) + (\Delta_{\mathit{shift}} + \Delta_2)$ as $\Delta_2 = \mathit{round}(\mathcal{GC}_2) \cdot \delta$; $v$ is decided with grade $1$ due to the strong validity property of $\mathcal{GC}_2$.
Therefore, every correct process decides (Step 5 of Task 1) by time $\tau + \Big( \Delta_{\mathit{shift}} + \Delta_1 \Big) + \Big( \mathcal{R} \cdot (\Delta_{\mathit{shift}} + \delta) \Big) + \Big( \Delta_{\mathit{shift}} + \Delta_2 \Big) = \tau + \Delta_{\mathit{total}}$, thus ensuring synchronicity.
\end{proof}

We now prove the last property of \block.

\begin{theorem} [Completion time]
\block satisfies completion time.
\end{theorem}
\begin{proof}
This property is ensured as every correct process incorporates a ``waiting step'' when executing $\mathcal{GC}_1$ (Step 1 of Task 1), $\mathcal{BA}^S$ (Step 2 of Task 1) and $\mathcal{GC}_2$ (Step 4 of Task 1).
\end{proof}

Finally, we prove the complexity of \block.

\begin{theorem} [Complexity]
Correct processes collectively send
\begin{equation*}
    \mathit{bit}(\block) = \mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B} \text{ bits.}
\end{equation*}
\end{theorem}
\begin{proof}
Correct processes collectively send (1) $\mathit{bit}(\mathcal{GC}_1)$ bits in $\mathcal{GC}_1$, (2) $\mathit{bit}(\mathcal{GC}_2)$ bits in $\mathcal{GC}_2$, and (3) $\mathit{bit}(\mathcal{VB})$ in $\mathcal{VB}$.
Moreover, each correct process sends at most $\mathcal{B}$ bits in $\mathcal{BA}^S$.
Therefore, correct processes collectively send $\mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B}$ bits.
\end{proof}

==> sections/former/algorithm.tex <==
\section{\name: Pseudocode \& Analysis}

\subsection{View Synchronization}

\begin{algorithm}
\caption{View Synchronization: Pseudocode (for process $P_i$)}
\label{algorithm:view_synchronization}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$
\State \hskip2em $\mathsf{Timer}$ $\mathit{view\_timer}_i$

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathit{view\_duration} \gets \Delta + 2\delta$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Epoch}$ $\mathit{epoch}_i \gets 1$
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$
\State \hskip2em $\mathit{view\_timer}_i.\mathsf{measure}(\mathit{view\_duration})$
\State \hskip2em \textbf{trigger} $\mathsf{advance}\big( 1 \big)$

\medskip
\State \textbf{upon} $\mathit{view\_timer}_i$ \textbf{expires}:
\State \hskip2em \textbf{if} $\mathit{view}_i < t + 1$:
\State \hskip4em $\mathit{view}_i \gets \mathit{view}_i + 1$
\State \hskip4em $\mathit{view\_timer}_i.\mathsf{measure}(\mathit{view\_duration})$
\State \hskip4em \textbf{trigger} $\mathsf{advance}\big( (\mathit{epoch}_i - 1)(t + 1) + \mathit{view}_i \big)$
\State \hskip2em \textbf{else:}
\State \hskip4em \textbf{trigger} $\mathit{brb}.\mathsf{broadcast}\big( \langle \textsc{epoch-complete}, \mathit{epoch}_i \rangle \big)$

\medskip
\State \textbf{upon} exists $\mathsf{Epoch}$ $e > \mathit{epoch}_i$ such that $\langle \textsc{epoch-complete}, e \rangle$ is received from $2t + 1$ processes:
\State \hskip2em $\mathit{view}_i \gets 1$
\State \hskip2em $\mathit{epoch}_i \gets e$
\State \hskip2em $\mathit{view\_timer}_i.\mathsf{measure}(\mathit{view\_duration})$
\State \hskip2em \textbf{trigger} $\mathsf{advance}\big( (\mathit{epoch}_i - 1)(t + 1) + \mathit{view}_i \big)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\name: Pseudocode (for process $P_i$)}
\label{algorithm:name}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em View Synchronization with $\Delta = 8\delta$, \textbf{instance} $\mathit{sync}$
\State \hskip2em Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets \bot$
\State \hskip2em $\mathsf{Value}$ $\mathit{locked\_value}_i \gets \bot$
\State \hskip2em $\mathsf{View}$ $\mathit{locked\_view}_i \gets \bot$
\State \hskip2em $\mathsf{Value}$ $\mathit{valid\_value}_i \gets \bot$
\State \hskip2em $\mathsf{View}$ $\mathit{valid\_view}_i \gets \bot$

\medskip
\State \textbf{upon} $\mathsf{propose}(\mathsf{Value} \text{ } proposal)$: 
\State \hskip2em $\mathit{proposal}_i \gets \mathit{proposal}$

\medskip
\State \textbf{upon} $\mathit{brb}.\mathsf{deliver}\big( \textsc{proposal}, \mathit{proposal}, \cdot \big)$, where the message is associated with some view $V > \mathit{valid\_view}_i$:
\State \hskip2em $\mathit{valid\_value}_i \gets \mathit{proposal}$
\State \hskip2em $\mathit{valid\_view}_i \gets V$

\medskip
\State \textbf{upon} $\mathit{sync}.\mathsf{advance}(\mathsf{View} \text{ } v)$:
\State \hskip2em \textbf{wait} $4\delta$ \BlueComment{wait to potentially update $\mathit{valid\_value}_i$ and $\mathit{valid\_view}_i$}

\smallskip
\State \hskip2em \textbf{if} $P_i = \mathsf{leader}(v)$:
\State \hskip4em $\mathsf{Value}$ $\mathit{proposal} \gets \mathit{proposal}_i$
\State \hskip4em \textbf{if} $\mathit{valid\_value}_i \neq \bot$:
\State \hskip6em $\mathit{proposal} \gets \mathit{valid\_value}_i$
\State \hskip4em \textbf{trigger} $\mathit{brb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, \mathit{proposal}, \mathit{valid\_view}_i \rangle \big)$

\smallskip
\State \hskip2em \textbf{upon} $\mathit{brb}.\mathsf{deliver}\big( \langle \textsc{proposal}, \mathit{proposal}, * \rangle \big)$:
\State \hskip4em $\mathit{locked\_value}_i \gets \mathit{proposal}$
\State \hskip4em $\mathit{locked\_view}_i \gets v$
\State \hskip4em $\mathit{valid\_value}_i \gets \mathit{proposal}$
\State \hskip4em $\mathit{valid\_view}_i \gets v$
\State \hskip4em \textbf{broadcast} $\langle \textsc{commit}, \mathit{locked\_value}_i \rangle$

\smallskip
\State \hskip2em \textbf{upon} exists $\mathsf{Value}$ $\mathit{dec}$ such that $2t + 1$ $\langle \textsc{commit}, \mathit{dec} \rangle$ is received:
\State \hskip4em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$
\end{algorithmic}
\end{algorithm}

In \Cref{algorithm:name}, we rely on the Byzantine reliable broadcast primitive.
However, we modify this primitive in the following way: a correct process $P$ echoes a received $\langle \textsc{proposal}, v, \mathit{vv} \rangle$ message if and only if (1) $P$ has previously reliably delivered the $\langle \textsc{proposal}, v, \cdot \rangle$ message associated with the view $\mathit{vv}$, and (2) $\mathit{vv} \geq \mathit{locked\_view}_i$.
Hence, the utilized variant of the reliable broadcast primitive ensures the following properties:
\begin{compactitem}
    \item \emph{Agreement:} If a correct process reliably delivers a message $m$ associated with some view $V$, and another correct process reliably delivers a message $m'$ associated with $V$, then $m = m'$.

    \item \emph{Validity:} If a correct process reliably broadcasts a message associated with some view $V$ at some time $\tau$, then that process eventually reliably delivers a message associated with $V$, and it does so by time $\max(\text{GST}, \tau) + 3\delta$.

    \item \emph{Totality:} If a correct process reliably delivers a message associated with some view $V$ at some time $\tau$, then all correct process eventually reliably deliver a message associated with $V$, and they all do so by time $\max(\text{GST}, \tau) + 2\delta$.
\end{compactitem}

\begin{lemma} \label{lemma:agreement_1}
Let a correct process $P$ decide a value $v$ in some view $V$.
Moreover, let a correct process $Q$ decide a value $v'$ in $V$.
Then, $v = v'$.
\end{lemma}
\begin{proof}
Follows from the fact that no correct process broadcasts a \textsc{commit} message more than once in a view.
\end{proof}

\begin{lemma} \label{lemma:agreement_2}
Let a correct process $P$ decide a value $v$ in some view $V$.
Then, no correct process reliably delivers a \textsc{proposal} message for any other value in any view $V' > V$.
\end{lemma}
\begin{proof}
Follows directly from the properties of the reliable broadcast primitive.
\end{proof}

\begin{theorem}
\name satisfies agreement.
\end{theorem}
\begin{proof}
Follows directly from \cref{lemma:agreement_1,lemma:agreement_2}.
\end{proof}



==> sections/former/application.tex <==
\section{Our Results in the Wild}

In this section, we investigate some well-studied validity properties. 
Specifically, we study the consequences our findings yield when applied to specific validity properties.

\subsection{Our Results in the Context of Well-Studied Validity Properties}

\paragraph{Strong Validity}
Recall that \emph{Strong Validity}~\cite{CGL18,civit2022byzantine,Momose2021} states that, if all correct processes propose the same value, only that value can be decided.
Observe that \emph{Strong Validity} is a non-trivial validity property.
As such, due to \Cref{theorem:triviality_main}, \emph{Strong Validity} is unsolvable with $n \leq 3t$.

Moreover, Dolev-Reischuk bound states that \emph{Strong Validity} requires $\Omega(t^2)$ messages (and words) to be sent by correct processes.
When $O(t) = O(n)$, the bound is tight: Civit \emph{et al.}~\cite{civit2022byzantine} introduced \textsc{Squad}, a Byzantine consensus algorithm with \emph{Strong Validity}, which achieves $O(n^2)$ message and communication complexities.
In this paragraph, we show that the structure of \textsc{Squad} is similar to the structure of our general algorithm.

\textsc{Squad} is built on top of \textsc{Quad}.
The authors assume an existence of a $(n - 2t, n)$-threshold signature scheme~\cite{libert2014born}.
In a nutshell, these are the steps taken by a correct process $P_i$ in \textsc{Squad}:
\begin{compactenum}
    \item Process $P_i$ broadcasts its proposal $v \in \mathcal{V}_I$, which is share-signed by $P_i$ (with the threshold $n - 2t$).

    \item Once $P_i$ collects $n - t$ proposals, it checks whether there exists a proposal $v^*$ sent by (at least) $n - 2t$.
    
    \begin{compactenum}
        \item If there is, $P_i$ creates a constant-sized threshold signature $\sigma^*$ and proposes $(v^*, \sigma^*)$ to \textsc{Quad}.

        \item Otherwise:
        \begin{compactenum}
            \item $P_i$ broadcasts a predetermined string ``any value'', which is share-signed by $P_i$ (with the threshold $n - 2t$).

            \item $P_i$ waits to obtain either a ``positivity'' proof $\sigma_p$ for some value $v_p$ ($n - 2t$ identical proposals for $p$) or a ``negativity'' proof $\sigma_n$ ($n - 2t$ ``any value'' messages).
            Once this happens, $P_i$ either proposes (1) $(v_p, \sigma_p)$, or (2) $(\mathit{default\_value}, \sigma_n)$ to \textsc{Quad}.
        \end{compactenum}
    \end{compactenum}
\end{compactenum}
Importantly, the pre-processing phase of \textsc{Squad} exists solely for ensuring that the proofs forwarded to \textsc{Quad} are of constant size.
Hence, the structure of \textsc{Squad} is similar to the structure of our general algorithm.
Indeed, our Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} could be modified (in the same way as the pre-processing phase of \textsc{Squad}) to allow constant-sized proofs in the case of \emph{Strong Validity}.

\paragraph{Weak Validity}
\emph{Weak Validity} says that, if all processes are correct and propose the same value, only that value can be decided.
As \emph{Weak Validity} is non-trivial, it cannot be solved with $n \leq 3t$ (by \Cref{theorem:triviality_main}).
Note that \textsc{Quad}~\cite{civit2022byzantine}, a Byzantine consensus algorithm with \emph{Weak Validity}, achieves $O(n^2)$ message and communication complexities.
However, until now, it was not known what the lower bound on message and communication complexities was for Byzantine consensus algorithm with \emph{Weak Validity}.
As we show, the lower bound are $\Omega(t^2)$, which further proves that \textsc{Quad} is indeed optimal (as $t = O(n)$ in \textsc{Quad}).

\paragraph{From-Correct Validity}
Thus far, we have not mentioned \emph{From-Correct Validity}.
\begin{compactitem}
    \item \emph{From-Correct Validity:} If a correct process decides a value $v$, then $v$ was proposed by a correct process.
\end{compactitem}
This validity property was used to define the \emph{strong consensus} problem~\cite{fitzi2003efficient}.

In their paper~\cite{fitzi2003efficient}, Fitzi and Garay show that Byzantine consensus algorithm with \emph{From-Correct Validity} is exists if and only if $n > (|\mathcal{D}| + 1)t$, where $\mathcal{D} = |\mathcal{V}_I|$.
We now show the same result using our formalism.

\begin{theorem} [new proof]
Solving the Byzantine consensus problem with \emph{From-Correct Validity} is possible if and only if $n > (d + 1)t$, where $d = |\mathcal{V}_I| = |\mathcal{V}_O|$.
\end{theorem}
\begin{proof}
First, we show that, if $n \leq (d + 1)t$, it is impossible to solve the Byzantine consensus problem with \emph{From-Correct Validity}.
By contradiction, suppose that it is possible to solve the Byzantine consensus problem with \emph{From-Correct Validity} with $n \leq (d + 1)t$.
Let $\mathit{base} \in \mathcal{I}$ be an input configuration such that (1) $|\mathit{base}| = n - t$, and (2) no proposal $v \in \mathcal{V}_I$ appears with more than $t$ processes in $\mathit{base}$; note that we can construct $\mathit{base}$ as $n - t \leq dt$.
For every value $v \in \mathcal{V}_I$, we construct an input configuration $c_v \in \mathcal{I}$ in the following way:
\begin{compactenum}
    \item Let $c_v \gets \mathit{base}$.

    \item We remove from $c_v$ all process-proposal pairs $\mathit{pp}$ with $\mathsf{proposal}(\mathit{pp}) = v$.

    \item For every process $P \notin \processes{\mathit{base}}$, we add $(P, v')$ to $c_v$, where $v' \neq v$.
\end{compactenum}
For every input configuration $c_v$, (1) $c_v \sim \mathit{base}$, and (2) $\text{\emph{From-Correct Validity}}(c_v) = \mathcal{V}_O \setminus{\{v\}}$.
Hence, \emph{From-Correct Validity} does not satisfy $\mathcal{C}_S$, which contradicts \Cref{theorem:similarity_condition_necessary}.
Thus, it is impossible that $n \leq (d + 1)t$.
\end{proof}

\subsection{On External Validity}


==> sections/former/byzantine.tex <==
\section{Validity Properties in the Byzantine Failure Model}

In this section, we investigate the validity properties of the consensus problem in the Byzantine failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can be Byzantine.
If a process is Byzantine, the process is \emph{faulty}; otherwise, the process is \emph{correct}.

\paragraph{Byzantine consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the Byzantine failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two correct processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, x]$, (2) $x \geq n - f$, and (3) every process-proposal pair is associated with a distinct process.
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$; if such process-proposal does not exist, $\mathit{input}[i] = \bot$.
% Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \,|\, (P, *) \text{ belongs to } \mathit{input}\}$ denotes the set of correct processes as established by $\mathit{input}$.
% Lastly, we define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\mathit{false}, \mathit{true}\}$ such that $\mathit{identical\_proposals}(i_1 \in \mathcal{I}, i_2 \in \mathcal{I}) = \top$ if and only if every process is associated with the same proposal in both $i_1$ and $i_2$.

By slightly abusing the notation, for any two input configurations $i_1, i_2 \in \mathcal{I}$, we define $i_1 \subseteq i_2$ in the following manner:
\begin{equation*}
    i_1 \subseteq i_2 \iff \forall j \in [1, n]: i_1[j] \neq \bot \implies i_2[j] = i_1[j].
\end{equation*}
In other words, $i_1 \subseteq i_2$ if and only if, the set that corresponds to the input configuration $i_1$ is a subset of the set that corresponds to the input configuration $i_2$.

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a Byzantine consensus algorithm $\mathcal{A}_B$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_B$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_B$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}

\subsection{Synchronous Environments}

First, we investigate validity properties of Byzantine consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
We start by introducing the \emph{Byzantine containment condition}.

\begin{definition} [Byzantine containment condition] \label{definition:Byzantine_containment}
Let $\mathit{val}$ be a validity property.
We say that $\mathit{val}$ satisfies the \emph{Byzantine containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: i_1 \subseteq i_2 \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
\end{definition}

We now show that the Byzantine containment condition (\Cref{definition:Byzantine_containment}) is necessary for a validity property to be satisfiable in a Byzantine environment.

\begin{lemma} [Byzantine containment condition is necessary] \label{lemma:byzantine_containment_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine containment condition.
No algorithm (even if synchronous) solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine containment condition, there exist two input configuration $i_1, i_2 \in \mathcal{I}$ such that (1) $i_1 \subseteq i_2$, and (2) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a Byzantine algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_B$ be a synchronous algorithm.

Since $\mathcal{A}_B$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_B$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first correct process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_B$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_B$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
We now show that the Byzantine containment condition is sufficient for a validity property to be satisfiable in a Byzantine setting.

\begin{theorem} [Byzantine containment condition is sufficient]
Let $\mathit{val}$ be a validity property that satisfies the Byzantine containment condition.
There exists an algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves $\mathit{val}$.

Before devising $\mathcal{A}_B$, we are implementing a synchronous Byzantine-tolerant consensus algorithm $\mathcal{A}_{\mathit{correct}}$ in which processes agree on an input configuration.
Specifically, $\mathcal{A}_{\mathit{correct}}$ satisfies the following validity property:
\begin{compactitem}
    \item \emph{All-correct validity:} Let the decided value be $i = \big[ (P_{i_1}, v_{i_1}), (P_{i_2}, v_{i_2}), ..., (P_{i_x}, v_{i_x}) \big]$.
    Then, for every correct process $P_x$, $(P_x, v_x)$ belongs to $i$, where $v_x$ is the proposed value by $P_x$.
\end{compactitem}
Intuitively, $\mathcal{A}_{\mathit{correct}}$ allows correct processes to agree on the input configuration that contains \emph{all} process-proposals associated with correct processes.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_{\mathit{correct}}$ that solves consensus with all-correct validity: Pseudocode for process $P_i$}
\label{algorithm:a_correct}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathit{brb}, \mathsf{broadcast}([\textsc{proposal}, \mathit{proposal}]) \rangle$

\medskip
\LineComment{$\mathit{brb}$ is implemented using synchronous HotStuff protocol accompanied by the certification phase given in the DISC submission}
\State \textbf{At time $8(f + 1)\Delta + 3\Delta$:} \label{line:decide_all_correct}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\text{the input configuration built out of all delivered \textsc{proposal} messages})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_{\mathit{correct}}$ (\Cref{algorithm:a_correct}) solves the Byzantine consensus problem with all-correct validity:
\begin{compactitem}
    \item Termination: Termination holds as every correct process decides at time $8(f + 1)\Delta + 3\Delta$ (line~\ref{line:decide_all_correct}).
    
    \item Agreement: Agreement follows from the agreement property of $\mathit{brb}$ and the fact that, if a correct process delivers a message from $\mathit{brb}$, it does so by time $8(f + 1)\Delta + 3\Delta$.
    
    \item All-correct validity: Follows from the validity property of $\mathit{brb}$ and the fact that a message $\mathit{brb}$-broadcast by a correct process is $\mathit{brb}$-delivered by time $8(f + 1)\Delta + 3\Delta$.
\end{compactitem}

Finally, we are ready to present $\mathcal{A}_B$.

\begin{algorithm}
\caption{Byzantine-tolerant algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Byzantine-Tolerant Consensus with All-Correct Validity, \textbf{instance} $\mathcal{A}_{\mathit{correct}}$
\State \hskip2em Synchronous Byzantine-Tolerant Consensu with External Validity, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{trigger} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{propose}(\mathit{proposal}) \rangle$

\medskip
\State \textbf{upon} $\langle \mathcal{A}_{\mathit{correct}}, \mathsf{decide}(i) \rangle$:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \text{a value from } \mathit{val}(i)$
\State \hskip2em \(\triangleright\) values which are valid for $c$ are all the values from $\mathit{val}(i)$
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$
\end{algorithmic}
\end{algorithm}

Termination of $\mathcal{A}_B$ follows from termination of $\mathcal{A}_{\mathit{correct}}$ and $c$.
Furthermore, agreement of $\mathcal{A}_B$ follows from agreement of $c$.
Hence, we need to prove the validity property of $\mathcal{A}_B$.

Fix an input configuration $\mathit{input}$.
Since all correct processes agree in $\mathcal{A}_{\mathit{correct}}$ on an input configuration $i$, all correct processes agree on the set of valid values in $c$.
Hence, the decided value $v \in \mathit{val}(i)$.
Moreover, we have that $\mathit{input} \subseteq i$ (due to the all-correct validity of $\mathcal{A}_{\mathit{correct}}$).
Thus, $v \in \mathit{val}(\mathit{input})$ (since $\mathit{val}$ satisfies the Byzantine containment condition), and the validity safety property is ensured.

As for the validity liveness, we can easily modify $\mathcal{A}_{\mathit{correct}}$ to take into account the exact time of decision.
Then, as done before, we can map the time into a specific value from $\mathit{val}(i)$.
Therefore, validity liveness is (i.e., can be) ensured by $\mathcal{A}_B$, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of Byzantine consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the Byzantine containment condition is necessary for a validity property to be satisfied in a partially synchronous environment (as this condition is necessary in a synchronous setting).
We now define when an input configuration is ``Byzantine-correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{ByzSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{ByzSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j] \neq \bot \land i'[j] \neq \bot \implies \mathit{input}[j] = i'[j]\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{Byzantine-correct-similar} to $\mathit{input}$ if all processes which belong to both $\mathit{input}$ and $i'$ propose the same values in both input configurations.

Next, we introduce the \emph{Byzantine-correct-similarity condition}.

\begin{definition} [Byzantine-correct-similarity condition] \label{definition:f+1_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{Byzantine-correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{ByzSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

We now show that the Byzantine-correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Byzantine-correct-similarity condition is necessary] \label{lemma:f+1_similarity_necessary}
Let $\mathit{val}$ be a validity property that does not satisfy the Byzantine-correct-similarity condition.
No partially synchronous algorithm solves the Byzantine consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the Byzantine-correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{ByzSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:f+1_similarity}).
By contradiction, suppose that there exists a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_B$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{ByzSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the Byzantine-correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_B$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item No process correct in both $e$ and $e'$ (there exist at least $f + 1$ such processes) hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_B$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_B$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that Byzantine containment and Byzantine-correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Byzantine containment and Byzantine-correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies Byzantine containment and Byzantine-correct-similarity conditions.
There exists a partially synchronous algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous Byzantine consensus algorithm $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous Byzantine algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Byzantine Consensus with External Validity, \textbf{instance} $c$
\State \hskip2em Byzantine Consistent Broadcast, \textbf{instance} $\mathit{bcb}$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{trigger} $\langle \mathit{bcb}, \mathsf{broadcast}\big([\textsc{proposal}, \mathit{proposal}]\big) \rangle$

\medskip
\State \textbf{upon} delivery of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i_byzantine}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{ByzSim}(i)$ \label{line:partially_set_to_propose}

\State \hskip2em \(\triangleright\) all values are associated with received \textsc{proposal} messages which proves the validity of the proposed values
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c_byzantine}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_B$ (\Cref{algorithm:partially_synchronous_byzantine}) solves the Byzantine consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous Byzantine consensus (instance $c$ in \Cref{algorithm:partially_synchronous_byzantine}).
Hence, it is left to show that $\mathcal{A}_B$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_B$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c_byzantine}) and let $i$ be the input configuration that corresponds to messages $P$ accompanies its proposal by.
We have the following: $i \in \mathit{ByzSim}(\mathit{input})$.
% ; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
% We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
% Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, the proposed value must belong to $\mathit{val}(\mathit{input})$.
% Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous Byzantine consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only values accompanied with \textsc{proposal} messages, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_byzantine}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_B$ relies on time.
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All correct processes propose their values according to $\mathit{input}$.
    All Byzantine processes immediately announce themselves by broadcasting ``I am Byzantine'' to all processes.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Every correct process receives messages from all correct processes before proposing to $c$.
\end{compactenum}
Hence, all correct processes build $\mathit{input}$ at line~\ref{line:partially_build_i_byzantine}.
Thus, all processes propose $v$ to $c$, which means $v$ is decided.
Let us underline that, in this case, the attack exploited in \Cref{lemma:f+1_similarity_necessary} cannot be used, which means that the execution preserves the safety violation (since $\mathit{val}$ satisfies the Byzantine containment property).
The theorem holds.
\end{proof}

==> sections/former/classification.tex <==
% \newpage
\section{Necessary solvability conditions}  \label{section:classification}

This section gives the necessary conditions for the solvability of validity properties. 
We start by focusing on the case of $n \leq 3t$: we prove that, if $n \leq 3t$, all solvable validity properties are trivial (\Cref{subsection:triviality_main}).
Then, we consider the case of $n > 3t$: we define the similarity condition, and prove its necessity for solvability (\Cref{subsection:necessary_condition}).

\subsection{Triviality of Solvable Validity Properties if $n \leq 3t$} \label{subsection:triviality_main}

%\manuel{It is doubtful whether we should include the next couple of sentences before the last.}
Some validity properties, such as \emph{Weak Validity} and \emph{Strong Validity}, are known to be unsolvable with $n \leq 3t$~\cite{DLS88,PeaseSL80}.
%\pierre{I would write Weak Validity (and maybe for Binary Consensus) to stress the fact that the result is known for quite weak validity properties, but we clarify the fact that there does not exists a super weak validity property that circumvents the $n/3$-bound}.
This seems to imply a split of validity properties depending on the resilience threshold.
We prove that such a split indeed exists for $n \leq 3t$, and, importantly, that it applies to \emph{all} solvable validity properties.
Implicitly, this means that there is no ``useful'' relaxation of the validity property that can tolerate $t \geq \lceil n / 3 \rceil$ failures.
Concretely, we prove the following theorem:

\begin{theorem} \label{theorem:triviality_main}
% Let $n$ denote the total number of processes, and $t$ the number of tolerated failures.
If a validity property is solvable with $n \leq 3t$, then the validity property is trivial, i.e., there exists a value $v' \in \mathcal{V}_O$ such that $v' \in \bigcap\limits_{c \in \mathcal{I}} \mathit{val}(c)$.
\end{theorem}

% Concretely, if $n \leq 3t$, all solvable validity properties are trivial (require no communication).
% % and can be solved without any communication.
% Let us start by formally defining the notion of a trivial validity property.

% \begin{definition} [Trivial validity property] \label{definition:trivial_validity}
% We say that a validity property $\mathit{val}$ is \emph{trivial} if and only if there exists a value $v' \in \mathcal{V}_O$ such that $v' \in \bigcap\limits_{c \in \mathcal{I}} \mathit{val}(c)$.
% \end{definition}

% Observe that the Byzantine consensus problem with a trivial validity property can be solved without any communication: processes decide the same always-admissible value.
% This subsection proves the following theorem:



Before presenting the proof of the theorem, we introduce the \emph{compatibility relation} between input configurations, which we use throughout this subsection.
% notion of \emph{compatible} input configurations.

\paragraph{Compatibility.}
We define the compatibility relation (``$\diamond$'') between input configurations:
\begin{equation*}
    \forall c_1, c_2 \in \allconfigurations: c_1 \diamond c_2 \iff \big(|\processes{c_1} \cap \processes{c_2}| \leq t\big) \land \big(\exists P \in \processes{c_1} \setminus{\processes{c_2}}\big) \land \big(\exists Q \in \processes{c_2} \setminus{\processes{c_1}}\big).
\end{equation*}

That is, $c_1$ is compatible with $c_2$ if and only if (1) there are at most $t$ processes in common, (2) there exists a process which belongs to $c_1$ and does not belong to $c_2$, and (3) there exists a process which belongs to $c_2$ and does not belong to $c_1$.
For example, when $n = 3$ and $t = 1$, $c = \big[ (P_1, 0), (P_2, 0) \big]$ is compatible with $\big[ (P_1, 1), (P_3, 1) \big]$, whereas $c$ is not compatible with $\big[ (P_1, 1), (P_2, 1), (P_3, 1) \big]$.
Observe that the compatibility relation is symmetric and irreflexive.
% Note that any trivial validity property satisfies $\mathcal{C}_S$: for every input configuration $c \in \mathcal{I}$, $\lambda(c)$ is defined as an always-admissible value.
% Moreover, the Byzantine consensus problem with a trivial validity property can be solved with no communication: processes immediately decide the same always-admissible value.

\paragraph{Proof of \Cref{theorem:triviality_main}.}
Throughout the rest of the subsection, we fix any validity property $\mathit{val}$ which is solvable with $n \leq 3t$; our aim is to prove the triviality of $\mathit{val}$.
Moreover:
\begin{compactitem}
    \item We assume that $n \leq 3t$.

    \item We fix any algorithm $\mathcal{A}$ which solves consensus with $\mathit{val}$.

    \item We fix any input configuration $\mathit{base} \in \mathcal{I}_{n - t}$ with exactly $n - t$ process-proposal pairs.

    \item We fix any infinite canonical execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{\mathit{base}}) = \mathit{base}$.
    As $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, and $\mathcal{E}_{\mathit{base}}$ is infinite, some value $v_{\mathit{base}} \in \mathit{val}(\mathit{base})$ is decided by a correct process in $\mathcal{E}_{\mathit{base}}$.
\end{compactitem}

%In our proof, we rely on a partitioning argument~\cite{LSP82}, as well as on canonical similarity (\Cref{subsection:intermediate_results}).

% Our proof works as follows:
% \begin{compactenum}
%     \item By applying the partitioning argument~\cite{LSP82}, we show that, in any canonical execution which corresponds to an input configuration compatible with $\mathit{base}$, $v_{\mathit{base}}$ must be decided.
    
%     \item We show that, for every input configuration with $n$ process-proposal pairs (i.e., every process is correct), there exists an execution in which $v_{\mathit{base}}$ is decided.
    
%     \item Finally, by ``removing'' process-proposal pairs from input configurations with $n$ process-proposal, we show that, for every input configuration $c$, $v_{\mathit{base}}$ is decided in (at least) one execution which corresponds to $c$.
% \end{compactenum}
% Recall that an input configuration $c_1 \in \mathcal{I}$ is compatible with an input configuration $c_2 \in \mathcal{I}$ (we write ``$c_1 \diamond c_2$'') if and only if (1) there are at most $t$ processes in common, (2) there exists a process which belongs to $c_1$ and does not belong to $c_2$, and (3) there exists a process which belongs to $c_2$ and does not belong to $c_1$.

First, we show that only $v_{\mathit{base}}$ can be decided in any canonical execution which corresponds to any input configuration compatible with $\mathit{base}$.
If a value different from $v_{\mathit{base}}$ is decided, we can apply the classical partitioning argument~\cite{LSP82}: the adversary causes a disagreement by partitioning processes into two disagreeing groups.

\begin{lemma} \label{lemma:triviality_compatible}
Let $c \in \mathcal{I}$ be any input configuration such that $c \diamond \mathit{base}$.
Let $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ be any (potentially infinite) canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_c) = c$.
If a value $v_c \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_c$, then $v_c = v_{\mathit{base}}$.
\end{lemma}
\begin{proof}
By contradiction, suppose that some value $v_c \neq v_{\mathit{base}}$ is decided by a correct process in $\mathcal{E}_c$.
Since $c \diamond \mathit{base}$, there exists a process $Q \in \processes{c}\setminus{\processes{\mathit{base}}}$.
If $\mathcal{E}_c$ is infinite, let $\mathcal{E}_c^Q \gets \mathcal{E}_c$.
Otherwise, let $\mathcal{E}_c^Q$ be an infinite canonical continuation of $\mathcal{E}_c$.
The following holds for process $Q$: (1) $Q$ decides $v_c$ in $\mathcal{E}_c^Q$ (as $\mathcal{A}$ satisfies \emph{Agreement} and \emph{Termination}), and (2) $Q$ is silent in $\mathcal{E}_{\mathit{base}}$.
Let $t_Q$ denote the time at which $Q$ decides in $\mathcal{E}_c^Q$.
Similarly, there exists a process $P \in \processes{\mathit{base}} \setminus{\processes{c}}$; note that (1) $P$ decides $v_{\mathit{base}}$ in $\mathcal{E}_{\mathit{base}}$, and (2) $P$ is silent in $\mathcal{E}_c^Q$.
Let $t_P$ denote the time at which $P$ decides in $\mathcal{E}_{\mathit{base}}$.

In the next step, we construct an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ by ``merging'' $\mathcal{E}_{\mathit{base}}$ and $\mathcal{E}_c^Q$:
\begin{compactenum}
    \item We separate processes into 4 groups: (1) group $A = \pi(\mathit{base}) \setminus{\pi(c)}$, (2) group $B = \pi(\mathit{base}) \cap \pi(c)$, (3) group $C = \pi(c) \setminus{\pi(\mathit{base})}$, and (4) group $D = \Pi \setminus{(A \cup B \cup C)}$.

    \item Processes in $B$ behave towards processes in $A$ as in $\mathcal{E}_{\mathit{base}}$, and towards processes in $C$ as in $\mathcal{E}_c^Q$.

    \item Communication between groups $A$ and $C$ is delayed until after time $\max(t_P, t_Q)$.

    \item Processes in group $D$ ``wake up'' at time $T_D > \max(t_P,t_Q)$ (with any proposals), and behave correctly throughout the entire execution.
    % $P$ has decided $v_{\mathit{base}}$ and $Q$ has decided $v_c$. 
    
    \item We set GST to after $T_D$.
\end{compactenum}
The following holds for $\mathcal{E}$:
\begin{compactitem}
    \item Processes in $\Pi \setminus{B}$ are correct in $\mathcal{E}$.
    In other words, only processes in $B$ are faulty in $\mathcal{E}$.
    Recall that $|B| \leq t$ as $\mathit{base} \diamond c$.

    \item Process $Q$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_c^Q$ until after time $\max(t_P, t_Q)$.
    % in which it decides $v_c$.
    Hence, process $Q$ decides $v_c$ in $\mathcal{E}$.

    \item Process $P$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_{\mathit{base}}$ until after time $\max(t_P, t_Q)$.
    % in which it decides $v_{\mathit{base}}$.
    Hence, process $P$ decides $v_{\mathit{base}} \neq v_c$ in $\mathcal{E}$.
\end{compactitem}
Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $v_c = v_{\mathit{base}}$.
\end{proof}


\iffalse
\begin{sketch}
By contradiction, suppose that some value $v_c \neq v_{\mathit{base}}$ is decided by a correct process in $\mathcal{E}_c$.
Since $c \diamond \mathit{base}$, there exists a correct process $Q \in \processes{c}\setminus{\processes{\mathit{base}}}$; note that (1) process $Q$ decides $v_c$ in $\mathcal{E}_c$ (as $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}), and (2) process $Q$ is silent in $\mathcal{E}_{\mathit{base}}$.
Similarly, there exists a process $P \in \processes{\mathit{base}} \setminus{\processes{c}}$; observe that (1) process $P$ decides $v_{\mathit{base}}$ in $\mathcal{E}_{\mathit{base}}$, and (2) process $P$ is silent in $\mathcal{E}_c$.

In order to prove the lemma, we construct an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ by ``merging'' $\mathcal{E}_{\mathit{base}}$ and $\mathcal{E}_c$:
\begin{compactenum}
    \item Processes in $\processes{c} \cap \processes{\mathit{base}}$ behave (1) towards processes in $\processes{\mathit{base}} \setminus{\processes{c}}$ as in $\mathcal{E}_{\mathit{base}}$, and (2) towards processes in $\processes{c} \setminus{\processes{\mathit{base}}}$ as in $\mathcal{E}_c$.

    \item Communication between (1) processes in $\processes{\mathit{base}} \setminus{\processes{c}}$ and (2) processes in $\processes{c} \setminus{\processes{\mathit{base}}}$ is delayed.
\end{compactenum}
The following holds for $\mathcal{E}$:
\begin{compactitem}
    \item Processes in $\processes{\mathit{base}} \ominus \processes{c}$ (symmetric difference) are correct in $\mathcal{E}$.

    \item Only processes in $\processes{\mathit{base}} \cap \processes{c}$ are faulty in $\mathcal{E}$.
    Recall that $|\processes{\mathit{base}} \cap \processes{c}| \leq t$ as $\mathit{base} \diamond c$.

    \item Process $Q$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_c$.
    Hence, process $Q$ decides $v_c$ in $\mathcal{E}$.

    \item Process $P$, which is correct in $\mathcal{E}$, cannot distinguish $\mathcal{E}$ from $\mathcal{E}_{\mathit{base}}$.
    Hence, process $P$ decides $v_{\mathit{base}} \neq v_c$ in $\mathcal{E}$.
\end{compactitem}
Therefore, \emph{Agreement} is violated in $\mathcal{E}$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $v_c = v_{\mathit{base}}$.
\end{sketch}
\fi

Observe that the proposals of an input configuration compatible with $\mathit{base}$ do not influence the decision: given an input configuration $c \in \mathcal{I}$, $c \diamond \mathit{base}$, only $v_{\mathit{base}}$ can be decided in any canonical execution which corresponds to $c$, \emph{irrespectively} of the proposals.

Next, we prove a direct consequence of \Cref{lemma:triviality_compatible}: for every input configuration $c_n \in \mathcal{I}_n$, there exists an infinite execution $\mathcal{E}_{n}$ such that (1) $\mathcal{E}_{n}$ corresponds to $c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$.
% Below, we give a proof sketch of the claim; the formal proof can be found in \Cref{section:triviality_appendix}.

% The results follows directly from \Cref{lemma:triviality_compatible}.

\begin{lemma} \label{lemma:triviality_complete}
For any input configuration $c_n \in \mathcal{I}_n$, there exists an infinite execution $\mathcal{E}_{n} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{n}) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$.
\end{lemma}
\begin{proof}
Fix any input configuration $c_n \in \mathcal{I}_n$.
We construct an input configuration $c_{n - t} \in \mathcal{I}_{n - t}$:
\begin{compactenum}
    \item For every process $P_i \notin \processes{\mathit{base}}$, we include a process-proposal pair $(P_i, v)$ in $c_{n - t}$ such that $v = \mathsf{proposal}(c_n[i])$.
    Note that there are $t$ such processes as $|\processes{\mathit{base}}| = n - t$.

    \item We include any $n - 2t$ process-proposal pairs $(P_i, v)$ in $c_{n - t}$ such that (1) $P_i \in \processes{\mathit{base}}$, and (2) $v = \mathsf{proposal}(c_n[i])$.
    That is, we ``complete'' $c_{n - t}$ (constructed in the step 1) with $n - 2t$ process-proposal pairs such that the process is ``borrowed'' from $\mathit{base}$, and its proposal is ``borrowed'' from $c_n$.
\end{compactenum}
Observe that $c_{n - t} \diamond \mathit{base}$ as (1) $|\processes{c_{n - t}} \cap \processes{\mathit{base}}| \leq t$ ($n - 2t \leq t$ when $n \leq 3t$), (2) there exists a process $P \in \processes{\mathit{base}} \setminus \processes{c_{n - t}}$ (while constructing $c_{n - t}$, we excluded $t > 0$ processes from $\mathit{base}$; step 2), and (3) there exists a process $Q \in \processes{c_{n - t}} \setminus{\processes{\mathit{base}}}$ (we included $t > 0$ processes in $\mathit{c_{n - t}}$ which are not in $\mathit{base}$; step 1).

Let $\mathcal{E}_{n - t} \in \mathit{execs}(\mathcal{A})$ denote any infinite canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_{n - t}) = c_{n - t}$.
As $\mathcal{A}$ satisfies \emph{Termination}, some value is decided by correct processes in $\mathcal{E}_{n - t}$; due to \Cref{lemma:triviality_compatible}, that value is $v_{\mathit{base}}$.
Finally, we are able to construct an infinite execution $\mathcal{E}_n \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_n$:
\begin{compactenum}
    \item All processes are correct in $\mathcal{E}_n$.

    \item Until some correct process $P \in \processes{c_{n - t}}$ decides $v_{\mathit{base}}$, $\mathcal{E}_n$ is identical to $\mathcal{E}_{n - t}$.
    Let $\mathcal{S}$ denote the set of all processes which take a computational step in $\mathcal{E}_{n - t}$ until $P$ decides $v_{\mathit{base}}$; note that $\mathcal{S} \subseteq \processes{c_{n - t}}$ and $P \in \mathcal{S}$.

    \item Afterwards, every process $Q \notin \mathcal{S}$ ``wakes up'' with the proposal specified in $c_n$.
    
    \item GST is set to after all processes have taken a computational step.
\end{compactenum}
Therefore, $v_{\mathit{base}}$ is indeed decided in $\mathcal{E}_n$ and $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, which concludes the proof.
\end{proof}

\iffalse
*********
\begin{sketch}
Fix any input configuration $c_n \in \mathcal{I}_n$.
There exists an input configuration $c_{n - t} \in \mathcal{I}_{n - t}$ such that (1) for every process $P \in \processes{c_n} \cap \processes{c_{n - t}}$, proposals of $P$ in $c_n$ and $c_{n - t}$ are identical, and (2) $c_{n - t} \diamond \mathit{base}$.
Hence, $v_{\mathit{base}}$ is decided in any infinite canonical execution $\mathcal{E}_{n - t}$ which corresponds to $c_{n - t}$ (by \Cref{lemma:triviality_compatible}).
Thus, by ``waking up'' processes in $\processes{c_n} \setminus{\processes{c_{n - t}}}$ after $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n - t}$, we build an execution $\mathcal{E}_n$ such that (1) $\mathcal{E}_n$ corresponds to $c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_n$.
\end{sketch}
**********
\fi


\iffalse
\begin{sketch}
Fix any input configuration $c \in \mathcal{I}_n$.
We construct another input configuration $c^* \in \mathcal{I}$:
\begin{compactenum}
    \item For every process $Q \notin \processes{\mathit{base}}$, we include a process-proposal pair $(Q, v)$ in $c^*$, for any value $v \in \mathcal{V}_I$.
    Note that there are $t$ such processes $Q$ as $|\processes{\mathit{base}}| = n - t$.

    \item We include $n - 2t$ process-proposal pairs $(P_i, v)$ in $c^*$ such that (1) $P_i \in \processes{\mathit{base}}$, and (2) $v = \mathsf{proposal}(c[i])$.
    That is, we ``complete'' $c^*$ (constructed in the step 1) with $n - 2t$ process-proposal pairs such that the process is ``borrowed'' from $\mathit{base}$ and its proposal is ``borrowed'' from $c$.
\end{compactenum}
Observe that $c^* \diamond \mathit{base}$ as (1) $|\processes{c^*} \cap \mathit{base}| \leq t$ (because $n - 2t \leq t$ when $n \leq 3t$), (2) there exists a process $P \in \processes{\mathit{base}} \setminus \processes{c^*}$ (because we excluded $t > 0$ processes from $\mathit{base}$ when constructing $c^*$; step 1), and (3) there exists a process $Q \in \processes{c^*} \setminus{\processes{\mathit{base}}}$ (because we included $t > 0$ processes in $\mathit{c^*}$ which are not in $\processes{\mathit{base}}$; step 1).

Let $\mathcal{E}_{c^*} \in \mathit{execs}(\mathcal{A})$ denote any infinite canonical execution such that $\mathsf{corresponds}(\mathcal{E}_{c^*}) = c^*$.
As $\mathcal{A}$ satisfies \emph{Termination}, some value is decided by correct processes in $\mathcal{E}_{c^*}$; due to \Cref{lemma:triviality_compatible}, that value is $v_{\mathit{base}}$.
Finally, we are able to construct an infinite execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{corresponds}(\mathcal{E}_c) = c$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_c$:
\begin{compactenum}
    \item All processes are correct in $\mathcal{E}_c$.

    \item Until some correct process $P \in \processes{c^*}$ decides $v_{\mathit{base}}$, $\mathcal{E}_c$ is identical to $\mathcal{E}_{c^*}$.

    \item Afterwards, every process $Q \notin \processes{c^*}$ ``wakes up'' with the proposal specified in $c$.
\end{compactenum}
Due to the construction, 
$v_{\mathit{base}}$ is indeed decided in $\mathcal{E}_c$ and $\mathsf{corresponds}(\mathcal{E}_c) = c$, which concludes the proof.
\end{sketch}
\fi

We are now ready to prove that $\mathit{val}$ is trivial.
We do so by showing that, for any input configuration $c \in \mathcal{I}$, $v_{\mathit{base}} \in \mathit{val}(c)$.

\begin{lemma}
\label{lemma:triviality_main_2} 
Validity property $\mathit{val}$ is trivial.
\end{lemma}
\begin{proof}
We fix any input configuration $c \in \mathcal{I}$.
Let us distinguish two possible scenarios:
\begin{compactitem}
    \item Let $c \in \mathcal{I}_n$.
    There exists an infinite execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_c) = c$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_c$ (by \Cref{lemma:triviality_complete}).
    As $\mathcal{A}$ satisfies $\mathit{val}$, $v_{\mathit{base}} \in \mathit{val}(c)$.

    \item Let $c \notin \mathcal{I}_n$.
    We construct an input configuration $c_n \in \mathcal{I}_n$ in the following way:
    \begin{compactenum}
        \item Let $c_n \gets c$.

        \item For every process $P \notin \processes{c}$, $(P, \text{any proposal})$ is included in $c_n$.
        % , where $v \in \mathcal{V}_I$ is any proposal.
    \end{compactenum}
    Due to the construction of $c_n$, $c_n \sim c$.
    By \Cref{lemma:triviality_complete}, there exists an infinite execution $\mathcal{E}_{n} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_n) = c_n$, and (2) $v_{\mathit{base}}$ is decided in $\mathcal{E}_{n}$; $\mathcal{E}_n$ is a canonical execution.
    Therefore, canonical similarity ensures that $v_{\mathit{base}} \in \mathit{val}(c)$ (\Cref{lemma:helper_main}).
\end{compactitem}
In both possible cases, $v_{\mathit{base}} \in \mathit{val}(c)$.
Thus, the theorem.
\end{proof}

% Given that $\mathit{val}$ is any solvable validity property with $n \leq 3t$ and it is shown that $\mathit{val}$ is trivial (\Cref{theorem:triviality_main}), every solvable validity property with $n \leq 3t$ is trivial.
\Cref{lemma:triviality_main_2} concludes the proof of \Cref{theorem:triviality_main}, as \Cref{lemma:triviality_main_2} proves that $\mathit{val}$, any solvable validity property with $n \leq 3t$, is trivial.
\Cref{fig:triviality} depicts the proof of \Cref{theorem:triviality_main}.
% Consensus with a trivial validity property can be solved without any communication: processes decide on the same always-admissible value.
Since this subsection shows that consensus cannot be useful when $n \leq 3t$, the rest of the paper focuses on the case of $n > 3t$.
% in the rest of the paper.
% Throughout the rest of the paper, we focus on the case of $n > 3t$.
% Throughout the rest of the paper, we focus on the case of $n > 3t$.

\begin{figure}[ht]
    \centering
    \includegraphics[scale = 0.44]{figures/export-13-crop.pdf}
    \caption{\Cref{theorem:triviality_main}: Overview of the proof in the case of $n = 6$, $t = 2$, and $\mathit{base} = \big[ (P_1, 0), (P_2, 0), (P_3, 0), (P_4, 0) \big]$.}
    \label{fig:triviality}
\end{figure}

% \newpage
\subsection{Similarity Condition: Necessary Solvability Condition} \label{subsection:necessary_condition}

This subsection defines the similarity condition, and proves its necessity for solvable validity properties.

\begin{definition} [Similarity condition] \label{definition:similarity_condition}
A validity property $\mathit{val}$ satisfies the \emph{similarity condition} ($\mathcal{C}_S$, in short) if and only if there exists a Turing-computable function $\Lambda: \mathcal{I}_{n - t} \to \mathcal{V}_O$ such that:
\begin{equation*}
 \forall c \in \mathcal{I}_{n - t}: \Lambda(c) \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c').
\end{equation*}
\end{definition}

$\mathcal{C}_S$ states that, for every input configuration $c \in \mathcal{I}_{n - t}$, there exists a Turing-computable function $\Lambda(c)$ which retrieves a common admissible decision among all input configurations similar to $c$.\footnote{A function is Turing-computable if there exists a finite procedure to compute the function.}
The necessity of $\mathcal{C}_S$ follows from the canonical similarity result: in any infinite canonical execution, a common admissible value must be decided (\Cref{lemma:helper_main}).

\begin{theorem} \label{theorem:similarity_condition_necessary}
Any solvable validity property satisfies $\mathcal{C}_S$.
\end{theorem}
\begin{proof}
By the means of contradiction, let there exist a validity property $\mathit{val}$ such that (1) $\mathit{val}$ does not satisfy $\mathcal{C}_S$, and (2) $\mathit{val}$ is solvable.
Let $\mathcal{A}$ be any algorithm which solves the Byzantine consensus problem with $\mathit{val}$.
As $\mathit{val}$ does not satisfy $\mathcal{C}_S$, there does not exist a Turing-computable function $\Lambda: \mathcal{I}_{n - t} \to \mathcal{V}_O$ such that, for every input configuration $c \in \mathcal{I}_{n - t}$, $\Lambda(c) \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
% (by \Cref{definition:similarity_condition}).

Fix any input configuration $c \in \mathcal{I}_{n - t}$ for which $\Lambda(c)$ is not defined or not Turing-computable.
% ; such an input configuration exists as $\mathit{val}$ does not satisfy $\mathcal{C}_S$.
Let $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ be an infinite canonical execution such that (1) $\mathsf{input\_conf}(\mathcal{E}_c) = c$, (2) the system is synchronous from the very beginning ($\text{GST} = 0$), and (3) the message delays are exactly $\delta$.
In other words, $\mathcal{E}_c$ unfolds in a ``lock-step'' manner.
As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_c$ is an infinite execution, some value $v_c \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_c$; observe that the prefix of $\mathcal{E}_c$ in which $v_c$ is decided is finite as processes take only finitely many steps in finite time.
By canonical similarity (\Cref{lemma:helper_main}), $v_c \in \bigcap\limits_{c' \in \similar{c}} \mathit{val}(c')$.
Hence, $\Lambda(c)$ is defined ($\Lambda(c) = v_c$) and Turing-computable ($\mathcal{A}$ computes it).
Thus, we reach a contradiction with the fact that $\Lambda(c)$ is not defined or not Turing-computable.
% , which concludes the proof.
% , which concludes the proof.
\end{proof}

Notice that, for proving the necessity of $\mathcal{C}_S$ (\Cref{theorem:similarity_condition_necessary}), we do not rely on the $n > 3t$ assumption.
% that $n > 3t$.
Hence, $\mathcal{C}_S$ is necessary for \emph{all} solvable validity properties (irrespectively of the resilience threshold).
However, as proven in \Cref{subsection:triviality_main}, $\mathcal{C}_S$ is not sufficient when $n \leq 3t$: e.g., \emph{Weak Validity} satisfies $\mathcal{C}_S$, but it is unsolvable with $n \leq 3t$~\cite{DLS88,PeaseSL80}.
(Observe that any trivial validity property satisfies $\mathcal{C}_S$.)

% \jovan{I believe we will need to cut the part below. No space.}
\paragraph{Similarity condition (example).}
Consider \emph{Correct-Proposal Validity}, a validity property which states that any decided value must have been proposed by a correct process.
Consensus with \emph{Correct-Proposal Validity} is also known as \emph{strong}  consensus~\cite{fitzi2003efficient,siu1998reaching}.
Strong  consensus assumes $\mathcal{V}_I = \mathcal{V}_O$.
It was shown that, in partial synchrony,  strong consensus  cannot be solved if $n \leq (|\mathcal{V}_I| + 1)t$~\cite{fitzi2003efficient}.
We now present an alternative proof.
Namely, we show that \emph{Correct-Proposal Validity} does not satisfy $\mathcal{C}_S$ if $n \leq (|\mathcal{V}_I| + 1)t$, which makes it unsolvable by \Cref{theorem:similarity_condition_necessary}.

\begin{theorem}
Strong consensus is unsolvable unless $n > (|\mathcal{V}_I| + 1)t$.
\end{theorem}
\begin{proof}
We prove the theorem by contradiction.
Let $|\mathcal{V}_I| = |\mathcal{V}_O| = m$.
Without loss of generality, let $n = (m + 1)t$.
We define an input configuration $\mathit{base} \in \mathcal{I}_{n - t}$ such that (1) $|\processes{\mathit{base}}| = n - t = mt$, and (2) every value $v \in \mathcal{V}_I$ is the proposal of exactly $t$ processes in $\mathit{base}$.
Therefore, all values are admissible for $\mathit{base}$ ($\mathit{val}(\mathit{base}) = \mathcal{V}_O$).
Next, for each value $v \in \mathcal{V}_I$, we design an input configuration $c_{\notni v}$ such that (1) $v$ is not admissible for $c_{\notni v}$, and (2) $c_{\notni v} \sim \mathit{base}$:
\begin{compactenum}
    \item Let $c_{\notni v} \gets \mathit{base}$.
    
    \item We remove from $c_{\notni v}$ all process-proposal pairs $\mathit{pp}$ with $\mathsf{proposal}(\mathit{pp}) = v$.

    \item For every process $P \notin \processes{\mathit{base}}$, we add $(P, v')$ to $c_{\notni v}$, for any value $v' \neq v$.
\end{compactenum}
Hence, \emph{Correct-Proposal Validity} does not satisfy $\mathcal{C}_S$ when $n \leq (m + 1)t$ as, for every $v \in \mathcal{V}_O$, there exists an input configuration $c_{\not\ni v} \sim \mathit{base}$ for which $v$ is not admissible.
% there does not exist a common admissible decision among input configurations similar to $\mathit{base}$.
Thus, \emph{Correct-Proposal Validity} is unsolvable if $n \leq (m + 1)t$ (by \Cref{theorem:similarity_condition_necessary}).
\end{proof}


% \medskip
% In this subsection, we introduced $\mathcal{C}_S$, and showed its necessity for solvable validity properties.
% % that any solvable validity property satisfies $\mathcal{C}_S$.
% In \Cref{subsection:general_algorithm}, we prove that, if a validity property satisfies $\mathcal{C}_S$ and $n > 3t$, the property is solvable.
% Therefore, $\mathcal{C}_S$ represents a necessary and sufficient condition for solvable validity properties when $n > 3t$.

% As $\mathit{val}$ is  shown to be trivial (by \Cref{theorem:triviality_main}), the corollary bellow directly follows.

% \begin{corollary} \label{corollary:triviality}
% If a validity property is solvable with $n \leq 3t$, the validity property is trivial.    
% \end{corollary}

% \subsection{Lower Bound on Message Complexity for Non Trivial and Solvable Validity Properties}
% \label{subsection:lower_bound}

% This subsection proves that any Byzantine consensus algorithm with a non-trivial and solvable validity property incurs $\Omega(t^2)$ message complexity.
% This result generalizes the seminal Dolev-Reischuk bound~\cite{dolev1985bounds}, which says that any Byzantine consensus algorithm with \emph{Strong Validity} exchanges (at least) $\Omega(t^2)$ messages.
% Our proof is by the means of contradiction and it consists of two steps: 
% \begin{compactenum}
%     \item If the message complexity of a Byzantine consensus algorithm is less than quadratic, we identify a process $Q$ which can decide some value $v \in \mathcal{V}_O$ without having received any message (from any other process).
%     The first step of our proof is identical to the first step of the original Dolev-Reischuk proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}.
    
%     \item We show that there exists an execution such that (1) $Q$ is faulty and silent, and (2) other processes decide a value $v' \neq v$.
%     We can then ``merge'' this execution with a valid behavior of $Q$ in which $Q$ decides $v$ without having received any message, thus constructing an execution in which \emph{Agreement} is violated.
    
%     The original proof of the Dolev-Reischuk bound follows the same idea.
%     However, given that the original bound concerns only \emph{Strong Validity}, the second step in the original proof is straightforward.
%     Conversely, as our bound considers \emph{all} validity properties, completing the second step proved more challenging.
% \end{compactenum}
% In this subsection, we give an informal proof of our lower bound; the formal treatment is delegated to \Cref{section:lower_bound_appendix}.

% Throughout the entire subsection, we fix any non-trivial and solvable validity property $\mathit{val}$.
% Moreover, we fix $\mathcal{A}$, any Byzantine consensus algorithm with $\mathit{val}$.
% Finally, $n > 3t$ as $\mathit{val}$ is non-trivial (see \Cref{theorem:triviality_main}).

% \paragraph{Execution $\mathcal{E}_{\mathit{base}}$ of $\mathcal{A}$.}
% We start by defining a specific infinite execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ in the following manner:
% \begin{compactenum}
%      \item $\text{GST}_{\mathit{base}} = 0$.
%      That is, the system is synchronous throughout the entire execution.
     
%      \item All processes are separated into two groups: (1) group $A$, with $|A| = n - \frac{t}{2}$, and (2) group $B$, with $|B| = \frac{t}{2}$.
     
%      \item All processes in the group $A$ are correct, whereas all processes in the group $B$ are faulty.
     
%      \item We fix any value $v^* \in \mathcal{V}_I$.
%      For every correct process $P \in A$, the proposal of $P$ in $\mathcal{E}_{\mathit{base}}$ is $v^*$.
     
%      \item For every faulty process $Q \in B$, $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $Q$ ignores the first $\frac{t}{2}$ messages received from other processes, and (2) $Q$ omits sending messages to other processes in $B$. 
% \end{compactenum}

% \medskip
% If correct processes send $(\frac{t}{2})^2$ (or more) messages in $\mathcal{E}_{\mathit{base}}$, the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
% Hence, in the rest of the subsection, we assume that correct processes send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$.

% The first step of our proof shows that, if correct processes indeed send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$, there must exist a process $Q \in B$ such that $Q$ can correctly decide some value $v \in \mathcal{V}_O$ without having received \emph{any} message from any other process.
% We prove this claim using the pigeonhole principle.

% \begin{lemma} \label{lemma:behavior_without_receptions}
% There exist a value $v \in \mathcal{V}_O$ and a process $Q \in B$ such that $Q$ can correctly decide $v$ without having received any message from any other process.
% \end{lemma}
% \begin{sketch}
% Recall that, by assumption, correct processes (i.e., processes in the group $A$) send less than $(\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$.
% Therefore, due to the pigeonhole principle, there exists a process $Q \in B$ which receives less than $\frac{t}{2}$ messages in $\mathcal{E}_{\mathit{base}}$.
% Recall that $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $Q$ ignores the first $\frac{t}{2}$ messages received from other processes, and (2) $Q$ does not send any messages to other processes in the group $B$.
% We denote by $S_Q$ the set of processes, not including $Q$, which send messages to $Q$ in $\mathcal{E}_{\mathit{base}}$; note that $|S_Q| \leq \frac{t}{2}$.

% Next, we construct an infinite execution $\mathcal{E}_{\mathit{base}}'$ in the following manner:
% \begin{compactenum}
%     % \item $\text{GST}_{\mathit{core}}' = 0$, i.e., the system is synchronous from the beginning.
    
%     \item Processes in $(A \cup \{Q\}) \setminus{S_Q}$ are correct; other processes are faulty.
%     That is, we make $Q$ correct in $\mathcal{E}'_{\mathit{base}}$, and we make all processes in $S_Q$ faulty in $\mathcal{E}'_{\mathit{base}}$.
    
%     \item Processes in $B \setminus{\{Q\}}$ behave exactly as in $\mathcal{E}_{\mathit{base}}$.
%     Moreover, processes in $S_Q$ behave exactly as in $\mathcal{E}_{\mathit{base}}$, except that they \emph{do not} send any message to $Q$.
% \end{compactenum}
% Importantly, there exists a process $P \in A \setminus{S_Q}$ (as $n > t$) such that $P$ cannot distinguish $\mathcal{E}_{\mathit{base}}'$ from $\mathcal{E}_{\mathit{base}}$.
% Hence, as $P$ decides some value $v \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}$ (as $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{\mathit{base}}$ is infinite), $P$ decides the same value $v$ in $\mathcal{E}_{\mathit{base}}'$.
% Moreover, due to the construction of $\mathcal{E}_{\mathit{base}}'$, process $Q$ does not receive any message (from any other process) in $\mathcal{E}_{\mathit{base}}'$.
% Due to the fact that $Q$ is correct in $\mathcal{E}_{\mathit{base}}'$ and $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}, $Q$ decides $v$ in $\mathcal{E}_{\mathit{base}}'$.
% Thus, $Q$ can indeed correctly decide $v \in \mathcal{V}_O$ without having received any message from any other process. 
% \end{sketch}
% % \jovan{Is this proof ok? Please, try to attack is much as possible. Can there be any problems with timers or I don't know what.
% % I am not seeing any problems. Just want us to be very careful!}

% In the second step, we show that there exists an execution $\mathcal{E}$ of $\mathcal{A}$ such that (1) $Q$ is faulty and silent, and (2) other processes decide a value $v' \neq v$.
% As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $c \in \mathcal{I}$ such that $v \notin \mathit{val}(c)$; recall that $v$ is the value that $Q$ can correctly decide without having received any message from any other process (by \Cref{lemma:behavior_without_receptions}).
% The following lemma shows that $Q \in \processes{c}$; otherwise, we could construct an execution in which $\mathcal{A}$ violates \emph{Agreement}.

% \begin{lemma} \label{lemma:q_in_c}
% $Q \in \processes{c}$.
% \end{lemma}
% \begin{sketch}
% By contradiction, let $Q \notin \processes{c}$.
% We fix any infinite canonical execution $\mathcal{E}_c \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{corresponds}(\mathcal{E}_c) = c$.
% Observe that $Q$ takes no computational steps in $\mathcal{E}_c$ as $Q \notin \processes{c}$.
% As $v \notin \mathit{val}(c)$, $\mathcal{E}_c$ is infinite and $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, some value $v' \neq v$ is decided by a correct process in $\mathcal{E}_c$.

% Next, we can construct another execution $\mathcal{E}'$ such that $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ is identical to $\mathcal{E}$, except that:
% \begin{compactenum}
%     \item Process $Q$ is correct in $\mathcal{E}'$.
    
%     \item All messages sent by and to $Q$ are delayed.
    
%     \item Process $Q$ exhibits the behavior in which (1) it receives no messages by other processes (until some time as in-flight messages must eventually be received by $Q$), and (2) $Q$ decides $v$.
%     Such a behavior of the process $Q$ exists due to \Cref{lemma:behavior_without_receptions}.
% \end{compactenum}
% As messages from $Q$ are delayed in $\mathcal{E}'$, all other correct processes cannot distinguish $\mathcal{E}'$ from $\mathcal{E}_c$ (until some time); hence, all other correct processes decide $v' \neq v$ in $\mathcal{E}'$.
% Therefore, there is a disagreement in $\mathcal{E}'$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
% Thus, $Q \in \processes{c}$.
% \end{sketch}

% The previous lemma shows that $Q \in \processes{c}$.
% Now, we construct an input configuration $c' \in \mathcal{I}$ such that $Q \notin \processes{c'}$:
% \begin{compactenum}
%     \item Let $c' \gets c$.

%     \item We remove $(Q, \cdot)$ from $c'$.

%     \item If $|\processes{c}| = n - t$, we add $(Z, \cdot)$ to $c'$, where $Z$ is any process such that $Z \notin \processes{c}$; note that such a process $Z$ exists as $t > 0$ and $Z \neq Q$ as $Q \in \processes{c}$ (by \Cref{lemma:q_in_c}).
% \end{compactenum}
% Due to the construction of $c'$, $c' \sim c$.
% Indeed, (1) $\processes{c'} \cap \processes{c} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c'} \cap \processes{c}$, the proposal of $P$ is identical in $c'$ and $c$ (by the step 1 of the construction).

% The lemma below shows that there exists a canonical execution $\mathcal{E}_{c'}$ such that (1) $\mathcal{E}_{c'}$ corresponds to $c'$, and (2) some value $v' \neq v$ is decided in $\mathcal{E}_{c'}$.

% \begin{lemma} \label{lemma:another execution}
% There exists a canonical execution $\mathcal{E}_{c'} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{c'}) = c'$, and (2) a value $v' \neq v$ is decided by a correct process in $\mathcal{E}_{c'}$.
% \end{lemma}
% \begin{proof}
% We fix any infinite canonical execution $\mathcal{E}_{c'} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{c'}) = c'$.
% As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{c'}$ is infinite, some value $v' \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{c'}$.
% As $c' \sim c$, $v' \in \mathit{val}(c)$ (by \Cref{lemma:helper_main}).
% Finally, $v' \neq v$ as (1) $v' \in \mathit{val}(c)$, and (2) $v \notin \mathit{val}(c)$, which concludes the proof.
% % Thus, xthe lemma.
% \end{proof}

% At last, we can ``merge'' the execution $\mathcal{E}_{c'}$ (from \Cref{lemma:another execution}) with the valid behavior of $Q$ in which $Q$ decides $v$ without having received any message (from \Cref{lemma:behavior_without_receptions}).
% Hence, we can construct an execution in which $\mathcal{A}$ violates \emph{Agreement}, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
% Therefore, correct processes send $\geq (\frac{t}{2})^2$ messages in $\mathcal{E}_{\mathit{base}}$, which means that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.

% \begin{theorem} [Lower bound on message complexity] \label{theorem:lower_bound_main}
% The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
% \end{theorem}

% Observe that, as each message contains (at least) a single word, \Cref{theorem:lower_bound_main} implies the $\Omega(t^2)$ lower bound on the communication complexity, as well.

% \subsection{Similarity \& Knowledge Conditions are Sufficient if $n > 3t$: General Algorithm \textsc{Complete}} \label{subsection:general_algorithm}

% In this subsection, we prove that $\mathcal{C}_S$ and $\mathcal{C}_K$ are sufficient conditions for a validity property to be solvable if $n > 3t$.\footnote{Recall that, when $n \leq 3t$, all solvable properties are trivial (\Cref{subsection:triviality_main}).}
% Namely, we present \textsc{Complete}, a Byzantine consensus algorithm with \emph{any} validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.
% Importantly, \textsc{Complete} achieves $O(n^2)$ message complexity, which makes it optimal (when $t \in \Omega(n)$); the communication complexity of \textsc{Complete} is $O(n^3)$.

% First, we formally define \emph{Interactive-Consistency Validity} \pierre{I guess interactive consistency is highly connoted with the desire to agree on the inputs of all correct processes, which is obviously possible iff the network is synchronous.}, and present a Byzantine consensus algorithm \textsc{Icon} with \emph{Interactive-Consistency Validity} (\Cref{subsubsection:interactive_consistency}).
% Then, we utilize \textsc{Icon} to obtain \textsc{Complete} (\Cref{subsubsection:Complete}).
% Throughout the entire subsection, $n > 3t$.

% % \newpage
% \subsubsection{\textsc{Icon}: Byzantine consensus with Interactive-Consistency Validity.} \label{subsubsection:interactive_consistency}
% In \textsc{Icon}, processes propose values, and agree on sets of $n - t$ process-proposal pairs.
% That is, processes agree on input configurations: $\mathcal{V}_O = \mathcal{I}_{n - t}$.

% Let us start by formally defining the \emph{Interactive-Consistency Validity} property:
% \begin{compactitem}
%      \item \emph{Interactive-Consistency Validity:} Let a correct process decide $\mathit{vector} \in \mathcal{I}_{n - t}$ such that (1) $(P, v)$ belongs to $\mathit{vector}$, for some value $v \in \mathcal{V}_I$, and (2) $P$ is a correct process.
%      Then, $v$ is $P$'s proposal.
% \end{compactitem}
% Intuitively, \emph{Interactive-Consistency Validity} states that, if a correct process decides that a value $v$ was proposed by a correct process $P$, then $P$'s proposal was indeed $v$.
% Observe that the Byzantine consensus problem with \emph{Interactive-Consistency Validity} is identical to the well-known interactive-consistency problem~\cite{ben2003resilient,thambidurai1988interactive,diamantopoulos2015interactive,fischer1982lower}, except that it does not require agreement on the proposals of \emph{all} processes: processes need to agree on the proposals of $n - t$ processes.

% The pseudocode of \textsc{Icon} is presented in \Cref{algorithm:interactive_consistency}.
% \textsc{Icon} achieves $O(n^2)$ message complexity and $O(n^3)$ communication complexity.
% We construct \textsc{Icon} by relying on \textsc{Quad}, a partially synchronous Byzantine consensus algorithm introduced by Civit \emph{et al.}~\cite{civit2022byzantine}; we give a brief description of \textsc{Quad} below.


% \paragraph{\textsc{Quad}.}
% Formally, \textsc{Quad} is concerned with two sets: (1) $\mathcal{V}_{\textsc{Quad}}$, a set of values, and (2) $\mathcal{P}_{\textsc{Quad}}$, a set of proofs.
% In \textsc{Quad}, processes propose and decide value-proof pairs.
% Moreover, there exists a function $\mathsf{valid}: \mathcal{V}_{\textsc{Quad}} \times \mathcal{P}_{\textsc{Quad}} \to \{ \mathit{true}, \mathit{false} \}$.
% As for the validity property, $\textsc{Quad}$ satisfies \emph{External Validity}: If a correct process decides a pair $(v, \Sigma)$, then $\mathsf{valid}(v, \Sigma) = \mathit{true}$.\footnote{We underline that our formalism in its current form is not expressive enough to describe \emph{External Validity}. However, we extend our formalism to accommodate for \emph{External Validity} in \Cref{subsection:external_validity}.}
% Importantly, \textsc{Quad} achieves $O(n^2)$ message complexity, which allows the message complexity of \textsc{Icon} to be $O(n^2)$.
% As for the communication complexity of \textsc{Quad}, it is $O(n^2 \cdot x)$, where $x$ denotes the maximum size of a proof.
% For completeness, we provide a detailed explanation of \textsc{Quad} in \Cref{section:quad_appendix}; 

% In our implementation of \textsc{Icon}
% (\Cref{algorithm:interactive_consistency}), we rely on a specific instance of \textsc{Quad} where (1) $\mathcal{V}_{\textsc{Quad}} = \mathcal{I}_{n - t}$ (i.e., processes propose input configurations), and (2) $\mathcal{P}_{\textsc{Quad}}$ is a set of $n - t$ \textsc{proposal} messages.
% Moreover, given an input configuration $c \in \mathcal{V}_{\textsc{Quad}}$ and a set of messages $\Sigma \in \mathcal{P}_{\textsc{Quad}}$, $\mathsf{valid}(c, \Sigma) = \mathit{true}$ if and only if, for every process-proposal pair $(P_j, v_j)$ which belongs to $c$, $\langle \textsc{proposal}, v_j \rangle_{\sigma_j} \in \Sigma$ (i.e., every process-proposal pair is accompanied by a properly signed \textsc{proposal} message).

% \paragraph{Description of \textsc{Icon}.}
% When a correct process $P_i$ proposes a value $v \in \mathcal{V}_I$ to \textsc{Icon} (line~\ref{line:propose}), the process broadcasts a signed \textsc{proposal} message (line~\ref{line:broadcast_proposal}).
% Once $P_i$ receives $n - t$ \textsc{proposal} messages (line~\ref{line:received_n_t_proposals}), $P_i$ constructs an input configuration $\mathit{vector}$ (line~\ref{line:construct_input_configuration}) and a proof 
% $\Sigma$ (line~\ref{line:construct_proof}) from the received \textsc{proposal} messages.
% Moreover, $P_i$ proposes $(\mathit{vector}, \Sigma)$ to \textsc{Quad} (line~\ref{line:propose_quad}).
% Finally, when $P_i$ decides a pair $(\mathit{vector}', \Sigma')$ from \textsc{Quad} (line~\ref{line:decide_quad}), $P_i$ decides $\mathit{vector}'$ 
%  from \textsc{Icon} (line~\ref{line:decide}).

% \begin{algorithm}
% \caption{\textsc{Icon}: Pseudocode for process $P_i$}
% \label{algorithm:interactive_consistency}
% \begin{algorithmic} [1]
% \State \textbf{Uses:}
% \State \hskip2em Best-Effort Broadcast, \textbf{instance} $\mathit{beb}$
% \State \hskip2em \textsc{Quad}, \textbf{instance} $\mathit{quad}$

% \medskip
% \State \textbf{upon} $\mathsf{init}$:
% \State \hskip2em $\mathsf{Integer}$ $\mathit{received\_proposals}_i \gets 0$ \Comment{the number of received proposals}
% \State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals}_i \gets \text{empty}$ \Comment{received proposals}
% \State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathsf{Message})$ $\mathit{messages}_i \gets \text{empty}$ \Comment{received \textsc{proposal} messages}

% \medskip
% \State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose}
% \State \hskip2em \textbf{trigger} $\mathit{beb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle_{\sigma_i} \big)$ \Comment{broadcast a signed proposal} \label{line:broadcast_proposal}

% \medskip
% \State \textbf{upon} reception of $\mathsf{Message}$ $m = \langle \textsc{proposal}, v_j \rangle_{\sigma_j}$ from process $P_j$ and $\mathit{received\_proposals} < n - t$:
% \State \hskip2em $\mathit{received\_proposals}_i \gets \mathit{received\_proposals}_i + 1$
% \State \hskip2em $\mathit{proposals}_i[P_j] \gets v_j$
% \State \hskip2em $\mathit{messages}_i[P_j] \gets m$

% \State \hskip2em \textbf{if} $\mathit{received\_proposals}_i = n - t$: \label{line:received_n_t_proposals}
% \State \hskip4em $\mathsf{Input\_Configuration}$ $\mathit{vector} \gets $ input configuration containing all process-proposal pairs from $\mathit{proposals}_i$ \label{line:construct_input_configuration}
% \State \hskip4em $\mathsf{Proof}$ $\Sigma \gets $ set of messages containing all \textsc{proposal} messages from $\mathit{messages}_i$ \label{line:construct_proof}
% \State \hskip4em $\mathit{quad}.\mathsf{propose}\big( (\mathit{vector}, \Sigma) \big)$ \label{line:propose_quad}

% \medskip
% \State \textbf{upon} $\mathit{quad}.\mathsf{decide}\big( (\mathsf{Input\_Configuration} \text{ } \mathit{vector}', \mathsf{Proof} \text{ } \Sigma') \big)$: \label{line:decide_quad}
% \State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector}')$ \label{line:decide}

% \end{algorithmic}
% \end{algorithm}

% \medskip
% For the lack of space, we delegate the proof of the correctness and complexity of \textsc{Icon} to \Cref{subsection:icon_appendix}
% \begin{theorem} [\textsc{Icon} is correct] \label{theorem:icon}
% \textsc{Icon} (\Cref{algorithm:interactive_consistency}) is a Byzantine consensus algorithm with Interactive-Consistency Validity.
% The message complexity of \textsc{Icon} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% % \begin{proof}
% % \emph{Agreement} follows directly from \emph{Agreement} of \textsc{Quad}.
% % Moreover, as there are (at least) $n - t$ correct processes, every correct process eventually proposes to \textsc{Quad} (line~\ref{line:propose_quad}).
% % Due to \emph{Termination} of \textsc{Quad}, every correct process eventually decides.
% % Therefore, \Cref{algorithm:interactive_consistency} satisfies \emph{Termination}.

% % It is left to prove that \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}.
% % Let $\mathit{vector}' \in \mathcal{I}_{n - t}$ be an input configuration decided by a correct process.
% % Due to \emph{External Validity} of \textsc{Quad}, if a process-proposal pair $(P_j, v_j)$ belongs to $\mathit{vector}'$, for some value $v_j \in \mathcal{V}_I$, $P_j$ has sent a properly signed \textsc{proposal} message for $v_j$.
% % If $P_j$ is correct, $v_j$ is its proposal as correct processes send \textsc{proposal} messages only for their proposals (line~\ref{line:broadcast_proposal}).
% % Thus, \Cref{algorithm:interactive_consistency} satisfies \emph{Interactive-Consistency Validity}.

% % The $O(n^2)$ message complexity of \textsc{Icon} follows from the following two facts: (1) correct processes only broadcast \textsc{proposal} messages (line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
% % As for the communication complexity of \textsc{Icon}, it is indeed $O(n^3)$ as (1) correct processes only broadcast $O(n^2)$ words (via the \textsc{proposal} messages; line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the communication complexity of \textsc{Quad} is $O(n^3)$ (because the maximum size of a proof is $O(n)$ words).
% % Thus, the theorem.
% % \end{proof}

% Observe that \textsc{Icon} (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed).
% We underline that a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} can be obtained even in a \emph{non-authenticated} setting; we provide such an algorithm in \Cref{section:appendix_non_authenticated}.

% \subsubsection{\textsc{Complete}: Byzantine consensus with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.} \label{subsubsection:Complete}
% The pseudocode of \textsc{Complete} is given in \Cref{algorithm:general}.
% \textsc{Complete} is directly obtained from \textsc{Icon}.
% When a correct process $P_i$ proposes (line~\ref{line:propose_general}) to \textsc{Complete}, the proposal is forwarded to \textsc{Icon} (line~\ref{line:propose_ic}).
% Once $P_i$ decides an input configuration $c \in \mathcal{I}_{n - t}$ from \textsc{Icon} (line~\ref{line:decide_ic}), $P_i$ decides the common value $\Lambda(c)$ from \textsc{Complete} (line~\ref{line:decide_general}).

% \begin{algorithm}
% \caption{\textsc{Complete}: Pseudocode for process $P_i$}
% \label{algorithm:general}
% \begin{algorithmic} [1]
% \State \textbf{Uses:}
% \State \hskip2em \textsc{Icon}, \textbf{instance} $\mathit{icon}$

% \medskip
% \State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose_general}
% \State \hskip2em \textbf{trigger} $\mathit{icon}.\mathsf{propose}(v)$ \label{line:propose_ic}

% \medskip
% \State \textbf{upon} $\mathit{icon}.\mathsf{decide}(\mathsf{Input\_Configuration} \text{ } c)$: \label{line:decide_ic}
% \State \hskip2em \textbf{trigger} $\mathsf{decide}\big( \Lambda(c) \big)$ \label{line:decide_general}
% \end{algorithmic}
% \end{algorithm}

% \begin{theorem} [\textsc{Complete} is correct] \label{theorem:general_algorithm}
% Let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$.
% \textsc{Complete} (\Cref{algorithm:general}) is a Byzantine consensus algorithm with $\mathit{val}$.
% The message complexity of \textsc{Complete} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% \begin{proof}
% \emph{Termination} and \emph{Agreement} of \textsc{Complete} follow from \emph{Termination} and \emph{Agreement} of \textsc{Icon}, respectively.
% Moreover, the message (resp., communication) complexity of \textsc{Complete} follows from the message (resp., communication) complexity of \textsc{Icon}.

% Finally, we prove that \textsc{Complete} satisfies $\mathit{val}$.
% Consider any execution $\mathcal{E}$ of $\textsc{Complete}$ such that $\mathsf{input\_conf}(\mathcal{E}) = c^*$, for some input configuration $c^* \in \mathcal{I}$.
% Let $c \in \mathcal{I}_{n - t}$ be the input configuration correct processes decide from \textsc{Icon} in $\mathcal{E}$ (line~\ref{line:decide_ic}).
% As \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}, we have that, for every process $P \in \processes{c^*} \cap \processes{c}$, $P$'s proposals in $c^*$ and $c$ are identical.
% Hence, $c \sim c^*$.
% Therefore, $\Lambda(c) \in \mathit{val}(c^*)$ (by the definition of the $\Lambda$ function).
% Thus, $\mathit{val}$ is satisfied by \textsc{Complete}, which concludes the proof.
% \end{proof}

% As \textsc{Complete} (\Cref{algorithm:general}) is a Byzantine consensus algorithm with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$ (\Cref{theorem:general_algorithm}), $\mathcal{C}_S$ and $\mathcal{C}_K$ are sufficient conditions for solvable validity properties when $n > 3t$.
% We underline that any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$ can be solved even in a non-authenticated setting: we simply use a non-authenticated version of \textsc{Icon} (see \Cref{section:non_auth}) in \Cref{algorithm:general}.

% Lastly, as \textsc{Complete} relies on \textsc{Icon}, we conclude that \emph{Interactive-Consistency Validity} is a \emph{strongest} validity property.
% That is, a Byzantine consensus algorithm with any solvable validity property (i.e., with any validity property which satisfies $\mathcal{C}_S$ and $\mathcal{C}_K$) can be obtained from a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity}.

\iffalse
\paragraph{\emph{$\textsc{IC}_{\mathit{non-auth}}$}: Solution in a non-authenticated setting.}
In order to implement $\textsc{IC}_{\mathit{non-auth}}$, we rely on the binary DBFT~\cite{CGL18} consensus algorithm.
DBFT is a partially synchronous Byzantine consensus algorithm, which (1) satisfies \emph{Strong Validity}, and (2) does not require digital signatures.

\begin{algorithm}
\caption{$\textsc{IC}_{\mathit{non-auth}}$: Pseudocode for process $P_i$}
\label{algorithm:interactive_consistency}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Byzantine Reliable Broadcast, \textbf{instance} $\mathit{brb}$
\State \hskip2em Binary DBFT, \textbf{instances} $\mathit{dbft}[1], ..., \mathit{dbft}[n]$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Integer}$ $\mathit{decided}_0 \gets 0$
\State \hskip2em $\mathsf{Integer}$ $\mathit{decided}_1 \gets 0$
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals} \gets \text{empty}$
\State \hskip2em $\mathsf{Set}(\mathsf{Integer})$ $\mathit{proposed\_to} \gets \emptyset$

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$:
\State \hskip2em \textbf{trigger} $\mathit{brb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle \big)$

\medskip
\State \textbf{upon} $\mathit{brb}.\mathsf{deliver}\big( \langle \textsc{proposal}, v_j \rangle \big)$ from process $P_j$:
\State \hskip2em $\mathit{proposals}[P_j] \gets v_j$
\State \hskip2em $\mathit{proposed\_to} \gets \mathit{proposed\_to} \cup \{j\}$
\State \hskip2em \textbf{trigger} $\mathit{dbft}[j].\mathsf{propose}(1)$

\medskip
\State \textbf{upon} $\mathit{dbft}[j].\mathsf{decide}(x)$:
\State \hskip2em $\mathit{decided}_x \gets \mathit{decided}_x + 1$

\medskip
\State \textbf{upon} $\mathit{decided}_1 \geq n - t$ for the first time:
\State \hskip2em \textbf{for every} $j \in [1, n] \setminus{\mathit{proposed\_to}}$:
\State \hskip4em \textbf{trigger} $\mathit{dbft}[j].\mathsf{propose}(0)$

\medskip
\State \textbf{upon} $\mathit{decided}_0 + \mathit{decided}_1 = n$ and, for the first $n - t$ processes $P_j$ with $\mathit{dbft}[j].\mathsf{decide}(1)$, $\mathit{proposals}[j] \neq \bot$:
\State \hskip2em $\mathit{vector} \gets \text{input configuration constructed of the first } n - t \text{ process-proposal pairs}$
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector})$

\end{algorithmic}
\end{algorithm}

\subsection{similarity and knowledge condition}

Let $\mathcal{A}$ be an algorithm with consensus interface and ensuring termination. Let $c\in \mathcal{I}$ be a an input configuration. The \emph{canonical execution w.r.t. $\mathcal{A}$ and $c$}, noted $\mathit{can}(\mathcal{A},c)$, is the infinite execution $e$ of $\mathcal{A}$ s.t. (1) $\mathit{GST}_e = 0$, (2) $\forall P_j \notin \pi(c)$, $P_j$ crashes immediately without any computational step, (3) $\forall P_i \in \pi(c)$, $P_i$ proposes the value $c[i]$, (4) All the messages are received in time $\delta$ exactly.
Let $c' \in \mathcal{I}$, s.t. $c' \sim c$. The \emph{dual execution w.r.t. $\mathcal{A}$, $c$ and $c'$}, noted $\mathit{dual}(\mathcal{A},c,c')$ is the infinite execution $e'$ s.t. (1) We note $e = \mathit{can}(\mathcal{A},c)$ and $T$ the minimum time s.t. all processes in $\pi(c)$ have decided in $e$, (2) the longest prefix of $e$ that does not exceed time $T$ is equal to the longest prefix of $e'$ that does not exceed time $T$ (3) $GST_{e'} = T$, (4) The processes in $\pi(c') \setminus \pi(c)$ start at time $T$, (5) The processes in $\pi(c) \setminus \pi(c')$ crash at time $T$.

Let $\mathit{val}$ be a validity property.
If $\mathcal{A}$ is a consensus algorithm ensuring $\mathit{val}$, then $\mathit{val}$ verifies similarity condition.

Indeed, otherwise we note $c$ s.t. $\bigcap_{c' \in \mathit{sim}(c)} \mathit{val}(c') = \emptyset$, $e = \mathit{can}(\mathcal{A},c)$, $\mathit{dec}$ the decision decided in $e$, $c'$ an input configuration in $\mathit{sim}(c)$ s.t. $dec \notin \mathit{val}(c')$ and $e' = \mathit{dual}(\mathcal{A},c,c')$.
By construction, there exists $P_j \in \pi(c) \cap \pi(c')$ with the same behavior in both $e$ and $e'$ until time $T$.
Thus $P_j$ decides $dec$ in $e'$, which contradicts the fact that $\mathcal{A}$ ensures $\mathit{val}$ since $\mathit{dec} \notin \mathit{val}(c')$.

Finally, we can note $\Lambda_{\mathcal{A},\mathit{val}} : c \in \mathcal{I} \mapsto \mathit{decision}(\mathit{can}(\mathcal{A},c))$.


\pierre{end of the discussion about knowledge condition about}
\jovan{I do not really understand the difference between what you wrote and what was already written before. What am I missing?}

\pierre{Ideally, I would like to stress that authencation is not required for computability. Here are some thoughts}
\jovan{I completely agree!}

\paragraph*{Brief Description of Vector Consensus Without Authentication}

Every correct process Reliable-Bcast its proposal (without Authentication). Upon, RB-delivery of message from $P_i$, propose $1$ to a binary-DBFT instance implementing a Binary Consensus with Strong Validity (without authentication). Eventually $n-t$ instances will be decided and their value will be $1$ because of strong validity. Then propose $0$ to the remaining instances. Decide the associated vector with at least $n-t$ components.

\jovan{Yes, definitely. Good point!}

\paragraph*{Sufficiency of similarity condition}

\begin{lemma}
Let $\mathit{val}$ be a validity property verifying similarity condition (with $t<n/3$), then there exists a $t$-resilient partially synchronous algorithm among $n$ processes that solves Byzantine consensus with validity $\mathit{val}$.
\end{lemma}

\begin{proof}
(Sketch)

We use a vector consensus that will allow the processes to agree on a vector of $n-t$ proposals associated with an id. We note $k$ the associated input configuration of size $|\pi(k)| \geq n-t$. Let us note that $P_j \in \pi(k)$ does not imply that $P_j$ is correct.
Then, every correct process decides $\Lambda(k)$.
Since $\mathit{val}$ verifies similarity condition, $\Lambda(k) \in \bigcap_{c \in \mathit{sim}(k)} \mathit{val}(c)$. Moreover, every input configuration $c$ matched by the execution $e$ that led to the pre-decision of vector $k$ is in $\mathit{sim}(k)$. Indeed, if a process $P_j$ in $\pi(k)$ is Byzantine, then its $P_j \notin \pi(c)$, while if a process $P_i \in \pi(c) \cap \pi(k)$, it is correct in $e$ and this is its input $c[i]$ that appears in $k[i]$ by property of Reliable-Broadcast.
\end{proof}

\paragraph*{A few comments}

\begin{itemize}
    \item The vector validity $\mathit{val}_{\mathit{vect}}$ (the decided value is a vector of $n-t$ values whose $n-2t$ among them correspond to the correct proposal of correct processes only) is the strongest achievable validity property in the sense that if you have an algorithm $\mathcal{A}_{\mathit{vect}}$ that achieves vector validity, then for every every satisfiable validity property $\mathit{val}$, it is possible to trivially design an algorithm $\mathcal{A}$ that returns $\Lambda_{\mathcal{A}}(\overset{\rightarrow}{v})$, where $\overset{\rightarrow}{v}$ is the value returned by $\mathcal{A}_{\mathit{vect}})$ as a black-box.
    Let us note that this transformation uses only one instance of $\mathcal{A}_{\mathit{vect}})$ and no additional communication nor latency.
    
    \item The impossibility results for validity properties that do not ensure similarity conditions only needs asynchrony and crash failures (we do not need to invocate Byzantine failures for this proof).
    
    \item If $\Theta(t^2)$ is a tight bound for partially synchronous Byzantine Agreement with strong validity or weak validity under threshold setup (Quad, SQuad and new lower bound for weak validity), here are some open problems:
    \begin{itemize}
        \item  bound for vector validity for any setup
        \item  bound for any validity for any setup except threshold setup
    \end{itemize}
\end{itemize}




\pierre{end of the discussion about sufficiency without authentication}
\jovan{I like it very much. All very good points! }

\subsection{The Similarity and Knowledge Conditions are Sufficient}

In this subsection, we prove that both the similarity and knowledge conditions together are sufficient for a validity property to be satisfiable.
We divide the subsection into two parts: (1) we consider the case of $n > 3t$, and (2) we consider the case of $n \leq 3t$.

\subsubsection{$n > 3t$}

We now prove the following theorem.

\begin{theorem} [The similarity and knowledge conditions are sufficient] \label{theorem:similarity_sufficient}
If a validity property satisfies the similarity and knowledge conditions, the validity property is satisfiable.
\end{theorem}

%In order to prove \ref{theorem:similarity_sufficient}, we will be constructing a general algorithm that solves consensus given any validity property that satisfies [GONE FOR LUNCH, WORK IN PROGRESS]


\begin{proof}
Let $\mathit{val}$ be any validity property that satisfies the similarity condition and the knowledge condition.
In order to conclude the theorem, we present an algorithm that solves the Byzantine consensus problem with $\mathit{val}$.

First, we assume an existence of a black-box Byzantine consensus protocol in which every value is proposed along with a matching proof. 
and where the protocol satisfies the following properties:
\begin{compactitem}
   \item Termination: Every correct process eventually decides.
   
   \item Agreement: No two correct processes decide different values.
   
   \item Validity-by-proof: If a correct process decides a value $v$, then $v$ is accompanied by a matching proof.
\end{compactitem}
The protocol is provided with the function $\mathit{matches}$ such that $\mathit{matches}(v, \mathit{proof}) = \mathit{true}$ if $\mathit{proof}$ matches $v$.
For example, by adding proofs to values and providing the $\mathit{matches}$ function, one can modify the HotStuff~\cite{yin2019hotstuff} or \textsc{quad}~\cite{civit2022byzantine} protocol to solve the aforementioned consensus problem with $n > 3t$. A more detailed explanation of the construction of this type of black-box can also be found in \textsc{quad}~\cite{civit2022byzantine}.

\begin{algorithm}
\caption{Partially synchronous Byzantine algorithm $\mathcal{A}_B$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_byzantine}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Byzantine Consensus with Validity-By-Proof, \textbf{instance} $c$
\State \hskip2em Byzantine Consistent Broadcast, \textbf{instance} $\mathit{bcb}$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{trigger} $\mathit{bcb}.\mathsf{broadcast}\big( [\textsc{proposal}, \mathit{proposal}] \big)$

\medskip
\State \textbf{upon} delivery of $n - t$ \textsc{proposal} messages:
\State \hskip2em $\mathsf{Input\_Configuration}$ $\mathit{input} \gets$ the input configuration built out of the received $n - t$ \textsc{proposal} messages
\State \hskip2em $\mathsf{Value}$ $\mathit{to\_propose} \gets $ find a common value among all input configurations that belong to $\mathit{sim}(\mathit{input})$
\State \hskip2em \(\triangleright\) $\mathit{to\_propose}$ is accompanied by the received \textsc{proposal} messages which act as a proof of $\mathit{to\_propose}$
\State \hskip2em \textbf{trigger} $c.\mathsf{propose}(\mathit{to\_propose}, \text{all received \textsc{proposal} messages})$ \label{line:partially_propose_c_byzantine}

% \medskip
% \State \textbf{upon} timer elapsed:
% \State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
% \State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i_byzantine}
% \State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
% \State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
% \State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
% \State \hskip2em \textbf{else:} 
% \State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{ByzSim}(i)$ \label{line:partially_set_to_propose}

% \State \hskip2em \(\triangleright\) all values are associated with received \textsc{proposal} messages which proves the validity of the proposed values
% \State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c_byzantine}

\medskip
\State \textbf{upon} $c.\mathsf{decide}(\mathit{dec})$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

First, \Cref{algorithm:partially_synchronous_byzantine} ensures termination as (1) every correct process eventually receives $n - t$ \textsc{proposal} messages, and (2) $c$ ensures termination.
Furthermore, \Cref{algorithm:partially_synchronous_byzantine} ensures agreement as $c$ ensures agreement.
Hence, it is left to prove that \Cref{algorithm:partially_synchronous_byzantine} ensures $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \allconfigurations$.
Let $P$ be a (faulty or correct) process that obtains a value $v$ with its proof; the proof of value $v$ is an input configuration $i$ which consists of $n - t$ process-proposal pairs such that $v \in \bigcap\limits_{i' \in \mathit{sim}(i)} \mathit{val}(i')$.
If there exist process-proposal pairs $\mathit{pp}$ and $\mathit{pp}'$ such that (1) $\mathit{pp}$ belongs to $\mathit{input}$, (2) $\mathit{pp}'$ belongs to $i$, and (3) $\mathit{pp}$ and $\mathit{pp}'$ are associated with the same process, then $\mathit{pp} = \mathit{pp}'$ as correct processes truthfully report their proposal via the \textsc{proposal} message.
Hence, $\mathit{i} \sim \mathit{input}$, which means that $v \in \mathit{val}(\mathit{input})$.
Thus, for any value $v^*$ for which a proof is obtained, $v^* \in \mathit{val}(\mathit{input})$.
Due to the validity-by-proof property of $c$, the decided value must belong to $\mathit{val}(\mathit{input})$, which means that \Cref{algorithm:partially_synchronous_byzantine} satisfies $\mathit{val}$.
Finally, $\mathit{val}$ is satisfiable, which concludes the proof of the theorem.
\end{proof}

\subsubsection{$n \leq 3t$}

If $n \leq 3t$, we prove that each satisfiable validity property is trivial, i.e., correct processes can decide with \emph{no communication}.
We fix a satisfiable validity property $\mathit{val}$ such that (1) $n \leq 3t$, and (2) a partially synchronous distributed protocol $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.

We start by defining compatibility of executions.

\begin{definition} [Compatible executions] \label{definition:compatible_executions}
Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $e'$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $x = |\mathit{Corr}_{\mathcal{A}}(e) \cap \mathit{Corr}_{\mathcal{A}}(e')|$.
We say that executions $e$ and $e'$ are \emph{compatible} if (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(e)|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(e')|$.
\end{definition}

Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without sending any message).
We denote by $\mathit{compatible}(e)$ the set of all infinite executions compatible with $e$, i.e., $\mathit{compatible}(e) = \{e' \,|\, e \text{ and } e' \text{ are compatible} \}$.

% Consider an infinite execution $e_1$ of $\mathcal{A}$ such that all faulty processes immediately crash (i.e., without sending any message).
% Let $c_1$ denote the number of correct processes in $e_1$; $c_1 \geq n - t$.
% Consider another infinite execution $e_2$ of $\mathcal{A}$ such that all faulty processes immediately crash (i.e., without sending any message).
% Let $c_2$ denote the number of correct processes in $e_2$; $c_2 \geq n -t$.
% We say that $e_2$ is \emph{compatible} with $e_1$ if the number of processes correct in both $e_1$ and $e_2$ is $x$ such that (1) $x \leq t$, (2) $x < c_1$, and (3) $x < c_2$.
% Finally, we denote by $\mathit{compatible}(e_1)$ the set of all infinite executions compatible with $e_1$, i.e., $\mathit{compatible}(e_1) = \{e \,|\, e \text{ is compatible with } e_1\}$.

\begin{lemma} \label{lemma:first_step}
Let $e$ be an infinite execution of $\mathcal{A}$ such that all faulty processes (if any) crash immediately (i.e., without taking any computational step).
Let $\mathit{dec}$ be the value decided in $e$.
For every execution $e' \in \mathit{compatible}(e)$, $\mathit{dec}$ is decided in $e'$.
\end{lemma}
\begin{proof}
By contradiction, let there exist an infinite execution $e' \in \mathit{compatible}(e)$ such that $\mathit{dec}$ is not decided in $e'$.
Let $x = |\mathit{Corr}_{\mathcal{A}}(e) \cap \mathit{Corr}_{\mathcal{A}}(e')|$.
As $e$ and $e'$ are compatible, we have: (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(e)|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(e')|$ (by \Cref{definition:compatible_executions}).
Hence, there exists a process $P$ such that (1) $P$ is correct in $e$, and (2) $P$ is not correct in $e'$ (as $x < |\mathit{Corr}_{\mathcal{A}}(e)|$).
Similarly, there exists another process $Q \neq P$ such that (1) $Q$ is correct in $e'$, and (2) $Q$ is not correct in $e$ (as $x < |\mathit{Corr}_{\mathcal{A}}(e')|$).
Thus, we can merge executions $e$ and $e'$ into an execution with $x \leq t$ faulty processes in which $P$ and $Q$ disagree.
Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies agreement while tolerating up to $t$ faulty processes, which concludes the proof of the lemma.
% The number of correct processes in $e$ is $c$, whereas the number of correct processes in $e'$ is $c'$.
% The number of correct processes in $e'$ is $\geq n - t$.
% Moreover, the number of processes which are correct in both $e_1$ and $e_2$ is $x$ such that (1) $x \leq t$, (2) $x < c$, and (3) $x < c'$.
% $< n - t$ and $\leq t$.
% Hence, there exists one process $P$ such that (1) $P$ is correct in $e$, and (2) $P$ is not correct in $e'$.
% Moreover, there exists another process $Q \neq P$ such that (1) $Q$ is correct in $e'$, and (2) $Q$ is not correct in $e$.
% Thus, we can merge executions $e$ and $e'$ into an execution with $x \leq t$ faulty processes in which $P$ and $Q$ disagree.
% The lemma holds.
\end{proof}  

We fix an input configuration with exactly $n - t$ process-proposal pairs; we denote this input configuration by $\mathit{base}$.
Let $E_{\mathit{base}}$ be an infinite execution of $\mathcal{A}$ such that (1) $E_{\mathit{base}}$ corresponds to $\mathit{base}$, and (2) all faulty processes ($t$ of them) crash immediately (i.e., without sending any message).
Let $\mathit{dec}$ be the value decided in $E_{\mathit{base}}$. 

\begin{lemma} \label{lemma:second_step}
$\mathit{compatible}(E_{\mathit{base}}) \neq \emptyset$.
\end{lemma}
\begin{proof}
Let us take a set $B$ of processes such that (1) $|B| = n - t$, and (2) $B$ contains all $t$ processes that do not belong to $\mathit{base}.\mathsf{processes}$.
Hence, $B \cap \mathit{base}.\mathsf{processes } = n - 2t$.
Moreover, $n - 2t \leq t$ as $n \leq 3t$.
Lastly, there exists a process $P \in B \setminus{\mathit{base}.\mathsf{processes}}$ (as $t > 0$ and $B$ contains $t$ processes which do not belong to $\mathit{base}.\mathsf{processes}$).
% Any two groups of $n - t$ processes intersect at at most $t$ processes as $n \leq 3t$.
% Indeed, $n - t + n - t - n \leq t$, which implies that $n - 2t \leq t$, which is always true as $n \leq 3t$.
% Furthermore, there exists a process $P$ which is faulty in $E_{\mathit{base}}$ as $t > 0$.
Hence, there exists an infinite execution $e$ such that (1) exactly $n - t$ processes are correct in $e$ (processes from the group $B$), (2) $P \in B$ is correct in $e$, and (3) all faulty processes ($t$ of them) crash immediately.
Moreover, $e$ and $E_{\mathit{base}}$ are compatible (by \Cref{definition:compatible_executions}).
Thus, the lemma.
\end{proof}


% By \Cref{lemma:first_step}, $\mathit{dec}$ must be decided in every execution of $\mathit{compatible}(e)$.
% Furthermore, $\mathit{dec} \in \mathit{val}(i)$, for every input configuration $i \in \allconfigurations$ that corresponds to an execution which belongs to $\mathit{compatible}(e)$.
% We now show that $\mathit{dec} \in \mathit{val}(i')$, for every $i' \in \allconfigurations$.

\begin{theorem} 
For every input configuration $i \in \allconfigurations$, $\mathit{dec} \in \mathit{val}(i)$.
\end{theorem}
\begin{proof}
By \Cref{lemma:second_step}, $\mathit{compatible}(E_{\mathit{base}}) \neq \emptyset$.
By \Cref{lemma:first_step}, $\mathit{dec}$ is decided in every execution compatible with $E_{\mathit{base}}$.
We fix one such execution; let this execution be denoted by $E_{i'} \in \mathit{compatible}(E_{\mathit{base}})$.
Let $x = |\mathit{Corr}_{\mathcal{A}}(E_{\mathit{base}}) \cap \mathit{Corr}_{\mathcal{A}}(E_{i'})|$.
As $e \in \mathit{compatible}(E_{\mathit{base}})$, we have: (1) $x \leq t$, (2) $x < |\mathit{Corr}_{\mathcal{A}}(E_{\mathit{base}})|$, and (3) $x < |\mathit{Corr}_{\mathcal{A}}(E_{i'})|$. 
Let $i'$ be an input configuration which corresponds to $E_{i'}$.
Recall that $\mathit{dec}$ is decided in $E_{i'}$.
% As $\mathit{dec}$ is decided in $e$, $\mathit{dec} \in \mathit{val}(i')$.

Let $i \in \allconfigurations$ be any input configuration.
Let $y = |i.\mathsf{processes} \cap i'.\mathsf{processes}|$.
We consider two possible cases:
\begin{compactitem}
   \item Let (1) $y \leq t$, (2) $y < |i.\mathsf{processes}|$, and (3) $y < |i'.\mathsf{processes}|$.
   Let $E_i$ be an infinite execution of $\mathcal{A}$ such that (1) $E_i$ corresponds to $i$, and (2) all faulty processes (if any) crash immediately.
   Hence, $E_i$ and $E_{i'}$ are compatible (by \Cref{definition:compatible_executions}).
   As $\mathit{dec}$ is decided in $E_{i'}$, $\mathit{dec}$ is decided in $E_i$ (by \Cref{lemma:first_step}).
   Therefore, $\mathit{dec} \in \mathit{val}(i)$, which concludes this case.
   
   \item Let (1) $y > t$, or (2) $y \geq |i.\mathsf{processes}|$, or (3) $y \geq |i'.\mathsf{processes}|$.
   We further distinguish three cases:
   \begin{compactitem}
        \item Let $y > t$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then (1) $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$, and (2) go to step 1.
                
                \item If $P_j \in i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i'$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (as $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Hence, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        Lastly, for every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a prefix of $E^*$ exists as $y > t > 0$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, the following holds for $E_i$: (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$, which confirms the statement of the lemma in this case.
        
        \item Let $y \geq |i.\mathsf{processes}|$.
        Hence, $y = |i.\mathsf{processes}|$, which means that, for every process $P \in i.\mathsf{processes}$, $P \in i'.\mathsf{processes}$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then (1) $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$, and (2) go to step 1.
                
                \item If $P_j \in i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i'$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by the construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (because $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Thus, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        For every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a process exists as every process that belongs to $i.\mathsf{processes}$ also belongs to $\mathit{Corr}_{\mathcal{A}}(E^*)$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$.
        
        \item Let $y \geq |i'.\mathsf{processes}|$.
        Hence, $y = |i'.\mathsf{processes}|$, which means that, for every process $P \in i'.\mathsf{processes}$, $P \in i.\mathsf{processes}$.
        We build an input configuration $i^* \in \allconfigurations$ in the following manner:
        \begin{compactenum}
            \item For every process $P_j \in \Psi$:
            \begin{compactenum}
                \item If $P_j \in i.\mathsf{processes} \cap i'.\mathsf{processes}$, then $(P_j, \mathit{proposal})$ is added to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$.
            \end{compactenum}
        \end{compactenum}
        Let $E^*$ be an infinite execution of $\mathcal{A}$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (if any) crash immediately.
        We have that $i^*.\mathsf{processes} = i'.\mathsf{processes}$ (by the construction of $i^*$).
        Therefore, $E^*$ and $E_{\mathit{base}}$ are compatible (because $E_{i'}$ and $E_{\mathit{base}}$ are compatible).
        Thus, $\mathit{dec}$ is decided in $E^*$ (by \Cref{lemma:first_step}).
        
        For every process $P$ such that (1) $P$ is correct in $E^*$, and (2) $P \in i.\mathsf{processes}$, $P$'s proposal in $E^*$ is identical to its proposal as specified by $i$ (follows from the construction of $i^*$).
        Hence, we can create an execution $E_i$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $P \in i.\mathsf{processes}$ that decides in $E^*_{\mathit{prefix}}$.
            Such a process exists as every process that belongs to $\mathit{Corr}_{\mathcal{A}}(E^*)$ also belongs to $i.\mathsf{processes}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, all processes that belong to $i.\mathsf{processes}$ are correct and live and have the proposals as specified by $i$.
            All other processes crash (if not have crashed before).
        \end{compactenum}
        Therefore, (1) $E_i$ corresponds to $i$, and (2) $\mathit{dec}$ is decided in $E_i$.
        Thus, $\mathit{dec} \in \mathit{val}(i)$.
   \end{compactitem}
\end{compactitem}
We have shown that, for every input configuration $i \in \allconfigurations$, $\mathit{dec} \in \mathit{val}(i)$.
Thus, the theorem.
\end{proof}

\begin{corollary} \label{corollary:trivial_validity}
Let $\mathit{val}$ be any satisfiable validity property.
Let $n \leq 3t$.
Then, $\mathit{val}$ is a trivial validity property, i.e., there exists a value $v \in \mathcal{V}$ such that, for every input configuration $i \in \allconfigurations$, $v \in \mathit{val}(i)$.
\end{corollary}


\iffalse
Let $\Pi \subseteq \Psi$ be any set of processes.
Moreover, let $x < |\Pi|$ be an integer.
We denote by $\mathit{execs}_{\mathcal{A}}(\Pi, x)$ a set of infinite executions of $\mathcal{A}$ such that (1) at most $x$ members of $\Pi$ does not crash immediately (i.e., without sending any message), and (2)  in every execution of $\mathit{execs}_{\mathcal{A}}(\Pi, x)$.
 




\paragraph{Let $n \leq 2t$.}
Let $\Pi \subseteq \Psi$ be any set of processes.
We denote by $\mathit{execs}_{\mathcal{A}}(\Pi)$ a set of infinite executions of $\mathcal{A}$ such that all processes from $\Pi$ crash immediately (i.e., without sending any message) in every execution of $\mathit{execs}_{\mathcal{A}}(\Pi)$.

We fix an input configuration $\mathit{input} \in \allconfigurations$ such that $\mathit{input}$ consists of exactly $n - t$ process-proposal pairs.
Let $\Pi$ denote the set of processes that belong to $\mathit{input}$; recall that $|\Pi| = n - t$.
We show that there exists a value $x \in \mathcal{V}$ such that (1) $x \in \mathit{val}(\mathit{input})$, and (2) $x$ is decided in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$.

\begin{lemma}
Let $\mathit{input} \in \allconfigurations$ be any input configuration such that $|\mathit{input}| = n - t$.
Let $\Pi$ denote the set of processes associated with $\mathit{input}$; $|\Pi| = n - t$.
There exists a value $x \in \mathit{val}(\mathit{input})$ such that $x$ is decided in every execution $e$ that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$.\footnote{Recall that $\mathit{execs}_{\mathcal{A}}(\Pi) \neq \emptyset$ as $n \leq 2t$.}
\end{lemma}
\begin{proof}
First, we show that, in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$, the decided value belongs to $\mathit{val}(\mathit{input})$.
By contradiction, let there exist an infinite $e \in \mathit{execs}_{\mathcal{A}}(\Pi)$ such that the decided value is $v \notin \mathit{val}(\mathit{input})$.
Let $\mathit{input}' \in \allconfigurations$ be an input configuration that corresponds to $e$.
We denote by $e^*$ the prefix of $e$ in which a process $P$ decides $v \notin \mathit{val}(\mathit{input})$.

Now, consider any execution $E$ that corresponds to $\mathit{input}$ in which all faulty processes (per $\mathit{input}$) crash immediately (i.e., without sending any messages).
As $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$, processes decide a value $v' \in \mathit{val}(\mathit{input})$ in $E$.
Hence, we can merge executions $e^*$ and $E$ to construct another execution in which two correct processes disagree (as one decides $v$ and another $v'$ such that $v \neq v'$). 
Thus, in every execution that belongs to $\mathit{execs}_{\mathcal{A}}(\Pi)$, the decided value belongs to $\mathit{val}(\mathit{input})$.

Finally, by contradiction, let there exist executions $e_1, e_2 \in \mathit{execs}_{\mathcal{A}}(\Pi)$ such that (1) the decided value in $e_1$ is $v_1 \in \mathit{val}(\mathit{input})$, (2) the decided value in $e_2$ is $v_2 \in \mathit{val}(\mathit{input})$, and (3) $v_1 \neq v_2$.
Let us take one execution $E$ that corresponds to $\mathit{input}$ in which all faulty processes (per $\mathit{input}$) crash without sending any message.
Hence, the value decided in $E$ is different from $v_1$ or different from $v_2$.
If it is different from $v_1$, we can merge executions $E$ and $e_1$ to reach disagreement.
Otherwise, we can merge executions $E$ and $e_2$ to reach disagreement.
Therefore, the lemma holds.
\end{proof}
\fi
\fi

==> sections/former/conclusion.tex <==
\section{Concluding Remarks} \label{section:conclusion}

This paper studies the validity property of partially synchronous Byzantine consensus.
Namely, we mathematically formalize validity properties, and give the necessary and sufficient conditions for a validity property to be solvable (i.e., for the existence of an algorithm which solves a consensus problem defined with that validity property, in addition to \emph{Agreement} and \emph{Termination}).
Moreover, we prove a quadratic lower bound on the message complexity for all non-trivial (and solvable) validity properties.
Previously, this bound was mainly known for \emph{Strong Validity}.
Lastly, we introduce \general, a general algorithm for  consensus with any solvable (and non-trivial) validity property; assuming a threshold signature scheme, \general achieves $O(n^2)$ message complexity, showing that the aforementioned lower bound is tight (with $t \in \Omega(n)$).

A reasonable future research direction is an extension of this work to synchronous environments.
Similarly, can we extend our results to randomized protocols?
% However, our proof technique for the lower bound on message complexity cannot be reused as such: this is because faults can be detected in a timely fashion in synchrony.
% Thus, we believe that the lower bound on message complexity for synchronous consensus is one of the most important open questions.
% Another interesting question is whether our lower bound holds for randomized consensus.
% In~\cite{DBLP:conf/podc/AbrahamCDNP0S19}, it is proven that randomized consensus with \emph{Strong Validity} has $\Omega(t^2)$ expected message complexity.
% Can this bound be extended to all non-trivial validity properties?
Furthermore, investigating consensus variants in which ``exact'' agreement among correct processes is not required (such as approximate~\cite{AbrahamAD04,MendesH13,GhineaLW22,ghinea2023multidimensional} or $k$-set~\cite{BouzidIR16,Delporte-Gallet20,Delporte-Gallet22,lynch1996distributed} agreement) constitutes another natural extension of this work.

Finally, we restate the question posed at the end of \Cref{subsection:general_algorithm}.
Is it possible to solve vector consensus with $o(n^3)$ exchanged bits and polynomial latency?
Recall that, due to the design of \general (\Cref{subsection:general_algorithm}), any (non-trivial) consensus variant can be solved using vector consensus.
Therefore, an upper bound on the complexity of vector consensus is an upper bound on the complexity of any consensus variant.
Hence, lowering the $O(n^3)$ communication complexity of vector consensus (while preserving polynomial latency) constitutes an important future research direction.

\begin{acks}
We would like to thank Rafael Pinot, Matteo Monti, Nirupam Gupta and Pierre-Louis Roman for the helpful discussions and comments.
This work was funded in part by the Hasler Foundation (\#21084), the Singapore grant MOE2018-T2-1-160, and the ARC Future Fellowship program (\#180100496).
\end{acks}
% Our (authenticated) implementation of vector consensus (\Cref{algorithm:interactive_consistency}) has $O(n^3)$ communication complexity.
% If the communication complexity of vector consensus can be reduced from $O(n^3)$ (while preserving a reasonable latency), then, by applying \general, all non-trivial consensus variants can be solved with $O(n^2)$ exchanged bits.
% Given our lower-bound on message complexity (\Cref{subsection:lower_bound}), this would imply another fundamental result: all non-trivial validity properties have the same optimal communication complexity, i.e., $\Theta(n^2)$, when $t \in \Omega(n)$.
% As it stands, the gap in communication complexity is linear ($\Omega(n^2)$ versus $O(n^3)$), which could indicate another hierarchy of validity properties, split by communication complexity.


% In the future, we aim to focus on \emph{External Validity}, a validity property whose analysis needs to incorporate a delicate cryptographic framework. (In \Cref{section:extended_formalim_appendix}, we give intuition about a formalism which might be suitable for the analysis of \emph{External Validity}.)
% Moreover, we have an intention of studying validity properties in a completely synchronous setting.

% focus on a classification of validity properties in a completely synchronous setting.
% \begin{compactitem}
%     \item \textbf{Matching the quadratic lower bound on communication complexity:}
%     As we prove, any non-trivial and solvable validity property requires $\Omega(t^2)$ bits.
%     In the literature, there exist Byzantine consensus algorithms achieving quadratic communication complexity for some validity properties (e.g., for \emph{Weak Validity}~\cite{civit2022byzantine}, for \emph{Strong Validity}~\cite{civit2022byzantine}).
%     Is it possible to match the quadratic lower bound for \emph{any} solvable and non-trivial validity property?
%     % We conjecture that we cannot: e.g., it seems improbable that \emph{Interactive-Consistency Validity} can be solved with $O(n^2)$ communication complexity as processes need to agree on a vector of $n - t$ values.
%     % Can we, then, match the quadratic lower bound for validity properties in which values are constant-sized?

%     \item \textbf{Validity properties of synchronous Byzantine consensus:}
%     In this work, we focus on partially synchronous Byzantine consensus.
%     A natural continuation is a study of validity properties in the synchronous case.
%     In particular, we are interested in investigating the lower bound on message complexity.
%     Does there exist a solvable and non-trivial validity property which allows for sub-quadratic Byzantine consensus algorithm in synchrony?
% \end{compactitem}

==> sections/former/crash-stop.tex <==
\section{Validity Properties In The Crash-Stop Failure Model}

In this section, we take a closer look at the validity properties of the consensus problem in the crash-stop failure model.

\subsection{Preliminaries}

\paragraph{System model.}
We consider a static system $\Psi = \{P_1, ..., P_n\}$ of $n$ processes among which $f < n$ processes can fail by \emph{crashing}.
If a process crashes, the process is \emph{faulty}; otherwise, the process is \emph{correct}.
This failure model is known as the \emph{crash-stop} failure model.

\paragraph{Crash-stop consensus.}
Each process has its \emph{proposal}, and it should eventually \emph{decide}.
We denote by $\mathcal{V}$ the set of values a process can propose and decide.
The consensus problem in the crash-stop failure model requires the following three properties to hold:
\begin{compactitem}
    \item \emph{Agreement:} No two processes decide different values.
    
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Validity}
\end{compactitem}

\paragraph{Validity property.}
First, we define a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$ is a value.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\top$ if and only if $\mathit{pp}$ is associated with a correct processes; $\mathit{pp}.\mathsf{correct}$ returns $\bot$ otherwise.

Next, an \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$, where (1) $\mathit{pp}_i$ is a process-proposal, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process, and (3) at most $f$ process-proposals refer to faulty processes (i.e., there can exist at most $f$ process-proposals of the format $(\bar{P}, v)$, where $P \in \Psi$ and $v \in \mathcal{V}$).
We denote by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

Furthermore, $\mathit{correct}(\mathit{input} \in \mathcal{I}) = \{P \in \Psi \,|\, \mathit{pp} \text{ belongs to } \mathit{input} \land \mathit{pp}.\mathsf{process} = P \land \mathit{pp}.\mathsf{correct} = \top\}$ denotes the set of correct processes as established by $\mathit{input}$.
We define $\mathit{identical\_proposals}: \mathcal{I} \times \mathcal{I} \to \{\top, \bot\}$ in the following manner:
\begin{equation*}
    \mathit{identical\_proposals}(i_1, i_2) = \top \iff \forall j \in [1, n]: i_1[j].\mathsf{proposal} = i_2[j].\mathsf{proposal}.
\end{equation*}

We define a \emph{validity property} $\mathit{val}$ as a function $\mathcal{I} \to 2^{\mathcal{V}}$ such that, for every $\mathit{input} \in \mathcal{I}$, $\mathit{val}(\mathit{input}) \neq \emptyset$.
Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item \emph{Validity safety:} In every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.
    
    \item \emph{Validity liveness:} For every input configuration $\mathit{input} \in \mathcal{I}$ and every value $v \in \mathit{val}(\mathit{input})$, there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
\end{compactitem}


% Finally, we say that a crash-stop consensus algorithm $\mathcal{A}_C$ satisfies a validity property $\mathit{val}$ if and only if, in every execution $e$ of $\mathcal{A}_C$, $\mathit{dec}_e \in \mathit{val}(\mathit{input})$, where (1) $\mathit{dec}_e$ is the decided value in $e$, and (2) $\mathit{input}$ is the input configuration that corresponds to $e$.

% \paragraph{Core valid values.}
% Consider a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies a validity property $\mathit{val}$.
% Let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
% We say that a value $v \in \mathit{val}(\mathit{input})$ is a \emph{core valid value} of $\mathit{input}$ in $\mathcal{A}_C$ if and only if there exists an execution $e$ of $\mathcal{A}_C$ such that (1) $e$ corresponds to $\mathit{input}$, and (2) the decided value in $e$ is $v$.
% We denote by $\mathit{core}(\mathcal{A}_C, \mathit{input})$ the set of core valid values of $\mathit{input}$ in $\mathcal{A}_C$; note that $\mathit{core}(\mathcal{A}_C, \mathit{input}) \subseteq \mathit{val}(\mathit{input})$.

% Why do we define core valid values?
% Consider an input configuration $\mathit{input} \in \mathcal{I}$.
% Since $\mathcal{A}_C$ satisfies $\mathit{val}$, $\mathcal{A}_C$ satisfies $\mathit{val}'$, which is a validity property identical to $\mathit{val}$, except that $\mathit{val}'(\mathit{input}) = \mathit{val}(\mathit{input}) \cup \{v^*\}$, where $v^* \notin \mathit{val}(\mathit{input})$.
% Indeed, $\mathcal{A}_C$ satisfies $\mathit{val}'$; however, $\mathcal{A}_C$ never decides $v^*$ in an execution that corresponds to $\mathit{input}$.
% Therefore, $v^*$ is not ``important'' to $\mathcal{A}_C$; we say that $v^*$ is \emph{not} a core valid value of $\mathit{input}$ in $\mathcal{A}_C$.
% In the rest of the section, we will usually talk about validity properties from the lenses of their core valid values.
 
\subsection{Synchronous Environments}

First, we investigate validity properties of crash-stop consensus in a synchronous setting.

\paragraph{Communication.}
In a synchronous environment, there exists an upper bound $\Delta$ on message delays between processes.
In other words, if a correct process sends a message to another correct process at time $t$, the message will be received by time $t + \Delta$; note that the message might be received at time $t^* \in [t, t + \Delta]$ (the actual message delay for each message is chosen by the adversary).

\paragraph{Necessary conditions.}
First, we define when two input configurations are similar.
Specifically, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{Sim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{Sim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \lor \mathit{i'}[j].\mathsf{correct} = \top \implies \mathit{input}[j] = \mathit{i'}[j]\}.
\end{equation*}
In other words, $i' \in \mathit{Sim}(\mathit{input})$ if and only if both input configurations have the identical ``set'' of process-proposals concerned with correct processes.
Note that $\mathit{Sim}(\mathit{input}) = \{\mathit{input}\}$ if, for every $j \in [1, n]$, $\mathit{input}[j].\mathsf{correct} = \top$.
Next, we introduce the \emph{similarity condition}.

\begin{definition} [Similarity condition] \label{definition:similarity_crash}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{Sim}(\mathit{input}) = \{\mathit{input'} \in \mathcal{I} \,|\, \text{all process-proposals concerned with correct processes are identical in } \mathit{input} \text{ and } \mathit{input}'\}$.
We say that $\mathit{val}$ satisfies the \emph{similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{Sim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

Now, we show that crash-stop consensus with a validity property that does not satisfy the similarity condition (\Cref{definition:similarity_crash}) cannot be satisfied by any algorithm.

\begin{lemma} [Similarity condition is necessary] \label{lemma:similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the similarity condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{Sim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:similarity_crash}).
Note that $i$ does not contain only process-proposals concerned with correct processes; otherwise, $\bigcap\limits_{i' \in \mathit{Sim}(i)} \neq \emptyset$ as $\mathit{Sim}(i) = \{i\}$.
By contradiction, suppose that there exists a crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); recall that there are faulty processes in $e$ as $i$ does not contain only process-proposals concerned with correct processes.
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{Sim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the similarity condition would be satisfied for $i$).
Again, note that there exist some faulty processes according to $i'$ (since there exist faulty processes according to $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item For each process who is faulty according to $e'$ (and $e$), we set its proposed value according to $e'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

Next, we define the \emph{containment condition}.

\begin{definition} [Containment condition] \label{definition:containment_crash}
Let $\mathit{val}$ be a validity property.
% and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
We say that $\mathit{val}$ satisfies the \emph{containment condition} if and only if the following holds:
\begin{equation*}
    \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{val}(i_2) \subseteq \mathit{val}(i_1).
\end{equation*}
% \begin{equation*}
%     \forall i_1, i_2 \in \mathcal{I}: \big(\mathit{identical\_proposals}(i_1, i_2) = \top \land \mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)\big) \implies \mathit{core}(\mathcal{A}_C, i_2) \subseteq \mathit{val}(i_1).
% \end{equation*}
\end{definition}

Next, we show that the containment condition is necessary for a validity property to be ``satisfiable''.

\begin{lemma} [Containment condition is necessary] \label{lemma:containment_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the containment condition.
No algorithm (even if synchronous) solves the crash-stop consensus problem with $\mathit{val}$.
% Let $\mathit{val}$ be a validity property and let $\mathcal{A}_C$ be an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies the containment condition with respect to $\mathcal{A}_C$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the containment condition, there exist two input configurations $i_1, i_2 \in \mathcal{I}$ such that (1) $\mathit{identical\_proposals}(i_1, i_2) = \top$, (2) $\mathit{correct}(i_1) \subseteq \mathit{correct}(i_2)$, and (3) $\mathit{val}(i_2) \not\subseteq \mathit{val}(i_1)$.
In other words, there exists a value $x \in \mathcal{V}$ such that $x \in \mathit{val}(i_2)$ and $x \notin \mathit{val}(i_1)$.

By contradiction, suppose that there exists a crash-stop algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.
Without loss of generality, let $\mathcal{A}_C$ be a synchronous algorithm.

Since $\mathcal{A}_C$ satisfies $\mathit{val}$, there exists an execution $e$ of $\mathcal{A}_C$ that corresponds to the input configuration $i_2$ in which the decided value is $x$ (due to the validity liveness).
We now create an execution $e'$ such that (1) $e'$ corresponds to $i_1$, and (2) the decided value in $e'$ is $x \notin \mathit{val}(i_1)$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    
    \item After the first process decides in $e'$, we crash all processes which are correct according to $i_2$ and faulty according to $i_1$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $x \notin \mathit{val}(i_1)$, which means that $\mathcal{A}_C$ does not satisfy $\mathit{val}$ in $e'$.
This contradicts the fact that $\mathcal{A}_C$ satisfies $\mathit{val}$, which concludes the lemma.
\end{proof}

% Hence, the similarity and containment conditions are necessary for a validity property to be ``satisfiable''.

% \begin{corollary}
% Let $\mathit{val}$ be a validity property for which there exists an algorithm $\mathcal{A}_C$ which solves the crash-stop consensus problem with $\mathit{val}$.
% Then, $\mathit{val}$ satisfies both similarity and containment conditions.
% % Then, $\mathit{val}$ satisfies both (1) the similarity condition, and (2) the containment condition with respect to $\mathcal{A}_C$.
% \end{corollary}

\paragraph{Sufficient conditions.}
We now show that the similarity and containment conditions are sufficient for a validity property to be satisfiable.

\begin{theorem} [Similarity and containment conditions are sufficient]
Let $\mathit{val}$ be a validity property that satisfies the similarity and the containment conditions.
There exists an algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{At time $0$:}
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{At time $\Delta$:}
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{Sim}(i)$ \label{line:set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a black-box synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P \in \Psi$ be a process that proposes to $c$ (at line~\ref{line:propose_c}) and let $i$ be the ``input configuration'' $P$ constructs at line~\ref{line:build_i} (if $P$ does not hear from all processes, $i$ is not, technically speaking, an input configuration as it does not contain $n$ process-proposals).
We separate two cases:
\begin{compactitem}
    \item $P$ receives \textsc{proposal} messages from all processes:
    In this case, we have that $\mathit{identical\_proposals}(i, \mathit{input}) = \top$.
    Moreover, $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i)$.
    Since $\mathit{to\_propose} \in \mathit{val}(i)$, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ (as $\mathit{val}$ satisfies the containment property). 
    Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$ in this case.
    
    \item $P$ does not receive \textsc{proposal} messages from all processes:
    In this case, $i$ does not contain proposals from all $n$ processes (i.e., $i$ is not, strictly speaking, an input configuration).
    Let $i^*$ be an input configuration identical to $i$, except that, for all processes whose proposal is missing in $i$, we add the process-proposal established by $\mathit{input}$; observe that all processes whose proposal is missing in $i$ are faulty according to $\mathit{input}$.
    
    Now, we ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not heard, we add $(\bar{P'}, \text{any value})$ to $i$.
    Observe that $i^* \in \mathit{Sim}(i)$.
    
    Let $\mathit{to\_propose} = v$ (set at line~\ref{line:set_to_propose}).
    Hence, $v \in \mathit{val}(i^*)$ (as $i^* \in \mathit{Sim}(i)$).
    
    Furthermore, we have that $\mathit{identical\_proposals}(i^*, \mathit{input}) = \top$ and $\mathit{correct}(\mathit{input}) \subseteq \mathit{correct}(i^*)$.
    According to the containment condition, $v \in \mathit{val}(\mathit{input})$.
\end{compactitem}
In both possible cases, we have that $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Hence, for every value $v$ proposed to the black-box synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$; we leave this modification for the future work).
We assume that the function mapping time to values is the same at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all processes faulty according to $\mathit{input}$ crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The validity liveness property is satisfied, which concludes the theorem.
\end{proof}

\subsection{Partially Synchronous Environments}

Next, we investigate validity properties of crash-stop consensus in a partially synchronous setting.

\paragraph{Communication.}
In a partially synchronous environment, there exists an unknown time Global Stabilization Time (GST) such that the system behaves asynchronously before GST, and behaves synchronously after GST.
Formally, there exist a known upper bound $\delta$ on message delays after GST.

\paragraph{Necessary conditions.}
First, note that the similarity and containment conditions are necessary for a validity property to be satisfied in a partially synchronous environment (as these conditions are necessary in a synchronous setting).
We now define when an input configuration is ``correct-similar'' to another configuration.
Formally, for every input configuration $\mathit{input} \in \mathcal{I}$, we define $\mathit{CorrectSim}(\mathit{input})$ in the following manner:
\begin{equation*}
    \mathit{CorrectSim}(\mathit{input}) = \{i' \in \mathcal{I} \,|\, \forall j \in [1, n]: \mathit{input}[j].\mathsf{correct} = \top \implies \mathit{input}[j].\mathsf{proposal} = i'[j].\mathsf{proposal}\}.
\end{equation*}
In other words, an input configuration $i' \in \mathcal{I}$ is \emph{correct-similar} to $\mathit{input}$ if proposed values of processes correct according to $\mathit{input}$ are identical in $i'$ and $\mathit{input}$.

Observe that $i_1 \in \mathit{CorrectSim}(i_2)$ does not imply $i_2 \in \mathit{CorrectSim}(i_1)$.
For example, let $i_1 = \big[(P_1, v_1), (P_2, v_2), (\bar{P}_3, v_3)\big]$ and $i_2 = \big[(\bar{P}_1, v_1), (P_2, v_2), (P_3, v_3')\big]$.
We have that $i_2 \in \mathit{CorrectSim}(i_1)$, but $i_1 \notin \mathit{CorrectSim}(i_2)$.
Next, we introduce the \emph{correct-similarity condition}.

\begin{definition} [Correct-similarity condition] \label{definition:correct_similarity}
Let $\mathit{val}$ be a validity property.
% Let $\mathit{input} \in \mathcal{I}$ be an input configuration.
% We define $\mathit{AlmostSim}(\mathit{input}) = \{\mathit{input}' \in \mathcal{I} \,|\, \text{proposed values of processes correct according to } i \text{ are identical}\}$.
We say that $\mathit{val}$ satisfies the \emph{correct-similarity condition} if and only if the following holds:
\begin{equation*}
    \forall \mathit{input} \in \mathcal{I}: \bigcap\limits_{i' \in \mathit{CorrectSim}(\mathit{input})} \big(\mathit{val}(i')\big) \neq \emptyset.
\end{equation*}
\end{definition}

% Note that, if all processes are correct according to $i \in \mathcal{I}$, $\mathit{AlmostSim}(i)$ contains input configurations $i' \in \mathcal{I}$ such that $\mathit{identical\_proposals}(i, i') = \top$ and $\mathit{correct}(i') \subseteq \mathit{correct}(i)$.
We now show that the correct-similarity condition is necessary in a partially synchronous setting.

\begin{lemma} [Correct-similarity condition is necessary] \label{lemma:correct_similarity_necessary_crash}
Let $\mathit{val}$ be a validity property that does not satisfy the correct-similarity condition.
No partially synchronous algorithm solves the crash-stop consensus problem with $\mathit{val}$.
\end{lemma}
\begin{proof}
Since $\mathit{val}$ does not satisfy the correct-similarity condition, there exists an input configuration $i \in \mathcal{I}$ such that $\bigcap\limits_{i' \in \mathit{CorrectSim}(i)} \big( \mathit{val}(i') \big) = \emptyset$ (by \Cref{definition:correct_similarity}).
By contradiction, suppose that there exists a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ that satisfies $\mathit{val}$.

Consider an execution $e$ of $\mathcal{A}_C$ that corresponds to $i$ (i.e., all processes propose the values as established by $i$, and $i$ establishes which processes are correct and which are faulty) such that all faulty processes in $e$ crash immediately (without sending any message); observe that there might be no faulty processes in $e$ (according to $i$).
Let the decided value in $e$ be $\mathit{dec}_e$.
Importantly, there exists an input configuration $i' \in \mathit{CorrectSim}(i)$ such that $\mathit{dec}_e \notin \mathit{val}(i')$ (otherwise, the correct-similarity condition would be satisfied for $i$).

Now, we create an execution $e'$ of $\mathcal{A}_C$ such that (1) $e'$ corresponds to $i'$, and (2) the decided value in $e'$ is $\mathit{dec}_e \notin \mathit{val}(i')$:
\begin{compactenum}
    \item We start with $e' \gets e$.
    We adjust the proposals according to $i'$.
    
    \item No process correct in $e$ hears from any process $P \in \Psi$ in $e'$ until a value is decided in $e'$, where $P$ is faulty in $e$ (i.e., according to $i$) and correct in $e'$ (i.e., correct according to $i'$).
    
    \item After a decision has been made in $e'$, we crash all processes which are faulty according to $i'$.
\end{compactenum}
Hence, the decided value in $e'$ is indeed $\mathit{dec}_e \notin \mathit{val}(i')$, which means that $\mathcal{A}_C$ does not satisfy the validity property in the execution $e'$ (as the validity safety property is not satisfied).
This contradicts the fact that $\mathcal{A}_C$ satisfies the validity property $\mathit{val}$, which concludes the lemma.
\end{proof}

\paragraph{Sufficient conditions.}
Finally, we are ready to show that similarity, containment and correct-similarity conditions are sufficient for a validity property to be satisfiable in a partially synchronous setting.

\begin{theorem} [Similarity, containment and correct-similarity conditions are sufficient in partial synchrony]
Let $\mathit{val}$ be a validity property that satisfies similarity, containment and correct-similarity conditions.
There exists a partially synchronous algorithm that solves the crash-stop consensus problem with $\mathit{val}$.
\end{theorem}
\begin{proof}
In order to prove the theorem, we devise a partially synchronous crash-stop consensus algorithm $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) that solves consensus with $\mathit{val}$.

\begin{algorithm}
\caption{Partially synchronous crash-stop algorithm $\mathcal{A}_C$ that solves consensus with $\mathit{val}$: Pseudocode for process $P_i$}
\label{algorithm:partially_synchronous_crash_stop}
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Partially Synchronous Crash-Stop Consensus, \textbf{instance} $c$

\medskip
\State \textbf{upon} $\mathsf{start}$:
\State \hskip2em \textbf{broadcast} $[\textsc{proposal}, \mathit{proposal}]$

\medskip
\State \textbf{upon} reception of $n - f$ \textsc{proposal} messages:
\State \hskip2em \textbf{trigger} timer for $\Delta$ time \Comment{$\Delta$ is some predefined constant}

\medskip
\State \textbf{upon} timer elapsed:
\State \hskip2em $\mathsf{Value} \text{ } \mathit{to\_propose} \gets \bot$
\State \hskip2em $\mathsf{Input\_Configuration} \text{ } i \gets $ the input configuration built out of the received \textsc{proposal} messages \label{line:partially_build_i}
\State \hskip2em \textbf{if} \textsc{proposal} messages are received from all processes:
\State \hskip4em $\mathsf{Time} \text{ } \mathit{first\_message\_time} \gets $ the time at which the first \textsc{proposal} message was received
\State \hskip4em $\mathit{to\_propose} \gets$ the value in $\mathit{val}(i)$ to which $\mathit{first\_message\_time}$ maps
\State \hskip2em \textbf{else:} 
\State \hskip4em $\mathit{to\_propose} \gets $ find a common value among all $\mathit{CorrectSim}(i)$ \label{line:partially_set_to_propose}
\State \hskip2em \textbf{trigger} $\langle c, \mathsf{propose}(\mathit{to\_propose}) \rangle$ \label{line:partially_propose_c}

\medskip
\State \textbf{upon} $\langle c, \mathsf{decide}(\mathit{dec}) \rangle$:
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{dec})$

\end{algorithmic}
\end{algorithm}

Let us prove that $\mathcal{A}_C$ (\Cref{algorithm:partially_synchronous_crash_stop}) solves the consensus problem with $\mathit{val}$.
First, termination and agreement follow directly from termination and agreement of a used partially synchronous crash-stop consensus (instance $c$ in \Cref{algorithm:partially_synchronous_crash_stop}).
Hence, it is left to show that $\mathcal{A}_C$ satisfies $\mathit{val}$.

Fix an input configuration $\mathit{input} \in \mathcal{I}$.
We first show that $\mathcal{A}_C$ satisfies the validity safety.
Let $P$ be a process that proposes to $c$ (at line~\ref{line:partially_propose_c}) and let $i$ be the input configuration $P$ constructs at line~\ref{line:partially_build_i}; observe that, if $P$ does not receive \textsc{proposal} messages from all processes, $i$ is not, strictly speaking, an input configuration.
We ``extend'' $i$ by adding process-proposals associated with processes from which $P$ has not heard, i.e., for every $P' \in \Psi$ from which $P$ has not received a \textsc{proposal} message, we add $(\bar{P}', \text{any value})$ to $i$.
Importantly, $\mathit{input} \in \mathit{CorrectSim}(i)$.
Hence, $\mathit{to\_propose} \in \mathit{val}(\mathit{input})$.
Therefore, for every value $v$ proposed to the black-box partially synchronous consensus $c$, $v \in \mathit{val}(\mathit{input})$.
Given that $c$ decides only proposed values, the decided value must belong to $\mathit{val}(\mathit{input})$.
Thus, the validity safety is satisfied by \Cref{algorithm:partially_synchronous_crash_stop}.

It is left to show that the validity liveness is satisfied.
In order to solve the validity liveness, $\mathcal{A}_C$ relies on time (importantly, $\mathcal{A}_C$ can avoid relying on time if $|\mathit{val}(\mathit{input})| < \infty$, for every $\mathit{input} \in \mathcal{I}$).
We assume that the time maps to a value in the same way at all processes.

Again, let us fix an input configuration $\mathit{input} \in \mathcal{I}$.
We need to show that, for every value $v \in \mathit{val}(\mathit{input})$, there exists an execution that corresponds to $\mathit{input}$ in which the decided value is $v$.
Hence, let us fix a value $v \in \mathit{val}(\mathit{input})$.
We construct an execution $e$ that corresponds to $\mathit{input}$ in which the decided value is $v$:
\begin{compactenum}
    \item All processes propose their values according to $\mathit{input}$.
    
    \item The first \textsc{proposal} message at each process is received at the \emph{exactly} the same time that maps to $v$.
    
    \item Once all processes have decided from $c$, all faulty processes crash.
\end{compactenum}
Since all processes receive the first \textsc{proposal} message at the same time (which maps to $v$), all processes propose $v$ to $c$.
Hence, the decided value must be $v$ (due to the validity property of $c$).
The theorem holds. 
\end{proof}

==> sections/former/crash.tex <==
\section{Validity Properties of the Crash-Stop Consensus}

In this section, we deal with the satisfiability of the validity properties of the crash-stop consensus problem.
First, we formally define a validity property of the crash-stop consensus (\Cref{subsection:crash_stop_definition}).
Then, we define necessary and sufficient conditions for satisfiability of a validity property in synchronous, and partially synchronous environments.

\subsection{Validity of the Crash-Stop Consensus: Formal Definition} \label{subsection:crash_stop_definition}

Let us fix the $f$-resilient crash-stop consensus problem $\mathcal{P}_C$.

We start by defining a \emph{process-proposal} pair as a pair $(P_x, \mathit{val}_x)$, where (1) $P_x$ is either $P \in \Psi$ or $\bar{P}$, with $P \in \Psi$, and (2) $\mathit{val}_x \in \mathcal{V}$.
Intuitively, $(P, \mathit{val})$ denotes that a \emph{correct} process $P \in \Psi$ has proposed a value $\mathit{val} \in \mathcal{V}$; on the other hand, $(\bar{P}, \mathit{val}')$ denotes that a \emph{faulty} process $P \in \Psi$ has proposed a value $\mathit{val}' \in \mathcal{V}$.
We denote by $\mathit{pp}.\mathsf{process}$ the process associated with a process-proposal $\mathit{pp}$, whereas $\mathit{pp}.\mathsf{proposal}$ denotes the proposal associated with $\mathit{pp}$.
Finally, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{true}$ if and only if $\mathit{pp}$ is associated with a correct process; otherwise, $\mathit{pp}.\mathsf{correct}$ returns $\mathit{false}$.

An \emph{input configuration} is a tuple $\big[\mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_n \big]$ such that (1) $\mathit{pp}_i$ is a process-proposal pair, for every $i \in [1, n]$, (2) every process-proposal pair is associated with a distinct process which belongs to $\Psi$, and (3) at most $f$ process-proposal pairs refer to faulty processes (i.e., there can exist at most $f$ process-proposal pairs of the format $(\bar{P}, \cdot)$, where $P \in \Psi$).
We denote    by $\mathcal{I}$ the set of all possible input configurations.
For every input configuration $\mathit{input} \in \mathcal{I}$ and every $i \in [1, n]$, we denote by $\mathit{input}[i]$ the process-proposal pair associated with process $P_i$.

==> sections/former/extensions.tex <==
\section{Beyond our Formalism}

\subsection{Extension to External Validity} \label{subsection:external_validity}

\subsection{Extension to Crash-Stop Validity}

==> sections/former/external_main.tex <==
\section{Extended Formalism: A Brief Introduction} \label{section:extended_formalism_main}

In this section, we briefly introduce an extended version of our formalism to accommodate for blockchain-specific validity properties.
Namely, we make our formalism more expressive by (1) allowing the input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) spaces to be unknown to processes, and (2) taking into account the ``proposals'' of faulty processes.
The full extended formalism can be found in \Cref{section:extended_formalim_appendix}. \Cref{section:classification_extended,section:blockchain_validity_appendix} are devoted to reestablishing, in the extended formalism, our previous results.

\paragraph{Intuition.}
In the original formalism, processes know the entire input ($\mathcal{V}_I$) and output ($\mathcal{V}_O$) space.
That is, processes are able to ``produce'' any value which belongs to $\mathcal{V}_I$ or $\mathcal{V}_O$.
However, this assumption limits the expressiveness of the formalism as it is impossible to describe a Byzantine consensus problem in which input or output spaces are unknown.
Let us give an example.

Imagine a committee-based blockchain which establishes two roles:
\begin{compactitem}
    \item \emph{Clients} are the users of the blockchain.
    They issue \emph{signed} transactions to the blockchain.
    
    \item \emph{Servers} are the operating nodes of the blockchain.
    Servers receive signed transactions issued by the clients, and solve the Byzantine consensus problem to agree on the exact order the transactions are processed.
\end{compactitem}
The Byzantine consensus problem at the heart of our blockchain satisfies \emph{External Validity}: if a transaction is processed, then it satisfies a predetermined $\mathsf{valid}$ predicate.
Notice that, for example, \emph{Strong Validity} is not suitable in this case, as, if not all correct processes propose the same transaction, \emph{any} transaction (even a ``useless'' one, such as $\bot$) can be decided.
Since servers rarely propose the same transactions, \emph{Strong Validity} would render our system useless a majority of the time.

As servers propose transactions \emph{signed by the clients} and servers do not have access to the private keys of the clients, servers do not know the input space $\mathcal{V}_I$ nor the output space $\mathcal{V}_O$.
% of the Byzantine consensus problem.
Hence, our original formalism is insufficient to describe the Byzantine consensus problem in the core of the aforementioned blockchain.
To address such scenarios, we introduce the extended formalism.

\paragraph{Extended vs. original formalism.}
As highlighted above, the main difference between the two formalisms is that the extended one allows us to specify the ``knowledge level'' of the input and output spaces.
In the extended formalism, a process is able to ``learn'' output values by observing input values.
That is, we define a \emph{discovery function} that specifies which output values are learned given observed input values.
In the committee-based blockchain example, once a server observes signed transactions $\mathit{tx}_1$ and $\mathit{tx}_2$, it learns the following output values: (1) $\mathit{tx}_1$, (2) $\mathit{tx}_2$, (3) $\mathit{tx}_1 || \mathit{tx}_2$, and (4) $\mathit{tx}_2 || \mathit{tx}_1$; we denote by ``$||$'' the concatenation.
% \footnote{We denote by ``$||$'' the concatenation operation.} 

The second difference between the original and the extended formalism is that the extended formalism takes into account the ``proposals'' of Byzantine processes.
Indeed, the original formalism does not allow us to define which values are admissible given the adversary's knowledge of the input space.
Think of the aforementioned example with a blockchain system.
If no process (correct or faulty) obtains a transaction $\mathit{tx}$ from the clients, $\mathit{tx}$ cannot be decided.
However, if \emph{only} a faulty process obtains a transaction $\mathit{tx}$, $\mathit{tx}$ is an admissible decision.
This scenario \emph{can} be expressed by the extended formalism (and not by the original one).



==> sections/former/lower_bound.tex <==
\section{Lower Bound on Message Complexity}

In this section, we show the quadratic lower bound on message complexity for any partially synchronous algorithm solving the Byzantine consensus problem with a non-trivial validity property.

\begin{definition} [Non-trivial validity property]
Let $\mathit{val}$ be a validity property.
We say that $\mathit{val}$ is \emph{non-trivial} if there does not exist a value $v \in \mathcal{V}$ such that, for every input configuration $i \in \mathcal{I}$, $v \in \mathit{val}(i)$.
\end{definition}

In the rest of the section, we fix a non-trivial validity property $\mathit{val}$ and a partially synchronous distributed algorithm $\mathcal{A}$ that solves the Byzantine consensus problem with $\mathit{val}$.
As $\mathit{val}$ is non-trivial, we have that $n > 3t$ (by \Cref{corollary:trivial_validity}).
In order to prove the lower bound, we show that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.

First, we define an infinite execution $E_{\mathit{base}}$ in the following manner:
\begin{compactitem}
    \item $\text{GST} = 0$.

    \item We separate all processes into two groups: (1) group $A$, where $|A| = n - t / 2$, and (2) group $B$, where $|B| = t / 2$.
    
    \item All processes from group $A$ are correct.
    
    \item All processes from group $B$ are faulty.
    For each process $P \in B$, $P$ behaves correctly, except that (1) $P$ ignores first $t / 2$ received messages (from other processes), and (2) $P$ does not send any message to any other process in group $B$. 
\end{compactitem}
Let $\mathit{base}$ denote the input configuration which corresponds to $E_{\mathit{base}}$.
Let $\mathit{dec}$ be the value decided in $E_{\mathit{base}}$.
As $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$, $\mathit{dec} \in \mathit{val}(\mathit{base})$.

If correct processes send $\geq (t / 2)^2$ messages in $E_{\mathit{base}}$, the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
In the rest of the proof, by contradiction, we assume that the number of messages sent by correct processes in $E_{\mathit{base}}$ is $< (t / 2)^2$.
We prove that there exists a process $P \in B$ with a valid behavior in which it decides $\mathit{dec}$ without having received any message (from other processes).

\begin{lemma} \label{lemma:p_without_any_message}
There exists a process $P \in B$ such that there exists a valid behavior of $P$ in which (1) $P$ does not receive any message (from other processes), and (2) $P$ decides $\mathit{dec}$.
\end{lemma}
\begin{proof}
Given that correct processes send $< (t / 2)^2$ messages in $E_{\mathit{base}}$, there exists a process $P \in B$ that receives $< t / 2$ messages in $E_{\mathit{base}}$.
Let $S \subset A$ denote the set of processes which send messages to $P$ in $E_{\mathit{base}}$.
Let us now create an infinite execution $E$, which is similar to $E_{\mathit{base}}$:
\begin{compactenum}
    \item We start with $E \gets E_{\mathit{base}}$.
    
    \item For every message which sending was omitted by $P$ in $E_{\mathit{base}}$, (1) the message is sent $E$ (recall that only omitted messages by $P$ are sent to processes in group $B$), and (2) the message is received in $E$ and ignored. 
    
    \item For every message sent to $P$, the sending and receiving events are removed.
\end{compactenum}
For every process $Q \in A \setminus{S}$, the behavior of process $Q$ in $E$ is identical to the one in $E_{\mathit{base}}$.
Hence, $\mathit{dec}$ is decided in $E$.
Moreover, $P$ is correct and it does not receive (from other processes) any message in $E$.
Due to the termination of $\mathcal{A}$, $P$ decides $\mathit{dec}$ in $E$, which concludes the lemma. 
\end{proof}

Finally, we conclude the proof of the lower bound.

\begin{theorem}
The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{theorem}
\begin{proof}
By \Cref{lemma:p_without_any_message}, there exists a valid behavior of $P$ in which (1) $P$ does not receive any message (from other processes), and (2) $P$ decides $\mathit{dec}$.
As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $i \in \mathcal{I}$ such that $\mathit{dec} \notin \mathit{val}(i)$.
We fix one such input configuration; let us denote this input configuration by $i$.

We distinguish two cases:
\begin{compactitem}
    \item Let $p \notin i.\mathsf{processes}$.
    In this case, we consider an execution $E_i$ such that (1) $E_i$ corresponds to $i$, and (2) all faulty processes (including $P$) crash immediately (i.e., without taking any computational step).
    In $E_i$, correct processes decide a value $\mathit{dec}_i$ such that $\mathit{dec}_i \neq \mathit{dec}$ (as $\mathit{dec} \notin \mathit{val}(i)$).
    Hence, we can merge execution $E_i$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
    Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
    
    \item Let $p \in i.\mathsf{processes}$.
    We further separate two cases:
    \begin{compactitem}
        \item Let $|i.\mathsf{processes}| > n - t$.
        Let $i^* \in \mathcal{I}$ be an input configuration identical to $i$ except that the process-proposal pair associated with $P$ is removed from $i^*$.
        Note that $|i^*.\mathsf{processes}| \geq n - t$, which means that $i^*$ is a legitimate input configuration.
        Moreover, $P \notin i^*.\mathsf{processes}$ and $i^*.\mathsf{processes} \subset i.\mathsf{processes}$.
        
        Consider an infinite execution $E^*$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (including $P$) crash immediately.
        Let $\mathit{dec}^* \in \mathit{val}(i^*)$ be the value decided in $E^*$.
        
        We prove that $\mathit{dec}^* \in \mathit{val}(i)$.
        By contradiction, suppose that $\mathit{dec}^* \notin \mathit{val}(i)$.
        We build another execution $E_i$ of $\mathcal{A}$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process that decides in $E^*_{\mathit{prefix}}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, process $P$ is correct and live and have the proposal as specified by $i$.
        \end{compactenum}
        Hence, $E_i$ corresponds to $i$ and the value decided in $E_i$ is $\mathit{dec}^*$.
        Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which implies that $\mathit{dec}^* \in \mathit{val}(i)$.
        
        As $\mathit{dec}^* \in \mathit{val}(i)$, $\mathit{dec}^* \neq \mathit{dec}$.
        Therefore, we can merge the execution $E^*$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
        Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
        
        \item Let $|i.\mathsf{processes}| = n - t$.
        In this case, there exists a process $Q$ such that $Q \notin i.\mathsf{processes}$ (as $t > 0$).
        We now build an input configuration similar to $i$:
        \begin{compactenum}
            \item We add $(Q, v)$ to $i^*$, where $v \in \mathcal{V}$ is any value.
        
            \item For every process $P_j \in i.processes \setminus{\{P\}}$, we add $(P_j, \mathit{proposal})$ to $i^*$ such that $(P_j, \mathit{proposal})$ belongs to $i$.
        \end{compactenum}
        Note that $|i^*.\mathsf{processes}| = n - t$, which means that $i^*$ is a legitimate input configuration.
        Moreover, $P \notin i^*.\mathsf{processes}$.
        
        Consider an infinite execution $E^*$ such that (1) $E^*$ corresponds to $i^*$, and (2) all faulty processes (including $P$) crash immediately.
        Let $\mathit{dec}^* \in \mathit{val}(i^*)$ be the value decided in $E^*$.
        
        We prove that $\mathit{dec}^* \in \mathit{val}(i)$.
        By contradiction, suppose that $\mathit{dec}^* \notin \mathit{val}(i)$.
        We build another execution $E_i$ of $\mathcal{A}$ in the following manner:
        \begin{compactenum}
            \item Let $E^*_{\mathit{prefix}}$ be a prefix of $E^*$ such that there exists a process $Q' \neq Q$ that decides in $E^*_{\mathit{prefix}}$.
            
            \item In the continuation of $E^*_{\mathit{prefix}}$, process $P$ is correct and live and have the proposal as specified by $i$.
            Moreover, process $Q$ crashes.
        \end{compactenum}
        Hence, $E_i$ corresponds to $i$ and the value decided in $E_i$ is $\mathit{dec}^*$.
        Therefore, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which implies that $\mathit{dec}^* \in \mathit{val}(i)$.
        
        As $\mathit{dec}^* \in \mathit{val}(i)$, $\mathit{dec}^* \neq \mathit{dec}$.
        Therefore, we can merge the execution $E^*$ with the valid behavior of $P$ in which $P$ decides $\mathit{dec}$ without having received any message.
        Thus, disagreement occurs, which contradicts the fact that $\mathcal{A}$ solves the Byzantine consensus problem with $\mathit{val}$.
    \end{compactitem}
\end{compactitem}
As the statement of the theorem is satisfied in every possible scenario, the theorem holds.
\end{proof}

\begin{corollary}
Let $\mathit{val}$ be any non-trivial validity property.
Let $\mathcal{A}$ be any partially synchronous distributed algorithm that solves the Byzantine consensus problem with $\mathit{val}$.
The message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{corollary}

==> sections/former/lower_bound_algorithm.tex <==
% \newpage
\section{Lower Bound \& General Algorithm}
\label{section:lower_upper_bounds}

This section is devoted to the cost of solving  consensus.
Specifically, we first show that any non-trivial and solvable validity property requires $\Omega(t^2)$ messages to be exchanged (\Cref{subsection:lower_bound}).
Then, we present \general, a general algorithm which, if $n > 3t$, solves consensus  with any validity property which satisfies $\mathcal{C}_S$ (\Cref{subsection:general_algorithm}).
Thus, \general proves the sufficiency of $\mathcal{C}_S$ when $n > 3t$.
% \footnote{Recall that, if $n \leq 3t$, any solvable validity property is trivial (see \Cref{subsection:triviality_main}).}

\subsection{Lower Bound on Message Complexity}
\label{subsection:lower_bound}

In this subsection, we prove the following theorem:

\begin{theorem} \label{theorem:lower_bound_main}
If an algorithm solves consensus  with a non-trivial validity property, the message complexity of the algorithm is $\Omega(t^2)$.
\end{theorem}

% This subsection proves that any algorithm which solves the Byzantine consensus problem with a non-trivial and solvable validity property incurs $\Omega(t^2)$ message complexity.
\Cref{theorem:lower_bound_main} extends the seminal Dolev-Reischuk bound~\cite{dolev1985bounds}, proven only for consensus algorithms with \emph{Strong Validity}, to all non-trivial variants of consensus.
% validity properties.
To prove \Cref{theorem:lower_bound_main}, we intertwine the idea of the original proof~\cite{dolev1985bounds} with the canonical similarity result (\Cref{subsection:similarity}).

% The proof of \Cref{theorem:lower_bound_main} follows the idea of the original proof~\cite{dolev1985bounds}.
% However, as \Cref{theorem:lower_bound_main} focuses on \emph{all} validity properties, our proof neatly conn

\paragraph{Proof of \Cref{theorem:lower_bound_main}.}
In our proof, we show that any algorithm which solves the Byzantine consensus problem with a non-trivial validity property has a synchronous execution ($\text{GST} = 0$) in which correct processes send 
more than $(\frac{t}{2})^2$ messages.
Hence, throughout the entire subsection, we fix a non-trivial and solvable validity property $\mathit{val}$.
Moreover, we fix $\mathcal{A}$, an algorithm which solves Byzantine consensus with $\mathit{val}$.
As $\mathit{val}$ is a non-trivial validity property, $n > 3t$ (\Cref{subsection:triviality_main}).


% Throughout the entire subsection, we fix a non-trivial and solvable validity property $\mathit{val}$.
% Moreover, we fix $\mathcal{A}$, an algorithm which solves the Byzantine consensus problem with $\mathit{val}$.
% Finally, $n > 3t$ as $\mathit{val}$ is non-trivial (see \Cref{subsection:triviality_main}).

% \paragraph{Overview of the proof.}
% We prove the lower bound by the means of contradiction.
% Hence, suppose that the message complexity of $\mathcal{A}$ is $o(t^2)$.
% Our proof consists of two steps: 
% \begin{compactenum}
%     \item We identify a process $Q$ such that $\mathcal{A}$ allows $Q$ to decide some value $v_Q \in \mathcal{V}_O$ without receiving any message (from any other processes).
%     The first step of our proof is identical to the first step of the original Dolev-Reischuk proof~\cite{dolev1985bounds,DBLP:conf/podc/AbrahamCDNP0S19}.
    
%     \item We show that there exists an execution of $\mathcal{A}$ such that (1) $Q$ is faulty and silent, and (2) other processes decide some value $v \neq v_Q$.
%     Hence, we can then ``merge'' this execution with a correct behavior of $Q$ in which $Q$ decides $v_Q$ without having received any message, thus constructing an execution in which \emph{Agreement} is violated.
    
%     The original proof of the Dolev-Reischuk bound follows the same idea.
%     However, given that the original bound concerns only \emph{Strong Validity}, the second step in the original proof is straightforward.
%     Conversely, as our bound considers \emph{all} non-trivial and solvable validity properties, completing the second step proved more challenging.
% \end{compactenum}
% In this subsection, we give an informal proof of our lower bound; the formal treatment is delegated to \Cref{section:lower_bound_appendix}.

% \paragraph{Execution $\mathcal{E}_{\mathit{base}}$ of $\mathcal{A}$.}
Next, we define a specific infinite execution $\mathcal{E}_{\mathit{base}} \in \mathit{execs}(\mathcal{A})$ in the following manner:
\begin{compactenum}
     \item $\text{GST} = 0$.
     That is, the system is synchronous throughout the entire execution.
     
     \item All processes are separated into two disjoint groups: (1) group $A$, with $|A| = n - \lceil \frac{t}{2} \rceil$, and (2) group $B$, with $|B| = \lceil \frac{t}{2} \rceil$.
     
     \item All processes in the group $A$ are correct, whereas all processes in the group $B$ are faulty.
     
     \item We fix any value $v^* \in \mathcal{V}_I$.
     For every correct process $P_A \in A$, the proposal of $P_A$ in $\mathcal{E}_{\mathit{base}}$ is $v^*$.
     
     \item For every faulty process $P_B \in B$, $P_B$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^*$, except that (1) $P_B$ ignores the first $\lceil \frac{t}{2} \rceil$ messages received from other processes, and (2) $P_B$ omits sending messages to other processes in $B$. 
\end{compactenum}
% \paragraph{Proof of the lower bound.}
To prove \Cref{theorem:lower_bound_main}, it suffices to show that the message complexity of $\mathcal{E}_{\mathit{base}}$ is greater than $ (\lceil \frac{t}{2} \rceil)^2$.
By contradiction, let the correct processes (processes in $A$) send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$.

The first step of our proof shows that, given that correct processes send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$, there must exist a process $Q \in B$ which can correctly decide some value $v_Q \in \mathcal{V}_O$ without receiving \emph{any} message from any other process.
We prove this claim using the pigeonhole principle.

\begin{lemma} \label{lemma:behavior_without_receptions}
There exist a value $v_Q \in \mathcal{V}_O$ and a process $Q \in B$ such that $Q$ has a correct 
local behavior $\beta_Q$ in which (1) $Q$ decides $v_Q$, and (2) $Q$ receives no messages from other processes.
% can correctly decide $v$ without having received any message from any other process.
\end{lemma}
\begin{proof}
By assumption, correct processes (i.e., processes in the group $A$) send $\leq (\lceil \frac{t}{2} \rceil)^2$ messages in $\mathcal{E}_{\mathit{base}}$.
Therefore, due to the pigeonhole principle, there exists a process $Q \in B$ which receives at most $\lceil \frac{t}{2} \rceil$ messages (from other processes) in $\mathcal{E}_{\mathit{base}}$.
Recall that $Q$ behaves correctly in $\mathcal{E}_{\mathit{base}}$ with its proposal being $v^* \in \mathcal{V}_I$, except that (1) $Q$ ignores the first $\lceil \frac{t}{2} \rceil$ messages received from other processes, and (2) $Q$ does not send any messages to other processes in the group $B$.
We denote by $S_Q$ the set of processes, not including $Q$, which send messages to $Q$ in $\mathcal{E}_{\mathit{base}}$; $|S_Q| \leq \lceil \frac{t}{2} \rceil$.

Next, we construct an infinite execution $\mathcal{E}_{\mathit{base}}'$.
Execution $\mathcal{E}_{\mathit{base}}'$ is identical to $\mathcal{E}_{\mathit{base}}$, except that we introduce the following modifications:
\begin{compactenum}
    % \item $\text{GST}_{\mathit{core}}' = 0$, i.e., the system is synchronous from the beginning.
    
    \item Processes in $(A \cup \{Q\}) \setminus{S_Q}$ are correct; other processes are faulty.
    That is, we make $Q$ correct in $\mathcal{E}'_{\mathit{base}}$, and we make all processes in $S_Q$ faulty in $\mathcal{E}'_{\mathit{base}}$.
    
    \item Processes in $B \setminus{\{Q\}}$ behave exactly as in $\mathcal{E}_{\mathit{base}}$.
    Moreover, processes in $S_Q$ behave exactly as in $\mathcal{E}_{\mathit{base}}$, except that they \emph{do not} send any message to $Q$.
\end{compactenum}
% Importantly, there exists a process $P \in A \setminus{S_Q}$ (as $n > 3t$) such that $P$ cannot distinguish $\mathcal{E}_{\mathit{base}}'$ from $\mathcal{E}_{\mathit{base}}$.
% Hence, as $P$ decides some value $v_Q \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}$ (as $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{\mathit{base}}$ is infinite), $P$ decides the same value $v_Q$ in $\mathcal{E}_{\mathit{base}}'$.
Due to the construction of $\mathcal{E}_{\mathit{base}}'$, process $Q$ does not receive any message (from any other process) in $\mathcal{E}_{\mathit{base}}'$.
As $Q$ is correct in $\mathcal{E}_{\mathit{base}}'$ and $\mathcal{A}$ satisfies \emph{Termination}, $Q$ decides some value $v_Q \in \mathcal{V}_O$ in $\mathcal{E}_{\mathit{base}}'$.
Thus, $Q$ indeed has a correct local behavior $\beta_Q$ in which it decides $v_Q \in \mathcal{V}_O$ without having received messages from other processes. 
\end{proof}
% \jovan{Is this proof ok? Please, try to attack is much as possible. Can there be any problems with timers or I don't know what.
% I am not seeing any problems. Just want us to be very careful!}

In the second step of our proof, we show that there exists an infinite execution in which (1) $Q$ is faulty and silent, and (2) correct processes decide some value $v \neq v_Q$.
% As $\mathit{val}$ is a non-trivial validity property, there exists some input configuration $c_{\notni v_Q} \in \mathcal{I}$ where $v_Q$ is not an admissible value, i.e., $v_Q\notin \mathit{val}(c_{\notni v_Q})$; recall that $v_Q$ is the value that $Q$ can correctly decide without having received any message from any other process (by \Cref{lemma:behavior_without_receptions}).
% The following lemma shows that $Q \in \processes{c_{\notni v_Q}}$; otherwise, $Q$ could be faulty and \emph{Agreement} would not necessarily be violated.

\begin{lemma} \label{lemma:conflicting_execution}
There exists an infinite execution $\mathcal{E}_{v}$ such that (1) $Q$ is faulty and silent in $\mathcal{E}_{v}$, and (2) a value $v \neq v_Q$ is decided by a correct process.
\end{lemma}
\begin{proof}
As $\mathit{val}$ is a non-trivial validity property, there exists an input configuration $c_{\notni v_Q} \in \mathcal{I}$ such that $v_Q \notin \mathit{val}(c_{\notni v_Q})$; recall that $v_Q$ is the value that $Q$ can correctly decide without having received any message from any other process (\Cref{lemma:behavior_without_receptions}).
We consider two possible cases:
\begin{compactitem}
     \item Let $Q \notin \processes{c_{\notni v_Q}}$.
     Thus, $\mathcal{E}_v$ is any infinite canonical execution which corresponds to $c_{\notni v_Q}$.
     As $v_Q \notin \mathit{val}(c_{\notni v_Q})$, the value decided in $\mathcal{E}_v$ must be different from $v_Q$ (as $\mathcal{A}$ satisfies $\mathit{val}$).
     
     \item Let $Q \in \processes{c_{\notni v_Q}}$.
     We construct an input configuration $c_{\notni Q} \in \mathcal{I}$ such that $Q \notin \processes{c_{\notni Q}}$:
     \begin{compactenum}
        \item Let $c_{\notni Q} \gets c_{\notni v_Q}$.

        \item We remove $(Q, \cdot)$ from $c_{\notni Q}$.
        That is, we remove $Q$'s process-proposal pair from $c_{\notni Q}$.

        \item If $|\processes{c_{\notni v_Q}}| = n - t$, we add $(Z, \text{any proposal})$ to $c_{\notni Q}$, where $Z$ is any process such that $Z \notin \processes{c_{\notni v_Q}}$; note that such a process $Z$ exists as $t > 0$.
    \end{compactenum}
    Due to the construction of $c_{\notni Q}$, $c_{\notni Q} \sim c_{\notni v_Q}$.
    Indeed, (1) $\processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}}$, the proposal of $P$ is identical in $c_{\notni Q}$ and $c_{\notni v_Q}$.
    
    In this case, $\mathcal{E}_v$ is any infinite canonical execution such that $\mathsf{input\_conf}(\mathcal{E}_{v}) = c_{\notni Q}$.
    As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{v}$ is infinite, some value $v \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{v}$.
    As $c_{\notni Q} \sim c_{\notni v_Q}$, $v \in \mathit{val}(c_{\notni v_Q})$ (by canonical similarity; \Cref{lemma:helper_main}).
    Finally, $v \neq v_Q$ as (1) $v \in \mathit{val}(c_{\notni v_Q})$, and (2) $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
\end{compactitem}
The lemma holds as its statement is true in both possible cases.
\end{proof}

\iffalse
\begin{lemma} \label{lemma:q_in_c}
$Q \in \processes{c_{\notni v_Q}}$.
\end{lemma}
\begin{proof}
By contradiction, let $Q \notin \processes{c_{\notni v_Q}}$.
We fix any infinite canonical execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}) = c_{\notni v_Q}$.
Observe that $Q$ takes no computational steps in $\mathcal{E}$.
% as $Q \notin \processes{c}$.
As $v_Q \notin \mathit{val}(c_{\notni v_Q})$, $\mathcal{E}$ is infinite and $\mathcal{A}$ satisfies \emph{Termination} and $\mathit{val}$, some value $v' \neq v_Q$ is decided in $\mathcal{E}$.
Let $t_c$ denote the time at which a correct process decides $v'$ in $\mathcal{E}$.
Moreover, let $t_Q$ denote the time at which $Q$ decides $v_Q$ in $\beta_Q$ (see \Cref{lemma:behavior_without_receptions}).

We now construct another execution $\mathcal{E}'$ such that $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ is identical to $\mathcal{E}$, except that:
\begin{compactenum}
    \item Process $Q$ is correct in $\mathcal{E}'$.
    
    \item All messages sent by and to $Q$ are delayed until after $\max(t_c, t_Q)$.
    
    \item Process $Q$ exhibits the behavior $\beta_Q$ (see \Cref{lemma:behavior_without_receptions}).
    
    \item Until $\max(t_c, t_Q)$, no process in $\processes{c}$ can distinguish $\mathcal{E}'$ from $\mathcal{E}$.
    % in which (1) it receives no messages by other processes (until some time as in-flight messages must eventually be received by $Q$), and (2) $Q$ decides $v_Q$.
    % Such a behavior of the process $Q$ exists due to \Cref{lemma:behavior_without_receptions}.
    
    % \item All messages sent by and to $Q$ are delayed until $Q$ decides $v_Q$ and some other correct process decides $v' \neq v_Q$.
    
    \item GST is set to after $\max(t_c, t_Q)$.
    % $Q$ decides $v_Q$ and some other correct process decides $v'$.
\end{compactenum}
As no process in $\processes{c_{\notni v_Q}}$ can distinguish $\mathcal{E}'$ from $\mathcal{E}$ until $\max(t_c, t_Q)$, $v' \neq v_Q$ is decided by a correct process in $\mathcal{E}'$.
Moreover, $Q$ decides $v_Q$ in $\mathcal{E}'$ (due to the step 3).
% As messages from $Q$ are delayed in $\mathcal{E}'$, all other correct processes cannot distinguish $\mathcal{E}'$ from $\mathcal{E}_c$ (until some time); hence, all other correct processes decide $v' \neq v_Q$ in $\mathcal{E}'$.
Therefore, there is a disagreement in $\mathcal{E}'$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, $Q \in \processes{c_{\notni v_Q}}$.
\end{proof}

The previous lemma shows that $Q \in \processes{c_{\notni v_Q}}$; recall that $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
Let us construct an input configuration $c_{\notni Q} \in \mathcal{I}$ such that $Q \notin \processes{c_{\notni Q}}$:
\begin{compactenum}
    \item Let $c_{\notni Q} \gets c_{\notni v_Q}$.

    \item We remove $(Q, \cdot)$ from $c_{\notni Q}$.
    That is, we remove $Q$'s process-proposal pair from $c_{\notni Q}$.

    \item If $|\processes{c_{\notni v_Q}}| = n - t$, we add $(Z, \text{any value})$ to $c_{\notni Q}$, where $Z$ is any process such that $Z \notin \processes{c_{\notni v_Q}}$; note that such a process $Z$ exists as $t > 0$.
\end{compactenum}
Due to the construction of $c_{\notni Q}$, $c_{\notni Q} \sim c_{\notni v_Q}$.
Indeed, (1) $\processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}} \neq \emptyset$ (as $n - t - 1 > 0$ when $n > 3t$ and $t > 0$), and (2) for every process $P \in \processes{c_{\notni Q}} \cap \processes{c_{\notni v_Q}}$, the proposal of $P$ is identical in $c_{\notni Q}$ and $c_{\notni v_Q}$ (by the step 1 of the construction).

The lemma below shows that there exists a canonical execution $\mathcal{E}_{c_{\notni Q}}$ such that (1) $\mathcal{E}_{c_{\notni Q}}$ corresponds to $c_{\notni Q}$, and (2) some value $v \neq v_Q$ is decided in $\mathcal{E}_{c_{\notni Q}}$.

\begin{lemma} \label{lemma:another_execution}
There exists a canonical execution $\mathcal{E}_{c_{\notni Q}} \in \mathit{execs}(\mathcal{A})$ such that (1) $\mathsf{input\_conf}(\mathcal{E}_{c_{\notni Q}}) = c_{\notni Q}$, and (2) a value $v \neq v_Q$ is decided by a correct process in $\mathcal{E}_{c_{\notni Q}}$.
\end{lemma}
\begin{proof}
We fix any infinite canonical execution $\mathcal{E}_{c_{\notni Q}} \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}_{c_{\notni Q}}) = c_{\notni Q}$.
As $\mathcal{A}$ satisfies \emph{Termination} and $\mathcal{E}_{c_{\notni Q}}$ is infinite, some value $v \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}_{c_{\notni Q}}$.
As $c_{\notni Q} \sim c_{\notni v_Q}$, $v \in \mathit{val}(c_{\notni v_Q})$ (by \Cref{lemma:helper_main}).
Finally, $v \neq v_Q$ as (1) $v \in \mathit{val}(c_{\notni v_Q})$, and (2) $v_Q \notin \mathit{val}(c_{\notni v_Q})$.
% , which concludes the proof.
% Thus, xthe lemma.
\end{proof}
\fi

As we have shown the existence of $\mathcal{E}_{v}$ (\Cref{lemma:conflicting_execution}), we can ``merge'' $\mathcal{E}_{v}$ with the valid local behavior $\beta_Q$ in which $Q$ decides $v_Q$ without having received any message (\Cref{lemma:behavior_without_receptions}).
Hence, we can construct an execution in which $\mathcal{A}$ violates \emph{Agreement}.
%, which represents a contradiction with the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Thus, correct processes must send more than $(\lceil \frac{t}{2} \rceil)^2 \in \Omega(t^2)$ messages in $\mathcal{E}_{\mathit{base}}$.
% , which implies an $\Omega(t^2)$ message complexity of $\mathcal{A}$.
% The formal proof of the following lemma, from which the lower bound on message complexity (\Cref{theorem:lower_bound_main}) follows directly, is given in \Cref{section:lower_bound_appendix}.

\begin{lemma} \label{lemma:final_lemma_lower_bound}
The message complexity of $\mathcal{E}_{\mathit{base}}$ is greater than $(\lceil \frac{t}{2} \rceil)^2$.
\end{lemma}
\begin{proof}
By \Cref{lemma:behavior_without_receptions}, there exists a local behavior $\beta_Q$ of process $Q$ in which $Q$ decides a value $v_Q$ without having received any message (from any other process).
Let $t_Q$ denote the time at which $Q$ decides $v_Q$ in $\beta_Q$.
Moreover, there exists an infinite execution $\mathcal{E}_{v}$ in which (1) $Q$ is faulty and silent, and (2) correct processes decide a value $v \neq v_Q$ (by \Cref{lemma:conflicting_execution}).
Let $t_{v}$ denote the time at which a correct process decides $v \neq v_Q$ in $\mathcal{E}_{v}$.

We now construct an execution $\mathcal{E}$ in the following way:
\begin{compactenum}
    \item Processes in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v}) \cup \{Q\}$ are correct in $\mathcal{E}$.
    All other processes are faulty.
    
    \item All messages from and to $Q$ are delayed until after $\max(t_Q, t_{v})$.
    
    \item Process $Q$ exhibits the local behavior $\beta_Q$.
    
    \item Until $\max(t_Q, t_{v})$, no process in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v})$ can distinguish $\mathcal{E}$ from $\mathcal{E}_{v}$.
    
    \item GST is set to after $\max(t_Q, t_{v})$ (and after all correct processes from the $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_v) \cup \{Q\}$ set have taken a computational step).
\end{compactenum}
As no process in $\mathit{Corr}_{\mathcal{A}}(\mathcal{E}_{v})$ can distinguish $\mathcal{E}$ from $\mathcal{E}_{v}$ until $\max(t_Q, t_{v})$, $v \neq v_Q$ is decided by a correct process in $\mathcal{E}$.
Moreover, $Q$ decides $v_Q$ in $\mathcal{E}$ as it exhibits $\beta_Q$ (step 3 of the construction).
Thus, \emph{Agreement} is violated in $\mathcal{E}$, which contradicts the fact that $\mathcal{A}$ satisfies \emph{Agreement}.
Hence, the starting assumption is not correct: in $\mathcal{E}_{\mathit{base}}$, correct processes send more than $(\lceil \frac{t}{2} \rceil)^2$ messages.
% , which concludes the proof.
% implies that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$.
\end{proof}

The following subsection shows that the quadratic bound on message complexity is tight with $t \in \Omega(n)$: \general exchanges $O(n^2)$ messages by relying on a threshold signature scheme (as all of the previous work on optimal consensus in partial synchrony~\cite{civit2022byzantine,lewis2022quadratic}).
We underline that our lower bound holds even for algorithms which employ threshold signatures.
Achieving the optimal quadratic message complexity without relying on threshold signatures (or any other signature variants) remains an important open question.

% Finally, as each message contains at least one word, \Cref{theorem:lower_bound_main} implies the $\Omega(t^2)$ lower bound on the communication complexity for any consensus algorithm with a non-trivial validity property.

% As \Cref{lemma:final_lemma_lower_bound} proves that the message complexity of $\mathcal{A}$ is $\Omega(t^2)$, the proof of \Cref{theorem:lower_bound_main} is concluded.

% With \Cref{lemma:final_lemma_lower_bound}, the proof of \Cref{theorem:lower_bound_main} is concluded.


% Observe that, as each message contains at least one word, \Cref{theorem:lower_bound_main} implies an $\Omega(t^2)$ lower bound on the communication complexity, as well.

% \newpage
\subsection{General Algorithm \general: Similarity Condition is Sufficient if $n > 3t$} \label{subsection:general_algorithm}

In this subsection, we show that $\mathcal{C}_S$ is sufficient for a validity property to be solvable when $n > 3t$.
Furthermore, we prove that, assuming a threshold signature scheme, the quadratic lower bound (\Cref{subsection:lower_bound}) is tight with $t \in \Omega(n)$.
In brief, we prove the following theorem:

\begin{theorem} \label{theorem:general}
Let $n > 3t$, and let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$.
Then, $\mathit{val}$ is solvable.
Moreover, assuming a threshold signature scheme, there exists an algorithm which solves Byzantine consensus with $\mathit{val}$, and has $O(n^2)$ message complexity.
\end{theorem}

To prove \Cref{theorem:general}, we present \general, an algorithm which solves the Byzantine consensus problem with \emph{any} validity property satisfying $\mathcal{C}_S$, given that $n > 3t$.
In other words, \general solves consensus with any solvable and non-trivial validity property.
Notably, assuming a threshold signature scheme, \general achieves $O(n^2)$ message complexity, making it optimal (when $t \in \Omega(n)$) according to our lower bound.

To construct \general, we rely on vector consensus~\cite{neves2005solving,vaidya2013byzantine,Doudou1998,correia2006consensus} (see \Cref{subsubsection:interactive_consistency}), a problem which requires correct processes to agree on the proposals of $n - t$ processes.
Specifically, when a correct process decides a vector $\mathit{vec}$ of $n - t$ proposals (from vector consensus), it decides (from \general) the common admissible value for all input configurations similar to $\mathit{vec}$, i.e., the process decides $\Lambda(\mathit{vec})$.
Note that the idea of solving consensus from vector consensus is not novel~\cite{Ben-Or94,CGL18,mostefaoui2000binary}.
For some validity properties it is even natural, such as \emph{Strong Validity}  (choose the most common value) or \emph{Weak Validity} (choose any value).
However, thanks to the necessity of $\mathcal{C}_S$ (\Cref{subsection:necessary_condition}), \emph{any} solvable  consensus variant can reuse this simple algorithmic design.

In this subsection, we first recall vector consensus (\Cref{subsubsection:interactive_consistency}).
% , a problem which requires correct processes to agree on the proposals of $n - t$ processes.
Then, we utilize vector consensus to construct \general (\Cref{subsubsection:Complete}).
Throughout the entire subsection, $n > 3t$.

% \newpage
\subsubsection{Vector Consensus.} \label{subsubsection:interactive_consistency}
In essence, vector consensus allows each correct process to infer the proposals of $n - t$ (correct or faulty) processes.
Formally, correct processes agree on input configurations (of vector consensus) with exactly $n - t$ process-proposal pairs: $\mathcal{V}_O = \mathcal{I}_{n - t}$. 
Let us precisely define \emph{Vector Validity}, the validity property of vector consensus:
\begin{compactitem}
     \item \emph{Vector Validity:} Let a correct process decide $\mathit{vector} \in \mathcal{V}_O$, which contains exactly $n - t$ process-proposal pairs, such that (1) $(P, v)$ belongs to $\mathit{vector}$, for some process $P \in \Pi$ and some value $v \in \mathcal{V}_I$, and (2) $P$ is a correct process.
     Then, $P$ proposed $v$ to vector consensus.
\end{compactitem}
Intuitively, \emph{Vector Validity} states that, if a correct process ``concludes'' that a value $v$ was proposed by a process $P$ and $P$ is correct, then $P$'s proposal was indeed $v$.

We provide two implementations of vector consensus: (1) a non-authenticated implementation (without any cryptographic primitives), and (2) an authenticated implementation (with threshold signatures).
% \pierre{I think this claim is controversial. A lot of similar (if not identical) reductions have been proposed  \cite{Ben-Or94} \cite{CGL18}}\manuel{We're just saying we provide implementations, not that we're solving the problem for the first time. We can maybe add a footnote: ``For alternative non-authenticated implementations of vector consensus, see~\cite{Ben-Or94, CGL18}''}\pierre{But can we say what is the difference between our proposal and \cite{CGL18} ?}\jovan{We discussed this already; will remove it.}
We give the pseudocode of the non-authenticated version in \Cref{subsection:nonauthenticated_vector}.
The pseudocode of the authenticated version is presented in \Cref{algorithm:interactive_consistency}.
This version relies on \textsc{Quad}, a Byzantine consensus algorithm recently introduced in~\cite{civit2022byzantine}; we briefly discuss \textsc{Quad} below.

% The pseudocode of \wic is presented in \Cref{algorithm:interactive_consistency}.
% \wic achieves $O(n^2)$ message complexity.
% % The \emph{communication complexity of \wic, the number of bits sent by correct processes, is $O(n^3)$.
% % , and $O(n^3)$ communication complexity.
% We construct \wic by relying on \textsc{Quad}, a Byzantine consensus algorithm introduced by Civit \emph{et al.}~\cite{civit2022byzantine}; we give a brief description of \textsc{Quad} below.


\paragraph{\textsc{Quad}.}
In essence, \textsc{Quad} is a partially-synchronous, ``leader-based'' Byzantine consensus algorithm, which achieves $O(n^2)$ message complexity.
Internally, \textsc{Quad} relies on a threshold signature scheme.
% \textsc{Quad} owes its complexity to its quadratic view synchronization~\cite{lewis2022quadratic, civit2022byzantine,naor2019cogsworth,naor2020expected} algorithm.
Formally, \textsc{Quad} is concerned with two sets: (1) $\mathcal{V}_{\textsc{Quad}}$, a set of values, and (2) $\mathcal{P}_{\textsc{Quad}}$, a set of proofs.
In \textsc{Quad}, processes propose and decide value-proof pairs.
There exists a function $\mathsf{verify}: \mathcal{V}_{\textsc{Quad}} \times \mathcal{P}_{\textsc{Quad}} \to \{ \mathit{true}, \mathit{false} \}$.
Importantly, $\mathcal{P}_{\textsc{Quad}}$ is not known a-priori: it is only assumed that, if a correct process proposes a pair $(v \in \mathcal{V}_{\textsc{Quad}}, \Sigma \in \mathcal{P}_{\textsc{Quad}})$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
\textsc{Quad} guarantees the following: if a correct process decides a pair $(v, \Sigma)$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
In other words, correct processes decide only valid value-proof pairs.
(See~\cite{civit2022byzantine} for full details on \textsc{Quad}.)

% As for the validity property, $\textsc{Quad}$ satisfies \emph{External Validity}:
% \begin{compactitem}
%      \item \emph{External Validity:} If a correct process decides a pair $(v, \Sigma)$, then $\mathsf{verify}(v, \Sigma) = \mathit{true}$.
% \end{compactitem}
% \textsc{Quad} achieves $O(n^2)$ message complexity, which enables the $O(n^2)$ message complexity of \wic, by relying on threshold signatures~\cite{libert2014born}.
% % The \emph{communication complexity}, the number of bits sent in messages by correct processes, of \textsc{Quad} is $O(n^2 \cdot x)$, where $x$ denotes the maximum size of a proof.
% (See the paper~\cite{civit2022byzantine} for more details on \textsc{Quad}.)
% For completeness, we provide a detailed explanation of \textsc{Quad} in \Cref{section:quad_appendix}; 

In our authenticated implementation of vector consensus
(\Cref{algorithm:interactive_consistency}), we rely on a specific instance of \textsc{Quad} where (1) $\mathcal{V}_{\textsc{Quad}} = \mathcal{I}_{n - t}$ (processes propose to \textsc{Quad} the input configurations of vector consensus), and (2) $\mathcal{P}_{\textsc{Quad}}$ is a set of $n - t$ \textsc{proposal} messages (sent by processes in vector consensus).
Finally, given an input configuration $\mathit{vector} \in \mathcal{V}_{\textsc{Quad}}$ and a set of messages $\Sigma \in \mathcal{P}_{\textsc{Quad}}$, $\mathsf{verify}(\mathit{vector}, \Sigma) = \mathit{true}$ if and only if, for every process-proposal pair $(P_j, v_j)$ which belongs to $\mathit{vector}$, $\langle \textsc{proposal}, v_j \rangle_{\sigma_j} \in \Sigma$ (i.e., every process-proposal pair of $\mathit{vector}$ is accompanied by a properly signed \textsc{proposal} message).

\paragraph{Description of authenticated vector consensus (\Cref{algorithm:interactive_consistency}).}
When a correct process $P_i$ proposes a value $v \in \mathcal{V}_I$ to vector consensus (line~\ref{line:propose}), the process broadcasts a signed \textsc{proposal} message (line~\ref{line:broadcast_proposal}).
Once $P_i$ receives $n - t$ \textsc{proposal} messages (line~\ref{line:received_n_t_proposals}), $P_i$ constructs an input configuration $\mathit{vector}$ (line~\ref{line:construct_input_configuration}), and a proof $\Sigma$ (line~\ref{line:construct_proof}) from the received \textsc{proposal} messages.
Moreover, $P_i$ proposes $(\mathit{vector}, \Sigma)$ to \textsc{Quad} (line~\ref{line:propose_quad}).
Finally, when $P_i$ decides a pair $(\mathit{vector}', \Sigma')$ from \textsc{Quad} (line~\ref{line:decide_quad}), $P_i$ decides $\mathit{vector}'$ from vector consensus (line~\ref{line:decide}).

\begin{algorithm}
\caption{Authenticated Vector Consensus: Pseudocode (for process $P_i$)}
\label{algorithm:interactive_consistency}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Best-Effort Broadcast~\cite{cachin2011introduction}, \textbf{instance} $\mathit{beb}$ \BlueComment{broadcast with no guarantees if the sender is faulty}
\State \hskip2em \textsc{Quad}~\cite{civit2022byzantine}, \textbf{instance} $\mathit{quad}$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{Integer}$ $\mathit{received\_proposals}_i \gets 0$ \BlueComment{the number of received proposals}
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathcal{V}_I)$ $\mathit{proposals}_i \gets \text{empty}$ \BlueComment{received proposals}
\State \hskip2em $\mathsf{Map}(\mathsf{Process} \to \mathsf{Message})$ $\mathit{messages}_i \gets \text{empty}$ \BlueComment{received \textsc{proposal} messages}

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose}
\State \hskip2em \textbf{invoke} $\mathit{beb}.\mathsf{broadcast}\big( \langle \textsc{proposal}, v \rangle_{\sigma_i} \big)$ \BlueComment{broadcast a signed proposal} \label{line:broadcast_proposal}

\medskip
\State \textbf{upon} reception of $\mathsf{Message}$ $m = \langle \textsc{proposal}, v_j \in \mathcal{V}_I \rangle_{\sigma_j}$ from process $P_j$ and $\mathit{received\_proposals}_i < n - t$:
\State \hskip2em $\mathit{received\_proposals}_i \gets \mathit{received\_proposals}_i + 1$
\State \hskip2em $\mathit{proposals}_i[P_j] \gets v_j$
\State \hskip2em $\mathit{messages}_i[P_j] \gets m$

\State \hskip2em \textbf{if} $\mathit{received\_proposals}_i = n - t$: \label{line:received_n_t_proposals} \BlueComment{received $n - t$ proposals; can propose to \textsc{Quad}}
\State \hskip4em $\mathsf{Input\_Configuration}$ $\mathit{vector} \gets $ input configuration constructed from $\mathit{proposals}_i$ \label{line:construct_input_configuration}
\State \hskip4em $\mathsf{Proof}$ $\Sigma \gets $ set of messages containing all \textsc{proposal} messages from $\mathit{messages}_i$ \label{line:construct_proof}
\State \hskip4em \textbf{invoke} $\mathit{quad}.\mathsf{propose}\big( (\mathit{vector}, \Sigma) \big)$ \label{line:propose_quad}

\medskip
\State \textbf{upon} $\mathit{quad}.\mathsf{decide}\big( (\mathsf{Input\_Configuration} \text{ } \mathit{vector}', \mathsf{Proof} \text{ } \Sigma') \big)$: \label{line:decide_quad}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{vector}')$ \label{line:decide}

\end{algorithmic}
\end{algorithm}

%\medskip
The message complexity of \Cref{algorithm:interactive_consistency} is $O(n^2)$ as (1) processes only broadcast \textsc{proposal} messages, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
We underline that the \emph{communication complexity} of \Cref{algorithm:interactive_consistency}, the number of bits sent by correct processes, is $O(n^3)$ as the communication complexity of \textsc{Quad} is $O(n^2 \cdot x) = O(n^3)$ (see~\cite{civit2022byzantine}), where $x$ is the size of a \textsc{Quad} proposal (in our case, $x \in \Theta(n)$).
% Lastly, the latency of \Cref{algorithm:interactive_consistency}, the time until processes decide (measured from GST), is linear (due to the linear latency of \textsc{Quad}; see~\cite{civit2022byzantine}).
We delegate the full proof of the correctness and complexity of \Cref{algorithm:interactive_consistency} to \Cref{subsection:authenticated_vector_proof}.
% , where we also include a solution to the vector consensus problem in the \emph{non-authenticated} setting (\Cref{algorithm:interactive_consistency} above relies on cryptographic signatures).
%Observe that \wic (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed, and \textsc{Quad} uses threshold signatures internally).
%We underline that the Byzantine consensus problem with \emph{Vector Validity} (i.e., vector consensus) can be solved even in a \emph{non-authenticated} setting, although with a higher cost; we provide such an algorithm in \Cref{section:algorithm_appendix}.
% Thus, the solvability of validity properties is \emph{independent} of the assumptions on authentication (as we show in \Cref{subsubsection:Complete}).

% \begin{theorem} [\textsc{Icon} is correct] \label{theorem:icon}
% \textsc{Icon} (\Cref{algorithm:interactive_consistency}) is a Byzantine consensus algorithm with Interactive-Consistency Validity.
% The message complexity of \textsc{Icon} is $O(n^2)$, whereas its communication complexity is $O(n^3)$.
% \end{theorem}
% \begin{proof}
% \emph{Agreement} follows directly from \emph{Agreement} of \textsc{Quad}.
% Moreover, as there are (at least) $n - t$ correct processes, every correct process eventually proposes to \textsc{Quad} (line~\ref{line:propose_quad}).
% Due to \emph{Termination} of \textsc{Quad}, every correct process eventually decides.
% Therefore, \Cref{algorithm:interactive_consistency} satisfies \emph{Termination}.

% It is left to prove that \textsc{Icon} satisfies \emph{Interactive-Consistency Validity}.
% Let $\mathit{vector}' \in \mathcal{I}_{n - t}$ be an input configuration decided by a correct process.
% Due to \emph{External Validity} of \textsc{Quad}, if a process-proposal pair $(P_j, v_j)$ belongs to $\mathit{vector}'$, for some value $v_j \in \mathcal{V}_I$, $P_j$ has sent a properly signed \textsc{proposal} message for $v_j$.
% If $P_j$ is correct, $v_j$ is its proposal as correct processes send \textsc{proposal} messages only for their proposals (line~\ref{line:broadcast_proposal}).
% Thus, \Cref{algorithm:interactive_consistency} satisfies \emph{Interactive-Consistency Validity}.

% The $O(n^2)$ message complexity of \textsc{Icon} follows from the following two facts: (1) correct processes only broadcast \textsc{proposal} messages (line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the message complexity of \textsc{Quad} is $O(n^2)$.
% As for the communication complexity of \textsc{Icon}, it is indeed $O(n^3)$ as (1) correct processes only broadcast $O(n^2)$ words (via the \textsc{proposal} messages; line~\ref{line:broadcast_proposal}) before proposing to \textsc{Quad}, and (2) the communication complexity of \textsc{Quad} is $O(n^3)$ (because the maximum size of a proof is $O(n)$ words).
% Thus, the theorem.
% \end{proof}

% Observe that \textsc{Icon} (\Cref{algorithm:interactive_consistency}) utilizes cryptographic signatures (\textsc{proposal} messages are signed).
% We underline that a Byzantine consensus algorithm with \emph{Interactive-Consistency Validity} can be obtained even in a \emph{non-authenticated} setting; we provide such an algorithm in \Cref{section:appendix_non_authenticated}.

\subsubsection{\general.} \label{subsubsection:Complete}
We construct \general (\Cref{algorithm:general}) directly from vector consensus (\Cref{subsubsection:interactive_consistency}).
When a correct process $P_i$ proposes to \general (line~\ref{line:propose_general}), the proposal is forwarded to vector consensus (line~\ref{line:propose_ic}).
Once $P_i$ decides an input configuration $\mathit{vector}$ from vector consensus (line~\ref{line:decide_ic}), $P_i$ decides $\Lambda(\mathit{vector})$ (line~\ref{line:decide_general}).

Note that our implementation of \general (\Cref{algorithm:general}) is independent of the actual implementation of vector consensus.
Thus, by employing our authenticated implementation of vector consensus (\Cref{algorithm:interactive_consistency}), we obtain a general consensus algorithm with $O(n^2)$ message complexity.
% : both authenticated and non-authenticated vector consensus implementations can be used in \Cref{algorithm:general}.
On the other hand, by employing a non-authenticated implementation of vector consensus (see \Cref{subsection:nonauthenticated_vector}), we obtain a non-authenticated version of \general, which implies that any validity property which satisfies $\mathcal{C}_S$ is solvable even in a non-authenticated setting (if $n > 3t$).

\begin{algorithm} [ht]
\caption{\general: Pseudocode for process $P_i$}
\label{algorithm:general}
\footnotesize
\begin{algorithmic} [1]
\State \textbf{Uses:}
\State \hskip2em Vector Consensus, \textbf{instance} $\mathit{vec\_cons}$

\medskip
\State \textbf{upon} $\mathsf{propose}(v \in \mathcal{V}_I)$: \label{line:propose_general}
\State \hskip2em \textbf{invoke} $\mathit{vec\_cons}.\mathsf{propose}(v)$ \label{line:propose_ic}

\medskip
\State \textbf{upon} $\mathit{vec\_cons}.\mathsf{decide}(\mathsf{Input\_Configuration} \text{ } \mathit{vector})$: \label{line:decide_ic}
\State \hskip2em \textbf{trigger} $\mathsf{decide}\big( \Lambda(\mathit{vector}) \big)$ \label{line:decide_general}
\end{algorithmic}
\end{algorithm}

% Magical vspace
% \vspace{-5pt}

Finally, we show that \general (\Cref{algorithm:general}) is a general Byzantine consensus algorithm and that its authenticated variant achieves $O(n^2)$ message complexity, which proves \Cref{theorem:general}.

\begin{lemma} \label{theorem:general_algorithm}
Let $\mathit{val}$ be any validity property which satisfies $\mathcal{C}_S$, and let $n > 3t$.
\general solves Byzantine consensus with $\mathit{val}$.
Moreover, if \general employs \Cref{algorithm:interactive_consistency} as its vector consensus building block, the message complexity of \general is $O(n^2)$.
% , whereas its communication complexity is $O(n^3)$.
% , whereas its communication complexity is $O(n^3)$.
\end{lemma}
\begin{proof}
\emph{Termination} and \emph{Agreement} of \general follow from \emph{Termination} and \emph{Agreement} of vector consensus, respectively.
Moreover, the message complexity of \general is identical to the message complexity of its vector consensus building block.

Finally, we prove that \general satisfies $\mathit{val}$.
Consider any execution $\mathcal{E}$ of \general; let $\mathsf{input\_conf}(\mathcal{E}) = c^*$, for some input configuration $c^* \in \mathcal{I}$.
Moreover, let $\mathit{vector} \in \mathcal{I}_{n - t}$ be the input configuration correct processes decide from vector consensus in $\mathcal{E}$ (line~\ref{line:decide_ic}).
As vector consensus satisfies \emph{Vector Validity}, we have that, for every process $P \in \processes{c^*} \cap \processes{\mathit{vector}}$, $P$'s proposals in $c^*$ and $\mathit{vector}$ are identical.
Hence, $\mathit{vector} \sim c^*$.
Therefore, $\Lambda(\mathit{vector}) \in \mathit{val}(c^*)$ (by the definition of the $\Lambda$ function).
Thus, $\mathit{val}$ is satisfied by \general.
\end{proof}

As \general (\Cref{algorithm:general}) solves the Byzantine consensus problem with any validity property which satisfies $\mathcal{C}_S$ (\Cref{theorem:general_algorithm}) if $n > 3t$, $\mathcal{C}_S$ is sufficient for solvable validity properties when $n > 3t$.
Lastly, as \general relies on vector consensus, we conclude that \emph{Vector Validity} is a \emph{strongest} validity property.
That is, a consensus solution to any solvable variant of the validity property can be obtained (with no additional cost) from vector consensus.

\paragraph{A note on the communication complexity of vector consensus.}
While the version of \general which employs \Cref{algorithm:interactive_consistency} (as its vector consensus building block) has optimal message complexity, its communication complexity is $O(n^3)$.
% (measured as total bits sent by all correct processes from GST to infinity).
This presents a linear gap to the lower bound for communication complexity (also $\Omega(n^2)$, implied by \Cref{theorem:lower_bound_main}), and to known optimal solutions for some validity properties (e.g., \emph{Strong Validity}, proven to be $\Theta(n^2)$ \cite{civit2022byzantine,lewis2022quadratic}).
At first glance, this seems like an issue inherent to vector consensus: the decided vectors are linear in size, suggesting that the linear gap could be inevitable.
However, this is not the case.
In~\Cref{subsection:better_communication}, we give a vector consensus algorithm with $O(n^2\log n)$ communication complexity, albeit with exponential latency.\footnote{Both our authenticated (\Cref{algorithm:interactive_consistency}) and our non-authenticated (see \Cref{subsection:nonauthenticated_vector}) variants of vector consensus have linear latency, which implies linear latency of \general when employing any of these two algorithms.}
Is it possible to construct vector consensus with subcubic communication and polynomial latency?
This is an important open question, as positive answers would lead to (practical) performance improvements of all consensus variants.

==> sections/former/model_preliminaries.tex <==
% \newpage
\section{Preliminaries} \label{section:preliminaries}

In this section, we present the computational model (\Cref{subsection:computational_model_main}), recall the  consensus problem (\Cref{subsection:byzantine_consensus}), formally define validity properties (\Cref{subsection:specifying_validity}), and introduce canonical similarity (\Cref{subsection:similarity}).

\subsection{Computational Model} \label{subsection:computational_model_main}

\paragraph{Processes.}
We consider a system $\allprocesses = \{P_1, P_2, ..., P_n\}$ of $n$ processes; each process is a deterministic state machine.
% Each process is polynomially-bounded.
% \add{For simplicity, we consider a \emph{static adversary} which corrupts up to $t$ ($0 < t < n$) processes before the start of the algorithm; these processes are \emph{faulty}, and can exhibit arbitrary behavior.\footnote{Note that all negative results proven against a static adversary extend to an adaptive one, which can corrupt processes at any point. Moreover, \Cref{section:algorithm_appendix} proves that \general (our positive result) is resilient to an adaptive adversary.}}
At most $t$ ($0 < t < n$) processes can be \emph{faulty}: those processes can exhibit arbitrary behavior.
A non-faulty process is said to be \emph{correct}.
Processes communicate by exchanging messages over an authenticated point-to-point network.
The communication network is \emph{reliable}: if a correct process sends a message to a correct process, the message is eventually received.
Each process has its own local clock, and no process can take infinitely many computational steps in finite time.
% Finally, we assume that local steps of processes take zero time, as the time needed for local computation is negligible in comparison with message delays. 

\paragraph{Executions.}
Given an algorithm $\mathcal{A}$, $\mathit{execs}(\mathcal{A})$ denotes the set of all executions of $\mathcal{A}$.
Furthermore, $\mathit{Corr}_{\mathcal{A}}(\mathcal{E})$ denotes the set of correct processes in an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$.
We say that an execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ is \emph{canonical} if and only if no faulty process takes any computational step in $\mathcal{E}$; note that faulty processes do not send any message in a canonical execution.

\paragraph{Partial synchrony.}
We consider the standard partially synchronous model~\cite{DLS88}. 
For every execution of the system, there exists a Global Stabilization Time (GST) and a positive duration $\delta$ such that message delays are bounded by $\delta$ after GST.
GST is not known to the processes, whereas $\delta$ is.
We assume that all correct processes start executing their local algorithm before or at GST.
Local clocks may drift arbitrarily before GST, but do not drift thereafter.

We remark that (almost) all results presented in the paper hold even if $\delta$ is unknown.
The only result that is not preserved is the message complexity of \general: if $\delta$ is unknown, \general may send arbitrarily many messages after GST (while processes are trying to estimate the message delays).
In fact, this subtle point is the main reason we consider the standard model in which $\delta$ is known since it provides a fair chance of designing \general with a quadratic number of exchanged messages, as is done in other consensus algorithms geared towards low complexity~\cite{civit2022byzantine,lewis2022quadratic,yin2019hotstuff}.

\paragraph{Cryptographic primitives.}
In one variant of the \general algorithm, we assume a $(k, n)$-threshold signature scheme~\cite{libert2014born} (see \Cref{subsection:general_algorithm}).
In fact, this variant relies on a closed-box consensus algorithm which internally utilizes threshold signatures.
In a threshold signature scheme, each process holds a distinct private key, and there exists a single public key.
Each process $P_i$ can use its private key to produce a (partial) signature of a message $m$; we denote by $\langle m \rangle_{\sigma_i}$ a message $m$ (partially) signed by the process $P_i$.
Moreover, a signature can be verified by other processes.
Finally, a set of signatures for a message $m$ from $k$ (the threshold) distinct processes can be combined into a single threshold signature for $m$, which proves that $k$ processes have signed $m$.
% , which proves that $k$ processes have signed the message.


% by invoking $\mathit{ShareSign}_i(m)$.
% A partial signature $\mathit{tsignature}$ of a message $m$ produced by a process $P_i$ can be verified by $\mathit{ShareVerify}_i(m, \mathit{tsignature})$.
% Finally, set $S = \{\mathit{tsignature}_i\}$ of partial signatures, where $|S| = k$ and, for each $\mathit{tsignature}_i \in S$, $\mathit{tsignature}_i = \mathit{ShareSign}_i(m)$, can be combined into a \emph{single} (threshold) signature by invoking $\mathit{Combine}(S)$; a combined signature $\mathit{tcombined}$ of message $m$ can be verified by $\mathit{CombinedVerify}(m, \mathit{tcombined})$.
% Where appropriate, invocations of $\mathit{ShareVerify}(\cdot)$ and $\mathit{CombinedVerify}(\cdot)$ are implicit in our descriptions of protocols.


% For \general, our general algorithm with $O(n^2)$ message complexity, we assume an idealized \emph{public-key infrastructure} (PKI): each process is associated with its public/private key pair which is used to (1) sign messages, and (2) verify signatures of other processes.
% The adversary is computationally bounded, i.e., faulty processes cannot forge signatures of correct processes.
% We denote by $\langle m \rangle_{\sigma_i}$ a message $m$ which is properly signed by the process $P_i$.
% Moreover, \general utilizes, as a closed-box, an algorithm which internally relies on a threshold signature scheme~\cite{libert2014born} (see \Cref{subsection:general_algorithm}).
% We emphasize that 
% Add a comment about threshold signatures

% \paragraph{Message \& communication complexities.}
% A \emph{word} contains a constant number of signatures and values.
% Each message contains at least a single word.
% Let $\mathcal{A}$ be any algorithm and let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any execution of $\mathcal{A}$.
% The message complexity of $\mathcal{E}$ is the number of messages sent by correct processes during $[\text{GST}, \infty]$.
% The communication complexity of $\mathcal{E}$ is the number of words sent in messages by correct processes during $[\text{GST}, \infty]$.

% The \emph{message complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{message complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

% The \emph{communication complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{communication complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

\paragraph{Message complexity.}
% A \emph{word} contains a constant number of signatures and values.
% Each message contains at least a single word.
Let $\mathcal{A}$ be any algorithm and let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any execution of $\mathcal{A}$.
The message complexity of $\mathcal{E}$ is the number of messages sent by correct processes during $[\text{GST}, \infty)$.
% The communication complexity of $\mathcal{E}$ is the number of words sent in messages by correct processes during $[\text{GST}, \infty]$.

The \emph{message complexity} of $\mathcal{A}$ is defined as
\begin{equation*}
    \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{message complexity of } \mathcal{E} \bigg\}.
\end{equation*}

% The \emph{communication complexity} of $\mathcal{A}$ is defined as
% \begin{equation*}
%     \max_{\mathcal{E} \in \mathit{execs}(\mathcal{A})}\bigg\{\text{communication complexity of } \mathcal{E} \bigg\}.
% \end{equation*}

\subsection{Consensus} \label{subsection:byzantine_consensus}

% In the Byzantine consensus problem, all processes start with their proposal and aim to agree on a common value despite Byzantine failures.
We denote by $\mathcal{V}_I$ the (potentially infinite) set of values processes can propose, and by $\mathcal{V}_O$ the (potentially infinite) set of values processes can decide.
% We underline that $\mathcal{V}_I$ might not be in
% Sometimes, we refer to $\mathcal{V}_I$ (resp., $\mathcal{V}_O$) as input (resp., output) space.
% We assume that $\mathcal{V}_I$ and $\mathcal{V}_O$ are known to all processes.
% \footnote{Our extended formalism, which can be found in \Cref{section:extended_formalim_appendix}, removes this assumption, thus making itself more expressive.}
The consensus\footnote{Throughout the paper, we use ``consensus'' and ``Byzantine consensus'' interchangeably.} problem exposes the following interface:
\begin{compactitem}
    \item \textbf{request} $\mathsf{propose}(v \in \mathcal{V}_I)$: a process proposes a value $v$.
    
    \item \textbf{indication} $\mathsf{decide}(v' \in \mathcal{V}_O)$: a process decides a value $v'$.
\end{compactitem}
A correct process proposes exactly once, and it decides at most once.
Consensus requires the following properties:
\begin{compactitem}
    \item \emph{Termination:} Every correct process eventually decides.
    
    \item \emph{Agreement:} No two correct processes decide different values.
\end{compactitem}
If the  consensus problem was completely defined by \emph{Termination} and \emph{Agreement}, a trivial solution would exist: processes decide on a default value.
Therefore, the specification of consensus additionally includes a validity property, which connects the proposals of correct processes to admissible decisions, precluding the aforementioned trivial solutions.

\subsection{Validity} \label{subsection:specifying_validity}
In a nutshell, our specification of a validity property includes a set of assignments of proposals to correct processes, and, for each such assignment, a corresponding set of admissible decisions.
% We provide a formal definition of a validity property below.

% \paragraph{Input configurations.}
We start by defining a \emph{process-proposal} pair as a pair $(P, v)$, where (1) $P \in \allprocesses$ is a process, and (2) $v \in \mathcal{V}_I$ is a proposal.
Given a process-proposal pair $\mathit{pp} = (P, v)$, $\mathsf{proposal}(\mathit{pp}) = v$ denotes the proposal associated with $\mathit{pp}$.
% $\process{\mathit{pp}} = P$ denotes the process associated with $\mathit{pp}$, and $\mathsf{proposal}(\mathit{pp}) = v$ denotes the proposal associated with $\mathit{pp}$.

An \emph{input configuration} is a tuple $\big[ \mathit{pp}_1, \mathit{pp}_2, ..., \mathit{pp}_x \big]$ of $x$ process-proposal pairs, where (1) $n - t \leq x \leq n$, and (2) every process-proposal pair is associated with a distinct process.
Intuitively, an input configuration represents an assignment of proposals to correct processes.
For example, an input configuration $\big[ (P_1, v), (P_2, v), (P_3, v), (P_4, v), (P_5, v) \big]$ describes an execution in which (1) only processes $P_1$, $P_2$, $P_3$, $P_4$ and $P_5$ are correct, and (2) all of them propose the same value $v$.

We denote by $\mathcal{I}$ the set of all input configurations.
Furthermore, for every $x \in [n - t, n]$, $\mathcal{I}_x \subset \mathcal{I}$ denotes the set of input configurations with \emph{exactly} $x$ process-proposal pairs.
For every input configuration $c \in \mathcal{I}$, we denote by $c[i]$ the process-proposal pair associated with process $P_i$; if such a process-proposal pair does not exist, $c[i] = \bot$.
Lastly, $\process{c} = \{ P_i \in \Pi \,|\, c[i] \neq \bot\}$ denotes the set of all processes included in $c$.

% \medskip
Given (1) an execution $\mathcal{E}$ of an algorithm $\mathcal{A}$, where $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, and (2) an input configuration $c \in \mathcal{I}$, we say that $\mathcal{E}$ \emph{corresponds} to $c$ ($\mathsf{input\_conf}(\mathcal{E}) = c$) if and only if (1) $\process{c} = \mathit{Corr}_{\mathcal{A}}(\mathcal{E})$, and (2) for every process $P_i \in \processes{c}$, $P_i$'s proposal in $\mathcal{E}$ is $\mathsf{proposal}(c[i])$.
% We denote by \add{$\mathsf{input\_conf}(\mathcal{E}) = c$} the input configuration to which $\mathcal{E}$ corresponds.

Finally, we define a validity property $\mathit{val}$ as a function $\mathit{val}: \allconfigurations \to 2^{\mathcal{V}_O}$ such that, for every input configuration $c \in \allconfigurations$, $\mathit{val}(\mathit{c}) \neq \emptyset$.
An algorithm $\mathcal{A}$, where $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, \emph{satisfies} a validity property $\mathit{val}$ if and only if, in any execution $\mathcal{E} \in \mathit{execs}(\mathcal{A})$, no correct process decides a value $v' \notin \mathit{val}\big( \mathsf{input\_conf}(\mathcal{E}) \big)$.
% if a correct process decides a value $v' \in \mathcal{V}_O$, then $v' \in \mathit{val}(\mathsf{input\_conf}(\mathcal{E}))$.
That is, an algorithm satisfies a validity property if and only if correct processes decide only admissible values.

\paragraph{Traditional properties in our formalism.}
% Let us take a look at two well-established validity properties, and how they can be expressed using the formalism above.
% \begin{compactitem}
%     \item \emph{Weak Validity}~\cite{milosevic2009unifying,lynch1996distributed,lamport1983weak}: If all processes are correct and propose the same value, only that value can be decided.
%     \item \emph{Strong Validity}~\cite{CGL18,civit2022byzantine,Momose2021,lamport2019byzantine}: If all correct processes propose the same value, only that value can be decided.
% \end{compactitem}
% Note that, 
To illustrate the expressiveness of our formalism, we describe how it can be used for \emph{Strong Validity}, \emph{Weak Validity} and \emph{Correct-Proposal Validity}.
For all of them, $\mathcal{V}_I = \mathcal{V}_O$.
\emph{Weak Validity} can be expressed as
\[
    \mathit{val}(c) =\begin{cases}
            \{v\}, & \text{if } (\processes{c} = \allprocesses) \land (\forall P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v) \\
            \mathcal{V}_O, & \text{otherwise,}
    \end{cases}
\]

whereas \emph{Strong Validity} can be expressed as
\[
    \mathit{val}(c) =\begin{cases}
            \{v\}, & \text{if } \forall P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v \\
            \mathcal{V}_O, & \text{otherwise.}
    \end{cases}
\]
Finally, \emph{Correct-Proposal Validity} can be expressed as
\[
    \mathit{val}(c) = \{v \,|\, \exists P_i \in \processes{c}: \mathsf{proposal}(c[i]) = v\}\text{.}
\]

% It is interesting to note how the difference between these two properties (and their relative ``strength'') is evident when expressed this way.
% The set of configurations for which \emph{Strong Validity} allows any value ($\mathcal{V}$) is strictly less than for \emph{Weak Validity}, as it lacks the $\processes{c} = \allprocesses$ term in the first case.

\paragraph{Consensus algorithms.}
An algorithm $\mathcal{A}$ solves consensus with a validity property $\mathit{val}$ if and only if the following holds:
\begin{compactitem}
    \item $\mathcal{A}$ exposes the $\mathsf{propose}(\cdot)/\mathsf{decide}(\cdot)$ interface, and
    
    \item $\mathcal{A}$ satisfies \emph{Termination}, \emph{Agreement} and $\mathit{val}$.
\end{compactitem}

Lastly, we formally define the notion of a solvable validity property.
% solvable validity properties.

\begin{definition} [Solvable validity property]
We say that a validity property $\mathit{val}$ is \emph{solvable} if and only if there exists an algorithm which solves  consensus 
with $\mathit{val}$.
\end{definition} 

\input{sections/similarity_lemma}

==> sections/former/related.tex <==
\section{Related work}
\label{section:related_work}

\paragraph{Solvability of consensus.}
The consensus problem has been thoroughly investigated in a variety of system settings and failure models.
It has been known (for long) that consensus can be solved in a synchronous setting, both with crash~\cite{lynch1996distributed,cachin2011introduction,raynal2002consensus} and arbitrary failures~\cite{abraham2017brief,kowalski2013synchronous,schmid2004synchronous,raynal2002consensus,Momose2021}.
% Moreover, the celebrated Dolev-Reischuk bound~\cite{dolev1985bounds} shows that any synchronous solution to the Byzantine consensus problem requires $\Omega(n^2)$ exchanged messages.
% Recently, this bound was shown to be tight by Momose and Ren~\cite{Momose2021}.
In an asynchronous environment, however, consensus cannot be solved deterministically even if a single process can fail, and it does so only by crashing; this is the seminal FLP impossibility result~\cite{fischer1985impossibility}.

A traditional way of circumventing the FLP impossibility result is \emph{randomization}~\cite{B83,aspnes2003randomized,abraham2019asymptotically,LL0W20,ezhilchelvan2001randomized}, where termination of consensus is not ensured deterministically.
Another well-established approach to bypass the FLP impossibility is to strengthen the communication model with \emph{partial synchrony}~\cite{DLS88}: the communication is asynchronous until some unknown time, and then it becomes synchronous.
The last couple of decades have produced many partially synchronous consensus algorithms~\cite{yin2019hotstuff,CGL18,CGG21,CL02,DLS88,BKM19,lynch1996distributed,lamport2001paxos,civit2022byzantine,lewis2022quadratic}.
% Recently, the aforementioned Dolev-Reischuk bound was shown to be tight even in partial synchrony~\cite{civit2022byzantine,lewis2022quadratic}.

Another line of research has consisted in weakening the definition of  consensus  to make it deterministically solvable under asynchrony.
In the \emph{condition-based} approach~\cite{mostefaoui2003conditions}, 
the specification of consensus is relaxed to require termination only if the assignment of proposals satisfies some predetermined conditions.
The efficiency of this elegant approach has been studied further in~\cite{mostefaoui2001hierarchy}.
Moreover, the approach is extended to the synchronous setting~\cite{mostefaoui2003using,zibin2003condition}, as well as  to the $k$-set agreement problem~\cite{hagit2002wait,mostefaoui2002condition}.

\paragraph{Solvability of general decision problems.}
% The question of which problems are solvable under which assumptions is crucial in distributed computing.
% Traditionally, 
A distributed decision problem has been defined in~\cite{crime_punishment,MendesTH14,HerlihyS99} 
as a mapping from input assignments to admissible decisions. 
Our validity formalism is of the same nature, and it is inspired by the aforementioned specification of decision problems.

The solvability of decision problems has been thoroughly studied in asynchronous, crash-prone settings.
It was shown in~\cite{moran1987extended} that the FLP impossibility result~\cite{fischer1985impossibility} can be extended to many decision problems.
In~\cite{biran1990combinatorial}, the authors defined the necessary and sufficient conditions for a decision problem to be asynchronously solvable with a single crash failure.
% the aforementioned work from Moran and Wolfstahl~\cite{moran1987extended}.
The asynchronous solvability of problems in which crash failures occur at the very beginning of an execution was studied in~\cite{taubenfeld1989initial}.
%using the game-theoretical approach, authors give necessary and sufficient conditions for a problem to be solvable in such a setting. 
The necessary and sufficient conditions for a decision problem to be asynchronously solvable (assuming a crash-prone setting) in a randomized manner were given in ~\cite{Chor1989}. 
The topology-based approach on studying the solvability of decision problems in asynchrony has proven to be extremely effective, both for crash~\cite{HerlihyS93,SaraphHG18,Herlihy2013} and arbitrary failures~\cite{MendesTH14,Herlihy2013}.
% \jovan{Pierre, please add some citations for topology (if you know them).} \pierre{Classically, results from algebraic topology address deterministic asynchronous computation (e.g. approximate agreement, $k$-set agreement, etc). I do no think they are topology-based results for consensus. I will take a look.}
Our results follow the same spirit as many of these approaches; however, we study the deterministic solvability and complexity of all consensus variants in a partially synchronous environment.

\paragraph{Validity of consensus.}
Various validity properties have been  associated with the consensus problem (beyond the aforementioned \emph{Strong Validity} and \emph{Weak Validity}).
\emph{Correct-Proposal Validity}~\cite{fitzi2003efficient,siu1998reaching} states that  a value decided by a correct process must have been proposed by a correct process. 
% (The consensus problem with \emph{Correct Proposal Validity} is usually referred to as strong Byzantine consensus.)
\emph{Median Validity}~\cite{stolz2016byzantine} is a validity property proposed in the context of synchronous consensus,  requiring the decision to be close to the median of the proposals of correct processes. \emph{Interval Validity}~\cite{melnyk2018byzantine}, on the other hand, requires the  decision to be close to the $k$-th smallest proposal of correct processes.
The advent of blockchain technologies has resurged the concept of \emph{External Validity}~\cite{Cachin2001,BKM19,yin2019hotstuff}.
This property requires the decided value to satisfy a predetermined predicate, typically asserting whether the decided value follows the rules of a blockchain system (e.g., no double-spending).
(This paper considers a simple formalism to express basic validity properties and derive our results. To express \emph{External Validity}, which is out of the scope of the paper, we propose an (incomplete) extension of our formalism in \Cref{section:extended_formalim_appendix}, and leave its full realization for future work.)
\emph{Convex-Hull Validity}, which states that the decision must belong to the convex hull of the proposals made by the correct processes, is employed in approximate agreement~\cite{AbrahamAD04,MendesH13,GhineaLW22,ghinea2023multidimensional}.
We underline that the approximate agreement problem is not covered in this paper since the problem allows correct processes to disagree as long as their decisions are ``close'' to each other.
However, this paper does study (in a general manner) the utilization of \emph{Convex-Hull Validity} in the classical consensus problem (in which the correct processes are required to ``exactly'' agree).


In interactive consistency~\cite{maneas2021achieving,fischer1981lower,ben2003resilient},  correct processes agree on the proposals of all correct processes. Given that the problem is  impossible in a non-synchronous setting, a weaker variant has been considered: vector consensus~\cite{neves2005solving,vaidya2013byzantine,Doudou1998,correia2006consensus,duan2023practical,Ben-Or94}. Here, processes need to agree on a vector of proposals which does not necessarily include the proposals of \emph{all} correct processes. Interactive consistency and vector consensus can be seen as specific consensus problems with a validity property requiring that, if a decided vector contains a proposal $v$ of a correct process, that correct process has indeed proposed $v$.
% which requires the decided vector to contain all the proposals of correct processes.
The design of \general, our general consensus algorithm for any solvable (and non-trivial) validity property, demonstrates that any non-trivial flavor of consensus which is solvable in partial synchrony can be solved using vector consensus (see \Cref{subsection:general_algorithm}).



==> sections/former/similarity_lemma.tex <==
\subsection{Canonical Similarity} \label{subsection:similarity}

In this subsection, we introduce \emph{canonical similarity}, a crucial intermediate result.
In order to do so, we first establish an important relation between input configurations, that of \emph{similarity}.

\paragraph{Similarity.}

We define the similarity relation (``$\sim$'') between input configurations:
\begin{equation*}
    \forall c_1, c_2 \in \allconfigurations: c_1 \sim c_2 \iff (\processes{c_1} \cap \processes{c_2} \neq \emptyset) \land (\forall P_i \in \processes{c_1} \cap \processes{c_2}: c_1[i] = c_2[i]).
\end{equation*}

In other words, $c_1$ is similar to $c_2$ if and only if (1) $c_1$ and $c_2$ have (at least) one process in common, and (2) for every common process, the process's proposal is identical in both input configurations.
For example, when $n = 3$ and $t = 1$, $c = \big[ (P_1, 0), (P_2, 1), (P_3, 0) \big]$ is similar to $\big[ (P_1, 0), (P_3, 0) \big]$, whereas $c$ is not similar to $\big[ (P_1, 0), (P_2, 0), (P_3, 0) \big]$.
Note that the similarity relation is symmetric (for every pair $c_1, c_2 \in \mathcal{I}$, $c_1 \sim c_2 \Leftrightarrow c_2 \sim c_1$) and reflexive (for every $c \in \mathcal{I}$, $c \sim c$).

For every input configuration $c \in \mathcal{I}$, we define its \emph{similarity set}, denoted by $\mathit{sim}(c)$:
\begin{equation*}
    \mathit{sim}(c) = \{ c' \in \mathcal{I} \,|\, c' \sim c \}.
\end{equation*}

% We rely on the similarity relation to define canonical simi larity (\Cref{subsection:intermediate_results}), and the similarity condition (\Cref{subsection:necessary_condition}).

% We later rely on the similarity relation in defining the similarity condition, which we prove to be a necessary condition for a validity property to be solvable (see \Cref{subsection:necessary_condition}).
% utilize to classify validity properties.

\paragraph{The result.}
Let $\mathcal{A}$ be an algorithm which solves  consensus  with some validity property $\mathit{val}$.
Our canonical similarity result states that $\mathcal{A}$, in any canonical execution which corresponds to some input configuration $c$, can only decide a value which is admissible for \emph{all} input configurations similar to $c$.
Informally, the reason is that correct processes cannot distinguish silent faulty processes from slow correct ones.

\begin{lemma}[Canonical similarity] \label{lemma:helper_main}
Let $\mathit{val}$ be any solvable validity property and let $\mathcal{A}$ be any algorithm which solves the consensus problem with $\mathit{val}$.
Let $\mathcal{E} \in \mathit{execs}(\mathcal{A})$ be any (potentially infinite) canonical execution and let $\mathsf{input\_conf}(\mathcal{E}) = c$, for some input configuration $c \in \mathcal{I}$.
If a value $v' \in \mathcal{V}_O$ is decided by a correct process in $\mathcal{E}$, then $v' \in \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
\end{lemma}
\begin{proof}
We prove the lemma by contradiction.
Suppose that $v' \notin \bigcap\limits_{c' \in \mathit{sim}(c)} \mathit{val}(c')$.
Hence, there exists an input configuration $c' \in \mathit{sim}(c)$ such that $v' \notin \mathit{val}(c')$.
If $\mathcal{E}$ is infinite, let $\mathcal{E}_P \gets \mathcal{E}$.
Otherwise, let $\mathcal{E}_P$ denote any infinite continuation of $\mathcal{E}$ such that (1) $\mathcal{E}_P$ is canonical, and (2) $\mathsf{input\_conf}(\mathcal{E}_P) = c$.
Let $P$ be any process such that $P \in \processes{c'} \cap \processes{c}$; such a process exists as $c' \sim c$.
As $\mathcal{A}$ satisfies \emph{Termination} and \emph{Agreement}, $\mathcal{E}_P$ is an infinite execution, and $P$ is correct in $\mathcal{E}_P$, $P$ decides $v'$ in $\mathcal{E}_P$.
Let $\mathcal{S}$ denote the set of all processes which take a computational step in $\mathcal{E}_P$ until $P$ decides $v'$; note that $\mathcal{S} \subseteq \processes{c}$ and $P \in \mathcal{S}$.

In the next step, we construct another execution $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}') = c'$:
\begin{compactenum}
    \item $\mathcal{E}'$ is identical to $\mathcal{E}_P$ until process $P$ decides $v'$.
    
    \item All processes not in $\processes{c'}$ are faulty in $\mathcal{E}'$ (they might behave correctly until $P$ has decided), and all processes in $\processes{c'}$ are correct in $\mathcal{E}'$.
    % Observe that processes behave correctly in $\mathcal{E}'$ until $P$ has decided.
    
    \item After $P$ has decided, processes in $\processes{c'} \setminus{\mathcal{S}}$ ``wake up'' with the proposals specified in $c'$.
    
    \item GST is set to after all processes in $\processes{c'}$ have taken a computational step.
\end{compactenum}
For every process $P_i \in \mathcal{S} \cap \processes{c'}$, the proposal of $P_i$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[i])$; recall that $c'[i] = c[i]$ as $c' \sim c$ and $\mathcal{S} \subseteq \processes{c}$.
Moreover, for every process $P_j \in \processes{c'} \setminus{\mathcal{S}}$, the proposal of $P_j$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[j])$ (due to the step 3 of the construction).
Hence, $\mathsf{input\_conf}(\mathcal{E}') = c'$.
Furthermore, process $P$, which is correct in $\mathcal{E}'$, decides a value $v' \notin \mathit{val}(c')$ (due to the step 1 of the construction).
Thus, we reach a contradiction with the fact that $\mathcal{A}$ satisfies $\mathit{val}$, which proves the lemma.
\end{proof}

We underline that \Cref{lemma:helper_main} does not rely on \emph{any} assumptions on $n$ and $t$.
In other words, \Cref{lemma:helper_main} is applicable to any algorithm irrespectively of the parameters $n$ and $t$ (as long as $0 < t < n$).

% We construct another execution $\mathcal{E}' \in \mathit{execs}(\mathcal{A})$ such that $\mathsf{input\_conf}(\mathcal{E}') = c'$:
% \begin{compactenum}
%     \item $\mathcal{E}'$ is identical to $\mathcal{E}_P$ until process $P$ decides $v'$.
    
%     \item All processes in $\Pi \setminus{\processes{c'}}$ are faulty in $\mathcal{E}'$ (they behave correctly until $P$ has decided), and all processes in $\processes{c'}$ are correct.
%     % Observe that processes behave correctly in $\mathcal{E}'$ until $P$ has decided.
    
%     \item After $P$ has decided, processes in $\processes{c'} \setminus{\processes{c}}$ ``wake up'' with the proposals specified in $c'$.
    
%     \item GST is set to after all processes in $\processes{c'}$ have taken a computational step.
% \end{compactenum}
% For every process $P_i \in \processes{c'} \cap \processes{c}$, the proposal of $P_i$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[i])$; recall that $c'[i] = c[i]$ as $c' \sim c$.
% Moreover, for every process $P_j \in \processes{c'} \setminus{\processes{c}}$, the proposal of $P_j$ in $\mathcal{E}'$ is $\mathsf{proposal}(c'[j])$ (due to the step 3 of the construction).

==> sections/repeater.tex <==
\section{\name Transformation}

This section introduces \name, our generic transformation that maps \emph{any} synchronous Byzantine agreement algorithm into a partially synchronous one.
Concretely, \name is a Byzantine agreement algorithm that internally utilizes multiple instances of \block (see \Cref{section:block}); recall that each instance of \block can be constructed using any synchronous agreement protocol.
Importantly, the bit complexity $\mathit{bit}(\name)$ of \name with constant-sized values is
\begin{equation*}
    \mathit{bit}(\name) = O\big(n^2 + \mathit{bit}(\block)\big).
\end{equation*}
Moreover, the bit complexity $\mathit{bit}(\name)$ of \name with $L$-bit (with $L \notin O(1)$) is 
\begin{equation*}
    \mathit{bit}(\name) = O\big(nL + n^2 \log n + \mathit{bit}(\block)\big).
\end{equation*}

This section first presents the pseudocode of \name (\Cref{subsection:name_pseudocode}), and then discusses \name's correctness (\Cref{subsection:name_correctness_complexity}).
Finally, this section presents some efficient and signature-less partially synchronous Byzantine agreement algorithms that can be constructed by \name (\Cref{subsection:concrete_algorithms}).

\subsection{Pseudocode} \label{subsection:name_pseudocode}

We present \name's pseudocode in \Cref{algorithm:name_pseudocode} described below.
For simplicity, we present \name assuming only constant-sized values.
We relegate a modification of \Cref{algorithm:name_pseudocode} for long $L$-bit values to \Cref{section:name_correctness_complexity_formal}.

\begin{algorithm}
\caption{\name for constant-sized values: Pseudocode (for process $p_i$)}
\label{algorithm:name_pseudocode}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em \block with parameter $\Delta_{\mathit{shift}} = 2\delta$, \textbf{instances} $\mathcal{CX}(V)$, for every $V \in \mathsf{View}$ \label{line:main_block_instance} \BlueComment{see \Cref{section:block}}

% \medskip
% \State \textbf{Local timers:}
% \State \hskip2em $\mathsf{Timer}$ $\mathit{help\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{enter\_timer}_i$

\medskip
\State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets \bot$
\State \hskip2em $\mathsf{Boolean}$ $\mathit{sent\_decide}_i \gets \mathit{false}$
\State \hskip2em $\mathsf{Map}(\mathsf{View} \to \mathsf{Boolean})$ $\mathit{helped}_i \gets \{\mathit{false}, \mathit{false}, ..., \mathit{false}\}$
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ \label{line:main_init_view}
% \State \hskip2em $\mathsf{View}$ $\mathit{last\_entered}_i \gets 1$
% \State \hskip2em $\mathsf{View}$ $\mathit{help\_view}_i \gets 1$ \label{line:init_help_view}

\medskip
\State \textbf{upon} $\mathsf{propose}(\mathit{pro}_i \in \mathsf{Value})$: \label{line:main_name_propose} \BlueComment{start participating in \name}
% \State \hskip2em $\mathit{proposal}_i \gets \mathit{proposal}$
\State \hskip2em \textbf{invoke} $\mathcal{CX}(1).\mathsf{propose}(\mathit{proposal})$ \BlueComment{start \block associated with view $1$ (i.e., enter view $1$)} \label{line:main_enter_1}

\medskip
\State \textbf{upon} $\mathcal{CX}(\mathit{view}_i).\mathsf{completed}$: \label{line:main_view_timer_expire} \BlueComment{current \block instance (i.e., current view) has completed}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i + 1 \rangle$ \label{line:main_send_complete_1} \BlueComment{start transiting to the next view}

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $V$ such that $\langle \textsc{start-view}, V \rangle$ is received from $t + 1$ processes and $\mathit{helped}_i[V] = \mathit{false}$: \label{line:main_receive_plurality}
\State \hskip2em $\mathit{helped}_i[V] \gets \mathit{true}$
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, V \rangle$ \label{line:main_send_complete_2}
% \label{line:main_send_complete_2_prime} 

% \State \hskip2em \textbf{if} $v > \mathit{help\_view}_i$: \label{line:check_help}
% \State \hskip4em $\mathit{help\_view}_i \gets v$ \label{line:update_help_view}
% \State \hskip4em $\mathit{help\_timer}_i.\mathsf{cancel}()$ \label{line:cancel_help}
% \State \hskip4em $\mathit{help\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_help}

% \medskip
% \State \textbf{upon} $\mathit{help\_timer}_i$ \textbf{expires}: \label{line:help_timer_expires}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i \rangle$ \label{line:send_complete_2}
% \State \hskip2em \textbf{if} $\mathit{help\_view}_i > 2$: \label{line:check_help_2}
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ \label{line:send_complete_2_prime} 
% \State \hskip2em \textbf{if} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ is received from $t + 1$ processes:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ 

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $V > \mathit{view}_i$ such that $\langle \textsc{start-view}, V \rangle$ is received from $2t + 1$ processes: \label{line:main_receive_quorum}
% \label{line:send_complete_3_prime}
\State \hskip2em \textbf{invoke} $\mathcal{CX}(\mathit{view}_i).\mathsf{abandon}$ \BlueComment{stop participating in the current \block instance} \label{line:main_leave_v}
\State \hskip2em \textbf{wait for} $\mathcal{CX}(V - 1).\mathsf{validate}(v \in \mathsf{Value})$ \label{line:main_wait_to_validate} \BlueComment{wait for a value to propose to the new \block instance}
\State \hskip2em \textbf{invoke} $\mathcal{CX}(V).\mathsf{propose}(v)$ \BlueComment{start the new \block instance (i.e., enter new view)}  \label{line:main_enter_v}
\State \hskip2em $\mathit{view}_i \gets V$ \label{line:main_update_view_i} \BlueComment{update the current view}
% \State \hskip2em $\mathit{last\_entered}_i \gets \mathit{view}_i$

% \medskip
% \State \textbf{upon} $\mathit{enter\_timer}_i$ \textbf{expires:} \label{line:enter_expires}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i \rangle$ \label{line:send_complete_3}
% \State \hskip2em \textbf{if} $\mathit{view}_i > 2$: \label{line:check_view}
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i - 1 \rangle$ \label{line:send_complete_3_prime}
% \State \hskip2em \textbf{invoke} $\mathit{core}(\mathit{last\_entered}_i).\mathsf{abandon}$ \BlueComment{stop participating in the current view core abstraction} \label{line:leave_v}
% \State \hskip2em \textbf{wait for} $\mathit{core}(\mathit{view}_i - 1).\mathsf{validate}(\mathit{val} \in \mathsf{Value})$
% \State \hskip2em \textbf{invoke} $\mathit{core}(\mathit{view}_i).\mathsf{propose}(\mathit{val})$ \BlueComment{start \block associated with view $\mathit{view}_i$}  \label{line:enter_v}
% \State \hskip2em $\mathit{last\_entered}_i \gets \mathit{view}_i$

\medskip
\State \textbf{upon} $\mathcal{CX}(\mathit{view}_i).\mathsf{decide}(v' \in \mathsf{Value})$ and $\mathit{sent\_decide}_i = \mathit{false}$: \label{line:main_decide_from_core} \BlueComment{decided from \block}
\State \hskip2em $\mathit{sent\_decide}_i \gets \mathit{true}$
\State \hskip2em \textbf{broadcast} $\langle \textsc{decide}, v' \rangle$ \label{line:main_send_decided_1} \BlueComment{disseminate the decision}

\medskip
\State \textbf{upon} exists $\mathsf{Value}$ $v'$ such that $\langle \textsc{decide}, v' \rangle$ is received from $t + 1$ processes and $\mathit{sent\_decide}_i = \mathit{false}$: \label{line:main_receive_decided_2}
\State \hskip2em $\mathit{sent\_decide}_i \gets \mathit{true}$
\State \hskip2em \textbf{broadcast} $\langle \textsc{decide}, v' \rangle$ \label{line:main_send_decided_2} \BlueComment{help dissemination of the \textsc{decide} messages}

\medskip
\State \textbf{upon} exists $\mathsf{Value}$ $v'$ such that $\langle \textsc{decide}, v' \rangle$ is received from $2t + 1$ processes: \label{line:main_receive_decided_3}
\State \hskip2em \textbf{broadcast} $\langle \textsc{decide}, v' \rangle$ \label{line:main_send_decided_3}
\State \hskip2em \textbf{trigger} $\mathsf{decide}(v')$  \label{line:main_name_decide} \BlueComment{decide from \name}
\State \hskip2em \textbf{halt} \BlueComment{stop sending any messages and reacting to any received messages}  \label{line:main_name_stop} 
\end{algorithmic} 
\end{algorithm}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% repeater correction for long inputs %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \pierre{I am writing the correction for long inputs, it will be polished later}

% \begin{algorithm}
% \caption{\name: Pseudocode for long inputs (for process $p_i$)}
% \label{algorithm:name_pseudocode_long_input}
% \footnotesize
% \begin{algorithmic} [1] 
% \State \textbf{Uses:}
% \State \hskip2em \block with parameter $\Delta_{\mathit{shift}} = 2\delta$, \textbf{instances} $\mathcal{CX}(V)$, for every $V \in \mathsf{View}$ \label{line_name_long_input:block_instance} \BlueComment{see \Cref{section:block}}

% \medskip
% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{decided}_i \gets \mathit{false}$
% \State \hskip2em $\mathsf{Boolean}$ $\mathit{add\_started}_i \gets \mathit{false}$
% \State \hskip2em $\mathsf{Map}(\mathsf{View} \to \mathsf{Boolean})$ $\mathit{helped}_i \gets \{\mathit{false}, \mathit{false}, ..., \mathit{false}\}$
% \State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ \label{line_name_long_input:init_view}


% \medskip
% \State \textbf{upon} $\mathsf{propose}(\mathit{pro}_i \in \mathsf{Value})$: \label{line_name_long_input:name_propose} \BlueComment{start participating in \name}
% \State \hskip2em \textbf{invoke} $\mathcal{CX}(1).\mathsf{propose}(\mathit{proposal})$ \BlueComment{start \block associated with view $1$ (i.e., enter view $1$)} \label{line_name_long_input:enter_1}

% \medskip
% \State \textbf{upon} $\mathcal{CX}(\mathit{view}_i).\mathsf{completed}$: \label{line_name_long_input:view_timer_expire} \BlueComment{current \block instance (i.e., current view) has completed}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i + 1 \rangle$ \label{line_name_long_input:send_complete_1} \BlueComment{start transiting to the next view}

% \medskip
% \State \textbf{upon} exists $\mathsf{View}$ $V$ such that $\langle \textsc{start-view}, V \rangle$ is received from $t + 1$ processes and $\mathit{helped}_i[V] = \mathit{false}$: \label{line_name_long_input:receive_plurality}
% \State \hskip2em $\mathit{helped}_i[V] \gets \mathit{true}$
% \State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, V \rangle$ \label{line_name_long_input:send_complete_2}
% \label{line_name_long_input:send_complete_2_prime} 

 
% \medskip
% \State \textbf{upon} exists $\mathsf{View}$ $V > \mathit{view}_i$ such that $\langle \textsc{start-view}, V \rangle$ is received from $2t + 1$ processes: \label{line_name_long_input:receive_quorum}
% \label{line_name_long_input:send_complete_3_prime}
% \State \hskip2em \textbf{invoke} $\mathcal{CX}(\mathit{view}_i).\mathsf{abandon}$ \BlueComment{stop participating in the current \block instance} \label{line_name_long_input:leave_v}
% \State \hskip2em \textbf{wait for} $\mathcal{CX}(V - 1).\mathsf{validate}(v \in \mathsf{Value})$ \label{line_name_long_input:wait_to_validate} \BlueComment{wait for a value to propose to the new \block instance}
% \State \hskip2em \textbf{invoke} $\mathcal{CX}(V).\mathsf{propose}(v)$ \BlueComment{start the new \block instance (i.e., enter new view)}  \label{line_name_long_input:enter_v}
% \State \hskip2em $\mathit{view}_i \gets V$ \label{line_name_long_input:update_view_i} \BlueComment{update the current view}

% \medskip
% \State \textbf{upon} $\mathcal{CX}(\mathit{view}_i).\mathsf{decide}(v' \in \mathsf{Value})$ and $\mathit{decided}_i = \mathit{false}$: \label{line_name_long_input:decide_from_core} \BlueComment{decided from \block}
% \State \hskip2em $\mathit{decided}_i \gets \mathit{true}$
% \State \hskip2em $\mathit{add\_started}_i \gets \mathit{true}$

% \State \hskip2em \textbf{invoke} $\mathsf{ADD.input}(v')$ \BlueComment{disseminate the decision}

% \State \hskip2em \textbf{broadcast} $\langle \textsc{add\_started}, \top \rangle$ \label{line_name_long_input:send_decided_1} 

% \medskip
% \State \textbf{upon} the reception of $2t + 1$ $\langle \textsc{add\_started}, * \rangle$  messages from as many different processes and $\mathit{add\_started}_i = \mathit{false}$: \label{line_name_long_input:receive_decided_3}

% \State \hskip2em $\mathit{add\_started}_i \gets \mathit{true}$

% \State \hskip2em \textbf{invoke} $\mathsf{ADD.input}(\bot)$

% \State \hskip2em \textbf{broadcast} $\langle \textsc{add\_started}, \bot \rangle$ 

% \medskip
% \State \textbf{upon} $\mathsf{ADD.output}(v')$ and $\mathit{decided}_i = \mathit{false}$: \label{line_name_long_input:receive_decided_3}

% \State \hskip2em \textbf{if} $\mathit{decided}_i = \mathit{false}$: 

% \State \hskip4em \textbf{trigger} $\mathsf{decide}(v')$  \label{line_name_long_input:name_decide} \BlueComment{decide from \name}
% \State \hskip2em \textbf{halt} \BlueComment{stop sending any messages and reacting to any received messages}  \label{line_name_long_input:name_stop} 
% \end{algorithmic} 
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %% end repeater correction for long inputs %%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% As with many partially synchronous algorithms~\cite{yin2019hotstuff,BKM19}, \name's execution unfolds in views.
% Concretely, let $\mathsf{View} = \{1, 2, ...\}$ denote the set of views.

\paragraph{Description.}
As with many partially synchronous algorithms~\cite{yin2019hotstuff,BKM19}, \name's executions unfold in views; $\mathsf{View} = \{1, 2, ...\}$ denotes the set of views.
Moreover, each view is associated with its instance of \block (see \Cref{section:block}); the instance of \block associated with view $V \in \mathsf{View}$ is denoted by $\mathcal{CX}(V)$ (line~\ref{line:block_instance}).
To guarantee liveness, \name ensures that all correct processes are brought to the same instance of \block for sufficiently long after GST, thus allowing \block to decide (due to its synchronicity property).
The safety of \name is ensured by the careful utilization of the \block instances.
We proceed to describe \name's pseudocode (\Cref{algorithm:name_pseudocode}) from the perspective of a correct process $p_i$.

% Moreover, each view 

% \name internally relies on the \block core consensus primitive (\Cref{section:block}).
% Precisely, \name associates each view with its own \block instance (line~\ref{line:block_instance}); we denote by $\mathit{core}(v)$ the \block instance associated with view $v$.
% In a nutshell, \name aims to ensure that all correct processes are brought together to the same instance of \block after GST, which then allows \block to decide.
% We say that a correct process $p_i$ \emph{enters} view $v$ if and only if $p_i$ invokes $\mathit{core}(v).\mathsf{propose}(\cdot)$.
% We proceed to describe the pseudocode from the perspective of a correct process $p_i$.

We say that process $p_i$ \emph{enters} view $V$ once $p_i$ invokes a $\mathcal{CX}(V).\mathsf{propose}(\cdot)$ request (line~\ref{line:enter_1} or line~\ref{line:enter_v}).
Moreover, a process $p_i$ \emph{completes} view $V$ once $p_i$ receives a $\mathsf{completed}$ indication from $\mathcal{CX}(V)$ (line~\ref{line:view_timer_expire}).
Process $p_i$ keeps track of its \emph{current view} using the $\mathit{view}_i$ variable: $\mathit{view}_i$ is the last view entered by $p_i$. 
When process $p_i$ proposes to \name (line~\ref{line:name_propose}), $p_i$ forwards the proposal to $\mathcal{CX}(1)$ (line~\ref{line:enter_1}), i.e., $p_i$ enters view $1$.
Once process $p_i$ completes its current view (line~\ref{line:view_timer_expire}), $p_i$ starts transiting to the next view: process $p_i$ sends a \textsc{start-view} message for the next view, illustrating its will to enter the next view (line~\ref{line:send_complete_1}).
When $p_i$ receives $t + 1$ \textsc{start-view} messages for the same view (line~\ref{line:receive_plurality}), $p_i$ ``helps'' a transition to that view by broadcasting its own \textsc{start-view} message (line~\ref{line:send_complete_2}).
Finally, when $p_i$ receives $2t + 1$ \textsc{start-view} messages for any view $V$ greater than its current view (line~\ref{line:receive_quorum}), $p_i$ performs the following steps: (1) $p_i$ abandons its current (stale) view (line~\ref{line:leave_v}), (2) waits until it validates any value $v$ from $\mathcal{CX}(V - 1)$ (line~\ref{line:wait_to_validate}), (3) enters view $V$ with value $v$ (line~\ref{line:enter_v}), and (4) updates its current view to $V$ (line~\ref{line:update_view_i}).

Once process $p_i$ decides some value $v'$ from a \block instance associated with its current view (line~\ref{line:decide_from_core}), process $p_i$ broadcasts a $\langle \textsc{decide}, v' \rangle$ message (line~\ref{line:main_send_decided_1}).
Similarly, if $p_i$ receives $t + 1$ \textsc{decide} messages for the same value (line~\ref{line:main_receive_decided_2}), $p_i$ disseminates that \textsc{decide} message (line~\ref{line:main_send_decided_2}) if it has not already broadcast a \textsc{decide} message.
Lastly, once $p_i$ receives $2t + 1$ \textsc{decide} messages for the same value $v'$ (line~\ref{line:main_receive_decided_3}), $p_i$ performs the following steps: (1) $p_i$ broadcasts a \textsc{decide} message for $v'$ (line~\ref{line:main_send_decided_3}) to help other correct processes receive $2t + 1$ \textsc{decide} messages, (2) $p_i$ decides $v'$ from \name (line~\ref{line:main_name_decide}), and (3) $p_i$ halts, i.e., $p_i$ stops sending and reacting to messages (line~\ref{line:main_name_stop}).
%\add{The \name's pseudocode from line~\ref{line:decide_from_core} to line~\ref{line:name_stop} is written for sake of presentation, but require additional technical efforts to efficiently handle long inputs \cite{das2021asynchronous}. Details are given in appendix TO CITE (see \Cref{algorithm:finisher_long_inputs}}

\paragraph{Remark on views entered by correct processes after GST}
Let us denote by $\vmax$ the greatest view entered by a correct process before GST.
We underline that the pseudocode of \name (\Cref{algorithm:name_pseudocode}) allows correct processes to enter every single view smaller than $\vmax$ after GST.
Indeed, a slow correct process might receive $2t + 1$ \textsc{start-view} messages (line~\ref{line:receive_quorum}) for every view preceding view $\vmax$.
Hence, the number of messages (and bits) correct processes send after GST (given the \name's implementation presented in \Cref{algorithm:name_pseudocode}) depends on $\vmax$.\footnote{As $\vmax$ depends on GST, clocks drifts and message delays before GST (and not on $n$), we treat $\vmax$ as a constant.}
However, we can modify \name to send $O(1)$ messages (and bits) after GST regardless of GST's value by incorporating the ``$\delta$-waiting step'' strategy introduced in~\cite{civit2022byzantine}.
Concretely, correct processes would not immediately enter a view upon receiving $2t + 1$ \textsc{start-view} messages.
Instead, a correct process would wait $\delta$ time to potentially learn about a more recent view than the one the process was about to enter.
For the sake of simplicity and presentation, we opted not to incorporate the aforementioned ``$\delta$-waiting step'' strategy proposed in~\cite{civit2022byzantine}.

\subsection{Correctness: Proof Sketch} \label{subsection:name_correctness_complexity}

In this subsection, we give a proof sketch of the following result:

\begin{theorem} \label{theorem:name_correctness_complexity}
\name (\Cref{algorithm:name_pseudocode}) is a correct partially synchronous Byzantine agreement algorithm that tolerates $t < n / 3$ faulty processes.
% Moreover, the bit complexity of \name is identical to the number of bits correct processes send in one instance of the underlying \block primitive.
\end{theorem}

We relegate the formal proof of \name's correctness and complexity to \Cref{section:name_correctness_complexity_formal}.
Our informal proof of \Cref{theorem:name_correctness_complexity} relies on a sequence of intermediate results that we introduce below.

\smallskip
\noindent \textbf{Result 1:} \emph{No two correct processes broadcast \textsc{decide} messages for different values.}

\noindent The first correct process $p_i$ that broadcasts a \textsc{decide} message does so upon deciding from $\mathcal{CX}(V)$ (line~\ref{line:decide_from_core}), where $V$ is some view.
Let that message be for some value $v$.
Due to the agreement property of $\mathcal{CX}(V)$, all correct processes that decide or validate from $\mathcal{CX}(V)$ do so with value $v$.
Therefore, every correct process that enters view $V + 1$ (i.e., proposes to $\mathcal{CX}(V + 1)$) does so with value $v$ (line~\ref{line:enter_v}).
Hence, the strong validity property of $\mathcal{CX}(V + 1)$ ensures that only $v$ can be decided or validated from $\mathcal{CX}(V + 1)$.
Applying the same reasoning inductively yields a conclusion that any correct process that decides from $\mathcal{CX}(V')$, for any view $V' \geq V$, does decide value $v$.

Utilizing another inductive argument shows that any correct process $p_j$ that broadcasts a \textsc{decide} message after process $p_i$ does so for value $v$.
Let us consider all possibilities for $p_i$ to broadcast a \textsc{decide} message:
\begin{compactitem}
    \item line~\ref{line:main_send_decided_1}: In this case, the message is for $v$ as only $v$ can be decided from the instances of \block (see the previous paragraph).

    \item line~\ref{line:main_send_decided_2} or line~\ref{line:main_send_decided_3}: Assuming that all previous \textsc{decide} messages broadcast by correct processes are for value $v$, the message sent by $p_j$ must be for $v$ as $p_j$ has received at least one \textsc{decide} message sent by a correct process (due to the rules at line~\ref{line:main_receive_decided_2} and line~\ref{line:main_receive_decided_3}).
\end{compactitem}

\smallskip
The agreement property of \name follows immediately from Result 1.

\smallskip
\noindent \textbf{Agreement:} \emph{No two correct processes decide different values.}

\noindent If a correct process $p_i$ (resp., $p_j$) decides a value $v$ (resp., $v'$) at line~\ref{line:main_name_decide}, then $p_i$ (resp., $p_j$) has previously received a \textsc{decide} message for $v$ (resp., $v'$) sent by a correct process (due to the rule at line~\ref{line:main_receive_decided_3}).
By Result 1, $v = v'$.

\smallskip
Another consequence of Result 1 is external validity of \name.

\smallskip
\noindent \textbf{External validity:} \emph{If a correct process decides a value $v'$, then $\mathsf{valid}(v') = \mathit{true}$.}

\noindent Let $v$ be the value carried by the first \textsc{decide} message sent by a correct process.
As that \textsc{decide} message is sent upon deciding from $\mathcal{CX}(V)$ (line~\ref{line:main_send_decided_1}), for some view $V$, the external validity property of $\mathcal{CX}(V)$ guarantees that $v$ is valid.
Since Result 1 states that all \textsc{decide} messages sent by correct processes are sent for value $v$, only $v$ can be decided by any correct process (line~\ref{line:main_name_decide}).
Given that $v$ is a valid value, external validity is satisfied by \name.

% \smallskip
% Integrity property is trivially satisfied.

% \smallskip
% \noindent \textbf{Integrity:} \emph{No correct process decides more than once.}
% \ayaz{we don't have this property in byzantine agreement (referring to the properties in the introduction)}
%\noindent Ensured by the fact that a correct process halts (line~\ref{line:name_stop}) as soon as it decides (line~\ref{line:name_decide}).

\smallskip
Next, we show that \name satisfies strong validity.

\smallskip
\noindent \textbf{Strong validity:} \emph{If all correct processes propose the same value $v$, no correct process decides any value $v' \neq v$.}

\noindent Suppose that all correct processes propose the same value $v$ (line~\ref{line:main_name_propose}).
Hence, all correct processes that enter view $1$ do so with value $v$ (line~\ref{line:main_enter_1}).
Due to the strong validity property of $\mathcal{CX}(1)$, only $v$ can be decided or validated from $\mathcal{CX}(1)$.
By repeating the inductive argument from the proof sketch of Result 1, only $v$ can be decided from any \block instance.
Given that the first \textsc{decide} message sent by a correct process is sent upon deciding from a \block instance (line~\ref{line:main_send_complete_1}), that message must be for value $v$.
Result 1 further guarantees that all \textsc{decide} messages sent by correct processes carry value $v$.
Thus, if a correct process decides (line~\ref{line:main_name_decide}), it indeed decides value $v$.

\smallskip
To show that \name satisfies termination, we introduce new intermediate results.
The first such result shows that a correct process cannot enter a view unless the previous view was completed by a correct process.

\smallskip
\noindent \textbf{Result 2:} \emph{If a correct process enters a view $V > 1$, then a (potentially different) correct process has previously entered and completed view $V - 1$.}

\noindent For a correct process to enter a view $V > 1$ (line~\ref{line:main_enter_v}), a correct process must have previously broadcast a $\langle \textsc{start-view}, V \rangle$ message (due to the rule at line~\ref{line:main_receive_quorum}).
As the first correct process to broadcast a $\langle \textsc{start-view}, V \rangle$ message does so upon completing view $V - 1$ (line~\ref{line:main_send_complete_1}), that process has previously completed and entered view $V - 1$.

\smallskip
The next intermediate result shows that, if any correct process decides, then all correct processes eventually decide.

\smallskip
\noindent \textbf{Result 3:} \emph{If any correct process decides, then all correct processes eventually decide.}

\noindent If any correct process $p_i$ decides (line~\ref{line:main_name_decide}), process $p_i$ has previously received $2t + 1$ \textsc{decide} messages (due to the rule at line~\ref{line:main_receive_decided_3}).
At least $t + 1$ messages out of the aforementioned $2t + 1$ messages are broadcast by correct processes, which implies that every correct process eventually receives at least $t + 1$ \textsc{decide} message.
Hence, every correct process eventually broadcasts a \textsc{decide} message (line~\ref{line:main_send_decided_2}).
Thus, every correct process eventually receives $2t + 1$ \textsc{decided} messages (line~\ref{line:main_receive_decided_3}), and decides (line~\ref{line:main_name_decide}).

\smallskip
We now show that, if no correct process ever decides, then all views are eventually entered by a correct process.

\smallskip
\noindent \textbf{Result 4:} \emph{If no correct process decides, then all views are eventually entered by a correct process.}

\noindent By contradiction, let $V^* + 1 > 1$ be the smallest view not entered by a correct process.
Due to Result 2, no view greater than $V^* + 1$ is ever entered by a correct process.
% In brief, every correct process eventually enters view $v^*$ (i.e., the greatest view entered by a correct process).
In brief, every correct process $p_i$ eventually (1) broadcasts a $\langle \textsc{start-view}, V^* \rangle$ message (line~\ref{line:main_send_complete_2}) upon receiving $t + 1$ $\langle \textsc{start-view}, V^* \rangle$ messages (line~\ref{line:main_receive_plurality}), (2) enters view $V^*$ (line~\ref{line:main_enter_v}) upon receiving $2t + 1$ $\langle \textsc{start-view}, V^* \rangle$ messages (line~\ref{line:main_receive_quorum}), (3) broadcasts a $\langle \textsc{start-view}, V^* + 1 \rangle$ message (line~\ref{line:main_send_complete_1}) upon completing view $V^*$, and (4) enters view $V^* + 1$ (line~\ref{line:main_enter_v}) upon receiving $2t + 1$ $\langle \textsc{start-view}, V^* + 1 \rangle$ messages (line~\ref{line:main_receive_quorum}), resulting in a contradiction.

\smallskip
Let $\vfinal$ be the smallest view that is first entered by a correct process at or after GST.
We are finally ready to show that \name satisfies termination.

\smallskip
\noindent \textbf{Termination:} \emph{Every correct process eventually decides.}

\noindent By contradiction, let us assume that no correct process ever decides.
(If at least one correct process decides, Result 3 shows that all correct processes eventually decide.)
Therefore, due to Result 4, view $\vfinal$ is eventually entered by a correct process.
Let the first correct process to enter view $\vfinal$ do so at time $t_{\vfinal}$; due to the definition of $\vfinal$, $t_{\vfinal} \geq \text{GST}$.
By the completion time property of $\mathcal{CX}(\vfinal)$ and Result 2, no correct process enters any view greater than $\vfinal$ by time $t_{\vfinal} + \Delta_{\mathit{total}}$ (a parameter of $\mathcal{CX}(\vfinal)$, i.e., \block).
Moreover, all correct processes enter view $\vfinal$ by time $t_{\vfinal} + 2\delta$.
Indeed, all correct processes receive at least $t + 1$ $\langle \textsc{start-view}, \vfinal \rangle$ messages (line~\ref{line:main_receive_plurality}) and disseminate their $\langle 
\textsc{start-view}, \vfinal \rangle$ message by time $t_{\vfinal} + \delta$.
Hence, all correct processes receive $2t + 1$ $\langle \textsc{start-view}, \vfinal \rangle$ messages (line~\ref{line:main_receive_quorum}) and enter view $\vfinal$ by time $t_{\vfinal} + 2\delta$.

Given that the $\Delta_{\mathit{shift}}$ parameter of $\mathcal{CX}(\vfinal)$ is equal to $2\delta$, the precondition of the synchronicity property of $\mathcal{CX}(\vfinal)$ is fulfilled.
Therefore, all correct processes decide from $\mathcal{CX}(\vfinal)$ (line~\ref{line:main_decide_from_core}), and broadcast a \textsc{decide} message (line~\ref{line:main_send_decided_1}).
Thus, all correct processes receive $2t + 1$ \textsc{decide} messages (line~\ref{line:main_receive_decided_3}), and decide (line~\ref{line:main_name_decide}).

\iffalse
\smallskip
To prove that the bit complexity of \name is identical to the number of bits exchanged in (one instances of) \block, we define the view $\vmax$ as the greatest view that is entered by a correct process before GST.
Note that Result 2 implies $\vfinal = \vmax + 1$.

\smallskip
\noindent \textbf{Bit complexity:} \emph{The bit complexity of \name is $O\big( \mathit{bit}(\block) \big)$, where $\mathit{bit}(\block)$ is the number of bits exchanged in (one instance of) \block.}

\noindent The termination property of \name states that all correct processes decide by time $t_{\vfinal} + \Delta_{\mathit{total}} + 2\delta$, where (1) $t_{\vfinal}$ denotes the first time a correct process enters view $\vfinal$, and (2) $\Delta_{\mathit{total}}$ is a parameter of \block.
Recall that $\Delta_{\mathit{total}} > \Delta_\mathit{shift} = 2\delta$ (see \Cref{algorithm:block}).
Importantly, (1) the first time a correct process enters view $\vfinal + 1$ is $t_{\vfinal} + \Delta_{\mathit{total}}$ (due to the time completion property of $\mathcal{CX}(\vfinal)$), and (2) the first time a correct process enters a view greater than $\vfinal + 1$ is $> t_{\vfinal} + \Delta_{\mathit{total}} + 2\delta$ (due to the time completion property of $\mathcal{CX}(\vfinal + 1)$ and and the fact that $\Delta_{\mathit{total}} > 2\delta$).
Hence, during the time period $[\text{GST}, t_{\vfinal} + \Delta_{\mathit{total}} + 2\delta]$, no correct process enters any view greater than $\vfinal + 1 = \vmax + 2$.
As $\vmax \in O(1)$ ($\vmax$ does not depend on $n$), only a constant number of \block instances are executed by correct processes.
Therefore, the bit complexity of \name is indeed $O\big( \mathit{bit}(\block) \big)$.

\iffalse
\smallskip
A direct consequence of Result 2 is \name's strong validity.

 
As the first correct process that broadcasts a \textsc{decide} message does so upon deciding from $\mathcal{CX}(V)$, for some view $V$, then the external validity property of $\mathcal{CX}(V)$

\paragraph{Proof of correctness.}
We start proving the correctness of \name by focusing on its agreement property.
Concretely, we first prove that no two correct processes receive $\mathsf{decide}(\cdot)$ indications for different values from (potentially different) \block instances.

\begin{lemma} \label{lemma:agreement_from_core}
If a correct process $p_i$ receives a $\mathsf{decide}(\mathit{val}_i)$ indication from $\mathit{core}(v_i)$ and a correct process $p_j$ receives a $\mathsf{decide}(\mathit{val}_j)$ indication from $\mathit{core}(v_j \geq v_i)$, then $\mathit{val}_i = \mathit{val}_j$.
\end{lemma}
\begin{proof}
If $v_i = v_j$, the statement of the lemma holds due to the agreement property of $\mathit{core}(v_i = v_j)$.

Hence, let $v_i < v_j$.
In order to prove the statement of the lemma, we show that all correct process that propose to $\mathit{core}(v^*)$, for every viewv $v^* > v_i$, do so with value $\mathit{val}_i$.

\smallskip
\emph{Base step: All correct processes propose value $\mathit{val}_i$ to $\mathit{core}(v_i + 1)$.}
The statement holds because any correct process that validates a value from $\mathit{core}(v_i)$ does validate value $\mathit{val}_i$ (due to the agreement property of $\mathit{core}(v_i)$).

\smallskip
\emph{Induction step: Assuming that all correct processes propose value $\mathit{val}_i$ to $\mathit{core}(v^*)$, for some view $v^* > v_i$, we prove that all correct processes propose value $\mathit{val}_i$ to $\mathit{core}(v^* + 1)$.}
The statement holds as any correct process that validates a value from $\mathit{core}(v^*)$ does so with value $\mathit{val}_i$ (due to the strong validity property of $\mathit{core}(v^*)$.

\smallskip
Due to the aforementioned intermediate result, all correct processes that propose to $\mathit{core}(v_j)$ do so with value $\mathit{val}_i$.
Thus, the strong validity property of $\mathit{core}(v_j)$ proves that $\mathit{val}_i = \mathit{val}_j$.
\end{proof}

Next, we show that no two correct processes broadcast \textsc{decide} messages for different values.

\begin{lemma} \label{lemma:agreement_from_decide_messages}
If a correct process $p_i$ broadcasts a $\langle \textsc{decide}, \mathit{val}_i \rangle$ message and another correct process $p_j$ broadcasts a $\langle \textsc{decide}, \mathit{val}_j \rangle$, then $\mathit{val}_i = \mathit{val}_j$.
\end{lemma} 
\begin{proof}
The first correct process that broadcasts a \textsc{decide} message does so after receiving a $\mathsf{decide}(\cdot)$ indication from \block (line~\ref{line:decide_from_core}); let that \textsc{decide} message be for some value $\mathit{val}^*$.
We prove the lemma by induction.

\smallskip
\emph{Base step: The second correct process that broadcasts a \textsc{decide} message does so for value $\mathit{val}^*$.}
We analyze all possible places at which the second correct process $p_2$ could send a \textsc{decide} message:
\begin{compactitem}
    \item line~\ref{line:send_decided_1}: In this case, the message is for $\mathit{val}^*$ due to \Cref{lemma:agreement_from_core}.

    \item line~\ref{line:send_decided_2}: In this case, the message is for $\mathit{val}^*$ as $p_2$ has received the first \textsc{decide} message sent by a correct process.

    \item line~\ref{line:send_decided_3}: This case is impossible as there are no $t + 1 > 1$ correct processes that have previously broadcast a \textsc{decide} message.
\end{compactitem}

\smallskip
\emph{Induction step: Assuming that the first $x > 1$ correct processes that broadcast a \textsc{decide} message do so for value $\mathit{val}^*$, we prove that the $(x + 1)$-st correct process that broadcasts a \textsc{decide} message does so for value $\mathit{val}^*$.}
Again, we analyze all possible places at which the $(x + 1)$-st correct process $p_{x + 1}$ could send a \textsc{decide} message:
\begin{compactitem}
    \item line~\ref{line:send_decided_1}: In this case, the message is for $\mathit{val}^*$ due to \Cref{lemma:agreement_from_core}.

    \item line~\ref{line:send_decided_2}: The message is for $\mathit{val}^*$ as $p_{x + 1}$ has received a \textsc{decide} message previously sent by a correct process.

    \item line~\ref{line:send_decided_3}: Same as above.
\end{compactitem}
The induction step concludes the proof of the lemma.
\end{proof}

We ready to prove that \name satisfies agreement.

\begin{theorem} [Agreement]
\name satisfies agreement.
\end{theorem}
\begin{proof}
Prior to deciding, any correct process receives a \textsc{decide} message from a correct process (due to the rule at line~\ref{line:receive_decided_3}).
Therefore, the theorem follows directly from \Cref{lemma:agreement_from_decide_messages}.
\end{proof}

Next, we prove that \name satisfies strong validity.

\begin{theorem} [Strong validity]
\name satisfies strong validity.
\end{theorem}
\begin{proof}
Suppose that all correct processes propose the same value $\mathit{val}$ to \name.
Following the same induction as the one presented in the proof of \Cref{lemma:agreement_from_core}, we conclude that all correct processes that propose to $\mathit{core}(v)$, for every view $v$, do so with value $\mathit{val}$.
Hence, given that the first correct process to broadcast a \textsc{decide} message does so at line~\ref{line:send_decided_1}, that message is for value $\mathit{val}$ (ensured by the strong validity property of \block).
Moreover, \Cref{lemma:agreement_from_decide_messages} proves that all correct processes that broadcast \textsc{decide} messages do so for value $\mathit{val}$.
Thus, no correct process decides any value $\mathit{val}' \neq \mathit{val}$ from \name.
\end{proof}

The following theorem proves that \name satisfies external validity.

\begin{theorem} [External validity]
\name satisfies external validity.
\end{theorem}
\begin{proof}
As the first correct process that broadcasts a \textsc{decide} message does so at line~\ref{line:send_decided_1}, the external validity property of \block and \Cref{lemma:agreement_from_decide_messages} prove that all \textsc{decide} messages sent by correct processes are sent for valid values.
Hence, no correct process can decide an invalid value from \name.
\end{proof}

Lastly, we need to prove that \name satisfies termination.
To this end, we first prove that, if any correct process decides, then all correct processes eventually decide.

\begin{lemma} \label{lemma:termination_all_from_one}
If a correct process decides, then every correct process eventually decides.
\end{lemma}
\begin{proof}
Let a correct process $p_i$ decide some value $\mathit{val}$ (line~\ref{line:name_decide}).
Hence, $p_i$ has received $2t + 1$ $\langle \textsc{decide}, \mathit{val} \rangle$ messages (line~\ref{line:receive_decided_3}) out of which (at least) $t + 1$ are sent by correct processes.
Therefore, every correct process $p_j$ eventually broadcasts a \textsc{decide} message for $\mathit{val}$, which implies that every correct process eventually receives $2t + 1$ \textsc{decide} messages for $\mathit{val}$ and decides.
\end{proof}

The previous lemma shows that it is sufficient to prove that one correct process decides to show that \name satisfies termination.
Next, we prove that, if a correct process enters any view $v > 1$, then a correct process has previously entered view $v - 1$.

\begin{lemma} \label{lemma:previously_entered}
If  correct process enters any view $v > 1$, then view $v - 1$ has been previously entered by a correct process.
\end{lemma}
\begin{proof}
Let $p_i$ be any correct process that enters view $v > 1$ (line~\ref{line:enter_v}).
Hence, $p_i$ has received a $\langle \textsc{start-view}, v \rangle$ message from a correct process (line~\ref{line:receive_quorum}).
As the first correct process that broadcasts a $\langle \textsc{start-view}, v \rangle$ message does so at line~\ref{line:view_timer_expire}, a correct process has completed view $v - 1$ before $p_i$ enters $v$.
Due to the integrity property of $\mathit{core}(v - 1)$, that correct process has previously entered view $v - 1$, which proves the statement of the lemma.
\end{proof}

The previous lemma allows us to prove that, if no correct process decides, then every view is eventually entered by a correct process.

\begin{lemma} \label{lemma:every_view_entered}
If no correct process decides, then every view is eventually entered by a correct process.
\end{lemma}
\begin{proof}
By contradiction, let $v^* + 1 > 1$ be the smallest view not entered by a correct process.
Due to \Cref{lemma:previously_entered}, no view greater than $v^* + 1$ is ever entered by a correct process.
% In brief, every correct process eventually enters view $v^*$ (i.e., the greatest view entered by a correct process).
In brief, every correct process $p_i$ eventually (1) broadcasts a $\langle \textsc{start-view}, v^* \rangle$ message (line~\ref{line:send_complete_2}) upon receiving $t + 1$ $\langle \textsc{start-view}, v^* \rangle$ messages (line~\ref{line:receive_plurality}), (2) enters view $v^*$ (line~\ref{line:enter_v}) upon receiving $2t + 1$ $\langle \textsc{start-view}, v^* \rangle$ messages (line~\ref{line:receive_quorum}), (3) broadcasts a $\langle \textsc{start-view}, v^* + 1 \rangle$ (line~\ref{line:send_complete_1}) upon completing view $v^*$, and (4) enters view $v^* + 1$ (line~\ref{line:enter_v}) upon receiving $2t + 1$ $\langle \textsc{start-view}, v^* + 1 \rangle$ (line~\ref{line:receive_quorum}), resulting in a contradiction.
\end{proof}

For each view $v$, we denote by $t_v$ the time at which the first correct process enters view $v$.
We now define view $\vfinal$ as the smallest view such that no correct process enters $\vfinal$ before GST.

\begin{definition} [View $\vfinal$]
We denote by $\vfinal$ the smallest view such that $t_{\vfinal} \geq \text{GST}$.
\end{definition}

Note that $\vfinal$ is well defined if no correct process decides due to \Cref{lemma:every_view_entered}.
The following lemma proves that every correct process enters view $\vfinal$ by time $t_{\vfinal} + 2\delta$.

\begin{lemma}
Every correct process enters view $\vfinal$ by time $t_{\vfinal} + 2\delta$.
\end{lemma}
\begin{proof}

\end{proof}

\paragraph{Proof of complexity.}
To prove the complexity of \name, we first define view $\vmax$ as the greatest view such that the first correct process that enters view $\vmax$ does so before GST.

\begin{definition} [View $\vmax$]
We denote by $\vmax$ the greatest view such that $t_{\vmax} < \text{GST}$.
\end{definition}

The following lemma proves that $\vfinal = \vmax + 1$.
Observe that $\vfinal = \vmax + 1$ due to \Cref{lemma:previously_entered}.

The following lemma proves that no correct process ever enters any view greater than $\vfinal$.

\begin{lemma}
No correct process enters any view greater than $\vfinal + 1$.
\end{lemma}
\begin{proof}
Let $t_d$ denote the time at which the first correct process decides.
By \Cref{lemma:termination_all_from_one}, all correct processes decide by time $\max(t_d, \text{GST}) + 2\delta$.
Moreover, if no correct process decides by time $t_{\vfinal} + \Delta_{\mathit{end}}$, it is guaranteed that every correct process receives a $\mathsf{decide}(\cdot)$ indication from \block.





It is proven that every correct process receives a $\mathsf{decide}(\cdot)$ indicatio 
\end{proof}
\fi
\fi

\subsection{From Generic Transformation to Concrete Algorithms} \label{subsection:concrete_algorithms}

We conclude this section by presenting a few efficient signature-free partially synchronous Byzantine agreement algorithms that \name yields (see \Cref{table:concrete_algorithms}).
As $\mathit{bit}(\name) = O\big( n^2 + \mathit{bit}(\block) \big)$ for constant-sized values and $\mathit{bit}(\block) = \mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B}$, the bit complexity $\mathit{bit}(\name)$ of \name for constant-sized values can be defined as
\begin{equation*}
    \mathit{bit}(\name) = O\big( n^2 + \mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B} \big)\text{, where}
\end{equation*}
$\mathcal{B}$ denotes the maximum number of bits any correct process sends in the \block's underlying synchronous Byzantine agreement algorithm.
Similarly, the bit complexity $\mathit{bit}(\name)$ of \name for $L$-bit values can be defined as
\begin{equation*}
    \mathit{bit}(\name) = O\big( nL + n^2 \log n + \mathit{bit}(\mathcal{GC}_1) + \mathit{bit}(\mathcal{GC}_2) + \mathit{bit}(\mathcal{VB}) + n \cdot \mathcal{B} \big).
\end{equation*}
% (1) $\mathit{bit}(\mathcal{GC}_1^A)$ (resp., $\mathit{bit}(\mathcal{GC}_2^A)$) denotes the number of bits sent in a specific implementation $\mathcal{GC}_1^A$ (resp., $\mathcal{GC}_2^A$) of asynchronous graded consensus, (2) $\mathit{bit}(\mathcal{VB}^A)$ denotes the number of bits sent in a specific implementation $\mathcal{VB}^A$ of asynchronous validation broadcast, and (3) $\mathcal{B}$ denotes the maximum number of bits any correct process sends in a specific implementation $\mathcal{BA}^S$ of synchronous Byzantine agreement.
Therefore, \Cref{table:concrete_algorithms} specifies, for each \name-obtained Byzantine agreement algorithm, the concrete implementations of (1) asynchronous graded consensus ($\mathcal{GC}_1$ and $\mathcal{GC}_2$), (2) synchronous Byzantine agreement ($\mathcal{BA}^S$), and (3) validation broadcast ($\mathcal{VB}$) required to construct the algorithm.


\begin{table}[ht]
% \centering
\footnotesize
\tabcolsep=0.08cm
\begin{tabular}{|p{3.05cm}|p{1.3cm}|p{2.32cm}|p{3cm}|p{2.32cm}|p{1.7cm}|  }
 \hline
 \centering \textbf{Bit complexity of \\the final algorithm} &
\centering Resilience ($n$) & \centering $\mathcal{GC}_1 = \mathcal{GC}_2$ \\ total bits & \centering $\mathcal{BA}^S$ \\ $n$ $\cdot$ (bits per process)  & \centering $\mathcal{VB}$ \\ total bits & \centering Cryptography \tabularnewline
 \hline
 \hline

\centering $O(n^2)$ \\(with $L \in O(1)$)  & \centering $3t + 1$ & \centering \cite{AttiyaWelch23} \\ $O(n^2)$ & \centering \cite{berman1992bit,CoanW92} \\ $O(n^2)$ & \centering \Cref{subsection:validation_broadcast_basic_implementation} \\ $O(n^2)$ & \centering None \tabularnewline

 % \hline
 % \hline

%  \centering $O(nL + n^2\log n\kappa)$ \\ (only strong validity) & \centering $3t + 1$ & \centering \Cref{subsection:graded_consensus_bounded} \\ $O(nL + n^2\log(n)\kappa)$  & \centering \cite{chen2021optimal} \\ $O(nL + n^2\log(n))$ & \centering \Cref{subsection:validation_bcast_long_3_4} \\ $O(nL + n^2\log(n)\kappa)$ & \centering Hash \tabularnewline
%  \hline

%   \centering $O(n\log(n)L + n^2\log(n)\kappa)$ & \centering $3t + 1$ & \centering \Cref{subsection:graded_consensus_bounded} \\ $O(nL + n^2\log(n)\kappa)$  & \centering 
%   \cite{errorFreeValidated}
% %\Cref{section:external_validity_sync_consensus}
%   \\ $O(
%   n\log(n)L + n^2\log(n))$ & \centering \Cref{subsection:validation_bcast_long_3_4} \\ $O(nL + n^2\log(n)\kappa)$ & \centering Hash \tabularnewline
 
 \hline
  \centering $O(nL + n^2\kappa\log n)$ \\ (only strong validity) & \centering $3t + 1$ & \centering \Cref{subsection:graded_consensus_bounded} \\ $O(nL + n^2\kappa\log n)$  & \centering \cite{chen2021optimal} \\ $O(nL + n^2\log n)$ & \centering \Cref{subsection:validation_bcast_long_3_4} \\ $O(nL + n^2\kappa)$ & \centering Hash \tabularnewline
 \hline

 \centering $O(nL\log n + n^2\kappa\log n)$ & \centering $3t + 1$ & \centering \Cref{subsection:graded_consensus_bounded} \\ $O(nL + n^2\kappa\log n)$  & \centering \cite{errorFreeValidated}%\Cref{section:external_validity_sync_consensus} 
 \\ $O(
  nL\log n + n^2\log n)$ & \centering \Cref{subsection:validation_bcast_long_3_4} \\ $O(nL + n^2\kappa)$ & \centering Hash \tabularnewline
 \hline

   \centering $O(nL + n^2\log n)$ \\ (only strong validity) & \centering $5t + 1$ & \centering \Cref{subsection:its_graded_consensus} \\ $O(nL + n^2\log n)$  & \centering \cite{chen2021optimal} \\ $O(nL + n^2\log n)$ & \centering \Cref{subsection:its_validation_broadcast} \\ $O(nL + n^2\log n)$ & \centering None \tabularnewline
 \hline

 \centering $O(nL\log n + n^2\log n)$ & \centering $5t + 1$ & \centering \Cref{subsection:its_graded_consensus} \\ $O(nL + n^2\log n)$  & \centering \cite{errorFreeValidated}%\Cref{section:external_validity_sync_consensus} 
 \\ $O(
  nL\log n + n^2\log n)$ & \centering \Cref{subsection:its_validation_broadcast} \\ $O(nL + n^2\log n)$ & \centering None \tabularnewline
 \hline
\end{tabular}
    \caption{Concrete partially synchronous Byzantine agreement algorithms obtained by \name.
    We emphasize that rows 2 and 4 satisfy only strong validity (i.e., they do not satisfy external validity).
    \\($L$ denotes the bit-size of a value, whereas $\kappa$ denotes the bit-size of a hash value. We consider $\kappa \in \Omega(\log n)$)}
\label{table:concrete_algorithms}
\end{table}

==> sections/repetear_old.tex <==
\section{\name}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\textwidth]{figures/Repeater-2.eps}
    \caption{Core}
    \label{fig:repeater_core}
\end{figure}


\subsection{Building Blocks}

This subsection introduces two problem specifications on which \name relies: (1) graded consensus, and (2) synchronous unauthenticated Byzantine consensus.

\subsubsection{Graded consensus.}

Graded consensus exposes the following interface:
\begin{compactitem}
    \item \textbf{request} $\mathsf{input}(b \in \{0, 1\})$: a process inputs a bit $b$.

    \item \textbf{request} $\mathsf{abandon}()$: a process abandons graded consensus.

    \item \textbf{indication} $\mathsf{output}(b' \in \{0, 1\}, g \in \{0, 1\})$: a process outputs a bit $b'$ with a grade $\mathit{g}$.
\end{compactitem}
Every correct process inputs and abandons graded consensus at most once.
Note that it is not guaranteed that all correct processes input their value.
The following properties are ensured:
\begin{compactitem}
    \item \emph{Consistency:} If a correct process outputs $(b', 1)$, then no correct process outputs $(1 - b', *)$. 

    \item \emph{Validity:} If all correct processes that input their value input the same bit $b$, then no correct process outputs $(1 - b, *)$ or $(b, 0)$. 

    \item \emph{Termination:} If all correct processes input their value and no correct process abandons it, every correct process eventually outputs some bit (with some grade).
\end{compactitem}




Importantly, there exists a graded consensus algorithm \textsc{gc} such that:
\begin{compactitem}
    \item \textsc{gc} is asynchronous, and

    \item \textsc{gc} is safe against a computationally unbounded adversary that can corrupt up to $t$ processes, and

    \item every correct process sends $O(n)$ bits in any execution of \textsc{gc}.
\end{compactitem}

\begin{lemma}
Any asynchronous graded consensus additionally satisfies the following property:
\begin{compactitem}
    \item \emph{Safety:} If all correct processes that input a bit input the same bit $b$, then no correct process outputs $(1 - b, *)$ or $(b, 0)$.
\end{compactitem}
\end{lemma}
\begin{proof}
If all correct processes input a bit, then the lemma follows from the validity property of graded consensus.
Hence, suppose that there exists a finite execution $\mathcal{E}$ in which not all correct processes input a value and a correct process outputs $(1 - b, *)$ or $(b, 0)$.
We now devise an execution $\mathcal{E}'$ in which all correct processes propose to graded consensus, but validity is violated.

Start with $\mathcal{E}' \gets \mathcal{E}$.
In continuation of $\mathcal{E}'$, we make all correct processes propose $b$ to graded consensus.
Hence, $\mathcal{E}'$ is an execution in which (1) all correct processes propose, (2) they all propose the same bit $b$, and (3) a correct process outputs $(1 - b, *)$ or $(b, 0)$.
Thus, validity is violated in $\mathcal{E}'$, which concludes the proof.
\end{proof}

\subsection{Pseudocode of \name}

\pierre{One Question about a potential multi-value version. What if instead of line \ref{line:rcv_enough_echo_to_help} of \Cref{algorithm:repeater_view_core}, we wait for (*) $2t+1$ $\textsc{echo}$ messages ? If (**) $t+1$ of them share the same value, we help that value, and otherwise, we can validate any value (e.g. former proposal or majority value in (*)). Upon the reception of (***) $2t+1$ $\textsc{echo}$ messages for the same value, we validate this value. What's the point ? First, consensus is preserved. Indeed, eventually (*) will be met by every correct process. If (**), it means no correct process has decided by validity of (multivalue) graded consensus, so it's safe to validate any value. If the view is successful, every correct process outputs the same value from the (multivalue) graded consensus, and so this value $v$ will meet (*) and then (***) at each future view.

Second, the protocol is now multi-value, with the validity provided by the synchronous consensus protocol.}


\begin{algorithm}
\caption{View core: simplified pseudocode version 1 (for process $p_i$)}
\label{algorithm:repeater_view_core}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em AW graded consensus~\cite{AttiyaWelch23}, \textbf{instances} $\mathit{gc\_start}$ and $\mathit{gc\_end}$
\State \hskip2em Synchronous consensus, \textbf{instance} $\mathit{sync\_consensus}$ \BlueComment{the synchronous consensus algorithm to be translated to partial synchrony}

\medskip
\State \textbf{Parameters:}
\State \hskip2em $\mathsf{View}$ $\mathit{view}$ \BlueComment{each view core abstraction is associated with a view}

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Time}$ $\mathit{gc\_duration} = 11\delta$ \BlueComment{AW graded consensus algorithm takes $7\delta$ to decide}
\State \hskip2em $\mathsf{Time}$ $\mathit{step\_duration} = 5\delta$ \BlueComment{each communication step takes $5\delta$ time}
\State \hskip2em $\mathsf{Time}$ $\mathit{sync\_consensus\_steps} = \mathcal{T}$ \BlueComment{synchronous consensus takes $\mathcal{T}$ communication steps}
\State \hskip2em $\mathsf{Time}$ $\mathit{echo\_duration} = 6\delta$ \BlueComment{\textsc{echo} step requires $2\delta$ to terminate}

%\medskip
%\State \textbf{Local timer:}
%\State \hskip2em $\mathsf{Timer}$ $\mathit{T}_i $
% \State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_start\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{sync\_consensus\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_end\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{end\_timer}_i$

% \medskip
% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Bit}$ $\mathit{validated}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_start}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_start}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_sync\_consensus}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_end}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_end}_i \gets \bot$
% \State \hskip2em $\mathsf{Boolean}[2]$ $\mathit{echo} \gets \{\mathit{false}, \mathit{false} \}$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{end\_delivered}_i \gets \bot$
 
\medskip
\State \textbf{procedure} $\mathsf{start}(\mathsf{Bit} \text{ } \mathit{proposal})$:
% \State \hskip2em \textbf{wait for} some $\mathsf{Bit}$ $b$ to be validated \BlueComment{this is a blocking call for this specific instance of the view core abstraction}
% \State \hskip2em $\mathit{bit\_validated} \gets \mathit{proposal}$
%\State \hskip2em $\mathit{T}_i.\mathsf{start\_timer}(0)$
% \State \hskip2em \textbf{let} $\mathit{validated}_i \gets b$
% \State \hskip2em \textbf{invoke} $\mathit{gc\_start\_timer}_i.\mathsf{measure}(\mathit{gc\_duration})$
\State \hskip2em \textbf{run} $\mathit{gc\_start}.\mathsf{input}(\mathit{proposal})$ \BlueComment{the instruction ``run'' runs the command in parallel. Similar to ``||'' notation}

\State \hskip2em \textbf{wait for} $\mathit{gc\_duration}$ \textbf{time}
\medskip

\State \hskip2em $(\mathit{bit\_gc\_start}, \mathit{grade\_gc\_start}) \gets \mathit{gc\_start}.\mathsf{output}$
\State \hskip2em \textbf{run} $\mathit{sync\_consensus}.\mathsf{propose}(\mathit{bit\_gc\_start})$ \BlueComment{run $\mathit{sync\_duration}$ with round duration of $5\delta$} \label{line:propose_sync_consensus}

\State \hskip2em \textbf{wait for} $\mathit{sync\_consensus\_step} \cdot \mathit{step\_duration}$  \textbf{time}
\medskip

\State \hskip2em $\mathit{bit\_sync\_consensus} \gets \mathit{sync\_consensus}.\mathsf{output}$  \BlueComment{The default is $\bot$ if there is still no decision}
\State \hskip2em \textbf{if} $\mathit{grade\_gc\_start} = 1$:
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_gc\_start})$ \label{line:gc_end_input_1}
\State \hskip2em \textbf{else if} $\mathit{bit\_sync\_consensus}_i \neq \bot$:
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_sync\_consensus}_i)$ \label{line:gc_end_input_2}
\State \hskip2em \textbf{else:}
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_validated})$ \label{line:gc_end_input_3}

\State \hskip2em \textbf{wait for} $\mathit{gc\_duration}$ \textbf{time}
\medskip
\State \hskip2em $(\mathit{bit\_gc\_end}, \mathit{grade\_gc\_end}) \gets \mathit{gc\_end}.\mathsf{output}$

\State \hskip2em \textbf{if} $\mathit{grade\_gc\_end}_i = 1$: \label{line:gc_end_grade_1}
\State \hskip4em $\textbf{decide}~\mathit{bit\_gc\_end}$ \label{line:decide}
\State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, \mathit{bit\_gc\_end}_i \rangle$ \label{line:bcast_echo_first}
\State \hskip2em $\mathit{echo\_value}[\mathit{bit\_gc\_end}] \gets \mathit{true}$

\State \hskip2em \textbf{run loop} $\mathit{echo}()$
\State \hskip2em \textbf{wait for} $\mathit{echo\_duration}$ \textbf{time}
\medskip
\State \hskip2em \textbf{wait for} $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $2t + 1$ processes. \label{line:rcv_enough_echo_to_leave}

\medskip

\State \textbf{procedure} $\mathsf{echo}()$:
\State \hskip2em \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $t + 1$ processes and $\mathit{echo\_value}[b] = \mathit{false}$: \label{line:rcv_enough_echo_to_help}
\State \hskip4em \textbf{broadcast} $\langle \textsc{echo}, b \rangle$ \label{line:bcast_echo_second}
\State \hskip4em $\mathit{echo\_value}[b] \gets \mathit{true}$

\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{View core: simplified pseudocode version 2 (for process $p_i$)}
\label{algorithm:repeater_view_core}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em AW graded consensus~\cite{AttiyaWelch23}, \textbf{instances} $\mathit{gc\_start}$ and $\mathit{gc\_end}$
\State \hskip2em Synchronous consensus, \textbf{instance} $\mathit{sync\_consensus}$ \BlueComment{the synchronous consensus algorithm to be translated to partial synchrony}

\medskip
\State \textbf{Parameters:}
\State \hskip2em $\mathsf{View}$ $\mathit{view}$ \BlueComment{each view core abstraction is associated with a view}

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Time}$ $\mathit{gc\_duration} = 11\delta$ \BlueComment{AW graded consensus algorithm takes $7\delta$ to decide}
\State \hskip2em $\mathsf{Time}$ $\mathit{step\_duration} = 5\delta$ \BlueComment{each communication step takes $5\delta$ time}
\State \hskip2em $\mathsf{Time}$ $\mathit{sync\_consensus\_steps} = \mathcal{T}$ \BlueComment{synchronous consensus takes $\mathcal{T}$ communication steps}
\State \hskip2em $\mathsf{Time}$ $\mathit{echo\_duration} = 6\delta$ \BlueComment{\textsc{echo} step requires $2\delta$ to terminate}
%\State \hskip2em $\mathsf{Time}$ $\mathit{view\_duration} = 2 \cdot \mathit{gc\_duration} + \mathit{sync\_consensus\_step} \cdot \mathit{step\_duration} + \mathit{echo\_duration}$ \BlueComment{minimum duration of each view} \label{line:init_view_duration}

\medskip
\State \textbf{Local timer:}
\State \hskip2em $\mathsf{Timer}$ $\mathit{T}_i $
% \State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_start\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{sync\_consensus\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_end\_timer}_i$
% \State \hskip2em $\mathsf{Timer}$ $\mathit{end\_timer}_i$

% \medskip
% \State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Bit}$ $\mathit{validated}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_start}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_start}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_sync\_consensus}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_end}_i \gets \bot$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_end}_i \gets \bot$
% \State \hskip2em $\mathsf{Boolean}[2]$ $\mathit{echo} \gets \{\mathit{false}, \mathit{false} \}$
% \State \hskip2em $\mathsf{Bit}$ $\mathit{end\_delivered}_i \gets \bot$
 
\medskip
\State \textbf{procedure} $\mathsf{start}(\mathsf{Bit} \text{ } \mathit{proposal})$:
\State \hskip2em \textbf{wait for} some $\mathsf{Bit}$ $b$ to be validated \BlueComment{this is a blocking call for this specific instance of the view core abstraction}
\State \hskip2em $\mathit{bit\_validated} \gets b$
\State \hskip2em $\mathit{T}_i.\mathsf{start\_timer}(0)$
%\State \hskip2em $\mathit{T}_i.\mathsf{start\_timer}(0)$
% \State \hskip2em \textbf{let} $\mathit{validated}_i \gets b$
% \State \hskip2em \textbf{invoke} $\mathit{gc\_start\_timer}_i.\mathsf{measure}(\mathit{gc\_duration})$
\State \hskip2em \textbf{run} $\mathit{gc\_start}.\mathsf{input}(b)$ \BlueComment{the instruction ``run'' runs the command in parallel. Similar to ``||'' notation}

\medskip
\State \hskip2em \textbf{wait for} $\mathit{T}_i \geq \mathit{gc\_duration}$
\medskip

\State \hskip2em $(\mathit{bit\_gc\_start}, \mathit{grade\_gc\_start}) \gets \mathit{gc\_start}.\mathsf{output}$
\State \hskip2em \textbf{run} $\mathit{sync\_consensus}.\mathsf{propose}(\mathit{bit\_gc\_start})$ \BlueComment{run $\mathit{sync\_duration}$ with round duration of $5\delta$} \label{line:propose_sync_consensus}

\medskip
\State \hskip2em \textbf{wait for} $\mathit{T}_i \geq \mathit{gc\_duration} + \mathit{sync\_consensus\_step} \cdot \mathit{step\_duration}$
\medskip

\State \hskip2em $\mathit{bit\_sync\_consensus} \gets \mathit{sync\_consensus}.\mathsf{output}$  \BlueComment{The default is $\bot$ if there is still no decision}
\State \hskip2em \textbf{if} $\mathit{grade\_gc\_start} = 1$:
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_gc\_start})$ \label{line:gc_end_input_1}
\State \hskip2em \textbf{else if} $\mathit{bit\_sync\_consensus}_i \neq \bot$:
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_sync\_consensus}_i)$ \label{line:gc_end_input_2}
\State \hskip2em \textbf{else:}
\State \hskip4em \textbf{run} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_validated})$ \label{line:gc_end_input_3}

\medskip
\State \hskip2em \textbf{wait for} $\mathit{T}_i \geq 2\cdot\mathit{gc\_duration} + \mathit{sync\_consensus\_step} \cdot \mathit{step\_duration}$
\medskip

\State \hskip2em $(\mathit{bit\_gc\_end}, \mathit{grade\_gc\_end}) \gets \mathit{gc\_end}.\mathsf{output}$

\State \hskip2em \textbf{if} $\mathit{grade\_gc\_end}_i = 1$: \label{line:gc_end_grade_1}
\State \hskip4em $\textbf{decide}~\mathit{bit\_gc\_end}$ \label{line:decide}
\State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, \mathit{bit\_gc\_end}_i \rangle$ \label{line:bcast_echo_first}
\State \hskip2em $\mathit{echo\_value}[\mathit{bit\_gc\_end}] \gets \mathit{true}$
\State \hskip2em \textbf{run loop} $\mathit{echo}()$

\medskip
\State \hskip2em \textbf{wait for} $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $2t + 1$ processes. \label{line:rcv_enough_echo_to_leave}
\State \hskip2em \textbf{wait for} $\mathit{T}_i \geq 2\cdot\mathit{gc\_duration} + \mathit{sync\_consensus\_step} \cdot \mathit{step\_duration} + \mathit{echo\_duration}$
\medskip

\State \textbf{procedure} $\mathsf{echo}()$:
\State \hskip2em \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $t + 1$ processes and $\mathit{echo\_value}[b] = \mathit{false}$: \label{line:rcv_enough_echo_to_help}
\State \hskip4em \textbf{broadcast} $\langle \textsc{echo}, b \rangle$ \label{line:bcast_echo_second}
\State \hskip4em $\mathit{echo\_value}[b] \gets \mathit{true}$

% \medskip
% \State \textbf{upon} $\mathsf{stop()}$:
% \State \hskip2em \textbf{invoke} $\mathit{gc\_start}.\mathsf{abandon()}$ if $\mathit{gc\_start}.\mathsf{propose}(\cdot)$ has previously been invoked
% \State \hskip2em \textbf{invoke} $\mathit{gc\_end}.\mathsf{abandon()}$ if $\mathit{gc\_end}.\mathsf{propose}(\cdot)$ has previously been invoked
% \State \hskip2em \textbf{stop participating} in $\mathcal{VC}(\mathit{view})$:

% \medskip
% \State \textbf{upon} $\mathit{gc\_start}.\mathsf{output}(\mathsf{Bit} \text{ } b, \mathsf{Bit} \text{ } g)$:
% \State \hskip2em $\mathit{bit\_gc\_start}_i \gets b$
% \State \hskip2em $\mathit{grade\_gc\_start} \gets g$

% \medskip
% \State \textbf{upon} $\mathit{gc\_start\_timer}_i$ expires and $\mathit{bit\_gc\_start}_i \neq \bot$ for the first time:
% \State \hskip2em \textbf{invoke} $\mathit{sync\_consensus\_timer}_i.\mathsf{measure}(\mathit{sync\_consensus\_steps} \cdot \mathit{step\_duration})$ \label{line:measure_sync_consensus_timer}
% \State \hskip2em \textbf{invoke} $\mathit{sync\_consensus}.\mathsf{propose}(\mathit{bit\_gc\_start}_i)$ \BlueComment{run $\mathit{sync\_duration}$ with round duration of $5\delta$} \label{line:propose_sync_consensus}

% \medskip
% \State \textbf{upon} $\mathit{sync\_consensus}.\mathsf{decide}(\mathsf{Bit} \text{ } b)$:
% \State \hskip2em $\mathit{bit\_sync\_consensus}_i \gets b$

% \medskip
% \State \textbf{upon} $\mathit{sync\_consensus\_timer}_i$ expires for the first time: \label{line:sync_consensus_timer_expire}
% \State \hskip2em \textbf{stop participating} in $\mathit{sync\_consensus}$  \BlueComment{$p_i$ does not decide from $\mathit{sync\_consensus}$ after this line has been executed} \label{line:sync_consensus_stop_participating}
% \State \hskip2em $\mathit{gc\_end\_timer}_i.\mathsf{measure}(\mathit{gc\_duration})$
% \State \hskip2em \textbf{if} $\mathit{grade\_gc\_start}_i = 1$:
% \State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_gc\_start}_i)$ \label{line:gc_end_input_1}
% \State \hskip2em \textbf{else if} $\mathit{bit\_sync\_consensus}_i \neq \bot$:
% \State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_sync\_consensus}_i)$ \label{line:gc_end_input_2}
% \State \hskip2em \textbf{else:}
% \State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{validated}_i)$ \label{line:gc_end_input_3}

% \medskip
% \State \textbf{upon} $\mathit{gc\_end}.\mathsf{output}(\mathsf{Bit} \text{ } b, \mathsf{Bit} \text{ } g)$:
% \State \hskip2em $\mathit{bit\_gc\_end}_i \gets b$
% \State \hskip2em $\mathit{grade\_gc\_end}_i \gets g$

% \medskip
% \State \textbf{upon} $\mathit{gc\_end\_timer}_i$ expires and $\mathit{bit\_gc\_end}_i \neq \bot$ for the first time:
% \State \hskip2em \textbf{if} $\mathit{grade\_gc\_end}_i = 1$: \label{line:gc_end_grade_1}
% \State \hskip4em \textbf{trigger} $\mathsf{decide}(\mathit{bit\_gc\_end}_i)$ \label{line:decide}
% \State \hskip2em \textbf{invoke} $\mathit{end\_timer}_i.\mathsf{measure}(\mathit{echo\_duration})$
% \State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, \mathit{bit\_gc\_end}_i \rangle$ \label{line:bcast_echo_first}
% \State \hskip2em $\mathit{echo}[\mathit{bit\_gc\_end}_i] \gets \mathit{true}$

% \medskip
% \State \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $t + 1$ processes and $\mathit{echo}[b] = \mathit{false}$: \label{line:rcv_enough_echo_to_help}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, b \rangle$ \label{line:bcast_echo_second}
% \State \hskip2em $\mathit{echo}[b] \gets \mathit{true}$

% \medskip
% \State \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $2t + 1$ processes: \label{line:rcv_enough_echo_to_leave}
% \State \hskip2em $\mathit{end\_delivered}_i \gets b$

% \medskip
% \State \textbf{upon} $\mathit{end\_timer}_i$ expires and $\mathit{end\_delivered}_i \neq \bot$ for the first time:
% \State \hskip2em \textbf{trigger} $\mathsf{finished}()$ \label{line:leave}
\end{algorithmic}
\end{algorithm}



\begin{algorithm}
\caption{View core: Pseudocode (for process $p_i$)}
\label{algorithm:repeater_view_core}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em AW graded consensus~\cite{AttiyaWelch23}, \textbf{instances} $\mathit{gc\_start}$ and $\mathit{gc\_end}$
\State \hskip2em Synchronous consensus, \textbf{instance} $\mathit{sync\_consensus}$ \BlueComment{the synchronous consensus algorithm to be translated to partial synchrony}

\medskip
\State \textbf{Parameters:}
\State \hskip2em $\mathsf{View}$ $\mathit{view}$ \BlueComment{each view core abstraction is associated with a view}

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathsf{Time}$ $\mathit{gc\_duration} = 11\delta$ \BlueComment{AW graded consensus algorithm takes $7\delta$ to decide}
\State \hskip2em $\mathsf{Time}$ $\mathit{step\_duration} = 5\delta$ \BlueComment{each communication step takes $5\delta$ time}
\State \hskip2em $\mathsf{Time}$ $\mathit{sync\_consensus\_steps} = \mathcal{T}$ \BlueComment{synchronous consensus takes $\mathcal{T}$ communication steps}
\State \hskip2em $\mathsf{Time}$ $\mathit{echo\_duration} = 6\delta$ \BlueComment{\textsc{echo} step requires $2\delta$ to terminate}
\State \hskip2em $\mathsf{Time}$ $\mathit{view\_duration} = 2 \cdot \mathit{gc\_duration} + \mathit{sync\_consensus\_step} \cdot \mathit{step\_duration} + \mathit{echo\_duration}$ \BlueComment{minimum duration of each view} \label{line:init_view_duration}

\medskip
\State \textbf{Local timers:}
\State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_start\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{sync\_consensus\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{gc\_end\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{end\_timer}_i$

\medskip
\State \textbf{Local variables:}
\State \hskip2em $\mathsf{Bit}$ $\mathit{validated}_i \gets \bot$
\State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_start}_i \gets \bot$
\State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_start}_i \gets \bot$
\State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_sync\_consensus}_i \gets \bot$
\State \hskip2em $\mathsf{Bit}$ $\mathit{bit\_gc\_end}_i \gets \bot$
\State \hskip2em $\mathsf{Bit}$ $\mathit{grade\_gc\_end}_i \gets \bot$
\State \hskip2em $\mathsf{Boolean}[2]$ $\mathit{echo} \gets \{\mathit{false}, \mathit{false} \}$
\State \hskip2em $\mathsf{Bit}$ $\mathit{end\_delivered}_i \gets \bot$
 
\medskip
\State \textbf{upon} $\mathsf{start}(\mathsf{Bit} \text{ } \mathit{proposal})$:
\State \hskip2em \textbf{wait for} some $\mathsf{Bit}$ $b$ to be validated \BlueComment{this is a blocking call for this specific instance of the view core abstraction}
\State \hskip2em $\mathit{validated}_i \gets b$
\State \hskip2em \textbf{invoke} $\mathit{gc\_start\_timer}_i.\mathsf{measure}(\mathit{gc\_duration})$
\State \hskip2em \textbf{invoke} $\mathit{gc\_start}.\mathsf{input}(b)$

\medskip
\State \textbf{upon} $\mathsf{stop()}$:
\State \hskip2em \textbf{invoke} $\mathit{gc\_start}.\mathsf{abandon()}$ if $\mathit{gc\_start}.\mathsf{propose}(\cdot)$ has previously been invoked
\State \hskip2em \textbf{invoke} $\mathit{gc\_end}.\mathsf{abandon()}$ if $\mathit{gc\_end}.\mathsf{propose}(\cdot)$ has previously been invoked
\State \hskip2em \textbf{stop participating} in $\mathcal{VC}(\mathit{view})$:

\medskip
\State \textbf{upon} $\mathit{gc\_start}.\mathsf{output}(\mathsf{Bit} \text{ } b, \mathsf{Bit} \text{ } g)$:
\State \hskip2em $\mathit{bit\_gc\_start}_i \gets b$
\State \hskip2em $\mathit{grade\_gc\_start} \gets g$

\medskip
\State \textbf{upon} $\mathit{gc\_start\_timer}_i$ has expired and $\mathit{bit\_gc\_start}_i \neq \bot$ for the first time:
\State \hskip2em \textbf{invoke} $\mathit{sync\_consensus\_timer}_i.\mathsf{measure}(\mathit{sync\_consensus\_steps} \cdot \mathit{step\_duration})$ \label{line:measure_sync_consensus_timer}
\State \hskip2em \textbf{invoke} $\mathit{sync\_consensus}.\mathsf{propose}(\mathit{bit\_gc\_start}_i)$ \BlueComment{run $\mathit{sync\_duration}$ with round duration of $5\delta$} \label{line:propose_sync_consensus}

\medskip
\State \textbf{upon} $\mathit{sync\_consensus}.\mathsf{decide}(\mathsf{Bit} \text{ } b)$:
\State \hskip2em $\mathit{bit\_sync\_consensus}_i \gets b$

\medskip
\State \textbf{upon} $\mathit{sync\_consensus\_timer}_i$ expires: \label{line:sync_consensus_timer_expire}
\State \hskip2em \textbf{stop participating} in $\mathit{sync\_consensus}$  \BlueComment{$p_i$ does not decide from $\mathit{sync\_consensus}$ after this line has been executed} \label{line:sync_consensus_stop_participating}
\State \hskip2em $\mathit{gc\_end\_timer}_i.\mathsf{measure}(\mathit{gc\_duration})$
\State \hskip2em \textbf{if} $\mathit{grade\_gc\_start}_i = 1$:
\State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_gc\_start}_i)$ \label{line:gc_end_input_1}
\State \hskip2em \textbf{else if} $\mathit{bit\_sync\_consensus}_i \neq \bot$:
\State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{bit\_sync\_consensus}_i)$ \label{line:gc_end_input_2}
\State \hskip2em \textbf{else:}
\State \hskip4em \textbf{invoke} $\mathit{gc\_end}.\mathsf{input}(\mathit{validated}_i)$ \label{line:gc_end_input_3}

\medskip
\State \textbf{upon} $\mathit{gc\_end}.\mathsf{output}(\mathsf{Bit} \text{ } b, \mathsf{Bit} \text{ } g)$:
\State \hskip2em $\mathit{bit\_gc\_end}_i \gets b$
\State \hskip2em $\mathit{grade\_gc\_end}_i \gets g$

\medskip
\State \textbf{upon} $\mathit{gc\_end\_timer}_i$ has expired and $\mathit{bit\_gc\_end}_i \neq \bot$ for the first time:
\State \hskip2em \textbf{if} $\mathit{grade\_gc\_end}_i = 1$: \label{line:gc_end_grade_1}
\State \hskip4em \textbf{trigger} $\mathsf{decide}(\mathit{bit\_gc\_end}_i)$ \label{line:decide}
\State \hskip2em \textbf{invoke} $\mathit{end\_timer}_i.\mathsf{measure}(\mathit{echo\_duration})$
\State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, \mathit{bit\_gc\_end}_i \rangle$ \label{line:bcast_echo_first}
\State \hskip2em $\mathit{echo}[\mathit{bit\_gc\_end}_i] \gets \mathit{true}$

\medskip
\State \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $t + 1$ processes and $\mathit{echo}[b] = \mathit{false}$: \label{line:rcv_enough_echo_to_help}
\State \hskip2em \textbf{broadcast} $\langle \textsc{echo}, b \rangle$ \label{line:bcast_echo_second}
\State \hskip2em $\mathit{echo}[b] \gets \mathit{true}$

\medskip
\State \textbf{upon} exists $\mathsf{Bit}$ $b$ such that $\langle \textsc{echo}, b \rangle$ is received from $2t + 1$ processes: \label{line:rcv_enough_echo_to_leave}
\State \hskip2em $\mathit{end\_delivered}_i \gets b$

\medskip
\State \textbf{upon} $\mathit{end\_timer}_i$ has expired and $\mathit{end\_delivered}_i \neq \bot$ for the first time:
\State \hskip2em \textbf{trigger} $\mathsf{finished}()$ \label{line:leave}
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{\name: Pseudocode (for process $p_i$)}
\label{algorithm:view_synchronization}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Local timers:}
% \State \hskip2em $\mathsf{Timer}$ $\mathit{view\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{help\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{enter\_timer}_i$

\medskip
\State \textbf{Local variables:}
\State \hskip2em $\mathsf{Bit}$ $\mathit{proposal}_i \gets \bot$
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ \label{line:init_view}
\State \hskip2em $\mathsf{View}$ $\mathit{last\_entered}_i \gets 1$
\State \hskip2em $\mathsf{View}$ $\mathit{help\_view}_i \gets 1$ \label{line:init_help_view}

\medskip
\State \textbf{upon} $\mathsf{propose}(\mathsf{Bit} \text{ } \mathit{proposal})$:
\State \hskip2em $\mathit{proposal}_i \gets \mathit{proposal}$
\State \hskip2em \textbf{invoke} $\mathcal{VC}(1).\mathsf{start}(\mathit{proposal}_i)$ \BlueComment{start the view core abstraction associated with view $1$} \label{line:enter_1}

\medskip
\State \textbf{upon} $\mathcal{VC}(\mathit{view}_i).\mathsf{finished}()$: \label{line:view_timer_expire}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i + 1 \rangle$ \label{line:send_complete_1}

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v$ such that (1) $v > \mathit{view}_i$, and (2) $\langle \textsc{start-view}, v \rangle$ is received from $t + 1$ processes: \label{line:receive_plurality}
\State \hskip2em \textbf{if} $v > \mathit{help\_view}_i$: \label{line:check_help}
\State \hskip4em $\mathit{help\_view}_i \gets v$ \label{line:update_help_view}
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{cancel}()$ \label{line:cancel_help}
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_help}

\medskip
\State \textbf{upon} $\mathit{help\_timer}_i$ \textbf{expires}: \label{line:help_timer_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i \rangle$ \label{line:send_complete_2}
\State \hskip2em \textbf{if} $\mathit{help\_view}_i > 2$: \label{line:check_help_2}
\State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ \label{line:send_complete_2_prime} 
% \State \hskip2em \textbf{if} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ is received from $t + 1$ processes:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ 

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v > \mathit{view}_i$ such that $\langle \textsc{start-view}, v \rangle$ is received from $2t + 1$ processes: \label{line:receive_quorum}
\State \hskip2em $\mathit{view}_i \gets v$ \label{line:update_view_2}
% \State \hskip2em \sout{$\mathit{view\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_view}}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_enter}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_enter}

\medskip
\State \textbf{upon} $\mathit{enter\_timer}_i$ \textbf{expires:} \label{line:enter_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i \rangle$ \label{line:send_complete_3}
\State \hskip2em \textbf{if} $\mathit{view}_i > 2$: \label{line:check_view}
\State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i - 1 \rangle$ \label{line:send_complete_3_prime}
\State \hskip2em \textbf{invoke} $\mathcal{VC}(\mathit{last\_entered}_i).\mathsf{stop}()$ \BlueComment{stop participating in the current view core abstraction} \label{line:leave_v}
\State \hskip2em \textbf{invoke} $\mathcal{VC}(\mathit{view}_i).\mathsf{start}(\mathit{proposal}_i)$ \BlueComment{start the view core abstraction associated with view $\mathit{view}_i$}  \label{line:enter_v}
\State \hskip2em $\mathit{last\_entered}_i \gets \mathit{view}_i$
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{\name's coordination: Pseudocode (for process $p_i$)}
% \label{algorithm:view_synchronization}
% \footnotesize
% \begin{algorithmic} [1] 
% \State \textbf{Variables:}
% \State \hskip2em $\mathsf{Bit}$ $\mathit{proposal}_i \gets \bot$

% \State \textbf{upon} $\mathsf{propose}(\mathsf{Bit} \text{ } b)$:
% \State \hskip2em $\mathit{proposal}_i \gets b$
% \State \hskip2em \textbf{invoke} $\mathsf{init}$ on view synchronization

% \State \textbf{upon} $\mathsf{enter}(\mathsf{View} \text{ } v)$:
% \State \hskip2em stop the current view core
% \State \hskip2em start view core $v$

% \State \textbf{upon} $\mathsf{leave}$ from view core:
% \State \hskip2em \textbf{invoke} $\mathsf{wish\_to\_advance()}$ on view synchronization

% \end{algorithmic}
% \end{algorithm}
\iffalse
\subsection{Proof of Correctness \& Complexity}

In this subsection, we present proof of \textsc{catch-up}'s correctness and complexity.

\begin{lemma} \label{lemma:started_before}
If a correct process enters a view $v > 1$, then (at least) one correct process has previously entered view $v - 1$.
\end{lemma}
\begin{proof}
Let a correct process $p_i$ enter $v > 1$ (line~\ref{line:enter_v}).
Let $p_v$ be the first correct process which sends the $m = \langle \textsc{start-view}, v \rangle$ message.
Importantly, $p_v$ sends $m$ at line~\ref{line:send_complete_1}; if $p_v$ sends $m$ at line~\ref{line:send_complete_2} or at line~\ref{line:send_complete_3}, then $p_v$ would not be the first correct process which sends $\langle \textsc{start-view}, v \rangle$ (line~\ref{line:receive_plurality}).

Process $p_i$ has received $\langle \textsc{start-view}, v \rangle$ message from $2t + 1$ processes (line~\ref{line:receive_quorum}), out of which (at least) $t + 1$ processes are correct.
Therefore, before $p_i$ enters $v$, $p_v$ sends the message $m$ at line~\ref{line:send_complete_1}.
Hence, $p_v$ indeed enters $v - 1$ before $p_i$ enters $v$.
\end{proof}

\begin{lemma}
Every view $v$ is eventually entered by a correct process.
\end{lemma}
\begin{proof}
By contradiction, suppose that the greatest view entered by a correct process is $v^*$; let $p^*$ be any correct process that enters $v^*$.
Note that $v^* > 1$ as every process enters the first view as soon as it starts executing \textsc{catch-up} (line~\ref{line:enter_1}).
As $p^*$ enters $v^* > 1$ (line~\ref{line:enter_v}), $p^*$ receives $\langle \textsc{start-view}, v^* \rangle$ from $2t + 1$ processes (line~\ref{line:receive_quorum}).
Therefore, each correct process eventually receives $t + 1$ $\langle \textsc{start-view}, v^* \rangle$ messages (line~\ref{line:receive_plurality}), which means that each correct process eventually broadcasts $\langle \textsc{start-view}, v^* \rangle$ (line~\ref{line:send_complete_2}).
Hence, every correct process eventually enters $v^*$ (line~\ref{line:receive_quorum}).

Eventually, for each correct process $p_i$, $\mathit{view\_timer}_i$ expires (line~\ref{line:view_timer_expire}).
Thus, every correct process eventually broadcasts $\langle \textsc{start-view}, v^* + 1 \rangle$, which implies that every correct process eventually receives $\langle \textsc{start-view}, v^* + 1 \rangle$ from $2t + 1$ correct processes (line~\ref{line:receive_quorum}), and enters $v^* + 1$ (line~\ref{line:enter_v}).
Therefore, $v^*$ is not the greatest view entered by a correct process, which proves the lemma.
\end{proof}

\begin{definition} [View $v_{\mathit{max}}$]
We denote by $v_{\mathit{max}}$ the greatest view entered by a correct process before GST; if such a view does not exist, $v_{\mathit{max}} = 0$.
\end{definition}

\begin{definition} [View $v_{\mathit{final}}$]
We denote by $v_{\mathit{final}}$ the smallest view first entered by a correct process after GST.
\end{definition}

\begin{lemma}
$v_{\mathit{final}} = v_{\mathit{max}} + 1$.
\end{lemma}
\begin{proof}
Follows directly from \Cref{lemma:started_before}.
\end{proof}

We denote by $t_v$ the first time a correct process enters the view $v$.

\begin{lemma} \label{lemma:view_duration}
For any view $v \geq v_{\mathit{final}}$, no correct process sends $\langle \textsc{view-complete}, v \rangle$ before time $t_v + \mathit{view\_duration}$.
\end{lemma}
\begin{proof}
As $v \geq v_{\mathit{final}}$, $t_v \geq \text{GST}$.
As local clocks do not drift after GST, the first time a correct process sends $\langle \textsc{view-complete}, v \rangle$ cannot be before $t_v + \mathit{view\_duration}$.
\end{proof}

\begin{lemma} \label{lemma:enter_final}
Every correct process enters $v_{\mathit{final}}$ by time $t_{v_{\mathit{final}}} + 4\delta$.
\end{lemma}
\begin{proof}
The first correct process $p$ enters $v_{\mathit{final}}$ at time $t_{v_{\mathit{final}}}$.
Importantly, by \Cref{lemma:view_duration}, no correct process $p_i$ updates its $\mathit{view}_i$ variable to $> v_{\mathit{final}}$ before time $t_{v_{\mathit{final}}} + \mathit{view\_duration}$.

By time $t_{v_{\mathit{final}}} + \delta$, every correct process $p_i$ that has not previously sent $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ receives $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ from $t + 1$ processes; as $t_{v_{\mathit{final}}} + \mathit{view\_duration} > t_{v_{\mathit{final}}} + \delta$, $\mathit{view}_i \leq v_{\mathit{final}}$ at process $p_i$.
Now, we separate two scenarios: 
\begin{compactitem}
    \item Let $\mathit{view}_i = v_{\mathit{final}}$.
    In this case, $p_i$ sent $\langle \textsc{start-view},  v_{\mathit{final}} \rangle$ (line~\ref{line:send_complete_3}).

    \item Otherwise, $p_i$ sends $\langle \textsc{start-view},  v_{\mathit{final}} \rangle$ by time $t_{v_{\mathit{final}}} + 2\delta$. (line~\ref{line:send_complete_2}).
\end{compactitem}
Hence, by time $t_{v_{\mathit{final}}} + 2\delta$, every correct process sends $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$.
Thus, by time $t_{v_{\mathit{final}}} + 4\delta$, all correct processes enter $v_{\mathit{final}}$; recall that $t_{v_{\mathit{final}}} + \mathit{view\_duration} > t_{v_{\mathit{final}}} + 4\delta$.
\end{proof}

\begin{lemma}
Correct processes overlap for (at least) $\Delta$ time in $v_{\mathit{final}}$.
\end{lemma}
\begin{proof}
Follows directly from \Cref{lemma:enter_final} and the fact that $\mathit{view\_duration} = \Delta + 6\delta$.
\end{proof}

\begin{lemma}
By time $\text{GST} + 6\delta$, every correct process enters $v_{\mathit{max}}$ or $v_{\mathit{final}}$.
\end{lemma}
\begin{proof}
To prove the lemma, we prove that every correct process broadcasts $\langle \textsc{start-view}, v_{\mathit{max}} \rangle$ or $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ by time $\text{GST} + 3\delta$.
Consider any process $p_i$ that does not satisfy the aforementioned claim.
By time $\text{GST} + \delta$, $p_i$ receives $t + 1$ $\langle 
\textsc{start-view}, v_{\mathit{max}} \rangle$ messages (line~\ref{line:receive_plurality}).
We consider the following cases:
\begin{compactitem}
    \item Let the check at line~\ref{line:receive_plurality} activates.
    We further distinguish two cases:
    \begin{compactitem}
        \item Let the check at line~\ref{line:check_help} pass.
        In this case, $\mathit{help\_view}_i \gets v_{\mathit{max}}$ by time $\text{GST} + \delta$.
        Therefore, $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.

        \item Otherwise, $\mathit{help\_view}_i \in \{v_{\mathit{max}}, v_{\mathit{final}}\}$, which implies that $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.
    \end{compactitem}

    \item Otherwise, $\mathit{view}_i \in \{v_{\mathit{max}}, v_{\mathit{final}}\}$.
    Again, $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.
\end{compactitem}
Therefore, every correct process broadcasts $\langle \textsc{start-view}, v_{\mathit{max}} \rangle$ or $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ by time $\text{GST} + 3\delta$.

Hence, by time $\text{GST} + 4\delta$, every correct process receives $2t + 1$ \textsc{start-view} messages for either $v_{\mathit{final}}$ or $v_{\mathit{max}}$.
Thus, by time $\text{GST} + 6\delta$, every correct process enters either $v_{\mathit{max}}$ or $v_{\mathit{final}}$.
\end{proof}

%%%%%%%%%%
% safety %
%%%%%%%%%%
\begin{lemma}\label{lemma:validity_of_core}
    If no correct process validates bit $1-b$ at view $v$, then 
    any correct process obtaining an output from the second instance of graded consensus at view $v$ will output $(b,1)$.
\end{lemma}

\begin{proof}
    Let $\mathsf{gc\_start}_{v}$ (resp., $\mathsf{gc\_end}_{v}$) be the first (resp., second) graded consensus instance of view $v$.
    By assumption, no correct process has validated bit $1-b$ at view $v$, and therefore, no correct process submits bit $1-b$ to $\mathsf{gc\_start}_{v}$.
    Consequently, by the validity of graded consensus, any correct process obtaining an output from $\mathsf{gc\_start}_{v}$ will output $(b,1)$.
    Therefore, no correct process submits bit $1-b$ to $\mathsf{gc\_end}_{v}$.
    Hence, by the validity of graded consensus, any correct process obtaining an output from $\mathsf{gc\_end}_{v}$ will output $(b,1)$.
\end{proof}

\begin{lemma}\label{lemma:lock_forever}
    Let $p_i$ be a correct process that decides on bit $b_i$ in view $v_i$.
    Then, for any view $v_j \geq v_i$, if a correct process validates or decides bit $b_j$ in view $v_j$, it must be that $b_j = b_i$.
\end{lemma}

\begin{proof}
    We proceed by induction.
    
    Base Case ($v_j = v_i$):
    
    According to lines \ref{line:gc_end_grade_1} and \ref{line:decide} in Algorithm \ref{algorithm:repeater_view_core}, process $p_i$ produces output $(b_i,1)$ from the second graded consensus in view $v_i$. 
    Due to the consistency of graded consensus, any correct process that produces an output from the second graded consensus in view $v_i$ will output $b_i$. Hence, no correct process decides $1-b_i$ at view $v_i$.
    For the same reason, no correct process broadcasts $\langle \textsc{echo}, 1-b_i \rangle$ at line \ref{line:bcast_echo_first}, nor at line \ref{line:bcast_echo_second}. Therefore, no correct process receives sufficient $\langle \textsc{echo}, 1-b_i \rangle$ messages in view $v_i$ to validate $1-b_i$.
    Thus, the only bit that can be validated in view $v_i$ is $b_i$.
    
    Inductive Step: Assume the lemma's statement holds up to view $v_j$. We prove it for view $v_j+1$. 
    
    %Let $\mathsf{gc\_start}_{v_j+1}$ (resp., $\mathsf{gc\_end}_{v_j+1}$) be the first (resp., second) graded consensus instance of view $v_j+1$.
    By the induction hypothesis, no correct process has validated bit $1-b_i$ at view $v_j$, and therefore, by Lemma \ref{lemma:validity_of_core}, any correct process obtaining an output from the second graded consensus instance, will output $(b_i,1)$.
    %no correct process submits bit $1-b_i$ to $\mathsf{gc\_start}_{v_j+1}$. Consequently, by the validity of graded consensus, any correct process obtaining an output from $\mathsf{gc\_start}_{v_j+1}$ will output $(b_i,1)$. Therefore, no correct process submits bit $1-b_i$ to $\mathsf{gc\_end}_{v_j+1}$. Again, by the validity of graded consensus, any correct process obtaining an output from $\mathsf{gc\_end}_{v_j+1}$ will output $(b,1)$.
    As a result, no correct process decides $1-b_i$ at view $v_j+1$.
    For the same reason, no correct process broadcasts $\langle \textsc{echo}, 1-b_i \rangle$ at line \ref{line:bcast_echo_first}, nor at line \ref{line:bcast_echo_second}. Thus, no correct process receives enough $\langle \textsc{echo}, 1-b_i \rangle$ messages in view $v_j+1$ to validate $1-b_i$.
    Therefore, the only bit that can be validated in view $v_j+1$ is $b_i$, completing the inductive step and the proof.
\end{proof}


\begin{lemma}\label{lemma:agreement}
    Agreement is ensured.
\end{lemma}

\begin{proof}
    By immediate application of Lemma \ref{lemma:lock_forever}.
\end{proof}


\begin{lemma}\label{lemma:strong_validity}
    Strong Validity is ensured.
\end{lemma}

\begin{proof}
    Assume every correct process start the protocol with input $b$. By Lemma \ref{lemma:validity_of_core}, the first correct process obtaining an output from the second instance of graded consensus at first view will output $(b,1)$.
    
\end{proof}
\fi

\begin{algorithm}
\caption{\name: Pseudocode (for process $p_i$)}
\label{algorithm:name_pseudocode}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em \block core consensus, \textbf{instances} $\mathit{core}(v)$, for every view $v$

\medskip
\State \textbf{Local timers:}
\State \hskip2em $\mathsf{Timer}$ $\mathit{help\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{enter\_timer}_i$

\medskip
\State \textbf{Local variables:}
% \State \hskip2em $\mathsf{Value}$ $\mathit{proposal}_i \gets \bot$
\State \hskip2em $\mathsf{Boolean}$ $\mathit{decided}_i \gets \mathit{false}$
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ \label{line:init_view}
\State \hskip2em $\mathsf{View}$ $\mathit{last\_entered}_i \gets 1$
\State \hskip2em $\mathsf{View}$ $\mathit{help\_view}_i \gets 1$ \label{line:init_help_view}

\medskip
\State \textbf{upon} $\mathsf{propose}(\mathit{proposal} \in \mathsf{Value})$:
% \State \hskip2em $\mathit{proposal}_i \gets \mathit{proposal}$
\State \hskip2em \textbf{invoke} $\mathit{core}(1).\mathsf{propose}(\mathit{proposal})$ \BlueComment{start \block associated with view $1$} \label{line:enter_1}

\medskip
\State \textbf{upon} $\mathit{core}(\mathit{view}_i).\mathsf{completed}$: \label{line:view_timer_expire} \BlueComment{current \block instance has completed}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i + 1 \rangle$ \label{line:send_complete_1} \BlueComment{start transiting to the next \block instance}

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v$ such that (1) $v > \mathit{view}_i$, and (2) $\langle \textsc{start-view}, v \rangle$ is received from $t + 1$ processes: \label{line:receive_plurality}
\State \hskip2em \textbf{if} $v > \mathit{help\_view}_i$: \label{line:check_help}
\State \hskip4em $\mathit{help\_view}_i \gets v$ \label{line:update_help_view}
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{cancel}()$ \label{line:cancel_help}
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_help}

\medskip
\State \textbf{upon} $\mathit{help\_timer}_i$ \textbf{expires}: \label{line:help_timer_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i \rangle$ \label{line:send_complete_2}
\State \hskip2em \textbf{if} $\mathit{help\_view}_i > 2$: \label{line:check_help_2}
\State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ \label{line:send_complete_2_prime} 
% \State \hskip2em \textbf{if} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ is received from $t + 1$ processes:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ 

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v > \mathit{view}_i$ such that $\langle \textsc{start-view}, v \rangle$ is received from $2t + 1$ processes: \label{line:receive_quorum}
\State \hskip2em $\mathit{view}_i \gets v$ \label{line:update_view_2}
% \State \hskip2em \sout{$\mathit{view\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_view}}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_enter}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_enter}

\medskip
\State \textbf{upon} $\mathit{enter\_timer}_i$ \textbf{expires:} \label{line:enter_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i \rangle$ \label{line:send_complete_3}
\State \hskip2em \textbf{if} $\mathit{view}_i > 2$: \label{line:check_view}
\State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i - 1 \rangle$ \label{line:send_complete_3_prime}
\State \hskip2em \textbf{invoke} $\mathit{core}(\mathit{last\_entered}_i).\mathsf{abandon}$ \BlueComment{stop participating in the current view core abstraction} \label{line:leave_v}
\State \hskip2em \textbf{wait for} $\mathit{core}(\mathit{view}_i - 1).\mathsf{validate}(\mathit{val} \in \mathsf{Value})$
\State \hskip2em \textbf{invoke} $\mathit{core}(\mathit{view}_i).\mathsf{propose}(\mathit{val})$ \BlueComment{start \block associated with view $\mathit{view}_i$}  \label{line:enter_v}
\State \hskip2em $\mathit{last\_entered}_i \gets \mathit{view}_i$

\medskip
\State \textbf{upon} $\mathit{core}(\mathit{view}_i).\mathsf{decide}(\mathit{val} \in \mathsf{Value})$ and $\mathit{decided}_i = \mathit{false}$:
\State \hskip2em $\mathit{decided}_i \gets \mathit{true}$
\State \hskip2em \textbf{broadcast} $\langle \textsc{decided}, \mathit{val} \rangle$

\medskip
\State \textbf{upon} exists $\mathsf{Value}$ $\mathit{val}$ such that $\langle \textsc{decided}, \mathit{val} \rangle$ is received from $t + 1$ processes and $\mathit{decided}_i = \mathit{false}$:
\State \hskip2em $\mathit{decided}_i \gets \mathit{true}$
\State \hskip2em \textbf{broadcast} $\langle \textsc{decided}, \mathit{val} \rangle$

\medskip
\State \textbf{upon} exists $\mathsf{Value}$ $\mathit{val}$ such that $\langle \textsc{decided}, \mathit{val} \rangle$ is received from $2t + 1$ processes:
\State \hskip2em \textbf{broadcast} $\langle \textsc{decided}, \mathit{val} \rangle$
\State \hskip2em \textbf{trigger} $\mathsf{decide}(\mathit{val})$
\State \hskip2em \textbf{stop participating} in \name (i.e., stop sending any messages and stop reacting to any received messages) \BlueComment{process $p_i$ halts}
\end{algorithmic}
\end{algorithm}

==> sections/subquadratic_solution.tex <==
\section{Randomized Solution}




\subsection{Cubic Reduction}

We studied the communication complexity of one flavor of consensus that is $\Omega(n^2)$ after GST in the partially synchronous model handling an unbounded adaptive adversary, even for randomized protocols. However, other problems can be considered such as the latency complexity and other agreement problems, such as agreement on a core set (ACS).

For some corresponding problems that only differ on the synchrony assumption, there is a significant gap between the synchronous and the asynchronous version.



Classic asynchronous reductions (\cite{Chor1989,CR93,BenOr1993}) allows asynchronous agreement on a core set (ACS). More concretely, we can use the transformation of \cite{ben1994asynchronous} and the reliable broadcast of  \cite{Alhaddad2022} to achieve ACS with communication complexity of $O(n^2L_{in}+ X_n)$ where $X_n$ denotes the communication complexity of $n$ parallel instances of binary BA with strong validity.
Against an unbounded adversary, even assuming private channels, no existing solution does better than \cite{AAPS23} with $\tilde{O}(n^4)$ communication complexity (with a collision resistant hash function, a cubic solution is possible \cite{das2024asynchronous}). Hence, a cubic information theoretic partially synchronous ACS can represent a good alternative.
Of course, a such a cubic solution can be trivially obtained from any information theoretic quadratic solutions. This includes solution with or without private channels, with a static or an adaptive adversary, with arbitrary failures or omission failures only.

With private channels, \cite{KingSaia10,King2011} implements binary Byzantine broadcast with $\tilde{O}(\sqrt{n})$ per-process bit complexity atop private channels agains an unbounded adversary that can adaptively corrupt up to $n/(3+\epsilon)$ processes.

In the full information model, achieving a satisfying latency against an adaptive adversary is particularly challenging because of the Bar-Joseph-Ben-Or lower bound \cite{Bar-JosephB98}.
With omission failures only 
\cite{hajiaghayi2024nearly} achieve a near optimal solution.

In the full information model, achieving a satisfying latency has been more investigated against a static adversary.  Goldwasser, Pavlov, and Vaikuntanathan \cite{GPV06}, considered a synchronized, full information model in which the adversary corrupts up to $f$ player sup front, that is,it is non-adaptive. They proved that Byzantine Agreement can be solved with resiliency $f < n/(3+\epsilon)$ in $O(\log n/\epsilon^2)$ rounds.
Consequently, it is possible to achieve a $O(1)$-round randomized BA protocol in a synchronous full-information network tolerating $t =
O( n/(\log n)^{1.58} )$ static corruptions.
Another research direction consists of extending the almost-everywhere protocol of King, Saia, Sanwalani, and Vee \cite{KSSV06,king2022corrigendum}. Specifically, their protocol succeeds with all but negligible probability of error and each party speaks to only $\tilde{O}(1)$ other parties (within $\tilde{O}(1)$ many rounds). It can tolerate
$1/3-\epsilon$ fraction of statically corrupted parties for every constant $\epsilon > 0.3$.
However, it fails to achieve correctness. It only achieves so-called almost-everywhere agreement, where $1-O(\log^{-1} n)$ fraction of the parties reach agreement. Extending almost-everywhere to full agreement (while preserving the efficiency properties) has been a major challenge since then. Information theoretic results include \cite{braud2013fast,Gelles23}




\subsection{Assuming secret channels}

Assuming secret channels Synchronous interactive consistency (resp., aynchronous agreement on a core set (ACS)) can be implemented with a constant expected number of rounds, and $O(n^2L_{in}) + \tilde{O}(n^3)$ (resp., $\tilde{O}(n^4)$) communication against an unbounded adaptive adversary
\cite{AsharovChandramouli24} \cite{AAPS23}.

(To do) Implement ACS with $O(n^2L_{in}) + \tilde{O}(n^3)$ and a constant expected number of rounds in partial snchrony.

\subsection{Balanced Propagation}

Each broadcast can be replaced by a propagation primitive, such as $\mathsf{Murmur}$ \cite{GKMPS19}.
Murmur is a probabilistic broadcast algorithm that uses simple message dissemination to establish validity (if the sender is correct, all correct processes eventually deliver the broadcast message). In this algorithm, each correct process relays the sender’s signed message to a randomly picked gossip sample of other processes. For the sample
size $\Omega(\log n )$, the resulting gossip network is a connected graph with $O( \log n/ \log \log n)$
diameter, with overwhelming probability.

\subsection{Verifiable Random Functions and Committee Sampling}

We follow the presentation of \cite{CKS20}.
We use verifiable random functions (VRFs) as defined below. Using VRFs, it is possible to implement validated committee sampling, a primitive that allows processes to elect committees without communication and later prove their election.

\paragraph*{VRF Setup}
A VRF provides every process $p_i$ with a private function $\mathsf{sample}_i(s, \lambda)$, which takes a string $s$ (typically the label of some specific step) and a threshold $\lambda \in [1:n]$, and returns a tuple $\langle v_i, \sigma_i \rangle$, where $v_i \in \{\mathit{true}, \mathit{false}\}$ and $\sigma_i$ is a proof that $v_i = \mathsf{sample}_i(s, \lambda)$. If $v_i = \mathit{true}$, we say that $p_i$ is sampled to the committee for $s$ and $\lambda$. The primitive ensures that $p_i$ is sampled with probability $\lambda / n$.

In addition, there is a public function, $\committeeval(s, \lambda, i, \sigma_i)$, which takes a string $s$, a threshold $\lambda$, a process identification $i$, and a proof $\sigma_i$, and returns $\mathit{true}$ or $\mathit{false}$.

We define the committee as:
\[
C(s, \lambda) = \{p_i \in \Pi \mid \mathsf{sample}_i(s, \lambda) \in \{ \langle \mathit{true}, \sigma \rangle \mid \sigma \in \{0,1\}^{*}\} \}
\]

Consider a string $s$. For every $i$, $1 \leq i \leq n$, let $\langle v_i, \sigma_i \rangle$ be the return value of $\mathsf{sample}_i(s, \lambda)$.

The following properties are satisfied for every $p_i$:
\begin{itemize}
    \item \textbf{Correctness:} $\committeeval(s, \lambda, i, \sigma_i) = v_i$.
    \item \textbf{Unpredictability:} If $p_i$ is correct, then it is infeasible for the adversary to compute $\mathsf{sample}_i(s, \lambda)$.
    \item \textbf{Unforgeability:} It is infeasible for the adversary to find $\langle v, \sigma \rangle$ such that $v \neq v_i$ and $\committeeval(s, \lambda, i, \sigma_i) = \mathit{true}$.
\end{itemize}

The committee system shares similar ideas with quorum systems, ensuring probabilistic intersection with overwhelming probability (1 minus a negligible function).

We define:
\begin{itemize}
    \item $W_{\delta} = \frac{2+\epsilon}{3}(1-\delta) \lambda$
    \item $B_{\delta'} = \frac{1-\epsilon}{3}(1+\delta') \lambda$
    \item apparently $\delta = 3\delta'$ is a good choice.
\end{itemize}

Using a standard Chernoff bound, we obtain the following lemma:
\begin{lemma}[Committee System]
Let $s$ be a string and $\lambda \in [1:n]$.
\begin{itemize}
    \item (Availibility) $\Pr[|C(s, \lambda) \cap \Corrects| \leq W_\delta] \leq \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)$
    \item (Non-Intrusion) $\Pr[|C(s, \lambda) \setminus \Corrects| \geq B_{\delta'}] \leq \exp\left(-\frac{(\delta')^2 (1-\epsilon) \lambda}{6 + 3\delta'}\right)$

    \item (Binary Partition) Let $(Q,Q')$, be a partition of $C(s, \lambda) \cap \Corrects$, with $|Q| \geq |Q'|$. 
    
    $\Pr[|Q| \leq B_{\delta'}] \leq \mathit{neg}(n)$

    \item (Committee Intersection) Let $Q,Q' \subseteq C(s, \lambda)$, such that $|Q|=W_\delta$.
    \begin{itemize}
    \item $\Pr[|Q \cap \Corrects| \leq B_{\delta''}] \leq \mathit{neg}(n)$
    
    \item If $|Q'|=W_\delta$, then

    \begin{itemize}
    \item $\Pr[|Q \cap Q'| \leq B_{\delta''}] \leq \mathit{neg}(n)$
    \item $\Pr[Q \cap Q' \cap \Corrects= \emptyset] \leq \mathit{neg}(n)$
    \end{itemize}
    
    \item If $|Q'|=B_{\delta'}$, then $\Pr[|Q \cap Q'| \leq B_{\delta''}] \leq \mathit{neg}(n)$
    \end{itemize}
\end{itemize}
\end{lemma}

\begin{proof}
$\;$
    \begin{itemize}
    \item (Availibility) Let $X_j$ be the Bernoulli random variable indicating if $p_j \in C(s, \lambda)$, so $\Pr[X_j = 1] = \lambda / n$. Define $Z_H = \sum_{p_j \in \Corrects} X_j$. By linearity of expectation,
\[
\mu_L \triangleq \mathbb{E}(Z_H) = \frac{2+\epsilon}{3} \lambda
\]
Thus, $|C(s, \lambda) \cap \Corrects| \sim Z_H$. By the Chernoff bound,
\[
\Pr[Z_H \leq (1 - \delta) \cdot \frac{2+\epsilon}{3} \lambda] \leq \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)
\]
    \item (Non-Intrusion) Let $Y_j$ be the Bernoulli random variable indicating if $p_j \notin \Corrects$ and $p_j \in C(s, \lambda)$, so $\Pr[Y_j = 1] = \lambda / n$. Define $Z_{B} = \sum_{p_j \notin \Corrects} Y_j$. By linearity of expectation,
\[
\mu_I \triangleq \mathbb{E}(Z_{B}) = \frac{1-\epsilon}{3} \lambda
\]
Thus, $|C(s, \lambda) \setminus \Corrects| \sim Z_{B}$. By the Chernoff bound,
\[
\Pr[Z_{B} \geq (1 + \delta) \cdot \frac{1-\epsilon}{3} \lambda] \leq \exp\left(-\frac{\delta^2 (1-\epsilon)}{6+3\delta} \lambda\right)
\]


    \item (Binary Partition) Consider the worst case $|Q|=|Q'|$. We have $|Q|\sim Z_H/2$.
    As stated above

    \[
\Pr[Z_H/2 \leq (1 - \delta) \cdot \frac{1+\epsilon/2}{3} \lambda] \leq \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)
\]
    
This concludes the proof.

    \item (Committee Intersection) 
    Define $Z_C = \sum_{p_j \in \Pi } X_j$. By linearity of the expectation, $\mu_C \triangleq \mathbb{E}(Z_C)= \lambda$.
    By the Chernoff bound, $\Pr[Z_C \geq (1 + \delta_c) \cdot \lambda] \leq \exp\left(-\frac{\delta_c^2}{2+\delta_c} \lambda \right) $.

    We remark that
    $|Q \cap Q'| \geq |Q|+|Q'|-|Q \cup Q'| \geq  W_{\delta} + |Q'| - Z_{C} $. 

    \begin{itemize}
        \item Assume $|Q'|=W_\delta$. 

        \begin{itemize}
        \item 

    $\Pr[2W_{\delta} - Z_C \leq 2W_{\delta} - (1 + \delta_c) \cdot \lambda] \leq \exp\left(-\frac{\delta_c^2}{2+\delta_c} \lambda \right) $

    $\Pr[|Q \cap Q'| \leq 2W_{\delta} - (1 + \delta_c) \cdot \lambda] \leq \exp\left(-\frac{\delta_c^2}{2+\delta_c} \lambda \right) $
    
        \item Moreover, for any $\delta''$, $\Pr[Q \cap Q' \cap \Corrects \neq \emptyset] \geq \Pr[|Q \cap Q'| \geq B_{\delta''}] \cdot \Pr[|C(s, \lambda) \setminus \Corrects| < B_{\delta''}]$. 
        Hence, for any $\delta''$, $\Pr[Q \cap Q' \cap \Corrects \neq \emptyset] \leq \Pr[|Q \cap Q'| \leq B_{\delta''}] + \Pr[|C(s, \lambda) \setminus \Corrects| \geq B_{\delta''}]$.
        The first factor has been dominated above, while the second factor is bounded by the non-intrusion property.
        Let us compute $\delta''$ such that $\frac{1-\epsilon}{3}(1+\delta'') = 2\frac{2+\epsilon}{3}(1-\delta) - (1+\delta_c)$

        \end{itemize}

        \item Assume $|Q'|=B_{\delta'}$

        $\Pr[W_{\delta} + B_{\delta'} - Z_C \leq W_{\delta} + B_{\delta'} - (1 + \delta_c) \cdot \lambda] \leq \exp\left(-\frac{\delta_c^2}{2+\delta_c} \lambda \right) $

    $\Pr[|Q \cap Q'| \leq W_{\delta} + B_{\delta'} - (1 + \delta_c) \cdot \lambda] \leq \exp\left(-\frac{\delta_c^2}{2+\delta_c} \lambda \right) $

    Let us compute $\delta''$ such that $\frac{1-\epsilon}{3}(1+\delta'') = 2\frac{2+\epsilon}{3}(1-\delta) + \frac{1-\epsilon}{3}(1+\delta') - (1+\delta_c)$
    \end{itemize}
\end{itemize}
\end{proof}

The former lemma is similar to the Claim 10, Corollary 11 and Corollary 11 of \cite{CKS20}.

\subsection{Subquadratic Double Echo}

\begin{module}
\caption{DoubleEcho$\langle \mathsf{String } \; \text{echo\_id} \rangle$}
\label{mod:vrf_double_echo}
\footnotesize
\begin{algorithmic}[1]

\Statex \textbf{Parameters:}
\Statex \hskip2em $\mathsf{String}$ $\mathsf{echo\_id}$ \BlueComment{unique identifier for the echo instance}
\Statex \hskip2em $\mathsf{Real}$ $\lambda$ \BlueComment{threshold parameter for committee selection}

\medskip
\Statex \textbf{Events:}
\Statex \hskip2em \emph{request} $\mathsf{init}()$: a process initiates the echo protocol.
\Statex \hskip2em \emph{notification} $\mathsf{react}()$: a process reacts to the echo protocol.
\Statex \hskip2em \emph{notification} $\mathsf{ack}()$: a process acknowledges the completion of the echo protocol.

\medskip 
\Statex \textbf{Properties used for the finisher and the view synchronizer:}

\Statex \hskip2em \emph{Obligation:} If every correct process triggers $\mathsf{init}$ by time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + \delta$.

\smallskip 
\Statex \hskip2em \emph{Totality:} If some correct process triggers $\mathsf{ack}$ at time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + 2\delta$.

\smallskip 
\Statex \hskip2em \emph{Justification:} If some correct process triggers $\mathsf{ack}$, then at least one correct process triggered $\mathsf{init}$.

\medskip 
\Statex \textbf{Properties used for the validation broadcast:}
\Statex \hskip2em \emph{Strong Obligation:} If one half of the correct processes triggers $\mathsf{init}$ by time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + 2\delta$.

%\Statex \hskip2em \emph{Partial Totality:} If some correct process triggers $\mathsf{ack}$ at time $\tau$, then every correct process triggers $\mathsf{react}$ by time $\max(\text{GST}, \tau) + \delta$, even if there exists a time $\tau'$ such that no correct sends any message after $\tau'$.

\end{algorithmic}
\end{module}


\begin{algorithm}
\caption{Subquadratic DoubleEcho$\langle \mathsf{String } \; \text{echo\_id} \rangle$ - Pseudocode (for process $p_i$)}
\label{algorithm:vrf_double_echo}
\footnotesize
\begin{algorithmic} [1] 
\medskip
\State \textbf{Local variables:}
\State \hskip2em $\mathsf{Set}(\mathsf{Process})$ $\mathit{from}_i \gets \emptyset$

\State \hskip2em $\mathsf{Boolean}$ $\mathit{propagated}_i \gets \mathit{false}$

\medskip
\State \textbf{upon} $\mathsf{init}()$: \label{line:init}
\State \hskip2em $\langle \mathit{elected}^v_i, \sigma^e_{i,v} \rangle \gets \mathsf{sample}(\text{echo\_id}, \lambda)$
\State \hskip2em \textbf{if} $\mathit{elected}^v_i$:

\State \hskip4em $\mathit{propagated}_i \gets \mathit{true}$

\State \hskip4em \textbf{propagate} $\langle \textsc{echo}, \text{echo\_id}, \sigma^e_{i,v} \rangle$

\medskip
\State \textbf{upon} $m_j = \langle \textsc{echo}, \text{echo\_id}, \sigma^e_{j,v}  \rangle$ \text{is received from process $p_j$}:
\State \hskip2em \textbf{if} $\committeeval (\text{echo\_id}, \lambda, j, \sigma^e_j)$
\State \hskip4em $\mathit{from}_i \gets \mathit{from}_i \cup \{p_j\} $

\medskip
\State \textbf{upon} $| \mathit{from}_i |\geq B_{\delta}$: \label{line:double_echo_amplication_check}

\State \hskip2em $\langle \mathit{elected}^v_i, \sigma^e_{i,v} \rangle \gets \mathsf{sample}(\text{echo\_id}, \lambda)$
\State \hskip2em \textbf{if} $\mathit{elected}^v_i \wedge \mathit{propagated}_i \neq \mathit{true}$:
\State \hskip4em $\mathit{propagated}_i \gets \mathit{true}$

\State \hskip4em \textbf{propagate} $\langle \textsc{echo}, \text{echo\_id}, \sigma^e_{i,v} \rangle$ \label{line:double_echo_amplication_propagate}

\State \hskip2em  \textbf{trigger} $\mathsf{react}()$

\medskip
\State \textbf{upon} $|\mathit{from}_i| \geq W_{\delta}$: \label{line:double_echo_ack_check}
\State \hskip2em \textbf{trigger} $\mathsf{ack}()$

\end{algorithmic} 
\end{algorithm}

\paragraph{Proof of Double Echo.}

%We begin the proof with a preliminary lemma.
%\begin{lemma}[Amplification] \label{lemma:double_echo_amplification}
%Assume $B_{\delta'}$ correct processes send an $\textsc{echo}$ message by time $\tau$, then, with overwhelming probability, every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + 2\delta$.
%\end{lemma}


\begin{lemma}[Obligation] \label{lemma:double_echo_obligation}
\Cref{algorithm:vrf_double_echo} ensures Obligation property of  Module~\ref{mod:vrf_double_echo} with overwhelming probability, that is,
if every correct process triggers $\mathsf{init}$ by time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + \delta$.
\end{lemma}
\begin{proof}
Let us note $s=\text{echo\_id}$.
Consider the event that every correct process triggers $\mathsf{init}$ by time $\tau$. This means that each correct process calls the function $\mathsf{sample}(s, \lambda)$ to determine if it is elected to propagate the echo message. 

By the Availability property, the probability that the number of correct processes in the committee $C(s, \lambda)$ is at least $W_\delta$ is overwhelming:
\[
\Pr[|C(s, \lambda) \cap \Corrects| \geq W_\delta] \geq 1 - \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)
\]

Hence, with overwhelming probability, every correct process receives $W_\delta$ $\textsc{ECHO}$ messages by time $\max(\text{GST}, \tau) + \delta$ before triggering $\mathsf{ack}$, which concludes the proof.
\end{proof}

We aim to show that if some correct process triggers $\mathsf{ack}$, then at least one correct process triggered $\mathsf{init}$.

%(Binary Partition) Let $(Q,Q')$, be a partition of $C(s, \lambda) \cap \Corrects$, with $|Q| \geq |Q'|$. $\Pr[|Q| \leq B_{\delta'}] \leq \mathit{neg}(n)$

\begin{lemma}[Justification] \label{lemma:double_echo_justification}
\Cref{algorithm:vrf_double_echo} ensures Justification property of  Module~\ref{mod:vrf_double_echo} with overwhelming probability, that is,
if some correct process triggers $\mathsf{ack}$, then at least one correct process triggered $\mathsf{init}$.
\end{lemma}
\begin{proof}
Let us note $s=\text{echo\_id}$. Consider the event that some correct process triggers $\mathsf{ack}$. This implies that the process received at least $W_\delta$ valid \textsc{ECHO} messages.

By the Non-Intrusion property, the probability that the number of incorrect processes in the committee $C(s, \lambda)$ is at least $B_\delta$ is bounded by:
\[
\Pr[|C(s, \lambda) \setminus \Corrects| \geq B_\delta] \leq \exp\left(-\frac{\delta^2 (1-\epsilon) \lambda}{6 + 3\delta}\right)
\]

Hence, if no correct process triggered $\mathsf{init}$, then, with overwhelming probability, the check at line~\ref{line:double_echo_amplication_check} does not pass for any correct process. Thus, no correct process sends any $\textsc{echo}$ message. Thus, with overwhelming probability, the check at line~\ref{line:double_echo_ack_check} does not pass for any correct process, concluding the proof.
\end{proof}

We aim to show that if some correct process triggers $\mathsf{ack}$ at time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + \delta$.

\begin{lemma} \label{lemma:double_echo_totality}
\Cref{algorithm:vrf_double_echo} ensures Totality property of  Module~\ref{mod:vrf_double_echo} with overwhelming probability, that is,
if some correct process triggers $\mathsf{ack}$ at time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + 2\delta$.
\end{lemma}
\begin{proof}
Let us note $s = \text{echo\_id}$. Consider the event that some correct process triggers $\mathsf{ack}$ at time $\tau$. This implies that the process received at least $|Q|=W_\delta$ valid \textsc{ECHO} messages from a set $Q \subset C(s,\lambda)$.

By the Committee Intersection property, the probability that the intersection of $Q$ with the set of correct processes is less than or equal to $B_{\delta''}$ is negligible:
\[
\Pr[|Q \cap \Corrects| \leq B_{\delta''}] \leq \mathit{neg}(n)
\]

Hence, with overwhelming probability, the check at line~\ref{line:double_echo_amplication_check} passes for every correct process, which means that every correct process that is elected propagates an $\textsc{echo}$ message (line line~\ref{line:double_echo_amplication_propagate}).

By the Availability property, that states that the probability that the number of correct processes in the committee $C(s, \lambda)$ is at least $W_\delta$ is overwhelming:
\[
\Pr[|C(s, \lambda) \cap \Corrects| \geq W_\delta] \geq 1 - \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)
\]

Thus, with overwhelming probability, every correct process receives $W_\delta$ $\textsc{ECHO}$ messages by time $\max(\text{GST}, \tau) + 2\delta$ before triggering $\mathsf{ack}$, which concludes the proof.




Given this high probability, consider any other correct process \(p_j\). This process will receive the same set of messages (or at least enough to ensure intersection) within time \(\delta\) after \(\tau\). Hence, these correct processes will also receive at least $W_\delta$ valid \textsc{ECHO} messages.

Therefore, every correct process will trigger $\mathsf{ack}$ by time \(\max(\text{GST}, \tau) + \delta\), concluding the proof.
\end{proof}

\begin{lemma}[Strong Obligation] \label{lemma:double_echo_strong_obligation}
\Cref{algorithm:vrf_double_echo} ensures Strong Obligation property of  Module~\ref{mod:vrf_double_echo} with overwhelming probability, that is,
if one half of the correct processes trigger $\mathsf{init}$ by time $\tau$, then every correct process triggers $\mathsf{ack}$ by time $\max(\text{GST}, \tau) + 2\delta$.
\end{lemma}
\begin{proof}
Let us note $s=\text{echo\_id}$.
Consider the event that one half of the correct processes trigger $\mathsf{init}$ by time $\tau$. This means that each correct process calls the function $\mathsf{sample}(s, \lambda)$ to determine if it is elected to propagate the echo message. 

By the Binary Partition property, with overwhelming probability, the corresponding elected set is of size at least $B_{\delta'}$. Hence, with overwhelming probability, every correct process receives $B_{\delta'}$ $\textsc{ECHO}$ messages by time $\max(\text{GST}, \tau) + \delta$ which allows the check line~\ref{line:double_echo_ack_check} to pqss, before propagating an $\textsc{ECHO}$ message in case of election.

By the Availability property, the probability that the number of correct processes in the committee $C(s, \lambda)$ is at least $W_\delta$ is overwhelming:
\[
\Pr[|C(s, \lambda) \cap \Corrects| \geq W_\delta] \geq 1 - \exp\left(-\frac{\delta^2 (2+\epsilon)}{6} \lambda\right)
\]

Hence, with overwhelming probability, every correct process receives $W_\delta$ $\textsc{ECHO}$ messages by time $\max(\text{GST}, \tau) + 2\delta$ before triggering $\mathsf{ack}$, which concludes the proof.
\end{proof}


\subsection{Subquadratic Finisher, View Synchronizer, and Binary Validation Broadcast}

\begin{module}
\caption{Recall Finisher}
\label{mod:subquadratic_finisher}
\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Events:}
\Statex \hskip2em \emph{request} $\mathsf{to\_finish}(v \in \mathsf{Value})$: a process aims to finish with value $v$.

\Statex \hskip2em \emph{indication} $\mathsf{finish}(v' \in \mathsf{Value})$: a process finishes with value $v'$.

\medskip 
\Statex \textbf{Properties:}

\Statex \hskip2em \emph{Integrity:} If a correct process receives a $\mathsf{finish}(v')$ indication, then a correct process has previously invoked a $\mathsf{to\_finish}(v')$ request.

\smallskip 
\Statex \hskip2em \emph{Termination:} Let $\tau$ be the first time such that all correct processes have invoked a $\mathsf{to\_finish}(\cdot)$ request by time $\tau$. Then, every correct process receives a $\mathsf{finish}(\cdot)$ indication by time $\max(\tau, \text{GST}) + 2\delta$.

\smallskip 
\Statex \hskip2em \emph{Totality:} If any correct process receives a $\mathsf{finish}(\cdot)$ indication at some time $\tau$, then every correct process receives a $\mathsf{finish}(\cdot)$ indication by time $\max(\tau, \text{GST}) + 2\delta$.

\end{algorithmic}
\end{module}


\begin{algorithm}
\caption{Subquadratic Finisher - Pseudocode (for process $p_i$)}
\label{algorithm:subquadratic_finisher}
\footnotesize
\begin{algorithmic} [1] 

\State \textbf{Uses:}
\State \hskip2em DoubleEcho$<\mathsf{Value} \; \mathit{val}>$ instances

\medskip
\State \textbf{upon} $\mathsf{to\_finish}(v)$: \label{line:to_finish}
\State \hskip2em \textbf{invoke} DoubleEcho$\langle v \rangle.\mathsf{init}()$

\medskip
\State \textbf{upon} DoubleEcho$\langle v \rangle.\mathsf{ack}()$:
\State \hskip2em \textbf{trigger} $\mathsf{finish}(v)$
\State \hskip2em \textbf{halt}
\end{algorithmic} 
\end{algorithm}


\begin{module}
\caption{Recall View Synchronizer}
\label{mod:subquadratic_view_sync}
\footnotesize
\begin{algorithmic}[1]
\Statex \textbf{Events:}
\Statex \hskip2em \emph{request} $\mathsf{to\_advance}(v \in \mathsf{View})$: a process aims to advance to view $v$.

\Statex \hskip2em \emph{indication} $\mathsf{advance}(v' \in \mathsf{View})$: a process can advance to view $v'$.

\medskip 
\Statex \textbf{Properties:}

\Statex \hskip2em \emph{Integrity:} If a correct process receives a $\mathsf{advance}(v')$ indication, then a correct process has previously invoked a $\mathsf{to\_advance}(v')$ request.

\smallskip 
\Statex \hskip2em \emph{Termination:} Let $\tau$ be the first time such that all correct processes have invoked a $\mathsf{to\_advance}(\cdot)$ request by time $\tau$. Then, every correct process receives a $\mathsf{advance}(\cdot)$ indication by time $\max(\tau, \text{GST}) + 2\delta$.

\smallskip 
\Statex \hskip2em \emph{Totality:} If any correct process receives a $\mathsf{advance}(\cdot)$ indication at some time $\tau$, then every correct process receives a $\mathsf{advance}(\cdot)$ indication by time $\max(\tau, \text{GST}) + 2\delta$.

\end{algorithmic}
\end{module}

\begin{algorithm}
\caption{Subquadratic View Synchronizer - Pseudocode (for process $p_i$)}
\label{algorithm:subquadratic_view_sync}
\footnotesize
\begin{algorithmic} [1] 

\State \textbf{Uses:}
\State \hskip2em DoubleEcho$<\mathsf{View} \; \mathit{view}>$ instances

\medskip
\State \textbf{upon} $\mathsf{to\_advance}(\mathit{view})$: \label{line:to_advance}
\State \hskip2em \textbf{invoke} DoubleEcho$\langle \mathit{view} \rangle.\mathsf{init}()$

\medskip
\State \textbf{upon} DoubleEcho$\langle \mathit{view} \rangle.\mathsf{ack}()$:
\State \hskip2em \textbf{trigger} $\mathsf{advance}(\mathit{view})$
\end{algorithmic} 
\end{algorithm}

\begin{algorithm}
\caption{Subquadratic Binary Validation Broadcast - Pseudocode (for process $p_i$)}
\label{algorithm:subquadratic_finisher}
\footnotesize
\begin{algorithmic} [1] 

\State \textbf{Uses:}
\State \hskip2em DoubleEcho$<0>$ 
\State \hskip2em DoubleEcho$<1>$ 


\medskip
\State \textbf{upon} $\mathsf{broadcast}(v \in \{0,1\})$: \label{line:binary_validation_broadcast_input}
\State \hskip2em \textbf{invoke} DoubleEcho$\langle v \rangle.\mathsf{init}()$

\medskip
\State \textbf{upon} DoubleEcho$\langle v \in \{0,1\} \rangle.\mathsf{ack}()$:
\State \hskip2em \textbf{trigger} $\mathsf{completed}$

\medskip
\State \textbf{upon} DoubleEcho$\langle v \in \{0,1\} \rangle.\mathsf{react}()$:
\State \hskip2em \textbf{trigger} $\mathsf{validate}(v)$
\end{algorithmic} 
\end{algorithm}

\subsection{Subquadratic Approver and Consequences}

Cohen, Keidar, and Spiegelman provides \cite[Section 6.1]{CKS20} an approver protocol $\mathcal{A}_{CKS}$ that corresponds to a $(1/2)$-binary approximate agreement. A sequential composition of $\mathcal{A}_{CKS}$ with itself leads to a $(1/4)$-binary approximate agreement, wchich is enough to solve binary graded consensus, as explained in \cite{AttiyaWelch23}.

\subsection{Simulating a synchronous randomized protocol despite a time shift}

The simulation $\mathsf{CryptoSim}$ (
\Cref{algorithm:simulation}) allows to simulate any synchronous randomized protocol with 
per-process bit-complexity $\mathcal{B}$ in a partially synchronous environment, with the same round complexity complexity $\mathcal{R}$ and per-process bit-complexity $max(O(n),\mathcal{B})$.


==> sections/synchronous_unauthenticated_agreement.tex <==
\section{\sync: Synchronous Unauthenticated Byzantine Agreement with $O(n^2)$ Bits}

In this section, we overview \sync, a synchronous unauthenticated Byzantine agreement algorithm concurrently introduced by Berman, Garay and Perry~\cite{berman1992bit} and Coan and Welch~\cite{CoanW92}.

\paragraph{\sync's structure.}
In a nutshell, \sync is a recursive unauthenticated Byzantine consensus algorithm.
Namely, \sync partitions all $n$ processes into two halves, where each half runs \sync (among $n / 2$ processes).
The partition continues until an instance of \sync with only a single process is reached.
When such an instance is reached, the single operating process decides its proposal.
For completeness, the pseudocode of \sync is presented below.

\smallskip
\begin{mdframed} [frametitle={\sync operating among $n$ processes}, frametitlealignment=\centering]
Let $p_i$ be a process, and let $b_i$ be $p_i$'s variable which is initialized to $p_i$'s proposal.

\smallskip
\noindent If $n = 1$, $p_i$ decides $b_i$ (i.e., $p_i$'s proposal).
Otherwise, $p_i$ executes the following steps:

\noindent (1) Run $\mathcal{GC}_1(\mathcal{S})$ with proposal $b_i$.
Let $(b_1, g_1)$ be the pair decided from $\mathcal{GC}_1(\mathcal{S})$.
Set $b_i$ to $b_1$.

\noindent (2) If $p_i \in \mathcal{S}_{1}$, run $\sync(\mathcal{S}_1)$ with input $b_i$, and send the decision of $\sync(\mathcal{S}_1)$ to all processes in $\mathcal{S}$.
Otherwise, wait for the step to finish.

\noindent (3) If $p_i$ receives the same bit $b$ from a majority of processes in $\mathcal{S}_1$ and $g_1 = 0$, set $b_i$ to $b$.

\noindent (4) Run $\mathcal{GC}_2(\mathcal{S})$ with proposal $b_i$.
Let $(b_2, g_2)$ be the pair decided from $\mathcal{GC}_2(\mathcal{S})$.
Set $b_i$ to $b_1$.

\noindent (5) If $p_i \in \mathcal{S}_{2}$, run $\sync(\mathcal{S}_2)$ with input $b_i$, and send the decision of $\sync(\mathcal{S}_2)$ to all processes in $\mathcal{S}$.
Otherwise, wait for the step to finish.

\noindent (6) If $p_i$ receives the same bit $b$ from a majority of processes in $\mathcal{S}_2$ and $g_2 = 0$, set $b_i$ to $b$.
\end{mdframed}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/SYNC_coolestest.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

\paragraph{\sync's round complexity.}
As explained in \Cref{section:introduction}, it is essential to know the number of rounds \sync takes to terminate.
The following recurrence defines the round complexity $\mathcal{RC}(n)$ of \sync operating among $n$ processes:
\begin{equation*}
    \mathcal{RC}(n) = \begin{cases}
0, &\text{ if $n = 1$}\\
16 + \mathcal{RC}(\lceil \frac{n}{2}) \rceil + \mathcal{RC}(\lfloor \frac{n}{2} \rfloor), &\text{ otherwise.}
\end{cases}
\end{equation*}
Let us explain the aforementioned recurrence.
If $n = 1$, a process immediately decides its own proposal. 
Therefore, $\mathcal{RC}(1) = 0$.
If $n > 1$, processes execute (1) two graded consensus algorithms (steps 1 and 4), (2) $\sync(\mathcal{S}_1)$ (step 2), (3) $\sync(\mathcal{S}_2)$ (step 5), and (4) two ``half-to-all'' communication steps after $\sync(\mathcal{S}_1)$ and $\sync(\mathcal{S}_2)$.
Assuming that \sync employs the graded consensus algorithm proposed by Attiya and Welch~\cite{AttiyaWelch23} that terminates in 7 rounds, $\mathcal{RC}(n > 1) = 7 + 7 + 1 + 1 + \mathcal{RC}(\lceil \frac{n}{2} \rceil) + \mathcal{RC}(\lfloor \frac{n}{2} \rfloor) = 16 + \mathcal{RC}(\lceil \frac{n}{2} \rceil) + \mathcal{RC}(\lfloor \frac{n}{2} \rfloor)$.

\paragraph{\sync's per-process message complexity.}
We now analyze the maximum number of messages any correct process sends while executing \sync.
The following recurrence defines the maximum number of messages $\mathcal{MC}_i(n)$ any correct process $p_i$ sends while executing \sync among $n$ processes:
\begin{equation*}
    \mathcal{MC}_i(n) = \begin{cases}
0, &\text{ if $n = 1$}\\
13n + \mathcal{MC}_i(\lceil \frac{n}{2} \rceil), &\text{ if $p_i \in \mathcal{S}_1$}\\
13n + \mathcal{MC}_i(\lfloor \frac{n}{2} \rfloor), &\text{ if $p_i \in \mathcal{S}_2$}.
\end{cases}
\end{equation*}
Let us elaborate on the aforementioned recurrence.
If $n = 1$, $p_i$ decides without sending any message.
If $n > 1$, $p_i$ executes (1) two graded consensus algorithms (steps 1 and 4), (2) $\sync(\mathcal{S}_1)$ or $\sync(\mathcal{S}_2)$ (but not both!), and (3) one ``half-to-all'' communication step.
Given that the concrete implementation of the graded consensus ensures that $p_i$ sends at most $6n$ messages, $\mathcal{MC}_i(n) = 6n + 6n + 1n + \mathcal{MC}_i(\lceil \frac{n}{2} \rceil) = 13n + \mathcal{MC}_i(\lceil \frac{n}{2} \rceil)$ (assuming $p_i \in \mathcal{S}_1$).
Importantly, note that $\mathcal{MC}_i(n) \in O(n)$.

==> sections/view_synchronization.tex <==
\section{View Synchronization for $n = 5t + 1$}

View synchronization represents a significant building block of \name.
We define view synchronization as a problem of bringing all correct processes to the same view.
Formally, let $\mathsf{View} = \{1, 2, ...\}$ be the set of views.
The view synchronization problem is associated with a parameter $\Delta > 0$, which denotes the desired duration of an overlap in each view.
View synchronization provides the following interface:
\begin{compactitem}
    \item \textbf{output} $\mathsf{advance}(v \in \mathsf{Value})$: the process advances to a view $v$.
\end{compactitem}
We define a synchronization point:
\begin{definition} [Synchronization point]
Time $t_s$ is a \emph{synchronization point} if and only if all correct processes are in the same view $v$ from time $t_s$ to (at least) time $t_s + \Delta$.
\end{definition}
Lastly, view synchronization ensures the following property:
\begin{compactitem}
    \item \emph{Eventual synchronization:} There exists a synchronization point $t_s$ such that $t_s \geq \text{GST}$.
\end{compactitem}

\subsection{\textsc{catch-up}}

This subsection introduces the pseudocode, our signature-free view synchronization protocol with $O(n^2)$ words exchanged in the time period $[\text{GST}, \infty)$.

\begin{algorithm}
\caption{\sync: Pseudocode (for process $p_i$)}
\label{algorithm:sync}
\footnotesize
\begin{algorithmic} [1] 
\State \textbf{Uses:}
\State \hskip2em $\mathsf{Timer}$ $\mathit{view\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{help\_timer}_i$
\State \hskip2em $\mathsf{Timer}$ $\mathit{enter\_timer}_i$

\medskip
\State \textbf{Constants:}
\State \hskip2em $\mathit{view\_duration} \gets \Delta + 6\delta$

\medskip
\State \textbf{upon} $\mathsf{init}$:
\State \hskip2em $\mathsf{View}$ $\mathit{view}_i \gets 1$ 
\State \hskip2em $\mathsf{View}$ $\mathit{help\_view}_i \gets 0$
\State \hskip2em $\mathit{view\_timer}_i.\mathsf{measure}(\mathit{view\_duration})$ \label{line:enter_1}
\State \hskip2em \textbf{trigger} $\mathsf{advance}\big( 1 \big)$ \BlueComment{enter view $1$}

\medskip
\State \textbf{upon} $\mathit{view\_timer}_i$ \textbf{expires}: \label{line:view_timer_expire}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i + 1 \rangle$ \label{line:send_complete_1}

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v$ such that (1) $v > \mathit{view}_i$, and (2) $\langle \textsc{start-view}, v \rangle$ is received from $t + 1$ processes: \label{line:receive_plurality}
\State \hskip2em \textbf{if} $v > \mathit{help\_view}_i$: \label{line:check_help}
\State \hskip4em $\mathit{help\_view}_i \gets v$
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{cancel}()$
\State \hskip4em $\mathit{help\_timer}_i.\mathsf{measure}(\delta)$

\medskip
\State \textbf{upon} $\mathit{help\_timer}_i$ \textbf{expires}:
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i \rangle$ \label{line:send_complete_2}
% \State \hskip2em \textbf{if} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ is received from $t + 1$ processes:
% \State \hskip4em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{help\_view}_i - 1 \rangle$ \label{line:send_complete_2_prime}

\medskip
\State \textbf{upon} exists $\mathsf{View}$ $v > \mathit{view}_i$ such that $\langle \textsc{start-view}, v \rangle$ is received from $2t + 1$ processes: \label{line:receive_quorum}
\State \hskip2em $\mathit{view}_i \gets v$ \label{line:update_view_2}
\State \hskip2em $\mathit{view\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_view}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{cancel()}$ \label{line:cancel_enter}
\State \hskip2em $\mathit{enter\_timer}_i.\mathsf{measure}(\delta)$ \label{line:measure_enter}

\medskip
\State \textbf{upon} $\mathit{enter\_timer}_i$ \textbf{expires:} \label{line:enter_expires}
\State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i \rangle$ \label{line:send_complete_3}
% \State \hskip2em \textbf{broadcast} $\langle \textsc{start-view}, \mathit{view}_i - 1 \rangle$ \label{line:send_complete_3_prime}
\State \hskip2em $\mathit{view\_timer}_i.\mathsf{measure}(\mathit{view\_duration})$ \label{line:measure_view}
\State \hskip2em \textbf{trigger} $\mathsf{advance}(\mathit{view}_i)$ \BlueComment{enter view $\mathit{view}_i$} \label{line:enter_v}
\end{algorithmic}
\end{algorithm}

\subsection{Proof of Correctness \& Complexity}

In this subsection, we present proof of \textsc{catch-up}'s correctness and complexity.

\begin{lemma} \label{lemma:started_before}
If a correct process enters a view $v > 1$, then (at least) one correct process has previously entered view $v - 1$.
\end{lemma}
\begin{proof}
Let a correct process $p_i$ enter $v > 1$ (line~\ref{line:enter_v}).
Let $p_v$ be the first correct process which sends the $m = \langle \textsc{start-view}, v \rangle$ message.
Importantly, $p_v$ sends $m$ at line~\ref{line:send_complete_1}; if $p_v$ sends $m$ at line~\ref{line:send_complete_2} or at line~\ref{line:send_complete_3}, then $p_v$ would not be the first correct process which sends $\langle \textsc{start-view}, v \rangle$ (line~\ref{line:receive_plurality}).

Process $p_i$ has received $\langle \textsc{start-view}, v \rangle$ message from $2t + 1$ processes (line~\ref{line:receive_quorum}), out of which (at least) $t + 1$ processes are correct.
Therefore, before $p_i$ enters $v$, $p_v$ sends the message $m$ at line~\ref{line:send_complete_1}.
Hence, $p_v$ indeed enters $v - 1$ before $p_i$ enters $v$.
\end{proof}

\begin{lemma}
Every view $v$ is eventually entered by a correct process.
\end{lemma}
\begin{proof}
By contradiction, suppose that the greatest view entered by a correct process is $v^*$; let $p^*$ be any correct process that enters $v^*$.
Note that $v^* > 1$ as every process enters the first view as soon as it starts executing \textsc{catch-up} (line~\ref{line:enter_1}).
As $p^*$ enters $v^* > 1$ (line~\ref{line:enter_v}), $p^*$ receives $\langle \textsc{start-view}, v^* \rangle$ from $2t + 1$ processes (line~\ref{line:receive_quorum}).
Therefore, each correct process eventually receives $t + 1$ $\langle \textsc{start-view}, v^* \rangle$ messages (line~\ref{line:receive_plurality}), which means that each correct process eventually broadcasts $\langle \textsc{start-view}, v^* \rangle$ (line~\ref{line:send_complete_2}).
Hence, every correct process eventually enters $v^*$ (line~\ref{line:receive_quorum}).

Eventually, for each correct process $p_i$, $\mathit{view\_timer}_i$ expires (line~\ref{line:view_timer_expire}).
Thus, every correct process eventually broadcasts $\langle \textsc{start-view}, v^* + 1 \rangle$, which implies that every correct process eventually receives $\langle \textsc{start-view}, v^* + 1 \rangle$ from $2t + 1$ correct processes (line~\ref{line:receive_quorum}), and enters $v^* + 1$ (line~\ref{line:enter_v}).
Therefore, $v^*$ is not the greatest view entered by a correct process, which proves the lemma.
\end{proof}

\begin{definition} [View $v_{\mathit{max}}$]
We denote by $v_{\mathit{max}}$ the greatest view entered by a correct process before GST; if such a view does not exist, $v_{\mathit{max}} = 0$.
\end{definition}

\begin{definition} [View $v_{\mathit{final}}$]
We denote by $v_{\mathit{final}}$ the smallest view first entered by a correct process after GST.
\end{definition}

\begin{lemma}
$v_{\mathit{final}} = v_{\mathit{max}} + 1$.
\end{lemma}
\begin{proof}
Follows directly from \Cref{lemma:started_before}.
\end{proof}

We denote by $t_v$ the first time a correct process enters the view $v$.

\begin{lemma} \label{lemma:view_duration}
For any view $v \geq v_{\mathit{final}}$, no correct process sends $\langle \textsc{view-complete}, v \rangle$ before time $t_v + \mathit{view\_duration}$.
\end{lemma}
\begin{proof}
As $v \geq v_{\mathit{final}}$, $t_v \geq \text{GST}$.
As local clocks do not drift after GST, the first time a correct process sends $\langle \textsc{view-complete}, v \rangle$ cannot be before $t_v + \mathit{view\_duration}$.
\end{proof}

\begin{lemma} \label{lemma:enter_final}
Every correct process enters $v_{\mathit{final}}$ by time $t_{v_{\mathit{final}}} + 4\delta$.
\end{lemma}
\begin{proof}
The first correct process $p$ enters $v_{\mathit{final}}$ at time $t_{v_{\mathit{final}}}$.
Importantly, by \Cref{lemma:view_duration}, no correct process $p_i$ updates its $\mathit{view}_i$ variable to $> v_{\mathit{final}}$ before time $t_{v_{\mathit{final}}} + \mathit{view\_duration}$.

By time $t_{v_{\mathit{final}}} + \delta$, every correct process $p_i$ that has not previously sent $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ receives $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ from $t + 1$ processes; as $t_{v_{\mathit{final}}} + \mathit{view\_duration} > t_{v_{\mathit{final}}} + \delta$, $\mathit{view}_i \leq v_{\mathit{final}}$ at process $p_i$.
Now, we separate two scenarios: 
\begin{compactitem}
    \item Let $\mathit{view}_i = v_{\mathit{final}}$.
    In this case, $p_i$ sent $\langle \textsc{start-view},  v_{\mathit{final}} \rangle$ (line~\ref{line:send_complete_3}).

    \item Otherwise, $p_i$ sends $\langle \textsc{start-view},  v_{\mathit{final}} \rangle$ by time $t_{v_{\mathit{final}}} + 2\delta$. (line~\ref{line:send_complete_2}).
\end{compactitem}
Hence, by time $t_{v_{\mathit{final}}} + 2\delta$, every correct process sends $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$.
Thus, by time $t_{v_{\mathit{final}}} + 4\delta$, all correct processes enter $v_{\mathit{final}}$; recall that $t_{v_{\mathit{final}}} + \mathit{view\_duration} > t_{v_{\mathit{final}}} + 4\delta$.
\end{proof}

\begin{lemma}
Correct processes overlap for (at least) $\Delta$ time in $v_{\mathit{final}}$.
\end{lemma}
\begin{proof}
Follows directly from \Cref{lemma:enter_final} and the fact that $\mathit{view\_duration} = \Delta + 6\delta$.
\end{proof}

\begin{lemma}
By time $\text{GST} + 6\delta$, every correct process enters $v_{\mathit{max}}$ or $v_{\mathit{final}}$.
\end{lemma}
\begin{proof}
To prove the lemma, we prove that every correct process broadcasts $\langle \textsc{start-view}, v_{\mathit{max}} \rangle$ or $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ by time $\text{GST} + 3\delta$.
Consider any process $p_i$ that does not satisfy the aforementioned claim.
By time $\text{GST} + \delta$, $p_i$ receives $t + 1$ $\langle 
\textsc{start-view}, v_{\mathit{max}} \rangle$ messages (line~\ref{line:receive_plurality}).
We consider the following cases:
\begin{compactitem}
    \item Let the check at line~\ref{line:receive_plurality} activates.
    We further distinguish two cases:
    \begin{compactitem}
        \item Let the check at line~\ref{line:check_help} pass.
        In this case, $\mathit{help\_view}_i \gets v_{\mathit{max}}$ by time $\text{GST} + \delta$.
        Therefore, $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.

        \item Otherwise, $\mathit{help\_view}_i \in \{v_{\mathit{max}}, v_{\mathit{final}}\}$, which implies that $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.
    \end{compactitem}

    \item Otherwise, $\mathit{view}_i \in \{v_{\mathit{max}}, v_{\mathit{final}}\}$.
    Again, $p_i$ broadcasts one of the messages by time $\text{GST} + 3\delta$.
\end{compactitem}
Therefore, every correct process broadcasts $\langle \textsc{start-view}, v_{\mathit{max}} \rangle$ or $\langle \textsc{start-view}, v_{\mathit{final}} \rangle$ by time $\text{GST} + 3\delta$.

Hence, by time $\text{GST} + 4\delta$, every correct process receives $2t + 1$ \textsc{start-view} messages for either $v_{\mathit{final}}$ or $v_{\mathit{max}}$.
Thus, by time $\text{GST} + 6\delta$, every correct process enters either $v_{\mathit{max}}$ or $v_{\mathit{final}}$.
\end{proof}

% \begin{lemma}
% $t_{v_\mathit{final}} \leq \text{GST} + \mathit{view\_duration} + 4\delta$.
% \end{lemma}
% \begin{proof}
% By contradiction, let $t_{v_\mathit{final}} > \text{GST} + \mathit{view\_duration} + 4\delta$.
% As a correct process enters $v_{\mathit{max}}$ before GST, at least $3t + 1$ correct processes send $\langle \textsc{view-complete}, v_{\mathit{max}} - 1 \rangle$ before GST.

% We prove this lemma through a sequence of intermediate results:
% \begin{compactenum}
%     \item By time $\text{GST} + \delta$, every correct process sends $\langle \textsc{view-complete}, v_{\mathit{max}} - 1 \rangle$.

%     Consider any process $p_i$ which does not send $\langle \textsc{view-complete}, v_{\mathit{max}} - 1 \rangle$ before GST.
%     By time $\text{GST} + \delta$, $p_i$ receives $t + 1$ $\langle \textsc{view-complete}, v_{\mathit{max}} - 1 \rangle$ messages.
%     Now, we separate two scenarios: 
%     \begin{compactitem}
%         \item Let $\mathit{view}_i \geq v_{\mathit{final}}$.
%         Impossible as it contradicts $t_{v_\mathit{final}} > \text{GST} + \mathit{view\_duration} + 4\delta$.

%         \item Otherwise, $p_i$ sends $\langle \textsc{view-complete},  v_{\mathit{max}} - 1 \rangle$ (line~\ref{line:send_complete_1} or line~\ref{line:send_complete_3}).
%     \end{compactitem}

%     \item By time $\text{GST}$
% \end{compactenum}
% \end{proof}
